Statistical Inference in the Differential Privacy Model

In modern settings of data analysis, we may be running our algorithms on datasets that are sensitive in nature. However, classical machine learning and statistical algorithms were not designed with these risks in mind, and it has been demonstrated that they may reveal personal information. These concerns disincentivize individuals from providing their data, or even worse, encouraging intentionally providing fake data. To assuage these concerns, we import the constraint of differential privacy to the statistical inference, considered by many to be the gold standard of data privacy. This thesis aims to quantify the cost of ensuring differential privacy, i.e., understanding how much additional data is required to perform data analysis with the constraint of differential privacy. Despite the maturity of the literature on differential privacy, there is still inadequate understanding in some of the most fundamental settings. In particular, we make progress in the following problems: $\bullet$ What is the sample complexity of DP hypothesis testing? $\bullet$ Can we privately estimate distribution properties with a negligible cost? $\bullet$ What is the fundamental limit in private distribution estimation? $\bullet$ How can we design algorithms to privately estimate random graphs? $\bullet$ What is the trade-off between the sample complexity and the interactivity in private hypothesis selection?

==> MRF/est-ub.tex <==
\section{Parameter Learning of Pairwise Graphical Models}
%The upper bound based on~\cite{WuSD19}, with privatized Franke-Wolfe.

The problem we consider in this section is to learn the weight matrix. To be specific, given $\ns$ i.i.d. samples $ \{z^1, \cdots, z^{\ns}\}$ generated from an unknown distribution $\cD(A,\theta)$, we want to design estimator $\hat{A}$ such that with probability at least $\frac{2}{3}$, $\max_{i,j\in[\dims]}\absv{A_{i,j} - \hat{A}_{i,j}} \le \dist$. Besides, we also require that $\hat{A}$ satisfies $(\eps,\delta)$-DP.

A nice observation of Ising model is that for any node $Z_i$, the probability of $Z_i=1$ conditioned on the remaining nodes $Z_{-i}$ simply follows from a logistic funtion. We formalize this observation by the following lemma.
\begin{lemma}
\label{lem:IsingToLR}
Let $Z \sim \cD(A,\theta)$ and $Z \in \{-1,1\}^{\dims}$, then $\forall i \in [\dims]$, $\forall x \in \{-1,1\}^{[\dims] \backslash \{i\}}$,
$$
\probof{Z_i=1|Z_{-i}=x} = \sigma\Paren{ \sum_{j\neq i}2A_{i,j}x_j + 2\theta_i} = \sigma\Paren{w^T x^{\prime}}.
$$
where $x^{\prime} = [x,1] \in \RR^{\dims}$ and $w= 2[A_{i,1},\cdots, A_{i,i-1}, A_{i,i+1},\cdots, A_{i,\dims},\theta_i]  \in \RR^{\dims}$. $\sigma(z) = \frac{1}{1+e^{-z}}$ is the sigmoid function. Moreover, $\norm{w} \le 2\lambda(A,\theta)$.
\end{lemma}

By Lemma~\ref{lem:IsingToLR}, a natural idea to estimate the weight matrix is to solve a logistic regression for each node.

\subsection{Private Sparse Logistic Regression~\cite{TalwarTZ14}}

\textbf{Problem definition:} Given a training data set $D$ consisting of n pairs of data $d_i = (x_i, y_i)$, where $x_i \in \RR^p$ and $y_i \in \RR$, a constraint set $\cC \in \RR^p$, and a loss function $\cL: \cC \times \RR^{p+1} \rightarrow \RR$, we want to find 
$w^{erm} = \arg\min_{w\in \cC} ~ \frac1\ns{\sum_{i=1}^{\ns} \cL(w; d_i)}$ in a DP way.

Before claiming their algorithm and results, we need the following two definitions.
\begin{definition}
A funtion $\cL : \cC \rightarrow \RR$ is $L_1$-Lipschitz with respect to $l_1$ norm, if the following holds.
$$\forall w_1, w_2 \in \cC, \absv{\cL(w_1) - \cL(w_2)} \le L_1 \norm{w_1-w_2}.$$
\end{definition}


\begin{definition}[Curvature constant]
For $\cL:\cC \rightarrow \RR$, $\Gamma_{\cL}$ is defined as 
$$ \Gamma_{\cL} = \sup_{w_1, w_2 \in \cC, \gamma \in (0,1], w_3 = w_1 + \gamma (w_2-w_1)}\frac{2}{\gamma^2} \Paren{\cL(w_3) - \cL(w_1) - \langle w_3-w_1, \nabla \cL(w_1) \rangle}.$$
\end{definition}

\begin{algorithm}[H]

\KwIn{Data set: $D = \{d_1,\cdots,d_n\}$, loss function: $\cL(w;D) = \frac1{\ns} \sum_{i=1}^{\ns} \cL(w;d_i)$ (with $l_1$-Lipschitz constant $L_1$), privacy parameters: $(\eps,\delta)$, convex set: $\cC = conv(S)$ with $\norm{\cC}$ = $\max_{s \in S} \norm{s}$, iteration times: $T$.}

Initialize $w$ from an arbitrary point in $\cC$.

\For{$t=1$ to $T-1$}{
$\forall s\in S$, $\alpha_s \leftarrow \langle s, \nabla \cL(w;D)\rangle+ \text{Lap}\Paren{\frac{L_1 \norm{C} \sqrt{8T\log(1/\delta)}}{\ns\eps}}$, where $\text{Lap}(\lambda)\sim \frac1{2\lambda}e^{-\absv{x}/\lambda}$.

$\tilde{w_t} \leftarrow \arg\min_{s \in S} \alpha_s$.

$w_{t+1} \leftarrow (1-\mu_t)w_{t} + \mu_t \tilde{w_t}$, where $\mu_t = \frac{2}{t+2}$.
}
\KwOut{ $w^{priv} = w_T$.}

\caption{$\cA_{FW}( D, \cL, \eps, \delta, \cC):$ Differentially Private Frank-Wolfie Algorithm}
\label{alg:privateFW}
\end{algorithm}

%\begin{lemma}[Privacy guarantee]
%Algorithm~\ref{alg:privateFW} satisfies $(\eps,\delta)$-DP.
%\end{lemma}

\begin{lemma}[Theorem 5.5 from~\cite{TalwarTZ14}]
\label{lem:PrivateFW}
Algorithm~\ref{alg:privateFW} satisfies $(\eps,\delta)$-DP. Furthermore, let $L_1$, $\norm{\cC}$ be defined as in Algorithm~\ref{alg:privateFW}. Let $\Gamma_{\cL}$ be an upper bound on the curvature constant for the loss function $\cL(\cdot;d)$ and $\absv{S}$ is the number of extreme points in $S$.
If we set $T=\frac{\Gamma_{\cL}^{\frac{2}{3}} (n\eps)^{\frac{2}{3}}}{L_1\norm{\cC}^{\frac{2}{3}}}$, then with probability at least $1-\beta$,

$$ \cL(w^{priv}; D) - \cL(w^{erm}; D) = O\Paren{ \frac{\Gamma_{\cL}^{\frac13} (L_1\norm{\cC}) ^{\frac{2}{3}}\log(\frac{ \ns\absv{S}}{\beta}) \sqrt{\log{\frac1{\delta}}} } {(\ns \eps)^{\frac{2}{3}}}}.$$

\end{lemma}

\begin{corollary}
\label{cor:EmpiricalError}

If we consider the problem of sparse logistic regression, i.e., $\cL(w;D) = \frac1{n} \sum_{i=1}^n \log(1+e^{-y_i \langle w, x_i \rangle})$, with the constraint that $\cC = \{w: \norm{w} \le \lambda\}$, and we further assume that $\forall i, \norminf{x_i} \le 1, y_i \in \{\pm 1\}$, let $T =  \lambda^{\frac{2}{3}} (\ns \eps)^{\frac{2}{3}}$,  then with probability at least $1-\beta$,

$$ \cL(w^{priv}; D) - \cL(w^{erm}; D) = O\Paren{ \frac{\lambda^{\frac{4}{3}}\log(\frac{ \ns\dims}{\beta}) \sqrt{\log{\frac1{\delta}}} } {(\ns \eps)^{\frac{2}{3}}}}.$$

\end{corollary}

\begin{proof}
First let we show $L_1 \le 2$. If we fix $d$, then for any $w_1, w_2\in \cC$,
$\absv{ \cL(w_1;d) -\cL(w_2;d)} \le \max_w \norminf{\nabla_w \Paren{ \cL(w;d)}} \cdot \norm{w_1 - w_2}.$
Since $\nabla_w \Paren{ \cL(w;d)} = \Paren{\sigma(\langle w, x \rangle) - y} x$, $\norminf{\nabla_w \Paren{ \cL(w;d)}} \le 2$.

Then we want to show $\Gamma_{\cL} \le \lambda^2$, where we need the following lemma.
\begin{lemma}[Remark 4 in~\cite{TalwarTZ14}]
For any $q,r \ge 1$ such that $\frac1q+\frac1r=1$, $\Gamma_{\cL}$ is upper bounded by $\alpha {\left\lVert \cC \right\rVert_q}^2$, where $\alpha = \max_{w \in \cC, {\left\lVert v \right\rVert_q=1}}  {\left\lVert \nabla^2 \cL(w) \cdot v \right\rVert_q}$.
\end{lemma}

If we take $q=1, r = +\infty$, then $\Gamma_{\cL} \le \alpha \lambda^2$, where 
$$\alpha = \max_{w \in \cC, \norm{v}=1}   \norminf{ \nabla^2 \cL(w;d) \cdot v} \le \max_{i,j \in[\dims]} \Paren{ \nabla^2 \cL(w;d)}_{i,j}.$$
Since $\nabla^2 \cL(w;d) = \sigma(\langle w, x \rangle)  \Paren{1- \sigma(\langle w, x \rangle)} x \cdot x^T$, given $\norminf{x}\le 1$, we have $\alpha \le 1$.

At last since $\cC = \{w: \norm{w}\le 1 \}$, the number of extreme points of $S$ equals $2\dims$. By replacing all these parameters in Lemma~\ref{lem:PrivateFW}, we prove the corollary. 

\end{proof}

\subsection{Privately Learning Ising Model}

\begin{algorithm}[H]

\KwIn{ $\ns$ i.i.d. samples $\{ z^1,\cdots, z^{\ns}\}$, where $z^m \in \{\pm1\}^{\dims}$ for $m\in [\ns]$; an upper bound on $\lambda(A,\theta) \le \lambda$, privacy parameter $\eps$, $\delta$.}


\For{$i=1$ to $\dims$}{
$\forall m \in [\ns]$, $x_m \leftarrow [z_{-i}^{m},1]$, $y_m \leftarrow z_i^m$.

$w^{priv} \leftarrow \cA( D, \cL, \eps^{\prime}, \delta^{\prime}, \cC)$
where $D=\{\Paren{x_m, y_m} \}_{m=1}^{\ns}$, $\cL(w;d) =  \log\Paren{1+e^{-y \langle w, x \rangle}}$, $\cC = \{ \norm{w}\le 2\lambda\}$, $\eps^{\prime}=\frac{\eps}{\sqrt{2\dims} \log(\frac{\dims}{\delta})}$ and $\delta^{\prime} =\frac{\delta}{\dims}$.

$\forall j \in \dims$, $\hat{A}_{i,j} \leftarrow w^{priv}_{\tilde{j}}$, where $\tilde{j} =j $ when $j<i$ and $\widetilde{j}  = j-1$ if $j>i$.

}

\KwOut{$\hat{A} \in \RR^{\dims \times \dims}$.}

\caption{Differentially Private Learning Ising Model}
\label{alg:DPIsing}
\end{algorithm}

\begin{theorem}[Privacy guarantee]
Algorithm~\ref{alg:privateFW} satisfies $(\eps,\delta)$-DP.
\end{theorem}


\begin{proof}

Every iteration satisfies $(\frac{\eps}{\sqrt{2\dims} \log(\frac{\dims}{\delta})},\frac{\delta}{\dims})$-DP. By strong composition theorem, the algorithm satisfies $(\eps,\delta)$-DP.

\end{proof}

\begin{theorem}[Utility]
Let $\cD(A,\theta)$ be an unknown $\dims$-variable Ising model distribution. Suppose that $\cD(A,\theta)$ has width $\lambda(A,\theta)\le \lambda$. Then with probability greater than $2/3$, Algorithm~\ref{alg:DPIsing} outputs $\hat{A}$ that satisfies $\max_{i,j \in [\dims]} \absv{A_{i,j} - \hat{A}_{i,j}} \le \dist$ if the number of i.i.d. samples satisfy
$$\ns = O\Paren{\frac{e^{\lambda} \lambda^2 \log(\dims)}{\dist^4}+ \frac{\sqrt{\dims} \lambda^2 \log^4(\dims) \cdot \log^{2}(\frac1{\delta}) \cdot e^{\lambda}}{\eps \alpha^3}}.$$
\end{theorem}

\begin{proof}

Let $P$ be a distribution over $\{-1,1\}^{\dims} \times \{-1,1\}$, where $d = (x,y) \sim P$ satisfies $\probof{y=1|x} = \sigma\Paren{\langle w^*, x\rangle}$ with $\norm{w^*}\le 2\lambda$.
Let $\cL(w;d) = \log\Paren{1+e^{-y \langle w, x \rangle}}$. Suppose we are given $\ns$ i.i.d. samples $D = (x_m,y_m)_{m=1}^{\ns}$, we use $w^{erm}$ to denote $\arg\min_w \sum_{m=1}^{\ns} \cL(w;d_m)$ s.t. $\norm{w} \le 2\lambda$. Our goal is to prove $\norminf{w^{priv} - w^*}$ is small when the samples are drawn from an Ising model, where $w^{priv} = \cA\Paren{ D, \cL, \frac{\eps}{\sqrt{2\dims} \log(\frac{\dims}{\delta})},\frac{\delta}{\dims},  \{w: \norm{w}\le 2\lambda \}}$.

First let we bound  $\expectationf{\cL(w^{priv};d)}{d\sim P} - \expectationf{\cL(w^*;d)}{d\sim P}$.  By triangle inequality,
\begin{align*}
&~\expectationf{\cL(w^{priv};d)}{d\sim P} - \expectationf{\cL(w^*;d)}{d\sim P} \nonumber\\
\le& \absv{ \expectationf{\cL(w^{priv};d)}{d\sim P} - \sum_{m=1}^{\ns} \cL(w^{priv};d_m) } + \absv{  \sum_{m=1}^{\ns} \cL(w^{priv};d_m) - \sum_{m=1}^{\ns} \cL(w^{erm};d_m) } \nonumber\\
+& \Paren{  \sum_{m=1}^{\ns} \cL(w^{erm};d_m) - \sum_{m=1}^{\ns} \cL(w^*;d_m) } + \absv{ \expectationf{\cL(w^{*};d)}{d\sim P} - \sum_{m=1}^{\ns} \cL(w^{*};d_m) } \nonumber
\end{align*}

Now we need to bound each term. We bound the third term first. According to the definition of $w^{erm}$, the third term should be smaller than 0. Then we turn to the first and last term. By the generalization error bound (Lemma 7 from~\cite{WuSD19}), when $\ns = O\Paren{\frac{ \lambda^2 \log(\dims)}{\gamma^2}}$, with probablity greater than $1 - \frac{1}{10 \dims}$, these two terms are upper bounded by $\frac13 \gamma$ at the same time. Last we look at the second term, by Corollary~\ref{cor:EmpiricalError}, when $\ns =O\Paren{ \frac{ \sqrt{\dims} \lambda^2 \log^4(\dims) \cdot \log^{2} (\frac1{\delta})}{\eps \gamma^{\frac{3}{2}}}}$, with probability greater than $1 - \frac{1}{10 \dims} $, it is bounded by $\frac13\gamma$.
Therefore, with probability greater than $1-\frac{3}{10\dims}$, $ \expectationf{\cL(w^{priv};d)}{d\sim P} - \expectationf{\cL(w^*;d)}{d\sim P} \le \gamma$.

The remaining proof follows from the same argument from~\cite{WuSD19}. Suppose the samples are drawn from Ising model and $ \expectationf{\cL(w^{priv};d)}{d\sim P} - \expectationf{\cL(w^*;d)}{d\sim P} \le O\Paren{\alpha^2 e^{-6\lambda}}$, then we have $\norminf{w^{priv} - w^*} \le \alpha$. By replacing $\gamma = \alpha^2 e^{-6\lambda}$ and uninon bound, we prove that with probability at least $\frac{2}{3}$, $\max_{i,j\in[\dims]}\absv{A_{i,j} - \hat{A}_{i,j}} \le \dist$.


\end{proof}
%to some value $x \in \{-1, 1\}^{[\dims-1]}$


==> MRF/preamble.tex <==
\def\eps{\ve}
\renewcommand{\epsilon}{\ve}
\def\ve{\varepsilon}

\newcommand{\Exp}{\mbox{\bf Exp}}
\newcommand{\E}{\mbox{\bf E}}
\newcommand{\Var}{\mbox{\bf Var}}
\newcommand{\sign}{\mbox{\bf sign}}
\newcommand{\erf}{\mbox{\text erf}}
\newcommand{\erfc}{\mbox{\text erfc}}
\newcommand{\pr}[2][]{\mathrm{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[#2\right]}
\newcommand{\R}{\mathbb{R}}
\newcommand{\U}{\mathcal{U}_n}
\newcommand{\dtv}{d_{\mathrm {TV}}}
\newcommand{\dk}{d_{\mathrm K}}
\newcommand{\dkl}{d_{\mathrm {KL}}}
\newcommand{\dskl}{d_{\mathrm {SKL}}}
\newcommand{\tr}{{\mathrm {tr}}}
\DeclareMathOperator{\argmax}{argmax}
\providecommand{\poly}{\operatorname*{poly}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\id}{\mathbb{I}}


\newtheorem{theorem}{Theorem}
\newtheorem{nontheorem}[theorem]{Non Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{case}[theorem]{Case}
\newtheorem{dfn}[theorem]{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{res}[theorem]{Result}

\numberwithin{theorem}{section}
\numberwithin{nontheorem}{section}
\numberwithin{proposition}{section}
\numberwithin{observation}{section}
\numberwithin{remark}{section}
\numberwithin{fact}{section}
\numberwithin{lemma}{section}
\numberwithin{claim}{section}
\numberwithin{corollary}{section}
\numberwithin{case}{section}
\numberwithin{dfn}{section}
\numberwithin{definition}{section}
\numberwithin{question}{section}
\numberwithin{openquestion}{section}
\numberwithin{res}{section}



\newenvironment{proofsketch}{\noindent {\em {Proof (sketch):}}}{$\blacksquare$\vskip \belowdisplayskip}
\newenvironment{prevproof}[2]{\noindent {\em {Proof of {#1}~\ref{#2}:}}}{$\hfill\qed$\vskip \belowdisplayskip}

\def \cA {{\cal A}}
\def \cC {{\cal C}}
\def \cD {{\cal D}}
\def \cL {{\cal L}}
\def \cS {{\cal S}}
\def \cV {{\cal V}}
\def \cW {{\cal W}}
\def \cX {{\cal X}}
\def \cY {{\cal Y}}

\newcommand{\RR}{\mathbb{R}}

\newcommand{\ab}{k}
\newcommand{\ns}{n}
\newcommand{\dist}{\alpha}
\newcommand{\Zon}{Z^\ns}
\newcommand{\Xon}{X^\ns}
\newcommand{\Yon}{Y^\ns}
\newcommand{\dims}{p}

\newcommand{\posa}{u}
\newcommand{\posb}{v}

\newcommand{\absv}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert_1}
\newcommand{\norminf}[1]{\left\lVert#1\right\rVert_{\infty}}
\newcommand{\norminfone}[1]{\left\lVert#1\right\rVert_{\infty,1}}
\def \Paren#1{{\left({#1}\right)}}
 
\newcommand{\probof}[1]{\Pr\Paren{#1}}
\newcommand{\proboff}[2]{\Pr_{#2}\Paren{#1}}
\newcommand{\expectation}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\expectationf}[2]{\mathbb{E}_{#2}\left[#1\right]}

\newcommand{\ham}[2]{d_{ham}(#1,#2)}

\def \Brack#1{{\left[{#1}\right]}}


==> back_up/toolbox copy/abstract.tex <==
Le Cam's method, Fano's inequality, and Assouad's lemma are three widely used techniques to prove lower bounds for statistical estimation tasks. We propose their analogues under central differential privacy. Our results are simple, easy to apply and we use them to establish sample complexity bounds in several estimation tasks. 

\noindent{We establish the optimal sample complexity of discrete distribution estimation under total variation distance and $\ell_2$ distance. We also provide lower bounds for several other distribution classes, including product distributions and Gaussian mixtures that are tight up to logarithmic factors. The technical component of our paper relates coupling between distributions to the sample complexity of estimation under differential privacy. 
}
%\anote{Perhaps add more in terms of upper bounds and some applications in the abstract?}
%Learning distributions from samples is a fundamental statistical learning task. When the samples are collected from users, how to protect each user's privacy has garnered wide interest in the recent years. We study the problem of learning $\ab$-ary discrete distributions under differential privacy. We show that the sample complexity of learning a distribution up to TV distance $\alpha$ ($\ell_2$ distance $\beta$) under $\eps$ pure differential privacy is $\Theta(\frac{k}{\alpha^2} + \frac{k}{\alpha \eps})$ ($\tilde{\Theta}(\frac{1}{\beta^2} + \frac{\min \{\sqrt{k}, 1/\beta\}}{\beta\eps})$ ). %\todo{HZ: this is incorrect, even if we change max to min. We do not have tight bounds in l2 distance.}
%The upper bound is obtained by adding Laplace noise to the empirical estimator. For the lower bound part, we extend the classical Fano's inequality to the case with differential privacy constraint, which can be of independent interest. The technique also gives tight lower bounds for learning product distributions and Gaussian mixtures.

==> back_up/toolbox copy/applications.tex <==
\subsection{Applications}
\label{sec:applications}
We now describe several applications of the theorems above. 

\medskip
\noindent\textbf{Applications of Theorem~\ref{thm:le_cam}.} 
%A result similar to Theorem 1 was developed by~\cite{AcharyaSZ18} who used it to establish sample complexity of differentially private uniformity testing  of $k$-ary distributions under total variation distance~\cite{AcharyaSZ18, AliakbarpourDR18}. and for differentially private entropy and support size estimation~\cite{AcharyaKSZ18}.  
~\cite{AcharyaSZ18} developed a result similar to Theorem~\ref{thm:le_cam}, which is used to establish sample complexity lower bounds for differentially private uniformity testing under total variation distance~\cite{AcharyaSZ18, AliakbarpourDR18}, and for differentially private entropy and support size estimation~\cite{AcharyaKSZ18}. In this paper, we use Theorem~\ref{thm:le_cam} as a stepping stone to prove private Assouad's method (Theorem~\ref{thm:assouad}). 

\medskip
\noindent\textbf{Distribution Estimation and Applications of Theorem~\ref{thm:dp_fano} and~\ref{thm:assouad}.} {We will apply Theorem~\ref{thm:dp_fano} (private Fano's inequality) and Theorem~\ref{thm:assouad} (private Assouad's lemma) to some classic distribution estimation problems. The results are summarized in Table~\ref{tab:pure} and Table~\ref{tab:approx}. Before presenting the results, we describe the framework of minimax distribution estimation.}

\medskip
\noindent\textit{Distribution estimation framework.} Let $\cQ$ be a collection of distributions over $\cX$, and for this $\cQ$, let $\cP=\cQ^{\ns}:=\{q^\ns:q\in\cQ\}$ be the collection of $n$-fold distributions over $\cX^\ns$ induced by i.i.d. draws from a distribution over $\cQ$. The parameter space is $\Theta=\cQ$, where $\theta(\q^n)=\q$, and $\ell$ is a distance measure between distributions in $\cQ$. 
Let $\alpha>0$ be a fixed parameter. The sample complexity,  $S(\cQ, \ell, \alpha, \eps, \delta)$ is the smallest number of samples $n$ to make $R(\cQ^\ns, \ell, \eps, \delta)\le \alpha$, \ie
\[
S(\cQ, \ell, \alpha, \eps, \delta)= \min \{n: R(\cQ^\ns, \ell, \eps, \delta)\le \alpha\}.
\]
When $\delta = 0$, we denote the sample complexity by $S(\cQ, \ell, \alpha, \eps)$. We will state our results in terms of sample complexity. The following corollary of Theorem~\ref{thm:dp_fano} can be used to prove lower bounds on the sample complexity in this distribution estimation framework.  The detailed proof of the corollary is in Section~\ref{sec:coro_fano_proof}.

\begin{restatable}[$\eps$-DP distribution estimation]{coro2}{distest}
	\label{coro:fano}
	Given $\eps>0$, let $\cV=\{\q_1, \q_2,...,\q_M\} \subseteq \cQ$ be a set distributions over $\cX$ with size $M$, such that for all $i\ne j$, 	\begin{enumerate}[label=(\alph*)]
		\item $\ell \Paren{\q_i, \q_j} \ge 3 \tau$,
		\item $D_{KL} \Paren{\q_i,\q_j} \le \beta$,
		\item $d_{TV} \Paren{\q_i,\q_j} \le \gamma$,
	\end{enumerate}
	then
\[
		S(\cQ, \ell, \tau, \eps) = \Omega\Paren{\frac{\log M}{\beta}+ \frac{\log M}{\gamma \eps}}.
\]
\end{restatable}
\noindent\textbf{Remark.} With only conditions $(a)$ and $(b)$, we obtain 
the first term of the sample complexity lower bound which is the original 
Fano's bound for sample complexity. \newnewzs{By Pinsker's inequality, 
a bound on the KL divergence (Condition $(c)$) would imply a bound on TV 
distance (Condition $(b)$), i.e., $\gamma \le \sqrt{\beta/2}$. Hence 
Conditions $(a)$ and $(b)$ can also imply a lower bound on the sample 
complexity. We include all three conditions here since it is possible that in 
certain applications $\gamma \ll \sqrt{\beta/2}$, and hence a better bound 
can be obtained.}
\input{toolbox/table}
\medskip

\medskip
\noindent We now present examples of distribution classes we consider.

\medskip
\noindent\textit{$k$-ary discrete distribution estimation.} {Suppose $\cX=[k]:=\{1, \ldots, \ab\}$, and $\cQ:=\Delta_k$ is the simplex of $k$-ary distributions over $[k]$.  We consider estimation in both total variation and $\ell_2$ distance.} 

\medskip
\noindent\textit{$(k,d)$-product distributions.} Consider $\cX=[k]^d$, and let $\cQ:=\Delta_k^d$ be the set of product distributions over $[k]^d$, where the marginal distribution on each coordinate is over $[k]$ and independent of the other coordinates. We study estimation under total variation distance. A special case of this is Bernoulli product distributions ($k=2$), where each of the $d$ coordinates is an independent Bernoulli random variable.  

\medskip
\noindent\textit{$d$-dimensional Gaussian mixtures.} Suppose $\cX=\RR^{\dims}$, and $\cG_{\dims} := \{ \cN (\mu, I_d): \norm{\mu}\le R\}$ is the set of all Gaussian distributions in $\RR^d$ with bounded mean and identity covariance matrix. The bounded mean assumption is unavoidable, since by~\cite{BunKSW2019}, it is not possible to learn a single Gaussian distribution under pure DP without this assumption. {We consider 
\[
\cQ = \cG_{\ab, \dims} :=\left\{\sum_{j=1}^{\ab} w_j \p_j: \forall j \in [k], w_j \ge 0, \p_j\in\cG_\dims, w_1+\ldots+w_k =1\right\},
\] the collection of mixtures of $k$ distributions from $\cG_\dims$.} 

\medskip
\noindent\textbf{Applications of Theorem~\ref{thm:dp_fano}.}
We apply Corollary~\ref{coro:fano} and obtain sample complexity lower bounds for the tasks mentioned above under pure  differential privacy.

\medskip
{\noindent\textit{$\ab$-ary distribution estimation.} Without privacy constraints, the sample complexity of $\ab$-ary discrete distributions under total variation, and $\ell_2$ distance is $\Theta(k/\alpha^2)$ and $\Theta(1/\alpha^2)$ respectively, achieved by the empirical estimator. Under $\eps$-DP constraint, an upper bound of $O \Paren{\ab/\alpha^2+\ab/\alpha\eps}$
%$O \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha\eps}}$
samples for total variation distance is known using Laplace 
mechanism~\cite{DworkMNS06} (e.g.~\cite{DiakonikolasHS15}). In 
Theorem~\ref{thm:pure-dv}, we establish the sample complexity of this 
problem by providing a lower bound that matches this upper 
bound. \newnewzs{The bound shows that when $\eps \ll \alpha$, the cost 
due 
to privacy dominates the statistical error and when $\eps \ge \alpha$, the 
privacy cost is almost negligible. The same break point (up to logarithmic 
factors) has also been observed for product distributions and mixtures of 
Gaussian distributions, as listed below.}} 

Under $\ell_2$ distance, in Theorem~\ref{thm:pure-l2} we design estimators and establish their optimality whenever $\dist< \ab^{-1/2}$ or $\dist \ge \ab^{-0.499}$, which contains almost all the parameter range. Note that under $\ell_2$ distance, estimation without privacy has sample complexity independent of $k$, whereas {an unavoidable} logarithmic dependence on $\ab$ is introduced due to privacy requirements. The results are presented in Section~\ref{sec:pdp_kary}. 
 
\medskip
\noindent\textit{$(\ab,\dims)$-product distribution estimation.} For $(\ab,\dims)$-product distribution estimation under $\eps$-DP,~\cite{BunKSW2019} proposed an algorithm that uses
%$O\Paren{\ab\dims \log \Paren{ \frac{\ab\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$ 
$O\Paren{\ab\dims \log \Paren{ \ab\dims/\dist} \Paren{1/\dist^2+1/\dist\eps}}$ samples. 
%For the lower bound, they argue that given the existence of an $\dist$-packing set of size M, there exists a lower bound of $\Omega\Paren{\frac{M}{\eps}}$.\amargin{I dont understand the previous sentence about packing. Could we clarify a bit?} However, no packing set is explicitly constructed in the paper. 
In this paper, we present a lower bound of $\Omega\Paren{{\ab\dims}/{\dist^2}+{\ab\dims}/{\dist\eps}}$, which matches their upper bound up to logarithmic factors. For Bernoulli product distributions, \cite{KamathLSU18} proved a lower bound of $\Omega\Paren{{d}/{\alpha \eps}}$ under $(\eps,{3}/{64\ns})$-DP, which is naturally a lower bound for pure DP. %Their proof is based on fingerprinting lemma~\cite{SteinkeU15}, \newhz{ which is defined for Boolean hypercube. It remains unclear whether the proof can be extended to $k$-ary product distributions.}  
The details are presented in Section~\ref{sec:product}.

\medskip
\noindent\textit{Estimating Gaussian mixtures.}{~\cite{BunKSW2019} provided an upper bound of $\widetilde{O}\Paren{{\ab\dims}/{\dist^2}+{\ab\dims}/{\dist\eps}}$ samples.} Without privacy, a tight bounds of $\Omega({\ab\dims}/{\alpha^2})$ was shown in~\cite{SureshOAJ14, DaskalakisK14, AshtianiBHLMP18}. {In this paper, we prove a lower bound of $\Omega\Paren{{\ab\dims}/{\dist^2}+{\ab\dims}/{\dist\eps}}$, which matches the upper bound up to logarithmic factors.} \newzs{For the special case of estimating a single Gaussian ($k=1$), a lower bound of $\ns = {\Omega}\Paren{{\dims}/{(\alpha\eps\log \dims)}}$ was given in~\cite{KamathLSU18} for $(\eps,{3}/{64\ns})$-DP, which implies a lower bound that is $\log d$ factor weaker than our result under pure DP.}
	%Our lower bound for $k = 1$ improves their result under pure DP.} The details are given in Section~\ref{sec:gaussian}.

%\newhzn{
%\noindent\textbf{Remark.} Using the classic packing lower bound instead of Corollary~\ref{coro:fano} leads to loose lower bounds for these estimation problems. For example, in the $\ab$-ary distribution estimation problem, the packing lemma can only give a lower bound of $\ns = \Omega\Paren{\frac{\ab \log \Paren{1/\dist}}{\eps}}$ instead of the optimal $\ns = \Omega\Paren{\frac{\ab}{\dist \eps}}$ lower bound, where there exists an exponential gap in the parameter $\frac1\dist$. This is non-trivial when $\dist$ is small, e.g., $\dist = \frac1{\ab}$.}

\medskip
\noindent\textbf{Applications of Theorem~\ref{thm:assouad}.} As remarked earlier, Theorem~\ref{thm:dp_fano} only works for pure DP (or approximate DP with very small $\delta$). 
%However, it was easy to use as Corollary~\ref{coro:fano}. 
Assouad's lemma can be used to obtain lower bounds for distribution estimation under $(\eps,\delta)$-DP. For $k$-ary distribution estimation under $TV$ distance, we get a lower bound of $\Omega\Paren{{k}/{\alpha^2} + {k}/{\alpha(\eps + \delta)}}$. This shows that even up to $\delta=O(\eps)$, the sample complexity for $(\eps,\delta)$-DP is the same as that under $\eps$-DP.

\newzs{For Bernoulli ($k = 2$) product distributions, \cite{KamathLSU18} provides an efficient $(\eps, \delta)$-DP algorithm that achieves an upper bound of $O\Paren{\dims \log \Paren{ \dims/\dist} \Paren{1/\dist^2+1/\dist\eps}}$.\footnote{\newzs{The algorithm in~\cite{BunKSW2019} works for $\eps$-DP and general $k$ but it is not computationally efficient.}}} The lower bound $\Omega ({d}/{\alpha^2} + {d}/{\alpha \eps})$ obtained in~\cite{KamathLSU18} by fingerprinting holds for small values of $\delta = O(1/\ns)$. Note by the definition of DP~\eqref{eqn:dp-definition}, if $\delta>1/\ns$, a DP algorithm can blatantly disregard the privacy of $\delta\ns$ users. Therefore in most of the literature, $\delta$ is assumed to be $O(1/\ns)$. We want to make a complimentary remark that we
%\footnote{\newhzn{In fact, their lower bound only holds given the loss is in the form of expectation. When the loss is in the form of high probability, they derive a worse lower bound of $\Omega\Paren{\frac{d}{\dist\eps\log d}}$. However, our lower bound holds for both cases.}} \snote{I think we agreed on not putting this footnote since it is not well justified in the current write up. Am I right?}
% We 
can obtain the same lower bound all the way up to $\delta = O(\eps)$. This shows that there is no gain even if we compromise the privacy of a $\delta$ fraction of users. Therefore, there is no incentive to do it. We describe the details about these applications in Section~\ref{sec:adp_applications}. 
%\newzs{
%Note that $\delta=O(1/n)$ is the interesting case for designing privacy-preserving schemes since otherwise one could blatantly disregard privacy of $\delta\ns$ users, which is a constant. However, our results improves our understanding of the estimation risk by showing that even with large $\delta$ (even as large as $\eps$), the same lower bounds hold as with $\delta =O(1/\ns)$ for various statistical estimation tasks. In other words, there is no utility gain by compromising the privacy of a fraction of users, and hence there is no incentive to do it.
%}
%For the results above, we note that while DP with $\delta>1/n$ is not really a privacy guarantee since the privacy of $\delta\ns$ users can be compromised. 
%\newhzn{
%Someone may argue that DP with $\delta>1/n$ is not really a privacy guarantee since the privacy of $\delta\ns$ users can be compromised.
%However, our results above show that the utility can not be improved even sacrificing the privacy of a constant fraction of the users. In other words there is no motivation for using large $\delta$ as opposed to $\delta=O(1/\ns)$. 
%}

==> back_up/toolbox copy/approx_dp_new2.tex <==
\section{$(\eps,\delta)$-DP distribution estimation} \label{sec:adp_applications}
{In the previous section we used Theorem~\ref{thm:dp_fano} to obtain sample complexity lower bounds for pure differential privacy. We will now use Theorem~\ref{thm:assouad} to prove sample complexity lower bounds under $(\eps, \delta)$-DP.}

\subsection{$\ab$-ary distribution estimation} \label{sec:adp_kary}
%In this section, we consider $\ab$-ary distribution estimation under $(\eps, \delta)$-DP.

%\approxdtv*

\begin{theorem}
\label{thm:ApproximateDiscreteTotalVariation}
The sample complexity of $(\eps, \delta)$-DP $\ab$-ary distribution estimation under total variation distance is 
\[
S(\Delta_k,  d_{TV}, \alpha, \eps, \delta) =\Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha(\eps+\delta)}}.
\]
\end{theorem}
{In practice, $\delta$ is chosen to be $\delta = O\Paren{\frac1\ns}$, and the privacy parameter is chosen as a small constant, $\eps = \Theta(1)$. In particular, when $\delta\le \eps$, the theorem above shows
\[
S(\Delta_k,  d_{TV}, \alpha, \eps, \delta) =\Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}.
\]
Since the sample complexity of $\eps$-DP is at most the sample complexity of $(\eps,\delta)$-DP, this shows that the bound above is tight for {$ \delta\le \eps$}. The lower bound part is proved using Theorem~\ref{thm:assouad} in Section~\ref{sec:approximate-tv}.}

\begin{theorem}
\label{thm:ApproximateDiscreteL2}
The sample complexity of $(\eps, \delta)$-DP discrete distribution estimation under $\ell_2$ distance,
\[
 \Omega \Paren {\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha (\eps+\delta)}} \le S(\Delta_k, \ell_2, \alpha, \eps, \delta) \le O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha\eps}},\ \ \ \ \text{for $\dist < \frac1{\sqrt{\ab}}$},
\] 
\begin{align}
\Omega\Paren{\frac{1}{\dist^2}+\frac{1}{\dist^2(\eps+\delta)}}\le S(\Delta_k, \ell_2, \alpha, \eps, \delta)  \le O\Paren{\frac{1}{\dist^2}+\frac{\log\ab}{\dist^2\eps}}, \ \ \ \text{for $\dist > \frac1{\sqrt{\ab}}$}. \nonumber
\end{align}
\end{theorem}
%{When $\delta = O(\eps)$, by Theorem~\ref{thm:pure-l2}, the bounds are tight up to logarithmic factor. We prove this result in Section~\ref{sec:approximate-l2}.}
{When $\delta = O(\eps)$, the bounds are tight when $\dist < 1/\sqrt{\ab}$ and differ by a factor of $\log k$ when $\dist \ge 1/\sqrt{\ab}$. We prove this result in Section~\ref{sec:approximate-l2}.}

\subsubsection{Proof of Theorem~\ref{thm:ApproximateDiscreteTotalVariation}.}
\label{sec:approximate-tv}

{The first term $k/\alpha^2$ is the tight sample complexity without privacy. We prove that $S(\Delta_{\ab}, d_{TV}, \alpha, \eps, \delta) = \Omega \Paren{\frac{\ab}{\alpha(\eps+\delta)}}$.} 

{Suppose $k$ is even and $\dist < 1/10$. Let $ \cE_{k/2} =\{-1,+1\}^{k/2}$, for  $e \in \cE_{k/2}$, we define $\p_e\in\Delta_k$ as follows. 
\begin{align}
\text{For $i=1, \ldots, k/2$}~~~~ \p_e(2i-1) = \frac{1+ 10 e_i \cdot \alpha}{\ab},  ~~ \p_e(2i) = \frac{1- 10e_i  \cdot \dist}{\ab}. \label{eqn:constr-approx-k-ary}
\end{align}}
{To apply Theorem~\ref{thm:assouad}, let $\cV_{\ab/2} = \{ \p_e^n, e \in \cE_{\ab/2}\}$. $\p_e^n$ is the distribution of $n$ i.i.d. samples from distribution $\p_e$, and $\theta(\p_e^n) = \p_e$. For $u, v \in \cE_{\ab/2}$,
\[
\ell( \theta(\p_u^n),  \theta(\p_v^n)) = d_{TV} (p_{u},p_{v}) = \frac{20\dist}{\ab} \cdot \sum_{i=1}^{\frac{k}{2}}\mathbb{I}\Paren{u_i \neq v_i}, 
\]
thus obeying~\eqref{eqn:assouad-loss} with $\tau=10\dist/k$.}
%\amargin{is the inequality an equality above? \newhzz{HZ: Yes}}

%First, we prove that
%\[
%	R(n, \Delta_{\ab}, d_{TV}, \eps, \delta) \ge \frac{1}{2}\min_{\he: \he \text{ is  $(\eps, \delta)$-DP}} ~ \max_{ e \in \cE_{\ab/2} } \EE_{\Xon \sim  \p_e^n} \left[ d_{TV}(\p_{\he},\p_e )\right].
%\]
%
%Given $\Xon$ generated from unknown $\p_e^{\ns} \in \cV_{\ab/2}$, for any distribution estimator $\hat p: \Xon \rightarrow \Delta_{\ab}$, we define $\he \in \{\pm1\}^{k/2}$ as follows:
%$$ \he(i)  = \left\{
%\begin{array}{rcl}
%1 ,       &      & when ~ \hat p (2i-1) \ge \hat p (2i),\\
%-1,       &      & when ~ \hat p (2i-1) < \hat p (2i).
%\end{array} \right. $$
%
%% We note that, given $\Xon$ generated from unknown $\p_e \in \cV_{\ab/2}$, it is enough if we can construct an index estimator $\hat e: \Xon \rightarrow  \{\pm1\}^{k/2}$ according to a feasible distribution estimator $\hat p: \Xon \rightarrow \Delta_{\ab}$ and we show that they have ``similar' performance. We define $\hat {e} \in \{\pm1\}^{k/2}$ as follows:
%%$$ \hat {e}(i)  = \left\{
%%\begin{array}{rcl}
%%1 ,       &      & when ~ \hat p (2i-1) \ge \hat p (2i),\\
%%-1,       &      & when ~ \hat p (2i-1) < \hat p (2i).
%%\end{array} \right. $$
%
%Since $\he$ is a post-processing of $\hat{p}$, so it also satisfies $(\eps,\delta)$-DP. Note that for any estimator $\hat {\p}$ and any distribution $\p_e$, if we have $\hat p (2i-1) < \hat p(2i) $ and $e(i)=1$. Then
%\[
%	\frac{1}{2} \Paren{ |\hat{\p}(2i -1) - \p_e(2i-1)| + |\hat{\p}(2i) - \p_e(2i)|} \ge \frac12|\p_e(2i-1) - \p_e(2i)| = \frac{10 \alpha}{k}.
%\]
%
%The same inequality holds if $\hat p (2i-1) \ge \hat p(2i) $ and $e(i)= -1$. For event $S$, let $\probofsub{e}{S}$ denote $\probofsub{\Xon \sim \p_e^{\ns}}{S}$. Hence for any $e \in \{\pm1\}^{k/2}$, we have
%\begin{align}
%          \expectationsub{\p_{e}}{d_{TV}(\hat p, \p_{e})} & = \frac{1}{2}\sum_{i = 1}^{k/2} \expectationsub{\p_{e}}{ |\hat{\p}(2i -1) - \p_e(2i-1)| + |\hat{\p}(2i) - \p_e(2i)|} \nonumber \\
%          %& \ge  \frac{10\alpha}{k} \sum_{i=1}^{k/2} \Big[ \mathbb{I} (e(i)=1) \cdot \probofsub{e}{\hat p (2i-1) < \hat p(2i) } 
%          %+  \mathbb{I} (e(i)  = -1) \cdot \probofsub{e}{\hat p (2i-1) >\hat p(2i) } \Big] \nonumber \\
%          &\ge  \frac{10\alpha}{k} \sum_{i=1}^{k/2} \Big[ \mathbb{I} (e(i)  =1 ) \cdot \probofsub{e}{\he(i)  =-1} 
%           +  \mathbb{I} ({e(i)}  = -1) \cdot \probofsub{e}{ \he_i =+1} \Big] \nonumber\\
%	 &= \frac1{2}\expectationsub{\p_{e}}{d_{TV}(\p_{\he},\p_{e})}.\nonumber
%\end{align}
%
%Hence we have:
%\begin{align}
%	R(n, \Delta_{\ab}, d_{TV}, \eps, \delta) & %= \min_{\hat p: \hat p \text{ is }(\eps,\delta)-DP} \max_{\p \in \cP} \EE_{\Xon \sim \p^n}\left[d_{TV}(\hat p(\Xon),\p)\right] \nonumber \\
%		 \ge  \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}} \max_{e \in \cE_{\ab/2} } \EE_{\Xon \sim \p_e^n} \left[d_{TV}(\hat p,\p_e)\right] \nonumber \\
%		& \ge \frac{1}{2} \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}}\max_{e \in \cE_{\ab/2}} \EE_{\Xon \sim \p^{\ns}_e} \left[d_{TV}(\p_{\he},\p_e)\right] \nonumber \\
%		& = \frac{1}{2} \min_{\he: \he \text{ is $(\eps,\delta)$-DP}} \max_{\p_e^{\ns} \in \cV_{\ab/2} } \EE_{\Xon \sim \p_e^{\ns}} \left[\ell(\p^{\ns}_{\he},\p_e^{\ns})\right]. \nonumber 
%\end{align}
%
%%Since $\sup_{\p_e \in \cV_{\ab} }\mathbb{E}_{\p_e} [d_{TV}(\hat{\p}, \p_e)]<  \sup_{\p \in \Delta_{\ab} }\mathbb{E}_{\p} [d_{TV}(\hat{\p}, \p)] \le \dist$, we have $R(n,  \cV_{\ab/2}, \ell, \eps, \delta) \le 2\dist$. By Theorem~\ref{thm:assouad}, we have
%%$$\sum_{i=1}^{\frac{\ab}{2}} \probofsub{+i }{ \hat {E}(i) \neq 1 } + \probofsub{-i }{\hat {E}(i) \neq -1 } \leq \frac{k}{5},$$
%%where
%%\[
%%\probofsub{+i }{S} = \probof{S | e(i) = +1} =   \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= + 1}\probof{S| E= e},
%%\]
%%\[
%%\probofsub{-i }{ S } =\probof{S | e(i) = -1} =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= - 1}\probof{S | E= e} .
%%\]
{Recall the mixture distributions $\p_{+i}$ and $\p_{-i}$,} 
\[
\dP_{+i}  =  \frac{2}{|\cE_{\ab/2}|} \sum_{e \in \cE_{\ab/2}: e_i= + 1} \p^{\ns}_e, ~~~ \dP_{-i}  =  \frac{2}{|\cE_{\ab/2}|} \sum_{e \in \cE_{\ab/2}: e_i= -1}\p^{\ns}_e.
\]
{To apply Theorem~\ref{thm:assouad}, we prove the following bound on the Hamming distance between a coupling between $\p_{+i}$ and $\p_{-i}$.
\begin{lemma} \label{lem:coupling_distance}
For any $i$, there is a coupling $(X,Y)$ between $\dP_{+i}$ and $\dP_{-i}$, such that
\[
\expectation{\ham{X}{Y}} \le \frac{20\dist \ns}{\ab}.
\]
\end{lemma}}
\begin{proof}
{By the construction in~\eqref{eqn:constr-approx-k-ary}, note that the distributions $\dP_{+i}$ and $\dP_{-i}$ only have a difference in the number of times $2i-1$ and $2i$ appear. To generate $Y\sim \p_{-i}$ from from $X\sim\p_{+i}$, we scan through $X$ and independently change the coordinates that have the symbol $2i-1$ to the symbol $2i$ with probability $\frac{20\alpha}{1+10\alpha}$. The expected Hamming distance is bounded by $\frac{20\alpha}{1+10\alpha} \cdot \frac{1+10\alpha}{\ab} \cdot \ns = \frac{20\alpha \ns}{\ab}$.}
\end{proof}

Note that $\cV\subset\cP := \{\p^n | \p \in \Delta_k \}$. By Theorem~\ref{thm:assouad}, using the bound on $D$ from Lemma~\ref{lem:coupling_distance}, and $\tau=10\dist/k$,
\[
R(\cP, d_{TV}, \eps, \delta) \ge \frac{5\alpha}{\ab} \cdot \ab \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}\ge  {5\alpha} \cdot \Paren{0.9 e^{-200 n\eps\alpha/k} - 200 \frac{n\eps\alpha\delta}k}.
\]
{To achieve $R(\cP, d_{TV}, \eps, \delta) \le \alpha$, either $n\eps\alpha/k=\Omega(1)$ or ${n\eps\alpha\delta}/k=\Omega(1)$, which implies that $n=\Omega( \frac{k}{\alpha(\eps+\delta)})$}.
%\amargin{Please check the constants above.}

\subsubsection{Proof of Theorem~\ref{thm:ApproximateDiscreteL2}} \label{sec:approximate-l2}

We first consider the case where $\dist < \frac1{\sqrt{\ab}}$.  By Cauchy-Schwarz inequality, $S(\Delta_k, \ell_2, \alpha, \eps, \delta) \ge S(\Delta_k,  d_{TV}, \sqrt{k}\alpha, \eps, \delta) $, and therefore $S(\Delta_k, \ell_2, \alpha, \eps, \delta) = \Omega\Paren{\frac{1}{\dist^2}+\frac{\sqrt{\ab}}{\dist (\eps+\delta)}}$ by Theorem~\ref{thm:ApproximateDiscreteTotalVariation}.

For $\alpha \ge \frac{1}{\sqrt{k}}$, we have $l = \lfloor \frac1{16\dist^2}\rfloor \le k$. Therefore, $\Delta_l \subset \Delta_k$ and $\dist < \frac1{\sqrt{l}}$. Hence,
\[
	S(\Delta_k, \ell_2, \alpha, \eps, \delta) \ge S(\Delta_l, \ell_2, \alpha, \eps, \delta) = \Omega\Paren{\frac{1}{\alpha^2} + \frac1{\dist^2(\eps+\delta)}}.
\]


==> back_up/toolbox copy/approx_dp_product.tex <==
\subsection{Binary product distribution estimation} 
\label{sec:adp_product}

{We now consider estimation of Bernoulli product distributions under total variation distance. A Bernoulli product distribution in $d$ dimensions is a distribution over $\{0,1\}^\dims$ parameterized by $\mu\in [0,1]^\dims$, where the $i$th coordinate is distributed $\ber(\mu_i)$, where $\ber(\cdot)$ is a Bernoulli distribution. Let $\Delta_{2,\dims}$ be the class of Bernoulli product distributions in $\dims$ dimensions.} 

\begin{theorem}
\label{thm:ApproximateProductTotalVariation}
The sample complexity of $(\eps, \delta)$-DP  binary product  distribution estimation satisfies 
\[
S(\Delta_{2,\dims}, d_{TV}, \alpha, \eps, \delta)  =\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha(\eps+\delta)}}.
\]
%Further, when $\delta\le\eps$,
%\[
%S(\Delta_{2,\dims}, d_{TV}, \alpha, \eps, \delta)   =\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha\eps}}.
%\]
\end{theorem}

\newzs{Compared to the upper bound of $O\Paren{\dims \log \Paren{\dims/\dist} \Paren{1/\dist^2+1/\dist\eps}}$ in~\cite{BunKSW2019, KamathLSU18}, our bound is tight up to logarithmic factors when $\delta \le \eps$. \cite{KamathLSU18} also presents a lower bound of $\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha(\eps+\delta)}}$ under $(\eps, \delta)$-DP when $\delta = O(1/\ns)$. Although $\delta = O(1/\ns)$ is the more interesting regime in practice, our bound complements the result by stating that the utility will not improve even if $\delta$ can be as large as $\eps$.}
\begin{proof}	
{Since $\Theta(\dims/\eps^2)$ is an established tight bound for non-private estimation, we only prove the second term.}

{We start by constructing a set of Bernoulli product distributions indexed by $\cE_{\dims} = \{ \pm1\}^{\dims}$. For all $e \in \cE_{\dims}$, let $\p_e = \ber(\mu^e_1) \times \ber(\mu^e_2) \times \cdots \times \ber(\mu^e_\dims)$, where 
\[
\mu^e_i = \frac{1+ e_i\cdot 20\dist}{\dims}.
\]}
%\amargin{I am changing the definitions here, since we wrote $e_i$ to be in 0,1 earlier.}
{Let $\cV = \{ \p_e^{\ns}, e \in \cE_{\dims}\}$, the set of distributions of 
$n$ i.i.d samples from $\p_e$, and $\theta\Paren{\p_e^{\ns}} = \p_e$. For 
$u, v\in \cE_{\dims},$, 	$\ell( \theta(\p_u^n),  \theta(\p_v^n)) = d_{TV} 
(p_{u},p_{v})$. We first prove that~\eqref{eqn:assouad-loss} holds under 
total variation distance for an appropriate $\tau$.} 


%By Lemma 6.4 in~\cite{KamathLSU18}, 
%for any pair of distributions $\p_i, \p_j \in \cV_{\dims}$, $C_1 \dist \le \dtv{\p_i}{\p_j} \le C_2\dist$, where $C_1$ and $C_2$ are some constants.

%We need the following lemma.
\begin{lemma}
\label{lem:binaryproducttv}
There exists a constant $C_1 > 5 $ such that $ \forall u, v \in \cE_{\dims}$,
\[ 
d_{TV} (\p_{u},\p_{v}) \ge \frac{C_1 \dist}{\dims}\cdot  \sum_{i=1}^{\dims}\mathbb{I}\Paren{u_i \neq v_i}.
\]
\end{lemma}

\begin{proof}
Let $S = \{i \in [\dims] : u_i \neq v_i\}$, and $S^{\prime} = \{i \in S : u_i = 1\} $. WLOG, let $\absv{S^{\prime}} \ge \frac12 \absv{S}$ (or else we can define $S^{\prime} = \{i \in S : u_i = -1\}$). Given a random sample $Z \in \{ \pm1\}^{\dims}$, we define an event $A = \{\forall i \in S^{\prime}, Z_i=0\}$. Now we consider the difference between the following two probabilities, which is a lower bound of the total variation distance between $\p_u$ and $\p_v$.
\begin{align}
d_{TV} (\p_{u},\p_{v}) &\ge \absv{\probofsub{Z \sim \p_{u}} {A} - \probofsub{Z \sim \p_{v}} {A}} \nonumber\\
&= \Paren{1-\frac{1-20\dist}{\dims}}^{\absv{S^{\prime}}} - \Paren{1-\frac{1+20\dist}{\dims}}^{\absv{S^{\prime}}} \nonumber\\
&\ge \frac{40\dist}{\dims} \cdot  \absv{S^{\prime}} \cdot  \Paren{1-\frac{1+20\dist}{\dims}}^{\absv{S^{\prime}}} \nonumber \\
& \ge \frac{40 \dist}{\dims} \cdot \absv{S'} e^{-(1+20\dist)} \ge \frac{C_1\dist}{\dims} \cdot \ham{u}{v}, \nonumber
\end{align}
where in the last two inequalities, we assume $\dims \ge 1000$ and $\dist<0.01$.
\end{proof} 

%First, we prove that
%\[
%	R(n, \cC_{\dims}, d_{TV}, \eps, \delta) \ge \frac{1}{2}\min_{\he: \he \text{ is  $(\eps, \delta)$-DP}} ~ \max_{ e \in \cE_{\dims} } \EE_{\Xon \sim  \p_e^n} \left[ d_{TV}(\p_{\he},\p_e )\right].
%\]
%
%Given $\Xon$ generated from unknown $\p_e^{\ns} \in \cV_{\dims}$, for any distribution estimator $\hat \p: \Xon \rightarrow \cC_{\dims}$, we define $\he \in \{\pm1\}^{\dims}$ as follows:
%$$ \he(i)  = \left\{
%\begin{array}{rcl}
%1 ,       &      & when ~ \hat \mu (i) \ge \frac1{\dims},\\
%-1,       &      & when ~ \hat \mu (i) < \frac1{\dims}.
%\end{array} \right. $$
%
%% We note that, given $\Xon$ generated from unknown $\p_e \in \cV_{\dims}$, it is enough if we can construct an index estimator $\hat e: \Xon \rightarrow  \{\pm1\}^{\dims}$ according to a feasible distribution estimator $\hat p: \Xon \rightarrow \cC_{\dims}$ and we show that they have ``similar' performance. We define $\hat {e} \in \{\pm1\}^{\dims}$ as follows:
%%$$ \hat {e}(i)  = \left\{
%%\begin{array}{rcl}
%%1 ,       &      & when ~ \hat p (2i-1) \ge \hat p (2i),\\
%%-1,       &      & when ~ \hat p (2i-1) < \hat p (2i).
%%\end{array} \right. $$
%
%Since $\he$ is a post-processing of $\hat{p}$, so it also satisfies $(\eps,\delta)$-DP. 
%%Note that for any estimator $\hat {\mu}$ and any distribution $\p_e$, if we have $\hat p (2i-1) < \hat p(2i) $ and $e(i)=1$. Then
%%\[
%%	\frac{1}{2} \Paren{ |\hat{\p}(2i -1) - \p_e(2i-1)| + |\hat{\p}(2i) - \p_e(2i)|} \ge \frac12|\p_e(2i-1) - \p_e(2i)| = \frac{10 \alpha}{k}.
%%\]
%%
%%The same inequality holds if $\hat p (2i-1) \ge \hat p(2i) $ and $e(i)= -1$.
% For event $S$, let $\probofsub{e}{S}$ denote $\probofsub{\Xon \sim \p_e^{\ns}}{S}$. Hence for any $e \in \{\pm1\}^{\dims}$, we have
%\begin{align}
%          \expectationsub{\p_{e}}{d_{TV}(\hat p, \p_{e})} & \ge C_1 \sum_{i = 1}^{\dims} \expectationsub{\p_{e}}{ |\hat{\mu}(i) - \mu_e(i)|} \nonumber \\
%          %& \ge  \frac{10\alpha}{k} \sum_{i=1}^{\dims} \Big[ \mathbb{I} (e(i)=1) \cdot \probofsub{e}{\hat p (2i-1) < \hat p(2i) } 
%          %+  \mathbb{I} (e(i)  = -1) \cdot \probofsub{e}{\hat p (2i-1) >\hat p(2i) } \Big] \nonumber \\
%          &\ge  \frac{C_1\alpha}{\dims} \sum_{i=1}^{\dims} \Big[ \mathbb{I} (e(i)  =1 ) \cdot \probofsub{e}{\he(i)  =-1} 
%           +  \mathbb{I} ({e(i)}  = -1) \cdot \probofsub{e}{ \he_i =+1} \Big] \nonumber\\
%	 &\ge \frac{C_1}{C_2}\expectationsub{\p_{e}}{d_{TV}(\p_{\he},\p_{e})}.\nonumber
%\end{align}
%
%Hence we have:
%\begin{align}
%	R(n, \cC_{\dims}, d_{TV}, \eps, \delta) & %= \min_{\hat p: \hat p \text{ is }(\eps,\delta)-DP} \max_{\p \in \cP} \EE_{\Xon \sim \p^n}\left[d_{TV}(\hat p(\Xon),\p)\right] \nonumber \\
%		 \ge  \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}} \max_{e \in \cE_{\dims} } \EE_{\Xon \sim \p_e^n} \left[d_{TV}(\hat p,\p_e)\right] \nonumber \\
%		& \ge\frac{C_1}{C_2} \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}}\max_{e \in \cE_{\dims}} \EE_{\Xon \sim \p^{\ns}_e} \left[d_{TV}(\p_{\he},\p_e)\right] \nonumber \\
%		& =\frac{C_1}{C_2} \min_{\he: \he \text{ is $(\eps,\delta)$-DP}} \max_{\p_e^{\ns} \in \cV_{\dims} } \EE_{\Xon \sim \p_e^{\ns}} \left[\ell(\p^{\ns}_{\he},\p_e^{\ns})\right]. \nonumber 
%\end{align}

%Since $\sup_{\p_e \in \cV_{\ab} }\mathbb{E}_{\p_e} [d_{TV}(\hat{\p}, \p_e)]<  \sup_{\p \in \cC_{\dims} }\mathbb{E}_{\p} [d_{TV}(\hat{\p}, \p)] \le \dist$, we have $R(n,  \cV_{\dims}, \ell, \eps, \delta) \le 2\dist$. By Theorem~\ref{thm:assouad}, we have
%$$\sum_{i=1}^{\frac{\ab}{2}} \probofsub{+i }{ \hat {E}(i) \neq 1 } + \probofsub{-i }{\hat {E}(i) \neq -1 } \leq \frac{k}{5},$$
%where
%\[
%\probofsub{+i }{S} = \probof{S | e(i) = +1} =   \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= + 1}\probof{S| E= e},
%\]
%\[
%\probofsub{-i }{ S } =\probof{S | e(i) = -1} =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= - 1}\probof{S | E= e} .
%\]
%Recall the definition of the two mixtures of distributions: \amargin{We just recalled this two pages ago. How many times should we recall?}
%$$
%\dP_{+i}  =  \frac{2}{|\cE_{\dims}|} \sum_{e \in \cE_{\dims}: e(i)= + 1} \p^{\ns}_e, ~~~ \dP_{-i}  =  \frac{2}{|\cE_{\dims}|} \sum_{e \in \cE_{\dims}: e(i)= -1}\p^{\ns}_e.
%$$
{Let $D$ be an upper bound on the expected Hamming distance for a coupling between $\dP_{+i}$ and $\dP_{-i}$ over all $i$.  Since $\cV_{\dims} \subset \Delta_{2,\dims}$, applying Theorem~\ref{thm:assouad} with Lemma~\ref{lem:binaryproducttv} we have
\[
R(\cP, d_{TV}, \eps, \delta) \ge \frac{C_1\alpha}{2\dims} \cdot \dims \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta} = \frac{C_1\alpha}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}. 
\]}

{Setting $R(\cP, d_{TV}, \eps, \delta) \le \alpha$, we get $D =\Omega\Paren{\frac1\eps}$ or $D =\Omega\Paren{\frac1\delta}$, or equivalently, $D =\Omega\Paren{\frac1{\eps+\delta}}$. Lemma~\ref{lem:coupling_distance} below shows that we can take $ D =\frac{40\dist\ns}{\dims}$, which proves the result.}
\end{proof}

\begin{lemma} \label{lem:coupling_distance}
There is a coupling between $(X,Y)$ between $\dP_{+i}$ and $\dP_{-i}$, such that
$\expectation{\ham{X}{Y}} \le \frac{40\dist \ns}{\dims}.$
\end{lemma}

\begin{proof}
We generate $Y\sim \dP_{-i}$ from $X\sim\dP_{+i}$ as follows. If the $i$th coordinate of a sample $X$ is $+1$, we independently flip it to $-1$ with probability  $\frac{40\alpha}{1+20\alpha}$ to obtain a sample $Y$. The expected Hamming distance is bounded by $\frac{40\alpha}{1+20\alpha} \cdot \frac{1+20\alpha}{\dims} \cdot \ns = \frac{40\alpha \ns}{\dims}$. 
\end{proof}



==> back_up/toolbox copy/coding-proofs.tex <==
\section{Proofs of existence of codes (Lemma~\ref{lem:GV} and Lemma~\ref{lem:constantGV2})}
\label{sec:codes}
%\amargin{This entire section is new, please read it thoroughly. I have changed the equations in Lemma~\ref{lem:GV}!}

\begin{proof}[Proof of Lemma~\ref{lem:GV}]
{This proof is a standard argument for Gilbert-Varshamov bound applied to constant weight codes. We use the following version (Theorem 7 in~\cite{GrahamS80}).}
\begin{lemma}
\label{lem:constantGV}
{There exists a length-$k$ constant weight binary code $\cC$ with weight $l$ and minimum Hamming distance $2\delta$, with $$\absv{\cC} \ge \frac{\binom{\ab}{l}}{\sum_{i=0}^{\delta} \binom{l}{i} \binom{\ab-l}{i}}.$$}
\end{lemma}
Applying this Lemma with $2\delta=\frac{l}{4}$, we have
\begin{align}
\absv{\cC} &\ge \frac{\binom{\ab}{l}} {\sum_{j=0}^{l/8} \binom{l}{j} \cdot \binom{\ab-l}{j}}\nonumber  \ge \frac{\binom{\ab}{l}}{\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} \cdot \binom{\ab}{\frac{l}{8}}}
  = \frac1 {\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} } \cdot \prod_{i = 0}^{\frac{7l}{8}- 1} \frac{k - \frac{l}{8}-i}{l - i} \\
& \ge \frac{2\sqrt{7} \pi}{e} \cdot (0.59)^{\frac{7l}{8}} \cdot \Paren{ \frac{\ab-\frac{l}{8}}{l}}^{\frac{7l}{8}} \label{eqn:gv-step}\\
 &\ge \Paren{\frac{\ab}{2^{7/8}l}}^{\frac{7l}{8}}, \nonumber 
\end{align}
{In~\eqref{eqn:gv-step}, we note that $\frac{k - \frac{l}{8}-i}{l - i}$ is monotonically increasing as $i$ increases.} And the first part is obtained by the Stirling's approximation $\sqrt{2\pi}\cdot l^{l+\frac12} \cdot e^{-l} \le l! \le e \cdot l^{l+\frac12} \cdot e^{-l}$ and the fact that $1.1^l \ge \sqrt{l}$ when $l \ge 20$. The last inequality comes from $l \le k/2$ and $15/16 \times 0.59 > 1/2^{7/8}$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:constantGV2}]
By the Gilbert-Varshamov bound (Lemma~\ref{lem:constantGV}),
\[
	\absv{\cH} \ge \frac{h^\dims}{\sum_{j=0}^{\frac{d}{2}-1} \binom{\dims}{j}(h-1)^j} \ge \frac{h^\dims}{\frac{\dims}{2} \cdot \binom{\dims}{\frac{\dims}{2}} \cdot h^{\frac{\dims}{2}}} \ge
	\frac{h^{\frac{\dims}{2}}} { \dims \cdot 2^{\dims} }  \ge \left(\frac{h}{16}\right)^{\frac{\dims}{2}}.
\]
\end{proof}

==> back_up/toolbox copy/gaussian.tex <==
\subsection{Gaussian mixtures 	estimation} \label{sec:gaussian}

%In this section, we show that our private Fano's inequality can be applied to derive the sample complexity lower bound of learning mixtures of distributions.   

%\begin{definition}
%	Let $\cG$ be some set of distributions. A $\ab$-mixture of $\cG$ is a distribution with density $\sum_{j=1}^{\ab} w_j \p_j$, where each $\p_j \in \cG$ and $\sum_{j=1}^{\ab} w_j =1$.
%\end{definition}

Recall $\cG_{\dims} = \{ \cN (\mu, I_d): \norm{\mu}\le R\}$ is the set of $\dims$-dimensional spherical Gaussians with unit variance and bounded mean and $\cG_{\ab,\dims} = \{ \p: \p \text{ is a $\ab$-mixture of } \cG_{\dims} \}$ consists of mixtures of $k$ distributions in $\cG_{\dims}$.~\cite{BunKSW2019} proves an upper bound of $\widetilde{O}\Paren{\frac{\ab\dims}{\dist^2}+\frac{\dims}{\dist\eps}}$ for estimating $k$-mixtures of Gaussians. We provide a sample complexity lower bound for estimating mixtures of Gaussians in Theorem~\ref{thm:main_Gaussian}, which matches the upper bound up to logarithmic factors. 

\begin{theorem}
\label{thm:main_Gaussian}
Given $\ab \le \dims$ and $R\ge \sqrt{64\log\Paren{\frac{8\ab}{\dist}}}$, {or $\ab \ge \dims$ and $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$,}
\begin{align}
&S(\cG_{\ab, \dims}, d_{TV}, \alpha, \eps) = \Omega \Paren{\frac{\ab\dims}{\dist^2}+\frac{\ab\dims}{\dist \eps}}. \nonumber
\end{align}
\end{theorem}

\begin{proof}
	
{We first consider the case when $\ab \le \dims$ and $R\ge \sqrt{64\log\Paren{\frac{8\ab}{\dist}}}$.} Let $\cC$ denote the codebook in Lemma~\ref{lem:GV} with weight $l=\frac{\dims}{2}$. Then we have $|\cC| \ge 2^{\frac{7\ab}{128}}$. Given $c_i$ in codebook $\cC$, we construct the following $\dims$-dimensional Gaussian distribution $\p_i$, with identity covariance matrix and mean $\mu_i$ satisfying %\amargin{This looks like the third time ... but this is ok this time I think}
%\[\mu_{i} (j)  = \left\{
%\begin{array}{rcl}
%+ \frac{\dist}{\sqrt{ \dims}} ,       &      & \text{for ~ } c_i (j)=1,\\
%- \frac{\dist}{\sqrt{\dims}},       &      & \text{for ~ } c_i (j)=0.
%\end{array} \right.
%\]

\[\mu_{i,j}  = \frac{\dist}{\sqrt{ \dims}} c_{i,j},\]
{ where   $\mu_{i,j}$ denotes the $j$-th coordinate of $\mu_i$.}

{Let $h = \absv{\cC}$. Similar to the product distribution case, using Lemma~\ref{lem:constantGV2}, we can get an $h$-ary codebook $\cH$ with length $d$ and minimum hamming distance $d/2$. Moreover, $|\cH| \ge (\frac{h}{16})^{\frac{\dims}{2}}$. }


$\forall i \in [h]$ and $j \in k$, define $\p_{i}^{(j)} = \cN(\mu_i + \frac{R}{2}e_j , I_d)$, where $e_j$ is the $j$th standard basis vector. It is easy to verify their means satisfy the norm bound. %By Claim~\ref{claim:constantGV2}, there exists an $h$-ary code $\cH \subset [h]^\ab$ with code length $\ab$ and minimum Hamming distance $\frac{\ab}{2}$, which satisfies $\absv{\cH} \ge (\frac{h}{16})^{\frac{\ab}{2}}$. 
For a codeword $b \in \cH$, let
\[
	\mP_b = \frac1k \Paren{ \p_{b_1}^{(1)} +  \p_{b_2}^{(2)}  +\ldots + \p_{b_k}^{(k)} }.
\]

Let $\cV_{\cG} = \{ \mP_b: b \in \cH\}$ be the set of the distributions defined above. Next we prove that $\forall \mP_b \neq \mP_{b'}\in \cV_{\cG}$, 
\begin{align}
	\dtv{\mP_b}{\mP_{b'}} \ge C \alpha, \label{eqn:dtv_gaussian} \\
	\dkl{\mP_b}{\mP_{b'}} \le 4 \alpha^2.\label{eqn:dkl_gaussian}
\end{align}
where $C$ is a constant. If these two inequalities hold, using~\eqref{eqn:dkl_gaussian}, by Pinsker's Inequality, we get $\dtv{\mP_b}{\mP_{b'}} \le \sqrt{2\dkl{\mP_b}{\mP_{b'}}  } \le 2\sqrt2\alpha$. Using Corollary~\ref{coro:fano}, we get
\[
S(\cG_{\ab, \dims}, d_{TV}, \alpha, \eps) =\Omega \Paren{\frac{\ab\dims}{\alpha^2}+\frac{\ab\dims}{\alpha \eps}}.
\]
It remains to prove~\eqref{eqn:dtv_gaussian} and~\eqref{eqn:dkl_gaussian}.

For~\eqref{eqn:dkl_gaussian}, note that for any distribution pair $\mP_b \neq \mP_{b'} \in \cV_{\cG}$,
\begin{align}
\dkl{\mP_b}{\mP_{b'}} &\le \frac1{k} \sum_{t=1}^{\ab} \dkl{\p^{(t)}_{b_t}}{\p^{(t)}_{b'_{t}}}\le \max_{i,j \in [h]} d_{KL}\Paren{\p_i, \p_j} \le 4\dist^2, \nonumber
\end{align}
{where the first inequality comes from the convexity of $KL$ divergence and the last inequality uses the fact that the KL divergence between two Gaussians with identity covariance is at most the $\ell_2^2$ distance between their means.} 

Next we prove~\eqref{eqn:dtv_gaussian}. Let $B_j = B_{j,1} \times \cdots \times B_{j,\dims}$, where

$$B_{j,i}=
\begin{cases}
[ \frac{R}{4}, \frac{3R}{4}], & \text{when $i=j$,}\\
[ -\frac{R}{4}, \frac{R}{4} ], & \text{when $i \neq j$ and $i \le \ab$,}\\
[-\infty, \infty], & \text{when $\ab<i \le \dims$.}
\end{cases}$$

Then by Gaussian tail bound and union bound, for any $\mP \in \cV_{\cG}$, the mass of the $j$-th Gaussian component outside $B_j$ is at most $2ke^{-\frac12 \cdot \Paren{\frac1{4} R}^2}$. And the mass of other Gaussian components inside $B_j$ is at most $e^{-\frac12 \cdot \Paren{\frac1{4} R}^2}$. Hence we have:
\begin{align}
	\dtv{\mP_b}{\mP_{b'}} &= \frac1{2\ab} \int_{z \in \RR^{\dims}} \absv{ \p_{b_1}^{(1)}(z) +\cdots+ \p_{b_{\ab}}^{(\ab)}(z)  - \p_{b'_{1}}^{(1)}(z)  - \cdots -  \p_{b'_{\ab}}^{(\ab)}(z) }  dz \nonumber\\
	&\ge \frac1{2\ab}  \sum_{j=1}^{\ab} \int_{z \in B_j} \absv{ \p_{b_1}^{(1)}(z) +\cdots+ \p_{b_{\ab}}^{(\ab)}(z)  - \p_{b'_{1}}^{(1)}(z)  - \cdots -  \p_{b'_{\ab}}^{(\ab)}(z) }  dz \nonumber\\
	& \ge \frac1{2\ab} \cdot \sum_{j=1}^{\ab} (\int_{z \in B_j}  \absv{  \p_{b_{j}}^{(j)}(z)  - \p_{b'_{j}}^{(j)}(z) } dz -(\ab - 1) \cdot e^{-\frac12 \cdot \Paren{\frac1{4} R}^2}) \nonumber \\
	& \ge \frac1{2\ab} \cdot \sum_{j=1}^{\ab} (\int_{z \in \RR^{\dims}}  \absv{  \p_{b_{j}}^{(j)}(z)  - \p_{b'_{j}}^{(j)}(z) } dz - 3\ab \cdot e^{-\frac12 \cdot \Paren{\frac1{4} R}^2}) \nonumber \\
	& = \frac1{2\ab} \cdot \sum_{j=1}^{\ab} \dtv{\p_{b_{j}}}{\p_{b'_{j}}} - \frac{3\dist^2}{64k}. \nonumber
\end{align}
By Fact 6.6 in~\cite{KamathLSU18}, there exists a constant $C_1$ such that for any pair $i \neq j \in [h]$, 
$$\dtv{\p_i}{\p_j} \ge C_1\dist.$$
Hence we have
\[
	\frac1{2\ab} \cdot \sum_{j=1}^{\ab} \dtv{\p_{b_{j}}}{\p_{b'_{j}}} \ge \frac{C_1\dist}{2\ab} \ham{b}{b'} \ge \frac{C_1\dist}{4},
\]
where the last inequality comes from the property of the codebook. WLOG, we can assume $
\frac{3\dist}{64k} < C_1/8$. Taking $C = \frac{C_1}{8}$ completes the proof of~\eqref{eqn:dtv_gaussian}.

%\begin{align}
%\dtv{P}{Q} &= \frac1{2\ab} \int_{z \in \RR^{\dims}} \absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%&\ge \frac1{2\ab}  \sum_{j=1}^{\ab} \int_{z \in B_j}\absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%& \ge \frac1{2\ab} \cdot \frac{\ab}{2} (C_1\dist - 2\ab\cdot e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}) \ge \frac14 \Paren{C_1 -\frac{1}{4}}\dist.
%\end{align}
%where in the last inequality, we only look at the balls such that $i_j$ differs from $i^{\prime}_j$, and there exists at least $\frac{\ab}{2}$ such balls by the property of the codebook. Besides, by Gaussian tail bound, for the other component other than $j$, it has at most $e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}$ mass in ball $j$.
%

%Let $h = \absv{\cC}$ denote the size of the codebook. Now we have designed a class of $h > 2^{\frac{\dims}{8}}$ distributions around the origin. Let $\cG = \{ \p_1, \p_2,\cdots, \p_h\}$. We note that by  For a distribution $\p$ over $\reals^{\dims}$ and $v \in \RR^{\dims}$, we define $\p+ v$ to be the distribution $\p$ shifted by $v$. 
%
%Now we are able to design the set of Gaussian mixtures. Each $(i_1, \cdots,i_k) \in [h]^\ab$ corresponds to the mixture of $\ab$ spherical Gaussians, with density
%$$ \frac1k \Paren{ \p_{i_1,1} +  \p_{i_2,2} +\cdots+ \p_{i_k,k}},$$
%where for $i \in [h]$ and $j \in [\ab]$, $\p_{i,j}\coloneqq \p_i + v_j$.
%Then by Claim~\ref{claim:constantGV}, there exists a $h$-ary code $\cH$ with code length $\ab$ and minimum Hamming distance $\frac{\ab}{2}$, which satisfies $\absv{\cH} \ge (\frac{h}{16})^{\frac{\ab}{2}}$. This implies that among the $h^{\ab}$ distributions, there exist a set of $\absv{\cH} \ge (\frac{h}{16})^{\frac{\ab}{2}}$ distributions among which any pair of tuples $(i_1,\cdots,i_k)$ and $(i^{\prime}_1,\cdots,i^{\prime}_k)$ corresponding to two distributions has Hamming distance at least $\frac{\ab}{2}$. We denote this distribution set as 
%$\cV_{\ab, \dims}$.
%
%Now let we set $v_j, j \in [\ab]$ far apart each other, in order to reduce the overlapping between each component of the mixture. To be specific, we set 
%$j \in [\ab], v_j = B \cdot t_j$, where $t_j$ is $j$-th standard basis vector. %We note that for any pair $i,j \in [\ab]$, $\norm{v_i-v_j} = \sqrt{2}B$.
%
%Following the same routine, we want to prove that for any pair $P, Q \in \cV_{\ab,\dims}$, $\dtv{P}{Q} \ge C_2\dist$ for some constant $C_2$. Let $P = \frac1\ab \Paren{ \p_{i_1,1} +  \p_{i_2,2} +\cdots+ \p_{i_\ab,\ab}}$, $Q  = \frac1\ab \Paren{ \p_{i^{\prime}_1,1} +  \p_{i^{\prime}_2,2} +\cdots+ \p_{i^{\prime}_\ab,\ab}}$, and we use $B_j$ to denote the $\dims$-dimensional ball with centre $v_j$ and radius $\frac{R}{2}$,
%\begin{align}
%\dtv{P}{Q} &= \frac1{2\ab} \int_{z \in \RR^{\dims}} \absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%&\ge \frac1{2\ab}  \sum_{j=1}^{\ab} \int_{z \in B_j}\absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%& \ge \frac1{2\ab} \cdot \frac{\ab}{2} (C_1\dist - 2\ab\cdot e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}) \ge \frac14 \Paren{C_1 -\frac{1}{4}}\dist.
%\end{align}
%where in the last inequality, we only look at the balls such that $i_j$ differs from $i^{\prime}_j$, and there exists at least $\frac{\ab}{2}$ such balls by the property of the codebook. Besides, by Gaussian tail bound, for the other component other than $j$, it has at most $e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}$ mass in ball $j$.
%
%
%By similar argument with Lemma~\ref{lem:reduction}, we can show $S(\cG_{\ab, \dims}, d_{TV}, \alpha, \eps)  \ge \Smc{\cV_{\ab, \dims}, \eps}$. Hence it is enough to show  $\Smc{\cV_{\ab, \dims}, \eps}=\Omega \Paren{\frac{\ab\dims}{\alpha^2}+\frac{\ab \dims}{\alpha \eps}}.$ Note that for any distribution pair $P,Q \in \cV_{\ab,\dims}$,
%\begin{align}
%	D_{KL} (P,Q) &\le \frac1{k} \sum_{j=1}^{\ab} D_{KL} (\p_{i_j},\p_{i^{\prime}_j}) \le \max_{i,j \in [h]} d_{KL}\Paren{\p_i, \p_j} \le 4\dist^2, \nonumber
%\end{align}
%where the first equality comes from the convexity of KL divergence. By Pinsker's inequality, $d_{TV}(P, Q) \le \sqrt{2D_{KL} (P,Q) } \le 2\sqrt2\alpha$.  Finally by Theorem~\ref{thm:fano} and the fact that $\exists c_1, c_2>0 , \absv{\cH} > c_1 \cdot 2^{c_2 \cdot \ab \dims}$, we have $\Smc{\cV_{\ab,\dims}, \eps} =\Omega \Paren{\frac{\ab\dims}{\alpha^2}+\frac{\ab\dims}{\alpha \eps}}$.

%\newhzz{Now we move to the case when $\ab \ge \dims$ and $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$. Let $r = \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$, we note that there exists a $r$-packing $S \subset \mathbb{R}^{\dims}$ with $|S| = \ab$ since $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$. Here we consider the same construction of the set of distributions as in the previous case, except that we set the centers of the $\ab$ components to be the points in $S$. Let $B_j$ denote the $\ell_2$ ball centering at the $j$-th point of $S$ with radius $\frac{r}{2}$. We note that by the tail bound of the Chi-squared distribution, the mass of the $j$-th Gaussian component outside $B_j$ is at most $O\Paren{\frac{\dist}{\ab}}$. Meanwhile, the mass of other Gaussian components inside $B_j$ is also at most $O\Paren{\frac{\dist}{\ab}}$. All the other analysis follows from the previous case.}

{Now we considers the case when $\ab \ge \dims$ and $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$. Let $r = \sqrt{16\dims \log\Paren{\frac{8\ab}{\dist}}}$, we note that there exists a packing set $S = \{v_1, v_2, ..., v_k\} \subset \mathbb{R}^{\dims}$ which satisfies $\forall u, v \in S$,
	\[
		\norm{u - v} > r,~~~~ \norm{u}\le R,~~~~, \norm{v}\le R/3, 
	\]
	and $|S| = \ab$ since $R\ge 2 (\ab)^{\frac1\dims}  r$. Consider the set of mixture distributions as following: 
	For a codeword $b \in \cH$, let
	\[
		\mP'_b = \frac1k \Paren{ \p_{b_1}^{(1)'} +  \p_{b_{2}}^{(2)'}  +\ldots + \p_{b_{\ab}}^{(k)'} },
	\]
	where $\forall i \in [k], \p_{b_j}^{(j)'} = \cN(\mu_{b_j} + v_j, I_d)$.
	Let $B'_j$ denote the $\ell_2$ ball centering at the $v_j$ with radius $\frac{r}{2}$. We note that by similar analysis using the tail bound of the Gaussian distribution, the mass of the $j$-th Gaussian component outside $B_j'$ is at most $\frac{\dist^2}{64\ab^2}$. Meanwhile, the mass of other Gaussian components inside $B_j'$ is also at most $\frac{\dist^2}{64\ab^2}$. Hence the remaining analysis follows from the previous case.}
\end{proof}

==> back_up/toolbox copy/glodef.tex <==
% Theorem-like environments

\usepackage{lmodern}
%\usepackage{xspace}
\usepackage[protrusion=true,expansion=true]{microtype}
%\usepackage{fullpage}
\usepackage{amsfonts, pbox}

% Colors (with names)

% Colors (with names)
%\usepackage[usenames,dvipsnames,table,xcdraw]{xcolor}


%\usepackage[usenames,dvipsnames,table]{xcolor}
%\usepackage[colorlinks,citecolor=blue, bookmarks=true]{hyperref}

% Required for the table of results
\usepackage{multirow}
\usepackage{dsfont} %\indic
%\usepackage{fullpage}

\newcommand{\insertref}[1]{\todo[color=green!40]{#1}}
\newcommand{\explainindetail}[1]{\todo[color=red!30]{#1}}
\newcommand{\inlinetodo}[1]{\todo[color=blue!25,inline]{#1}}

% Algorithm environment
%\usepackage{algorithmicx,algpseudocode,  algorithm}
\providecommand\algorithmname{Algorithm}
\providecommand*{\factautorefname}{Fact}

% compact lists, and handy shortcuts for items
\usepackage[shortlabels]{enumitem}
\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
\setenumerate{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}


\makeatletter
\@ifundefined{theorem}{% Theorems (each with its own style)
  \theoremstyle{plain}
  \newtheorem{theorem}{Theorem}
  \newtheorem{corollary}[theorem]{Corollary}
  %\newtheorem{corollary}{Corollary}
  \newtheorem{lemma}[theorem]{Lemma}
  \newtheorem{claim}[theorem]{Claim}
  \newtheorem{fact}{Fact}
  \newtheorem*{unnumberedfact}{Fact}
   \theoremstyle{definition}
  \newtheorem{definition}[theorem]{Definition}
  \theoremstyle{remark}
  \newtheorem{remark}{Remark}
  \newtheorem{question}{Question}
  \newtheorem*{notation}{Notation}
  \newtheorem{example}{Example}
  \newtheorem{observation}{Observation}
}{}
\makeatother
\newenvironment{proofof}[1]{\noindent{\bf Proof of {#1}:~~}}{\(\qed\)}

% Begin / End Theorems

\def \bthm#1{\begin{#1}\upshape\quad}
\def \ethm#1{\rqed\end{#1}}
\def \ethmp#1{\end{#1}}     % No box, when ends in displayed equation

\def \bClaim     {\bthm{Claim}}
\def \eClaim     {\ethm{Claim}}
\def \eClaimp    {\ethmp{Claim}}
\def \bConjecture {\bthm{Conjecture}}
\def \eConjecture {\ethm{Conjecture}}
\def \eConjecturep{\ethmp{Conjecture}}
\def \bCorollary {\bthm{Corollary}}
\def \eCorollary {\ethm{Corollary}}
\def \eCorollaryp{\ethmp{Corollary}}
\def \bCounter   {\bthm{CounterExample*}}
\def \eCounter   {\ethm{CounterExample*}}
\def \eCounterp  {\ethmp{CounterExample}}
\def \bDefinition{\bthm{Definition}}
\def \eDefinition{\ethm{Definition}}
\def \eDefinitionp{\ethmp{Definition}}
\def \bExample   {\bthm{Example}}
\def \eExample   {\ethm{Example}}
\def \eExamplep  {\ethmp{Example}}
\def \bExercise  {\bthm{Exercise}}
\def \eExercise  {\ethm{Exercise}}
\def \eExercisep {\ethmp{Exercise}}
\def \bIntuition {\bthm{Intuition}}
\def \eIntuition {\ethmp{Intuition}}
\def \bJoke      {\bthm{Joke}}
\def \eJoke      {\ethm{Joke}}
\def \bLemma     {\bthm{Lemma}}
\def \eLemma     {\ethm{Lemma}}
\def \eLemmap    {\ethmp{Lemma}}
\def \bOpen      {\bthm{Open problem}}
\def \eOpen      {\ethm{Open problem}}
\def \eOpenp     {\ethmp{Open problem}}
\def \bProperty  {\bthm{Property}}
\def \eProperty  {\ethm{Property}}
\def \ePropertyp {\ethmp{Property}}
\def \bQuestion  {\bthm{Question}}
\def \eQuestion  {\ethm{Question}}
%\def \bRemark    {\bthm{Remark}}
%\def \eRemark    {\ethm{Remark}}
\def \bResult    {\bthm{Result}}
\def \eResult    {\ethm{Result}}
\def \bTheorem   {\bthm{Theorem}}
\def \eTheorem   {\ethm{Theorem}}
\def \eTheoremp  {\ethmp{Theorem}}

% Environments

\newenvironment{Problem}{\textbf{Problem}\\ \begin{enumerate}}{\end{enumerate}}
\newenvironment{Problems}{\textbf{Problems}\\ \begin{enumerate}}{\end{enumerate}}

%\newenvironment{Problems}{\begin{trivlist}\item[]{\textbf{Problems}}{\end{trivlist}}}

% Headers

\def \skpbld#1{\par\noindent\textbf{#1}\quad}
\def \skpblds#1{\skpbld{#1}\par\noindent}

\def \Answer   {\skpbld{Answer}}
\def \Answers  {\skpblds{Answers}}
\def \Basis    {\skpbld{Basis}}
\def \Check    {\skpbld{Check}}
%\def \Example  {\skpbld{Example}}
\def \Examples {\skpbld{Examples}}
\def \Intuition{\skpbld{Intuition}}
\def \Method   {\skpbld{Method}}
\def \Methods  {\skpblds{Methods}}
\def \Outline  {\skpbld{Outline}}
\def \Proof    {\skpbld{Proof}}
\def \Proofs   {\skpblds{Proofs}}
%\def \Problem  {\skpbld{Problem}}
%\def \Problems {\skpblds{Problems}}
\def \Proline  {\skpbld{Proof Outline}}
%\def \Remark   {\skpbld{Remark}}
\def \Remarks  {\skpblds{Remarks}}
\def \Solution {\skpbld{Solution}}
\def \Solutions{\skpblds{Solutions}}
\def \Verify   {\skpbld{Verify}}
\def \Step     {\skpbld{Step}}

% Ignores

\newcommand{\ignore}[1]{}

% Problems & solutions

\newcommand{\problem}[1]{#1}
\newcommand{\solution}[1]{{\\ \bf Solution}\quad #1}
%\newcommand{\solution}[1]{\mbox{}\\ \medskip\noindent{\bf Solution\medskip}#1}
%\newcommand{\solution}[1]{}

\newcommand{\source}[1]{(Taken from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\modifiedfrom}[1]{(Modified from~\cite{#1})}
%\newcommand{\modifiedfrom}[1]{}

\newcommand{\takenfrom}[1]{(Taken from~\cite{#1})}
%\newcommand{\takenfrom}[1]{}

\newcommand{\reportedby}[1]{Reported by #1.}
%\newcommand{\reportedby}[1]{}

\newcommand{\hint}[1]{Hint: #1}
%\newcommand{\hint}[1]{}

\newcommand{\joke}[1]{\footnote{#1}}
\newcommand{\trivia}[1]{\footnote{#1}}

% Equation formatting

\newcommand{\spreqn}[1]{{\qquad\text{#1}\qquad}}

% Blackboard fonts
\newcommand{\II}{\mathbb{I}} % Added by Theertha on April 16th 2013.
\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}

% probability
\newcommand{\expectation}[1]{\EE\left[#1\right]}
\newcommand{\variance}[1]{Var\left(#1\right)}

% Number sets

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\positives}{\PP}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}

\newcommand{\realsge}{{\reals_{\ge}}}
\newcommand{\realsp}{\reals^+}
\newcommand{\integersp}{\integers^+}
\newcommand{\integerss}[1]{\integers_{\ge{#1}}}

% boldface

\def \ba     {{\bf a}}
\def \bx     {{\bf x}}
\def \by     {{\bf y}}

\def \bA     {{\bf A}}
\def \bB     {{\bf B}}
\def \bC     {{\bf C}}
\def \bD     {{\bf D}}
\def \bF     {{\bf F}}
\def \bG     {{\bf G}}
\def \bL     {{\bf L}}
\def \bQ     {{\bf Q}}
\def \bR     {{\bf R}}
\def \bS     {{\bf S}}
\def \bT     {{\bf T}}
\def \bX     {{\bf X}}
\def \bY     {{\bf Y}}
\def \bZ     {{\bf Z}}

% caligraphics

\def \cA     {{\cal A}}
\def \cB     {{\cal B}}
\def \cC     {{\cal C}}
\def \cD     {{\cal D}}
\def \cE     {{\cal E}}
\def \cF     {{\cal F}}
\def \cG     {{\cal G}}
\def \cH     {{\cal H}}
\def \cI     {{\cal I}}
\def \cK     {{\cal K}}
\def \cL     {{\cal L}}
\def \cM     {{\cal M}}
\def \cN     {{\cal N}}
\def \cO     {{\cal O}}
\def \cP     {{\cal P}}
\def \cQ     {{\cal Q}}
\def \cR     {{\cal R}}
\def \cS     {{\cal S}}
\def \cT     {{\cal T}}
\def \cU     {{\cal U}}
\def \cV     {{\cal V}}
\def \cW     {{\cal W}}
\def \cX     {{\cal X}}
\def \cY     {{\cal Y}}
\def \cZ     {{\cal Z}}

% vectors

\def \vct#1{{\overline{#1}}}

\def \vcta  {{\vct a}}
\def \vctb  {{\vct b}}
\def \vctq  {{\vct q}}
\def \vcts  {{\vct s}}
\def \vctu  {{\vct u}}
\def \vctv  {{\vct v}}
\def \vctx  {{\vct x}}
\def \vcty  {{\vct y}}
\def \vctz  {{\vct z}}
\def \vctp  {{\vct p}}

\def \vctV  {{\vct V}}
\def \vctX  {{\vct X}}
\def \vctY  {{\vct Y}}
\def \vctZ  {{\vct Z}}

\def \vctbeta  {{\vct\beta}}

% Random variables

\newcommand{\rnd}[1]{{\boldsymbol #1}}

\newcommand{\rndd}{{\rnd d}}
\newcommand{\rndl}{{\rnd l}}
\newcommand{\rndp}{{\rnd p}}
\newcommand{\rnds}{{\rnd s}}
\newcommand{\rndx}{{\rnd x}}
\newcommand{\rndy}{{\rnd y}}
\newcommand{\rndz}{{\rnd z}}

%\newcommand{\poi}{{\rm poi}}
\newcommand{\Var}{{\rm Var}}

% following should not exist (indicate random sets)

\newcommand{\rndR}{{\rnd R}}
\newcommand{\rndT}{{\rnd T}}

% arrow vectors

\newcommand{\rvc}{{\overrightarrow c}}

% Abbreviations - \xspace puts space iff there is space after command

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish
%\newcommand{\iid}{\textit{i.i.d.}\xspace} 
\newcommand{\iid}{\textit{i.i.d.}} % Edit by Theertha, \xspace not compiling

\newcommand{\etc}{etc.\@\xspace}

% Colors

%\definecolor{light}{gray}{.75}


% marginal notes

\newcommand{\mrgs}[2]{\# #1 \#{\marginpar{#2}}}

\newcommand{\mrgcgd}[1]{\mrgs{#1}{CHANGED}}
\newcommand{\mrgchk}[1]{\mrgs{#1}{CHECK}}
\newcommand{\mrgfix}[1]{\mrgs{#1}{FIX}}
\newcommand{\mrgnew}[1]{\mrgs{#1}{NEW}}

% qed's --  Also consider \qedhere

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}

\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \ok    {1\upto k}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \set#1#2{{\sets{{#1}\upto{#2}}}}

\def \setpmo   {\sets{\pm 1}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \setok    {\{\ok\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \inseg#1{{[#1]}} % use \intsgm instead
\newcommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations


%\DeclareMathOperator*{\union}{\cup}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Union}{\bigcup}  %Commented by Theertha on April 15

\newcommand{\unionl}{\union\limits}
\newcommand{\Unionl}{\Union\limits}
 
%\DeclareMathOperator*{\inter}{\cap}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Inter}{\bigcap}   %Commented by Theertha on April 15

\newcommand{\interl}{\inter\limits}
\newcommand{\Interl}{\Inter\limits}

% Floors, Ceilings, Absolute value

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}
\def \absvlu#1{{|#1|}}
\def \Absvlu#1{{\left|{#1}\right|}}
\newcommand{\absv}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|_2}
% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}
\def \Brace#1{\left\{#1\right\}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory

\newcommand{\base}[2]{{[#1]_{#2}}}

% equalities

\newcommand{\ed}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{{:=}}

\newcommand{\cnvprb}{\stackrel{\mathrm{p}}{\to}}
\newcommand{\cnvdst}{\stackrel{\mathrm{d}}{\to}}
\newcommand{\cnvas}{\stackrel{\mathrm{a.s.}}{\to}}

\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

\newcommand{\al}[1]{\stackrel{\mathit{{#1}}}{<}}
\newcommand{\ag}[1]{\stackrel{\mathit{{#1}}}{>}}
\newcommand{\ale}[1]{\stackrel{\mathit{{#1}}}{\le}}
\newcommand{\age}[1]{\stackrel{\mathit{{#1}}}{\ge}}
\newcommand{\aeq}[1]{\stackrel{\mathit{{#1}}}{=}}

%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

\newcommand{\re}{\sim}
\newcommand{\rle}{\stackrel<\sim} % roughly (asymptotically taken) <=
%\newcommand{\rl}{\stackrel<\sim}
\newcommand{\rge}{\stackrel>\sim}
%\newcommand{\rg}{\stackrel>\sim}

\newcommand{\ere}{\approx} % exponentially roughly equal
\newcommand{\erle}{\stackrel<\approx}
%\newcommand{\erl}{\stackrel<\approx}
\newcommand{\erge}{\stackrel>\approx}
%\newcommand{\erg}{\stackrel>\approx}

% Relations

\newcommand{\independent}{\perp\!\!\!\perp}

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% probability

\newcommand{\pr}{{p}} % phase out in favor of \prb
\newcommand{\prb}{{p}} 

\newcommand{\prbs}[1]{{\prb^{(#1)}}}

\newcommand{\Prb}{\text{Pr}}
%\newcommand{\Pr}{{\text{Pr}}} % phase out in favor of \Prb
\newcommand{\Prn}{\text{Pr}}  % phase out in favor of \Prb

\newcommand{\Prs}[1]{\Pr\Paren{#1}} % phase out in favor of \Prbs
\newcommand{\Prbs}[1]{{\Prb^{(#1)}}} % Check if used - phase out
\newcommand{\probof}[1]{\Pr\Paren{#1}}

% notation

\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\newcommand{\flnpwr}[2]{{#1^{\underline{#2}}}} % Falling power

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\pfx}{{\prec}}
\newcommand{\pfxeq}{{\preceq}}

\newcommand{\sfx}{{\succ}}
\newcommand{\sfxeq}{{\succeq}}

% for old documents

\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{				% grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}


\newcommand{\Sparen}[1]{\left[#1\right]}
\newcommand{\Order}{O}
\newcommand{\order}{o}


\newtheorem{prop2}[theorem]{Proposition}
\newtheorem{lem2}[theorem]{Lemma}
\newtheorem{coro2}[theorem]{Corollary}







==> back_up/toolbox copy/intro2.tex <==
\section{Introduction}
{
Statistical estimation tasks are often characterized by the optimal trade-off between the sample size and estimation error. There are two steps in establishing tight sample complexity bounds: An information theoretic lower bound on sample complexity and an algorithmic upper bound that achieves it.}
%Statistical estimation tasks are often characterized by their rates or sample complexity which characterizes the optimal trade-off between the sample size and error in estimation. There are two parts to establishing sample complexity bounds: An information theoretic lower bound on sample complexity, and an algorithmic upper bound that achieves it.
Several works %\amargin{Get bunch of references from YU, BIN?}
have developed general tools to obtain the lower bounds (e.g.,~\cite{LeCam73, Assouad83, IbragimovK13, BickelR88, devroye1987course, verdu1994generalizing, CoverT06, ScarlettC19}, and references therein), {and three prominent techniques are Le Cam's method, Fano's inequality, and Assouad's lemma.} An exposition of {these three methods and their connections} is presented in~\cite{Yu97}\footnote{The title of~\cite{Yu97}, ``Assouad, Fano, and Le Cam'' is the inspiration for our title.}. 

%\noindent\textbf{Setting.} Let $\cP$ be a family of distributions over $\cX^\ns$, and let $\ell:\cP\times\cP\to\RR_{\ge0}$ be a distance measure between distributions in $\cP$. Here $\ns$ denotes the number of samples, and $\cX$ is the underlying domain of the individual samples.

In several estimation tasks, individual samples have sensitive information that must be protected. 
%has gathered much attention when the samples are collected from different users with the concern of each user's privacy.  %The data samples used in several applications can contain sensitive information about individuals who contribute to the samples. 
This is particularly of concern in applications such as healthcare, finance, geo-location, etc. Privacy-preserving computation has been studied in various fields including database, cryptography, statistics and machine learning~\cite{Warner65, Dalenius77, DinurN03, WassermanZ10, DuchiJW13, ChaudhuriMS11}. Differential privacy (DP)~\cite{DworkMNS06}, which allows statistical inference while preserving the privacy of the individual samples, has become one of the most {popular notions of privacy}~\cite{DworkMNS06, WassermanZ10, DworkRV10, BlumLR13, McSherryT07, DworkR14, KairouzOV17}. Differential privacy has been adopted by the US Census Bureau for the 2020 census and several large technology companies, including Google, Apple, and Microsoft~\cite{ErlingssonPK14, AppleDP17, DingKY17}.

\medskip
\noindent\textit{Differential privacy}~\cite{DworkMNS06}. {Let $\cX$ denote an underlying data domain of individual data samples} and {$\cX^\ns$ be the set of all possible length-$n$ sequences over $\cX$}. For $x, y\in \cX^\ns$, $\ham{x}{y}$ is their Hamming distance, the number of coordinates they differ at. A (randomized) estimator $\hat\theta:\cX^\ns\to\Theta$ is \emph{$(\eps,\delta)$-differentially private} (denoted {as} $(\eps,\delta)$-DP) if for any $S \subseteq \Theta$, and all $x, y\in\cX^\ns$ with $\ham{x}{y}\le 1$, the following holds:
	\begin{align}
		\probof{\hat\theta(x)\in S}\le e^{\eps} \cdot \probof{\hat\theta(y)\in S}+\delta.\label{eqn:dp-definition}
	\end{align}

The case $\delta=0$ is \emph{pure differential privacy} and is denoted by $\eps$-DP. We consider problems of parameter estimation and {goodness-of-fit (hypothesis testing)} under differential privacy constraints.
\medskip

\noindent\textbf{Setting.} Let $\cP$ be \emph{{any}} collection of distributions over $\cX^\ns$, {where $\ns$ denotes the number of samples.}\footnote{In the general setting, we are not assuming i.i.d. distribution over $\cX^\ns$, although we will specialize to this case later.} {Let $\theta:\cP\to\Theta$ be a parameter of the distribution that we want to estimate}. {Let $\ell:\Theta\times\Theta\to\RR_+$ be a pseudo-metric which is the loss function for estimating $\theta$. We now describe the minimax framework of parameter estimation, and hypothesis testing.}
%Let $\ell:\Theta\times\Theta\to\RR_+$ be a loss function (distance) between parameters.

\medskip

\noindent\textit{Parameter estimation.} The risk of an estimator $\hat{\theta}:\cX^\ns\to\Theta$ under loss $\ell$ is $\max_{\p \in \cP} \EE_{X \sim \p}\left[\ell(\hat \theta (X),\theta(p))\right]$, {the worst case expected loss of $\hat\theta$ over $\cP$. Note that $X\in\cX^\ns$, since $\p$ is a distribution over $\cX^\ns$. The minimax risk of estimation under $\ell$ for the class $\cP$ is}
\begin{align*}
R(\cP, \ell) := \min_{\hat \theta}\ \max_{\p \in \cP}\ \EE_{X \sim \p}\left[\ell(\hat \theta (X),\theta(p))\right].
\end{align*}
{The minimax risk under differentially private protocols is given by restricting $\hat\theta$ to be differentially private. For $(\eps, \delta)$-DP, we study the following minimax risk:} 
\begin{align}
R(\cP, \ell, \eps, \delta) := \min_{\hat \theta \text{ is }(\eps,\delta)\text{-DP}}\ \max_{\p \in \cP}\ \EE_{X \sim \p}\left[\ell(\hat \theta (X),\theta(p))\right].\label{eqn:minmax-risk}
\end{align}
For $\delta=0$, the above minimax risk under $\eps$-DP is denoted as $R(\cP, \ell, \eps)$. 

\medskip

\noindent\textit{Hypothesis testing.} Hypothesis testing can be cast in the framework of parameter estimation as follows. {Let $\cP_1\subset \cP$, and $\cP_2\subset \cP$ be two disjoint subsets of distributions denoting the two hypothesis classes. Let $\Theta=\{1,2\}$, such that for $\p\in\cP_i$, let $\theta(p)=i$. For a test $\hat\theta:\cX^n\to \{1,2\}$, and $\ell(\theta, \theta')=\II\{\theta\ne\theta'\}=|\theta-\theta'|$,} {the error probability is the worst case risk under this loss function:}
\begin{align}
P_e(\hat\theta, \cP_1, \cP_2):= \max_i \max_{\p\in \cP_i}\probofsub{ 
\newnewzs{X\sim \p}}{\hat\theta(X)\ne i } = \max_i \max_{\p\in 
\cP_i}\EE_{X\sim \p} 
\left[{|\hat\theta(X)-\theta(p)}|\right].\label{eqn:error-prob}
\end{align}


%\noindent\textit{Hypothesis testing.} Hypothesis testing can be cast in the framework of parameter estimation as follows. \newa{Let $\cP_1\subset \cP$, and $\cP_2\subset \cP$ be two disjoint subsets of distributions denoting the two hypothesis classes. Let $\Theta=\{1,2\}$, such that for $\p\in\cP_i$, let $\theta(p)=i$. For a test $\hat\theta:\cX^n\to \{1,2\}$, and $\ell(\theta, \theta')=\II\{\theta\ne\theta'\}=|\theta-\theta'|$. The error probability is the minimax risk under this loss function:}
%\begin{align}
%P_e(\hat\theta, \cP_1, \cP_2):= \max_i \max_{\p\in \cP_i}\probof{\hat\theta(X)\ne i \mid X\sim \p} = \max_i \max_{\p\in \cP_i}\EE_{X\sim \p} \left[{|\hat\theta(X)-\theta(p)}|\right].\label{eqn:error-prob}
%\end{align}



%\vspace{-20pt}

\smallskip
\noindent\textbf{Organization.} The remainder of the paper is organized as follows. In Section~\ref{sec:dp-lecam},~\ref{sec:dp-fano}, and~\ref{sec:dp-assouad} we state the privatized versions of Le Cam, Fano, and Assouad's method respectively. In Section~\ref{sec:applications} we discuss the applications of these results to several estimation tasks. In Section~\ref{sec:related} we discuss some related and prior work. In Section~\ref{sec:pdp_estimation} and~\ref{sec:adp_applications} we prove the bounds for distribution estimation under pure DP and approximate DP respectively. In Section~\ref{sec:proofs}, we prove the main theorems stated in Section~\ref{sec:results}.  
 
\section{Results}
\label{sec:results}
Le Cam's method is used to establish lower bounds for hypothesis testing and functional estimation. Fano's inequality, and Assouad's lemma prove {lower bounds} for multiple hypothesis testing problems and can be applied to parameter estimation tasks such as estimating distributions. We \newhzn{develop} extensions of these results with differential privacy. 


\medskip

{
\noindent\textit{An observation.} 
A \emph{coupling} between distributions $\p_1$ and $\p_2$ over 
$\cX^\ns$ is a joint distribution $(X,Y)$ over $\cX^\ns \times\cX^\ns$ 
whose marginals satisfy $X \sim \p_1$ and $Y \sim 
\p_2$\footnote{\newnewzs{We use the term coupling to refer to both the random 
variable $(X,Y)$ and the joint distribution.}}. 
%For simplicity, we treat coupling as a randomized function $f: \cX^\ns\to\cX^\ns$ such that if $X\sim\p$, then $Y=f(X)\sim\q$. Note that $X$, and $Y$ are not necessarily independent. 
Our lower bounds are based on the following observation. If there is a coupling $(X,Y)$ between distributions $\p_1$ and $\p_2$ over $\cX^\ns$ with $\expectation{\ham{X}{Y}}=D$, then a draw from $\p_1$ can be converted to a draw from $\p_2$ by changing $D$ coordinates in expectation. 
%We then apply~\eqref{eqn:dp-definition} for any DP algorithm that distinguishes $p_1$ and $p_2$ about $D$ times.}
\newzs{By the group property of differential privacy, roughly speaking, for 
any $(\eps,\delta)$-DP estimator $\hat{\theta}$, it must satisfy $$\forall 
S\subseteq \Theta, \probofsub{ 
		\newnewzs{X\sim \p}}{\hat\theta(X) \in S} \le e^{D\eps}\cdot 
		\probofsub{ 
		\newnewzs{X\sim \q}}{\hat\theta(Y) \in S}+ \delta D e^{\eps(D-1)}.$$
	Hence, if there exists an algorithm that distinguishes between $\p_1$ and $\p_2$ reliably, $D$ must be large ($\Omega\Paren{1/\eps+\delta}$).}


\subsection{DP Le Cam's method}
\label{sec:dp-lecam}
\newhz{
Le Cam's method (Lemma 1 of~\cite{Yu97}) is widely used to prove lower bounds for composite hypothesis testings such as uniformity testing~\cite{Paninski08}, density estimation~\cite{Yu97, ray2016cam}, and estimating functionals of distributions~\cite{JiaoVHW15, WuY16, polyanskiy2019dualizing}.}
%\amargin{Find more applications ... check this paper to add ... Dualizing le cam by Yihong wu and yury}  

%We use the expected Hamming distance between couplings of distributions in the two classes to obtain the following extension of Le Cam's method with $(\eps, \delta)$-DP. \anew{Coupling based lower bounds for DP appeared independently in~\cite{AcharyaSZ18, KarwaV18}.~\cite{KarwaV18} established their results for simple hypothesis testing where $\p_1$ and $\p_2$ below are i.i.d. distributions. The result below is similar to the result in~\cite{AcharyaSZ18} which was stated for arbitrary distributions over $\cX^\ns$ and used to establish sample complexity lower bounds for composite hypothesis testing problems.} For the hypothesis testing problem described above, let $\text{co}(\cP_i)$ be the convex hull of distributions in $\cP_i$, which are also families of distributions over $\cX^\ns$.

We use the expected Hamming distance between couplings of distributions in the two classes to obtain the following extension of Le Cam's method with $(\eps, \delta)$-DP, which is an adaptation of a similar result in~\cite{AcharyaSZ18}. For the hypothesis testing problem described above, let $\text{co}(\cP_i)$ be the convex hull of distributions in $\cP_i$, which are also families of distributions over $\cX^\ns$.

\begin{restatable}[$(\eps, \delta)$-DP Le Cam's method]{theorem}{dplecam}
	\label{thm:le_cam}
	Let $\p_1\in\text{co}(\cP_1)$ and $\p_2\in\text{co}(\cP_2)$. Let $(X,Y)$ be a coupling between $\p_1$ and $\p_2$ with $D=\expectation{\ham{X}{Y}}$. Then for $\eps\ge0, \delta\ge0$, any $(\eps,\delta)$-differentially private  hypothesis testing algorithm $\hat{\theta}$ must satisfy 
	\begin{align}
	P_e(\hat{\theta}, \cP_1, \cP_2)  \ge  \frac12 \max \left\{  1-\dtv{p_1}{p_2}, 0.9 e^{-10 \eps D} - 10 D \delta\right\},\label{eqn:le-cam}
	\end{align}
	{where $\dtv{p_1}{p_2} := \sup_{A \subseteq \cX^\ns} 
	\Paren{p_1(A)-p_2(A)}=\frac12\|\p_1 -  \p_2\|_1$ is the total 
	variation (TV) distance of $p_1$ and $p_2$.}
\end{restatable}
%\begin{theorem}[$(\eps, \delta)$-DP Le Cam's method]
%\label{thm:le_cam}
%Let $\p_1\in\text{co}(\cP_1)$ and $\p_2\in\text{co}(\cP_2)$. Let $(X,Y)$ be a coupling between $\p_1$ and $\p_2$ with $D=\expectation{\ham{X}{Y})}$. Then for $\eps\ge0, \delta\ge0$, any $(\eps,\delta)$-differentially private binary hypothesis testing algorithm $\cA$ must satisfy 
%\begin{align*}
%	P_e(\cA, \cP_1, \cP_2)  \ge  \frac12 \max \big\{  1-\dtv{p_1}{p_2}, \left(0.9 e^{-10 \eps D} - 10 D \delta\right) \big\}.
%\end{align*}
%\end{theorem}
The first term here is the original Le Cam's result~\cite{LeCam73, LeCam86, Yu97, Canonne15} and the second term is a lower bound on the additional error due to privacy. \newzs{Note that the second term increases when $D$ decreases. Choosing $\p_1, \p_2$ with small $D$ makes the RHS of~\eqref{eqn:le-cam} large, hence giving better testing lower bounds.} {A similar result (Theorem 1 in~\cite{AcharyaSZ18})}, along with a suitable coupling was used in~\cite{AcharyaSZ18} to obtain the optimal sample {complexity of testing discrete distributions}. We defer the proof of this theorem to Section~\ref{sec:le}.
%{~\cite{AcharyaSZ18} used their result with a suitable coupling to obtain the optimal sample complexity of the composite hypothesis testing problem of testing discrete distributions (see Section~\ref{??}). \anew{An independent result of~\cite{KarwaV18} obtained a similar result for testing simple hypotheses, where $\p_1$ and $\p_2$ are both i.i.d. distributions over $\cX^\ns$, and $D$ is }
%\medskip

%\noindent\textbf{Applications.} The \newhz{private} Le Cam's method has found usage in several applications. Theorem~\ref{thm:le_cam} can be used to establish optimal sample complexity for testing uniformity of discrete distributions~\cite{AcharyaSZ18, AliakbarpourDR18}, and for establishing lower bounds of differentially private entropy and support size estimation~\cite{AcharyaKSZ18}. The key component to use this result is to design couplings with small \newhz{expected} Hamming distance. 

\subsection{DP Fano's inequality}
\label{sec:dp-fano}
\newzs{Theorem~\ref{thm:le_cam} (DP Le Cam's method) characterizes lower bounds for binary hypothesis testing. In estimation problems with multiple parameters, it is common to reduce the problem to a multi-way hypothesis testing problem. The following theorem, proved in Section~\ref{sec:fano_pro}, provides a lower bound on the risk of multi-way hypothesis testing under $\eps$-DP.}
%\amargin{I am adding definition of KL, not sure if we ever did.}
Let 
\[
D_{KL}\Paren{\p_i,\p_j}:=\sum_{x\in\cX^\ns}p_i(x)\log \frac{p_i(x)}{p_j(x)}
\]
 be the $KL$ divergence between (discrete) distributions $\p_i$ and $\p_j$. \footnote{\newzs{For continuous distributions, the summation is replaced with an integral and the probability mass functions are replaced with densities. We focus on discrete distributions in the proof while the results hold for continuous distributions as well.}}
%\begin{theorem} [$\eps$-DP Fano's inequality] \label{thm:dp_fano}
%	Let $\p_1, \p_2,...,\p_M\in\cP$ such that 
%	\begin{enumerate}[label=(\alph*)]
%		\item $\forall i \neq j \in [M]$, $\ell \Paren{\theta(\p_i),\theta(\p_j)} \ge \alpha$,
%		\item $\forall i,j \in [M]$, $D_{KL} \Paren{\p_i,\p_j} \le \beta$,
%		\item \label{item:dham} $\forall i,j \in [M]$, there exists a coupling $(X, Y)$ between $\p_i$ and $\p_j$ such that
%		\[
%		\expectation{\ham{X}{Y}} \le D, 
%		\]
%	\end{enumerate}
%	then
%	\begin{align} \label{eqn:fano_result}
%	R(\cP, \ell, \eps) \ge \max \Bigg\{ & \frac{\alpha}{2} \left(1 - \frac{\beta + \log 2}{\log M}\right), 0.4\alpha \min\left\{1, \frac{M}{e^{10\eps D}}\right\} \Bigg\}. \nonumber 
%	\end{align}
%\end{theorem}
%\amargin{remember to define coupling.}
\begin{restatable} [$\eps$-DP Fano's inequality] {theorem}{dpfano}
	\label{thm:dp_fano}
	Let $\cV=\{\p_1, \p_2,...,\p_M\}\subseteq \cP$ such that {for all $i\ne j$,} 
	\begin{enumerate}[label=(\alph*)]
		\item  $\ell \Paren{\theta(\p_i),\theta(\p_j)} \ge \alpha$,
		\item $D_{KL} \Paren{\p_i,\p_j} \le \beta$,
		\item \label{item:dham} there exists a coupling $(X, Y)$ between $\p_i$ and $\p_j$ such that $\expectation{\ham{X}{Y}} \le D$, then
	\end{enumerate}
	\begin{align} \label{eqn:fano_result}
		R(\cP, \ell, \eps) \ge \max \Bigg\{ & \frac{\alpha}{2} \left(1 - \frac{\beta + \log 2}{\log M}\right), 0.4\alpha \min\left\{1, \frac{M}{e^{10\eps D}}\right\} \Bigg\}. 
	\end{align}
\end{restatable}

\newzs{Under pure DP constraints, Theorem~\ref{thm:dp_fano} extends Theorem~\ref{thm:le_cam} to the multiple hypothesis case.} Non-private Fano's inequality (e.g., Lemma 3 of~\cite{Yu97}) requires only conditions $(a)$ and $(b)$ and provides the first term of the risk bound above. {Now, if we consider the second term, which is the additional cost due to privacy, we would require $\exp(10\eps D)\ge M$, \ie $D \ge {\log M}/{(10\eps)}$ to achieve a risk less than $0.4\alpha$.} Therefore, for reliable estimation, the expected Hamming distance between any pair of distributions cannot be too small. In Corollary~\ref{coro:fano}, we provide a corollary of this result to establish sample complexity lower bounds for several distribution estimation tasks.

	Theorem~\ref{thm:dp_fano} ($\eps$-DP Fano's inequality) can also be seen as a probabilistic generalization of the classic packing lower bound~\cite{Vadhan17}. The packing argument, with its roots in database theory, considers inputs to be deterministic datasets whose pairwise Hamming distances are bounded with probability one, while Theorem~\ref{thm:dp_fano} considers randomly generated datasets whose Hamming distances are bounded in expectation. This difference makes Theorem~\ref{thm:dp_fano} better suited for proving lower bounds for statistical estimation problems. We discuss this difference in details in Section~\ref{sec:related}.

\smallskip
\noindent\textbf{Remark.} {Theorem~\ref{thm:dp_fano} is a bound on the risk for pure differential privacy ($\delta=0$). Our proof extends to $(\eps,\delta)$-DP for \newhz{$\delta = O \Paren{\frac1M}$},  which is not sufficient to establish meaningful bounds since in most problems $M$ will be chosen to be exponential in the problem parameters. To circumvent this difficulty, in the next section we provide a private analogue of Assouad's method, which also works for $(\eps,\delta)$-DP.} 


%\noindent\textbf{Remark.} In Corollary~\ref{coro:fano} we present a corollary of this theorem that is easily applicable to establish sample complexity lower bounds for distribution estimation problems under $\eps$-DP.

%\medskip

%\noindent\textbf{Applications.} We use this theorem to establish the optimal sample complexity of estimating $k$-ary discrete distributions under total variation distance (Theorem~\ref{thm:pure-dv}), $k$-ary discrete distributions under $\ell_2$ distance (Theorem~\ref{thm:pure-l2}), and improved \newhz{sample complexity} lower bounds for product distributions (Theorem~\ref{thm:main_product}) and Gaussian mixtures (Theorem~\ref{thm:main_Gaussian}). 

\subsection{DP Assouad's method}
\label{sec:dp-assouad}
{Our next result is a private version of Assouad's lemma (Lemma 2 of~\cite{Yu97}, and~\cite{Assouad83}). Recall that $\cP$ is a set of distributions over $\cX^\ns$. Let $\cV\subseteq\cP$ be} a set of distributions indexed by the hypercube $ \cE_{\ab} := \{\pm 1\}^{\ab}$, and the loss  $\ell$ is such that
\begin{align}
\forall u,v \in \cE_{\ab}, \ell(\theta(\p_u), \theta(\p_v)) \ge 2\tau \cdot \sum_{i=1}^{\ab} \mathbb{I}\Paren{u_i\neq v_i}.
\label{eqn:assouad-loss}
\end{align}

{Assouad's method provides a lower bound on the estimation risk for distributions in $\cV$, which is a lower bound for $\cP$. For each coordinate $i\in[k]$, consider the following mixture distributions obtained by averaging over all distributions with a fixed value at the $i$th coordinate,}
\[
	\p_{+i}  =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e_i= + 1}\p_e, ~~~ \p_{-i}  =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e_i= -1}\p_e.
\]
Assouad's lemma provides a lower bound on the risk by using~\eqref{eqn:assouad-loss} and considering the problem of distinguishing $\p_{+i}$ and $\p_{-i}$. 
{Analogously, we prove the following privatized version of Assouad's lemma by considering the minimax risk of a private hypothesis testing $\phi:\cX^\ns\to\{-1,+1\}$ between $\p_{+i}$ and $\p_{-i}$. The detailed proof is in Section~\ref{sec:private_assouad}.
}
%In particular, we consider the minimax risk of a hypothesis test $\phi:\cX^\ns\to\{-1,+1\}$ between $\p_{+i}$ and $\p_{-i}$ to prove the following privatized version of Assouad's lemma, and prove it in Section~\ref{sec:private_assouad}. 
\begin{restatable} [DP Assouad's method] {theorem} {dpassouad}
	\label{thm:assouad} 
{$\forall i \in [k]$, let $\phi_i:\cX^\ns\to\{-1,+1\}$ be a binary classifier.%\amargin{I dont understand how we can have $\phi$ inside the summation below, and define one $\phi$ above.
	\begin{align*}
	R(\cP, \ell, \eps, \delta) \ge \frac{\tau}{2} \cdot \sum_{i=1}^{\ab} \min_{\phi_i \text{ is $(\eps, \delta)$-DP}}   ( \probofsub{ X\sim \p_{+i} }{ \phi_i(X) \neq 1 } 
	+ \probofsub{X\sim \p_{-i} }{\phi_i(X) \neq -1 } ). \nonumber
	\end{align*}
	Moreover, if $\forall i\in [\ab]$, there exists a coupling $(X,Y)$ between $\p_{+i}$ and $\p_{-i}$ with $\expectation{\ham {X} {Y}} \le D$,
	\begin{equation} \label{eqn:assouad}
	R(\cP, \ell, \eps, \delta) \ge \frac{\ab \tau}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}. 
	\end{equation} }
%	\begin{align*}
%	R(\cP, \ell, \eps, \delta) \ge R_1:= \frac{\tau}{2} \cdot \sum_{i=1}^{\ab} \min_{\phi_i \text{ is $(\eps, \delta)$-DP}}   ( \probofsub{ X\sim \p_{+i} }{ \phi_i(X) \neq 1 } 
%	+ \probofsub{X\sim \p_{-i} }{\phi_i(X) \neq -1 } ). \nonumber
%	\end{align*}
%Moreover, if $\forall i\in [\ab]$, there exists a coupling $(X,Y)$ between $\p_{+i}$ and $\p_{-i}$ with $\expectation{\ham {X} {Y}} \le D$,
%	\begin{equation} \label{eqn:assouad}
%	R(\cP, \ell, \eps, \delta) \ge \max\left\{R_1, \frac{\ab \tau}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}\right\}.
%	\end{equation}
\end{restatable}

%\begin{theorem}
%\label{thm:assouad}
%Let $\cE_{\ab}$, \newhz{ $\cV_k \subseteq \cP$} be as previously defined, and $\phi: X \rightarrow \{\pm1\}$ be a binary classifier.
%\begin{align*}
%	R(\cP, \ell, \eps, \delta) \ge \frac{\tau}{2} \cdot \sum_{i=1}^{\ab} \min_{ \phi: \phi \text{ is DP}}   ( \probofsub{ X\sim \p_{+i} }{ \phi(X) \neq 1 } 
%	+ \probofsub{X\sim \p_{-i} }{\phi(X) \neq -1 } ). \nonumber
%\end{align*}
%
%%\begin{equation}
%%\sup_{\p \in \cV_{\ab} } \EE_{X \sim \p} \left[ \ell(\p_{\he}, \p )\right] \ge \tau \cdot \sum_{i=1}^{\ab} \inf_{ \phi: \phi \text{ is DP}}  \Paren{ \probofsub{ X\sim \p_{+i} }{ \phi(X) \neq 1 } + \probofsub{X\sim \p_{-i} }{\phi(X) \neq -1 }}. \nonumber
%%\end{equation}
%Moreover, if $\forall i\in [\ab]$, there exists a coupling $(X,Y)$ between $\p_{+i}$ and $\p_{-i}$ with $\expectation{\ham {X} {Y}} \le D$,
%\begin{equation} \label{eqn:assouad}
%	R(\cP, \ell, \eps, \delta) \ge \frac{\ab \tau}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}. \nonumber
%\end{equation}
%\end{theorem}
\noindent The first bound is the classic Assouad's Lemma and~\eqref{eqn:assouad} is the loss due to privacy constraints. Once again note that~\eqref{eqn:assouad} grows with decreasing $D$. \newzs{Compared to Theorem~\ref{thm:dp_fano} (DP Fano's inequality), Theorem~\ref{thm:assouad} works under $(\eps, \delta)$-DP, which is a less stringent privacy notion.}
%\medskip
%\noindent\textbf{Applications.} We use Theorem~\ref{thm:assouad} to establish optimal sample complexity for $k$-ary discrete distributions under total variation distance (Theorem~\ref{thm:ApproximateDiscreteTotalVariation}), and $\ell_2$ distance (Theorem~\ref{thm:ApproximateDiscreteL2}). \newhz{say something about product}



 

==> back_up/toolbox copy/locdef.tex <==
 \newcommand{\anew}[1]{{\color{black}#1}}
 \newcommand{\newzs}[1]{{\color{black}#1}}
  \newcommand{\newnewzs}[1]{{\color{black}#1}}
  
 \newcommand{\newhz}[1]{{\color{black}#1}}
 \newcommand{\newhzz}[1]{{\color{black}#1}}
 \newcommand{\newzz}[1]{{\color{black}#1}}
 
  \newcommand{\newhzn}[1]{{\color{black}#1}}

\newcommand{\Dk}{\Delta_k}
\newcommand{\D}{\Delta}
\newcommand{\Du}{\Delta_u}

\newcommand{\absz}{k}
\newcommand{\ab}{k}
\newcommand{\dims}{d}
\newcommand{\ns}{n}
\newcommand{\ber}{\cB}
\newcommand{\dP}{p}
\newcommand{\dQ}{q}
\newcommand{\mP}{p}
\newcommand{\mQ}{q}


\newcommand{\verify}[1]{\textcolor{black}{#1}}


\newcommand{\p}{p}
\newcommand{\q}{q}
\newcommand{\pn}[1]{\p^{#1}}
\newcommand{\qn}[1]{\q^{#1}}


\newcommand{\expectationsub}[2]{\EE_{#1}\left[#2\right]}
\newcommand{\probofsub}[2]{\Pr\nolimits_{#1}\Paren{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Sitnp}{S({\tt IT}, \ab, \dist)}

\newcommand{\Sit}{S({\tt IT}, \ab, \dist,\eps)}
\newcommand{\Sitd}{S({\tt IT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sut}[2]{S({\tt UT}, #1, #2,\eps)}
\newcommand{\Sutd}{S({\tt UT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sutnp}[2]{S({\tt UT}, #1, #2)}
\newcommand{\Sittwo}{S({\tt IT}, \ab, \dist,\eps)}
\newcommand{\Sct}{S({\tt CT}, \ab, \dist,\eps)}
\newcommand{\Sctd}{S({\tt CT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sctnp}{S({\tt CT}, \ab, \dist)}

\newcommand{\Smc}[1]{S({\tt MC},#1)}
\newcommand{\Sdl}[1]{S({\tt DL},\Delta_{\ab}, \alpha,\eps, #1)}
\newcommand{\Sdla}[1]{S({\tt DL},\Delta_{\ab}, \alpha,\eps,\delta, #1)}
\newcommand{\Sdlat}[2]{S({\tt DL},#1, \alpha,\eps,\delta, #2)}

\newcommand{\Pds}{C_{\ab, \dims}}
\newcommand{\Spl}{S({\tt PL},\Pds, \alpha,\eps, d_{TV})}
\newcommand{\Spla}{S({\tt PL},\Pds, \alpha,\eps, \delta, d_{TV})}

\newcommand{\absvn}[1]{\left\|#1\right\|_1}



\newcommand{\unif}{u}
\newcommand{\unifab}{\unif[{\ab}]}
\newcommand{\unifabs}[1]{\unif[{#1}]}


\newcommand{\smb}{x}
\newcommand{\psmb}{\p_\smb}
\newcommand{\ps}[1]{\p_{#1}}
\newcommand{\Xon}{X^\ns}
\newcommand{\Yon}{Y^\ns}
\newcommand{\Zon}{Z^\ns}
\newcommand{\xon}{x^\ns}
\newcommand{\yon}{y^\ns}
\newcommand{\Xot}{X_1^t}
\newcommand{\Yot}{Y_1^t}
\newcommand{\Xos}{X_1^s}
\newcommand{\Xosp}{X_1^{'s}}
\newcommand{\Yos}{Y_1^s}
\newcommand{\Yosp}{Y_1^{'s}}
\newcommand{\Xosmo}{X_1^{s-1}}
\newcommand{\Yosmo}{Y_1^{s-1}}




\newcommand{\Mestxon}{\Mest\Paren{\Xon}}
\newcommand{\Mest}{{M}}
\newcommand{\Mestgtxon}{\Mest^{\texttt{GT}}\Paren{\Xon}}


\newcommand{\Moxon}{M_0(\Xon)}

\newcommand{\prf}[2]{\Phi_{#1}(#2)}
\newcommand{\prfi}[1]{\Phi_{#1}}

\newcommand{\kp}{k^{'}}

\newcommand{\eps}{\varepsilon}
\newcommand{\he}{\hat{E}}

\newcommand{\mltx}[1]{\mu_{#1}}
\newcommand{\mlty}[1]{\nu_{#1}}

\newcommand{\bias}{b}
\newcommand{\Bern}[1]{B(#1)}

\newcommand{\ham}[2]{d_{\text{Ham}}(#1,#2)}
\newcommand{\alg}{\hat \theta}


\newcommand{\Mltsmb}[2]{M_{#1}(#2)}
\newcommand{\prfsmb}[2]{\Phi_{#1}(#2)}


\newcommand{\dist}{\alpha}

\newcommand{\dtv}[2]{d_{TV}(#1, #2)}
\newcommand{\dkl}[2]{d_{KL}(#1, #2)}


%\ifnum\withcolors=1
%  \newcommand{\new}[1]{{\color{red} {#1}}} % new
%  \newcommand{\newer}[1]{{\color{blue} {#1}}} % even newer
%  \newcommand{\newest}[1]{{\color{orange} {#1}}} % even even newer
%  \newcommand{\newerest}[1]{{\color{blue!10!black!40!green} {#1}}} % you get the idea.
%  \newcommand{\acolor}[1]{{\color{ForestGreen}#1}} % Jayadev
%  \newcommand{\scolor}[1]{{\color{RubineRed}#1}} % Clement
%  \newcommand{\zcolor}[1]{{\color{Orange}#1}} % Himanshu
%  \newcommand{\zscolor}[1]{{\color{Purple}#1}} % Himanshu
%\else
%  \newcommand{\new}[1]{{{#1}}}
%  \newcommand{\newer}[1]{{{#1}}}
%  \newcommand{\newest}[1]{{{#1}}}
%  \newcommand{\newerest}[1]{{{#1}}}
%  \newcommand{\acolor}[1]{{#1}}
%  \newcommand{\scolor}[1]{{#1}}
%  \newcommand{\zcolor}[1]{{#1}}
%\fi
%
%\ifnum\withnotes=1
%  \newcommand{\anote}[1]{\par\acolor{\textbf{J: }\sf #1}} % Jayadev
%  \newcommand{\snote}[1]{\par\scolor{\textbf{ZS: }\sf #1}} % Clement
%  \newcommand{\znote}[1]{\par\zcolor{\textbf{H: }\sf #1}} % Himanshu
%  \newcommand{\afootnote}[1]{\footnote{{\bf \acolor{Jayadev}}: {#1}}}
%  \newcommand{\sfootnote}[1]{\footnote{{\bf \scolor{Cl\'ement}}: {#1}}}
%  \newcommand{\zfootnote}[1]{\footnote{{\bf \zcolor{Himanshu}}: {#1}}}
%
%
%  \newcommand{\todonote}[2][]{\todo[size=\scriptsize,color=red!40,#1]{#2}}  
%	\newcommand{\questionnote}[2][]{\todo[size=\tiny,color=blue!30]{#2}}
%	\newcommand{\todonotedone}[2][]{\todo[size=\scriptsize,color=green!40]{$\checkmark$ #2}}
%	\newcommand{\todonoteinline}[2][]{\todo[inline,size=\scriptsize,color=orange!40,#1]{#2}}  
%  \newcommand{\marginnote}[1]{\todo[color=white,linecolor=black]{{#1}}}
%\else
%  \newcommand{\anote}[1]{}
%  \newcommand{\snote}[1]{}
%  \newcommand{\znote}[1]{}
%  \newcommand{\todonote}[2][]{\ignore{#2}}
%	\newcommand{\questionnote}[2][]{\ignore{#2}}
%	\newcommand{\todonotedone}[2][]{\ignore{#2}}
%	\newcommand{\todonoteinline}[2][]{\ignore{#2}}
%  \newcommand{\marginnote}[1]{\ignore{#1}}
%\fi
%
%\newcommand{\amargin}[1]{\questionnote{\acolor{#1}}} % Jayadev
%\newcommand{\smargin}[1]{\questionnote{\ccolor{#1}}} % Clement
%\newcommand{\zmargin}[1]{\questionnote{\hcolor{#1}}} % Himanshu
%\newcommand{\zsmargin}[1]{\questionnote{\zscolor{#1}}} %Ziteng
%
%\ifnum\withnotes=1
%  \usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}
%\fi



%%%%%%%%%%%%%%%%%%%%%%

==> back_up/toolbox copy/product_new.tex <==
\subsection{Product distribution estimation} \label{sec:product}

%\begin{definition}
%A $(\ab,\dims)$-product distribution is a distribution over $[\ab]^{\dims}$, such that its marginal distribution on each dimension is independent.
%\end{definition}

Recall that $\Delta_{\ab, \dims}$ is the set of all $(\ab,\dims)$-product distributions.~\cite{BunKSW2019} proves an upper bound of $O\Paren{\ab\dims \log \Paren{ \frac{\ab\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$. We prove a sample complexity lower bound for $\eps$-DP $(\ab,\dims)$-product distribution estimation in Theorem~\ref{thm:main_product}, which is optimal up to logarithmic factors.

%\product*
\begin{theorem}
\label{thm:main_product}
The sample complexity of $\eps$-DP $(\ab,\dims)$-product distribution estimation satisfies
\begin{align}
&S(\Delta_{\ab, \dims}, d_{TV}, \alpha, \eps) = \Omega \Paren{\frac{\ab\dims}{\dist^2}+\frac{\ab\dims}{\dist \eps}}. \nonumber
\end{align}
\end{theorem}

\begin{proof}
%We start with the construction of the distribution set. First we utilize the same binary code as in Claim~\ref{clm:GV}, restated below:
%\amargin{A total repeat again ...!}
%\GVcode*
{
We start with the construction of the distribution set. First we use the same binary code as in Lemma~\ref{lem:GV} with weight $l = \frac{\ab}{2}$.
Let $h := \absv{\cC}$ denote the size of the codebook. Given $j \in [h]$, we construct the following $\ab$-ary distribution $\p_j$ based on $c_j \in \cC$:}

{$$ \p_{j} (i)  = \frac{1}{\ab} +\frac{\dist}{\ab\sqrt{\dims}} \cdot \mathbb{I}\Paren{ c_{j,i}=1},$$}
{ where $ c_{j,i}$ denotes the $i$-th coordinate of $c_j$.}
%
%$$ \p_{j} (i)  = \left\{
%\begin{array}{rcl}
%\frac{1}{\ab} + \frac{\dist}{\ab \sqrt{ \dims}} ,       &      & when ~ c_j (i)=1,\\
%\frac{1}{\ab} - \frac{\dist}{\ab\sqrt{\dims}},       &      & when ~c_j (i)=0.
%\end{array} \right. $$


Now we have designed a set of $\ab$-ary distributions of size $h = \Omega \Paren{2^{\frac{7\ab}{128}}}$. To construct a set of product distributions, {we use the codebook construction in Lemma~\ref{lem:constantGV2} to get an $h$-ary codebook $\cH$ with length $d$ and minimum hamming distance $d/2$. Moreover, $|\cH| \ge (\frac{h}{16})^{\frac{\dims}{2}}$. }

Now we can construct the distribution set of $(\ab,\dims)$-product distributions.
Given $b \in \cH$, define
$$\dP_b = \p_{b_1} \times  \p_{b_2}\times \cdots \times \p_{b_d}.$$

Let $\cV_{\ab,\dims}$ denote the set of distributions induced by $\cH$. We want to prove that $\forall \dP \neq \dQ \in \cV_{\ab,\dims},$
\begin{align}
	\dtv{\dP}{\dQ} \ge C\dist, \label{eqn:dtv_prod}\\
	D_{KL} (\dP,\dQ)  \le 4\dist^2, \label{eqn:dkl_prod}
\end{align}
for some constant $C$. Suppose these two inequalities hold, using~\eqref{eqn:dkl_prod}, by Pinsker's Inequality, we get $d_{TV}(\dP, \dQ) \le \sqrt{2D_{KL} (\dP, \dQ) } \le 2\sqrt2\alpha$. Then using Corollary~\ref{coro:fano}, we can get
\begin{align}
&S(\Delta_{\ab, \dims}, d_{TV}, \alpha, \eps) = \Omega \Paren{\frac{\ab\dims}{\dist^2}+\frac{\ab\dims}{\dist \eps}}. \nonumber
\end{align}
Now it remains to prove~\eqref{eqn:dtv_prod} and~\eqref{eqn:dkl_prod}. For~\eqref{eqn:dkl_prod}, note that for any distribution pair $\dP,\dQ \in \cV_{\ab,\dims}$,
\begin{align}
	D_{KL} (\dP,\dQ) \le \dims \cdot \max_{i, j \in [h]} d_{KL}\Paren{\p_i, \p_j} \le 4\dist^2, \nonumber
\end{align}
\newzs{
where the first inequality comes from the additivity of $KL$ divergence for independent distributions and $\forall i, j \in [h]$, 
\[
	d_{KL}\Paren{\p_i, \p_j} = \sum_{x \in [k]} \p_i(x) \log \frac{\p_i(x)}{\p_j(x)} \le \sum_{x \in [\dims]} \frac{(\p_i(x) - \p_j(x))^2}{\p_j(x)} \le \ab \Paren{\frac{\dist}{\ab\sqrt{\dims}}}^2/ \frac{1}{\ab} = \frac{\alpha^2}{d}.
\]
}
Next we prove~\eqref{eqn:dtv_prod}. For any $b \in \cH$ and $\forall i \in[k]$, define set
\[
	S_i  = \{j \in [\ab] : c_{ b_{i},j} = 1\},
\]
which contains the locations of $+1$'s in the code at the $i$th coordinate of $b$. Based on this, we define a product distribution
\[
	\dP'_{b} = \prod_{i = 1}^{d} \cB(\mu_{i} ),
\]
where $\mu_{i} = \sum_{j \in S_i} \p_{b_{i}} (j)$ and $\cB(t)$ is a Bernoulli distribution with mean $t$. For any $b' \neq b \in \cH$, we define
\[
	\dP'_{b'} = \prod_{i = 1}^{d} \cB(\mu'_{i} ),
\]
 where $\mu'_{i} = \sum_{j \in S_i} \p_{b'_{i}}(j)$. Then we have:
 \[
 	\dtv{\dP'_{b}}{\dP'_{b'}} \le \dtv{\dP_{b}}{\dP_{b'}},
 \]
since $\dP'_{b}$ and $\dP'_{b'}$ can be viewed as a post processing of $\dP_{b}$ and $\dP_{b'}$ by mapping elements in $S_i$ to 1 and others to 0 at the $i$-th coordinate. Moreover, we have $\ham{b}{b'} \ge \frac{d}{2}$, and $\forall i$, if $b_{i} \neq b'_{i}$, we have $d_{H}(c_{b_{i}}, c_{b'_{i}}) > \frac{k}{8}$. By the definition of $\p_i$'s, we have
\[
	\| \mu_1 - \mu_2 \|_2^2 \ge \frac{d}{2} \times \left( \frac{\ab}{8} \times \frac{\dist}{\ab \sqrt{d}} \right)^2 = \frac{\dist^2}{128}.
\] 
By Lemma 6.4 in~\cite{KamathLSU18}, there exists a constant $C$ such that $\dtv{\dP'_{b}}{\dP'_{b'}} \ge C\dist$, proving~\eqref{eqn:dtv_prod}.

%start by looking at the marginal distribution of $\dP$ and $\dQ$ on the first coordinate, which we denote as $\p$ and $\q$.  Let $S(\p) = \{j \in [\ab] : \p(j) = \frac{1}{\ab} + \frac{\dist}{\ab \sqrt{ \dims}} \}$, and we design the following mapping $f: \Delta_{\ab} \to \Delta_2$ such that given distribution $\p^{\prime}$, $f (\p^{\prime}) = \cB(\mu_{\p^{\prime}})$, with $\mu_{\p^{\prime}} = \sum_{j \in S(\p)} \p^{\prime}(j)$. By the properties of the code $\cC$, we note that $\mu_{\p} = \frac12+ \frac{\dist}{\sqrt{\dims}}$ and $\mu_p - \mu_q \ge \frac{\dist}{8\sqrt{\dims}}$. Now we apply similar mapping on all the dimensions and after the mapping, we get two $(2,\dims)$-product distributions $\dP^{\prime}$ and $\dQ^{\prime}$, such that $\norm{\mu(\dP^{\prime}) - \mu(\dQ^{\prime})} \ge \frac{\dist}{8}$, where $\mu(\dP^{\prime})$ is the bias vector of the $(2,\dims)$-product distribution $\dP^{\prime}$. By Lemma 6.4 in~\cite{KamathLSU18}, there exists some constant $C$ such that $\dtv{\dP^{\prime}}{\dQ^{\prime}}  \ge C\dist$.  Besides, by the definition of TV distance, we have $\dtv{\dP}{\dQ} \ge \dtv{\dP^{\prime}}{\dQ^{\prime}}\ge C\dist$. 


\end{proof}

==> back_up/toolbox copy/proof_of_theorem.tex <==
\section{Proof of Theorems}
\label{sec:proofs}
\subsection{Proof of DP Le Cam's method (Theorem~\ref{thm:le_cam})}
\label{sec:le}
%We now prove Theorem~\ref{thm:le_cam}, restated below. 
The proof technique is similar to the proof of coupling lemma in~\cite{AcharyaSZ18}. However, we directly characterize the error probability in Theorem~\ref{thm:le_cam}, which we then use to prove Theorem~\ref{thm:assouad} (DP Assouad's method).

\dplecam*

%\amargin{Why are we using $\cA$ instead of $\hat \theta$, when we have used $\theta$ everywhere else in the paper, including when we defined the hypothesis testing problem in the beginning.}
\begin{proof}
{From~\eqref{eqn:error-prob},} 
	\[
	P_e(\hat \theta, \cP_1, \cP_2) \ge \frac12 \Paren{ \probofsub{ X\sim \p_1 }{ \hat \theta(X) \neq \p_1 } + \probofsub{X\sim \p_2 }{\hat \theta(X) \neq \p_2 }}.
	\]
	
{The first term in Theorem~\ref{thm:le_cam} follows from the classic Le Cam's method (Lemma 1 in~\cite{Yu97}). For the second term, let $(X, Y)$ be distributed according to a coupling of $\p_1$ and $\p_2$ with $\expectation{\ham{X}{Y}} \le D$. 
	By Markov's inequality, 
	$\probof{\ham{X}{Y}>10D}<0.1$.
	Let $x$ and $y$ be the realization of $X$ and $Y$.  $W := \{ (x,y) \in \cX^n \times \cX^n| \ham{x}{y} \le 10D \}$ be the set of pairs of realizations with Hamming distance at most $10D$.} Then we have 
	\begin{align}
	\probof{\alg\Paren{X}=\p_2}  = & \sum_{x,y} \probof{X = x, Y = y} \cdot \probof{\alg\Paren{x}=\p_2} \nonumber\\
	\ge &  \sum_{(x,y)\in W} \probof{X = x, Y = y} \cdot \probof{\alg\Paren{x}=\p_2}.
	\end{align}
Let  $\beta_1=\probof{\alg\Paren{X}=\p_2} $, so we have 
	$$ \sum_{(x,y)\in W} \probof{X = x, Y = y}  \cdot\probof{\alg\Paren{x}=\p_2} \le \beta_1$$
	
	Next, we need the following group property of differential privacy.
	
	\begin{lemma} \label{lem:group}
		Let $\alg$ be a $(\eps,\delta)$-DP algorithm, then for sequences $x$, and $y$ with $\ham{x}{y} \le t$, and $\forall S$, 
		$		\probof{\hat \theta(x)\in S}\le e^{t\eps}\cdot\probof{\hat \theta(y)\in S}+ \delta t e^{\eps (t-1)}$. 
	\end{lemma}
	
	\noindent By Lemma~\ref{lem:group}, and $\probof{\ham{X}{Y}>10D}<0.1$, let $\probof{\alg\Paren{Y}=\p_2}=1- \beta_2$,
	\begin{align}
	1- \beta_2=&  
	\sum_{(x,y)\in W} \probof{x,y}  \cdot \probof{\alg\Paren{y}=\p_2}+ 
	\sum_{(x,y)\notin W} \probof{x,y} \cdot \probof{\alg\Paren{y}=\p_2} \nonumber \\
	\leq& \sum_{(x,y)\in W} \probof{x,y}  \cdot \Paren{ e^{\eps \cdot 10D} \probof{\alg\Paren{x}=\p_2} + 10 D\delta \cdot e^{\eps \cdot 10(D-1)}} +0.1	 \nonumber \\
	\leq& \beta_1 \cdot e^{\eps\cdot 10 D} +  10 D\delta \cdot e^{\eps \cdot 10D} + 0.1. \nonumber
	\end{align}
	Similarly, we get
	\begin{align}
	1- \beta_1 \le  \beta_2 \cdot e^{\eps\cdot 10 D} +  10 D\delta \cdot e^{\eps \cdot 10D} + 0.1. \nonumber
	\end{align}
	
	Adding the two inequalities and rearranging terms,
	\[
	\beta_1 + \beta_2 \ge \frac{1.8 - 20D\delta e^{\eps \cdot 10D} }{1 + e^{\eps\cdot 10 D}} \ge 0.9 e^{-10 \eps D} - 10 D \delta.
	\]
\end{proof}

\subsection{Proof of private Fano's inequality (Theorem~\ref{thm:dp_fano})}
\label{sec:fano_pro}
In this section, we prove $\eps$-DP Fano's inequality (Theorem~\ref{thm:dp_fano}), restated below. 
%\amargin{If the theorem statement is identical, why are we restating it again? \newhzz{ HZ: I am fine with the theorem restating, especially when there is enough space. I think it is easier for the readers since they do not need to go to previous pages. Let Ziteng decide.}}

\dpfano*

The proof is based on the observation that if you can change a sample from $\p_i$ to $\p_j$ by changing $D$ coordinates in expectation, then an algorithm that  algorithm that correctly outputs a sample as from $\p_i$ has to output $\p_j$ with probability roughly $e^{-\eps D}$. With a total of $M$ distributions in total, we show that the error probability is large as long as $\frac{M}{e^{\eps D}}$ is large.

\begin{proof}
{The first term in~\eqref{eqn:fano_result} follows from the non-private Fano's inequality (Lemma~3 in~\cite{Yu97}).}
{For an observation $X\in\cX^\ns$,} 
\[
	\hat{\p}(X) := \arg \min_{\p \in \cV} \ell \Paren{\theta(\p),  \hat \theta(X)},
\]
{be the distribution in $\cP$ closest in parameters to an $\eps$-DP estimate $\hat \theta(X)$. Therefore, $\hat{\p}(X)$ is also $\eps$-DP. By the triangle inequality,
	\[
	\ell\Paren{\theta(\hat \p), \theta(\p)} \le \ell \Paren{\theta(\hat \p), \hat \theta(X)}  + \ell \Paren{ \theta(\p), \hat \theta(X)} \le 2\ell \Paren{\theta(\p), \hat \theta(X)}.
	\]}
	Hence,
	\begin{align} 
	\max_{\p \in \cP} \EE_{X \sim \p} \left[\ell(\hat \theta (X),\theta (\p)) \right]  
	\ge \max_{\p \in \cV} \EE_{X \sim \p} \left[\ell(\hat \theta (X),\theta (\p)) \right]
	&\ge \frac{1}{2}\max_{\p \in \cV} \EE_{X \sim \p} \left[\ell(\theta(\hat \p) ,\theta (\p)) \right]  \nonumber \\
	& \ge \max_{\p \in \cV} \frac{\alpha}{2}\probofsub{X \sim \p}{\hat{\p} (X) \neq \p} \nonumber \\
	&\ge \frac{\alpha}{2M}\sum_{\p \in \cV} \probofsub{X \sim \p}{\hat{\p} (X) \neq \p}.
	\label{eqn:reduction}
	\end{align}
	Let $\beta_i = \probofsub{X \sim \p_i}{\hat{\p} (X) \neq \p_i}$ be the probability that $\hat p(X)\ne\p_i$ when the underlying distribution generating $X$ is $\p_i$. For $\p_i, \p_j \in \cV$, let $(X,Y)$ be the coupling in condition $(c)$. By Markov's inequality $\probof{\ham{X}{Y}>10D}<1/{10}.$

{Similar to the proof of Theorem~\ref{thm:le_cam} in the previous section, let $W := \{ (x,y) | \ham{x}{y} \le 10D \}$ and $\probof{x,y}  = \probof{X = x, Y = y}$ . Then
	\begin{align}
	1- \beta_j = \probof{\hat{\p}\Paren{Y} =\p_j}  \leq  \sum_{(x, y)\in W} \probof{x,y}  \cdot \probof{\hat{\p} \Paren{y}  = \p_j} + \sum_{(x, y)\notin W} \probof{x,y}  \cdot 1. \nonumber
	\end{align}}
Therefore, 
	\[ \sum_{(x, y)\in W} \probof{x,y}  \cdot \probof{\hat{\p} \Paren{y}  = \p_j} \ge 0.9 - \beta_j.\] Then, we have
	\begin{align}
	\probof{\hat{\p} \Paren{X}  = \p_j} & \ge  \sum_{(x,y)\in W} \probof{x, y} \cdot \probof{\hat{\p} \Paren{x}  = \p_j}\nonumber \\ 
	&\ge \sum_{(x,y)\in W} \probof{x, y} e^{-10 \eps D} \probof{\hat{\p} \Paren{y}  = \p_j} \label{eqn:step-dp} \\
	& \ge ( 0.9 - \beta_j)  e^{-10 \eps D},\nonumber
	\end{align}
	where~\eqref{eqn:step-dp} uses that $\hat p$ is $\eps$-DP and $\ham{x}{y} \le 10D$. Similarly, for all $j' \neq i$, 
	\[
	\probof{\hat{\p} \Paren{X}  = \p_{j'}} \ge ( 0.9 - \beta_{j'})  e^{-10 \eps D}.
	\]
	Summing over $j'\ne i$, we obtain
	\begin{align}
	\beta_i &= \sum_{j' \neq i} \probof{\hat{\p} \Paren{X} = \p_{j'}}  \ge \Paren{ 0.9(M-1) - \sum_{j' \neq i}\beta_{j'} } e^{-10 \eps D}.\nonumber
	\end{align}
	Summing over $i \in [M]$,
	\[
	\sum_{i \in [M]} \beta_i \ge  \Paren{ 0.9 M (M-1) - (M - 1)\sum_{i \in [M]} \beta_{i} } e^{-10 \eps D}.
	\]
	Rearranging the terms
	\[
	\sum_{i \in [M]} \beta_i \ge \frac{0.9 M (M - 1)}{M - 1 + e^{10 \eps D}} \ge 0.8M \min\left\{1,  \frac{M}{e^{10 \eps D}}\right\}.
	\]
	Combining this with~\eqref{eqn:reduction} completes the proof.
\end{proof}


\subsection{Proof of Corollary~\ref{coro:fano}} \label{sec:coro_fano_proof}
%{We restate the corollary before proving it.} 
%
\distest*
%\amargin{Dont know how to make the number to Corollary 4.}
\begin{proof}
Recall that $\cQ^{\ns} := \{ \q^\ns | \q \in \cQ \}$ is the set of induced distributions over $\cX^\ns$ and $\q^\ns \in \cQ^\ns, \theta(\q^\ns) = \q$. Then,
	$\forall i \neq j \in [M]$,
$\ell \Paren{\theta(\q_i^n),\theta(\q_j^n)} \ge 3 \tau$, and $D_{KL} \Paren{\q_i^n,\q_j^n} = n D_{KL} \Paren{\q_i,\q_j}  \le n \beta.$

{The following lemma is a corollary of maximal coupling~\cite{Hollander12}, which states that for two distributions there is a coupling of their $n$ fold product distributions with an expected Hamming distance $n$ times their total variation distance.}
	\begin{lemma}
		\label{lem:couplingdistance}
		Given distributions $\q_1,\q_2$ over $\cX$, there exists a coupling $(X,Y)$ between $\q_1^n$ and $\q_2^n$ such that  
		\[\expectation{\ham{X}{Y}} = \ns \cdot d_{TV} \Paren{\q_1,\q_2},
		\]
		where $X \sim \q_1^n$ and $Y \sim \q_2^n.$
	\end{lemma}
\noindent By Lemma~\ref{lem:couplingdistance}, $\forall i,j \in [M]$, there exists a coupling $(X, Y)$ between $\q_i^n$ and $\q_j^n$ such that $\expectation{\ham{X}{Y}} \le n\gamma. $
	Now by Theorem~\ref{thm:dp_fano},
	\begin{align}
	R(\cQ^*, \ell, \eps) \ge \max \Bigg\{\frac{3\tau}{2} \left(1 - \frac{n \beta + \log 2}{\log M}\right), 1.2\tau \min\left\{1, \frac{M}{e^{10\eps n \gamma}}\right\} \Bigg\}.
	\end{align}
Therefore, for $R(\cQ^\ns, \ell, \eps) \le \tau$, 
	\[
	S(\cQ, \ell, \tau, \eps) = \Omega\Paren{\frac{\log M}{\beta}+ \frac{\log M}{\gamma \eps}}.
	\]
\end{proof}


\subsection{{Proof of private Assouad's method (Theorem~\ref{thm:assouad})}}
\label{sec:private_assouad}
\newzs{We restate the theorem below and the notions are the same as defined in Section~\ref{sec:dp-assouad}.}
\dpassouad*
\begin{proof}
{The first part is from the non-private Assouad's lemma, which we include here for completeness. Let $\p\in\cV \subset \cP$ and $X\sim\p$. For an estimator $\hat \theta(X)$, consider an estimator $\he(X) = \arg \min_{e \in \cE_{\ab}} \ell \Paren{\hat \theta(X), \theta(\p_e)}$.} Then, by the triangle inequality,
		\[
	\ell \Paren{ \theta(\p_{\he}), \theta(\p) } \le \ell \Paren{ \hat \theta, \theta(\p_{\he})}  + \ell \Paren{ \hat \theta, \theta(\p) } \le 2 \ell \Paren{ \hat \theta, \theta(\p) }.
	\]
	Hence,
	\begin{equation} \label{eqn:reduce_index}
	R(\cV, \ell, \eps, \delta) = \min_{\hat \theta \text{ is }(\eps,\delta)-DP}\ \max_{\p \in \cV}\ \EE_{X \sim \p}\left[\ell(\hat \theta (X),\theta(p))\right] \ge \frac{1}{2} \min_{\he \text{ is }(\eps,\delta)-DP}\ \max_{\p \in \cV}\ \EE_{X \sim \p}\left[\ell(\theta(\p_{\he(X)}),\theta(p))\right]
	\end{equation}
	
\noindent For any $(\eps, \delta)$-DP index estimator $\he$, and by~\eqref{eqn:assouad-loss},
	\begin{align}
	\max_{\p \in \cV }\expectationsub{X \sim \p} {\ell(\theta(\p_{\he}), \theta(\p))} \geq \frac1{|\cE_{\ab}|} \sum_{ e \in \cE_{k}} \expectationsub{X \sim \p_{e}} {\ell(\theta(\p_{\he}),\theta(\p_{e}) )} 
	\geq  \frac{2\tau}{|\cE_{\ab}|}  \sum_{i=1}^{k}  \sum_{ e \in \cE_{k}} \probof{\he_i \neq {e}_i| E = e }. \nonumber 
	\end{align}
	%
	%\begin{align}
	%\sup_{\p \in \cV_{\ab} }\expectationsub{X \sim \p} {\ell(\p_{\he}, \p)} \geq \frac1{|\cE_{\ab}|} \sum_{ e \in \cV } \expectationsub{X \sim \p_{e}} {\ell(\p_{\he},\p_{e} )} 
	%\geq  \frac{2\tau}{|\cE_{\ab}|}  \sum_{i=1}^{k}  \sum_{ e \in \cE_{k}} \probof{\he(i) \neq {e}(i) | E = e }. \nonumber 
	%\end{align}
	
\noindent For each $i$, we divide $ \cE_{k} =  \{\pm1\}^{k}$ into two sets according to the value of $i$-th position,
	\begin{align}
	\max_{\p \in \cV }\expectationsub{X \sim \p} {\ell(\theta(\p_{\he}), \theta(\p))} & \geq  \frac{2\tau}{|\cE_{\ab} |} \sum_{i=1}^{k}  \Brack {\sum_{e:e_i=1} \probof{ \he_i\neq 1| E=e }+\sum_{e:e_i=-1} \probof{\he_i \neq -1  | E = e} }\nonumber\\
	&= \tau \cdot \sum_{i=1}^{\ab}  \Paren{ \probofsub{ X\sim \p_{+i} }{ \he_i\neq 1 } + \probofsub{X\sim \p_{-i} }{\he_i\neq -1 }}  \nonumber \\
	&\ge \tau \cdot \sum_{i=1}^{\ab} \min_{ \phi_i: \phi_i \text{ is DP}}  \Paren{ \probofsub{ X\sim \p_{+i} }{ \phi_i(X) \neq 1 } + \probofsub{X\sim \p_{-i} }{\phi_i(X) \neq -1 }}.  \nonumber
	\end{align}
	Combining with~\eqref{eqn:reduce_index}, we have
	\[
	R(\cP, \ell, \eps, \delta)  \ge R(\cV, \ell, \eps, \delta) \ge  \frac{\tau}{2} \cdot \sum_{i=1}^{\ab} \min_{ \phi_i: \phi_i \text{ is DP}}  \Paren{ \probofsub{ X\sim \p_{+i} }{ \phi_i(X) \neq 1 } + \probofsub{X\sim \p_{-i} }{\phi_i(X) \neq -1 }},
	\]
	proving the first part.

	For the second part. Note that for each $i \in [\ab]$, the summand above is the error probability of hypothesis testing between the mixture distributions $\p_{+i}$ and $\p_{-i}$. Hence, using Theorem~\ref{thm:le_cam}, 
	\[
	R(\cP, \ell, \eps, \delta) \ge \frac{\ab \tau}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}.
	\]
\end{proof}


==> back_up/toolbox copy/pure_dp.tex <==
\section{$\eps$-DP distribution estimation} \label{sec:pdp_estimation}
In this section, we use Corollary~\ref{coro:fano} to prove sample complexity lower bounds for various $\eps$-DP distribution estimation problems. The general idea is to construct a subset of distributions in $\cQ$ such that they are close in both $TV$ distance and $KL$ divergence while being separated {in the loss function $\ell$}. The larger the subsets we construct, {the better} the lower bounds we can get. In Section~\ref{sec:pdp_kary}, we {derive} sample complexity lower bounds for $k$-ary distribution estimation under both \emph{TV} and $\ell_2$ distance that are tight up to constant factors. Tight sample complexity lower bounds up to logarithmic factors for $(k,d)$-product distributions and $d$-dimensional Gaussian mixtures are derived in Section~\ref{sec:product} and~\ref{sec:gaussian} respectively. 

{Corollary~\ref{coro:fano} requires a \emph{packing} of distributions with pairwise distance at least $3\tau$ apart in $\ell$. A standard method to construct such distributions is using results from coding theory.}

\newzs{We start with some definitions. An $h$-ary code of length $k$ is a set $\cC\subseteq \{0,1, \ldots, h-1\}^k$, and each $c\in\cC$ is a \emph{codeword}. The \emph{minimum distance} of a code $\cC$ is the smallest Hamming distance between two codewords in $\cC$. The code is called binary when $h = 2$. The weight of a binary codeword $c\in\cC$ is $wt(c)= |\{i:c_i=1\}|$, the number of 1's in $c$. A binary code $\cC$ is a \emph{constant weight code} if each $c\in\cC$ has the same weight.  We now present some useful variants of the classic Giblert Varshamov bounds on the existence of codes with certain properties. We prove these in Section~\ref{sec:codes}.
}
{
\begin{lemma}
\label{lem:GV}
Let $l$ be an integer at most $k/2$ and at least $20$. There exists a constant weight binary code $\cC$ which has code length $k$, weight $l$, minimum distance $l/4$ with $|\cC|\ge \Paren{\frac{k}{2^{7/8}l}}^{7l/8}$.
\end{lemma}} 

%\noindent{An $h$-ary code of length-$k$ is a subset of $\{0,1,\ldots, h-1\}^k$. 
\begin{lemma}
\label{lem:constantGV2}
There exists an $h$-ary code $\cH$ with code length $\dims$ and minimum Hamming distance $\frac{\dims}{2}$, which satisfies that $\absv{\cH} \ge (\frac{h}{16})^{\frac{\dims}{2}}$.
\end{lemma}}


%We start with some definitions. A binary code of length $k$ is a set $\cC\subseteq \{0,1\}^k$, and each $c\in\cC$ is a \emph{codeword}. The weight of a binary codeword $c\in\cC$ is $wt(c)= |\{i:c_i=1\}|$, the number of 1's in $c$. $\cC$ is a \emph{constant weight code} if each $c\in\cC$ has the same weight. The \emph{minimum distance} of a code $\cC$ is the smallest Hamming distance between two codewords in $\cC$. We now present some useful variants of the classic Giblert Varshamov bounds on the existence of codes with certain properties. We prove these in Section~\ref{sec:codes}.
%
%{
%	\begin{lemma}
%		\label{lem:GV}
%		Let $l$ be an integer at most $k/2$ and at least $20$. There exists a constant weight binary code $\cC$ which has code length $k$, weight $l$, minimum distance $l/4$ with $|\cC|\ge \Paren{\frac{k}{2^{7/8}l}}^{7l/8}$.
%\end{lemma}} 
%
%\noindent{An $h$-ary code of length-$k$ is a subset of $\{0,1,\ldots, h-1\}^k$. 
%	\begin{lemma}
%		\label{lem:constantGV2}
%		There exists an $h$-ary code $\cH$ with code length $\dims$ and minimum Hamming distance $\frac{\dims}{2}$, which satisfies that $\absv{\cH} \ge (\frac{h}{16})^{\frac{\dims}{2}}$.
%\end{lemma}}

\input{toolbox/pure_dp_kary}

\input{toolbox/product_new}

\input{toolbox/gaussian}

==> back_up/toolbox copy/pure_dp_kary.tex <==
\subsection{$\ab$-ary distribution estimation} \label{sec:pdp_kary}
We establish the sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $TV$ and $\ell_2$ distance. 
%\puredtv*
\begin{theorem}
\label{thm:pure-dv}
The sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $TV$ distance  is
\begin{align}
S(\Delta_{\ab}, d_{TV}, \alpha, \eps)=\Theta \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha\eps}}.
\end{align}
\end{theorem}

\begin{theorem}
\label{thm:pure-l2}
The sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $\ell_2$ distance is
\begin{align}
S(\Delta_{\ab}, \ell_2, \alpha, \eps) =\Theta \Paren{\frac{1}{\dist^2}+\frac{\sqrt{\ab}}{\dist\eps}},\ \ \ \text{for $\dist < \frac1{\sqrt{\ab}}$, and}
\end{align}
\begin{align}
\Omega\Paren{\frac{1}{\dist^2}+\frac{\log(\ab\dist^2)}{\dist^2\eps}}\le S(\Delta_{\ab}, \ell_2, \alpha, \eps) \le O\Paren{\frac{1}{\dist^2}+\frac{\log\ab}{\dist^2\eps}} \ \ \ \text{for $\dist > \frac1{\sqrt{\ab}}$.} 
\end{align}
\end{theorem}
 

For $\ell_2$ loss, our bounds are tight within constant factors when $\dist < \frac1{\sqrt{\ab}}$ or $\dist > \ab^{-(\frac12- 0.001)}$.
%With regarding to approximate DP, we have matching upper and lower bounds when $\eps \ge O(\delta)$, which is a weak condition (practically people $\eps = O(1)$ and $\delta = O\Paren{\frac1{\ns}}$). 

\subsubsection {Total variation distance}
\label{sec:puredp-tv}

In this section, we derive the sample complexity of $\eps$-DP $k$-ary distribution estimation under $TV$ distance, which is stated in Theorem~\ref{thm:pure-dv}.

\medskip

\noindent \textbf{Upper bound:}
\cite{DiakonikolasHS15} provides an upper bound based on Laplace mechanism~\cite{DworkMNS06}. {We state the algorithm and a proof for completeness and we will use it for estimation under $\ell_2$ distance.}

Given a $\Xon$ from an unknown distribution $\p$ over $[\ab]$. Let $M_x(\Xon)$ be the number of appearances of $x$ in $\Xon$. {Let $p^{\text{erm}}$ be the empirical estimator where $ p^{\text{erm}}(x) :=\frac{M_x(\Xon)}{\ns}$. We note that changing one $X_i$ in $X^n$ can change at most two coordinates of $p^{\text{erm}}$, each by at most $\frac1n$, and thus changing one $X_i$ changes the $p^{\text{erm}}$ by at most $2/n$ in $\ell_1$ distance. Therefore, by~\cite{DworkMNS06}, adding a Laplace noise of parameter $2/\ns\eps$ to each coordinate of $p^{\text{erm}}$ makes it $\eps$-DP. For $x\in[k]$, let
\[ 
h(x) = p^{\text{erm}}(x)+\text{Lap}\Paren{\frac{2}{n \eps}}, \]
where $Lap(\beta)$ is a Laplace random variable with parameter $\beta$.}
The final output $\hat{p}$ is the projection of $h$ on the simplex $\Delta_k$ {in $\ell_2$ distance}.
%We first give the proof of the sample complexity under $\ell_2$ loss. Then we can attain the result with respect to  total variation distance by Cauchy-Schwartz Inequality.
The expected $\ell_2$ loss between $h$ and $p$ can be upper bounded by
\begin{align}
\Paren{\expectation{\norm{h-p}}}^2 &\le \expectation{\norms{h-p}} \le \expectation{\norms{p^{\text{erm}}-p}}+\expectation{\norms{h - p^{\text{erm}}}}, \nonumber
\end{align}
where the first inequality comes from the Jensen's inequality and the second inequality comes from the triangle inequality.


The first term $\expectation{\norms{p^{\text{erm}} -p}}$ is upper bounded by $\frac{1}{n}$ by an elementary analysis of the empirical estimator. For the second term, note that $\expectation{\norms{h - p^{\text{erm}}}} = \sum_{i=1}^\ab \expectation{Z_i^2}$, where $\forall i, Z_i \sim \text{Lap}\Paren{\frac{2}{\ns\eps}}$. %\amargin{Which property of Laplace distribution?} 
{By the variance of Laplace distribution}, we have $\expectation{\norms{p^{\text{erm}} -h}} = O\Paren{\frac{k}{n^2 \eps^2}}$.  Therefore $\expectation{\norm{h-p}}\le O\Paren{\frac1{\sqrt{\ns}}+\frac{\sqrt{k}}{\ns\eps}}$.
%Therefore $\expectation{\norm{\hat{p}-p}} \le \frac1{10}\alpha$ when $n= O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{k}}{\alpha\eps}}$.
%By simply applying Markov inequality, we have $\norm{h-\p} \le \alpha$ with probability higher than $\frac{9}{10}$.

Note that since $\Delta_k$ is convex, $\norm{\hat{p}-p} \le\norm{h-p}$. Finally, by Cauchy-Schwarz Inequality, $\expectation{\absvn{\hat{p}- p}} \le \sqrt{\ab}\cdot \expectation{\norm{\hat{p}-\p}}  \le \sqrt{\ab}\cdot\expectation{\norm{h-\p}} = O\Paren{\sqrt{\frac{k}{n}}+ {\frac{k}{n \eps}}} $. Therefore $\expectation{\absvn{\hat{p}- p}} \le \alpha$ when $n= O \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}$.

%As to the lower bounds, we first give a proof under total variation distance by a standard packing argument. Then we extend it to $\ell_2$ distance by using Cauchy–Schwarz inequality. We begin by constructing packing set.
\medskip

\noindent \textbf{Lower bound.}
{We will construct a large set of distributions such that the conditions of Corollary~\ref{coro:fano} hold.} 
\ignore{Our lower bound is through the following two steps. The first step is to construct a set of distributions $\cV_\ab \subset \Delta_k$, such that each pair of distributions in $\cV_\ab$ is $\Omega(\dist)$-separated in total variation distance and with $|\cV_\ab|$ as large as possible. 
In the second step, we bound the $KL$ divergence and $TV$ distance between each pair of distributions, and apply Corollary~\ref{coro:fano} to get the sample complexity lower bound.}
%The following claim is a corollary of Varshamov-Gilbert's lemma (Lemma 4.7 in~\cite{Massart07}). First we need the following binary code to construct packing set.
%\begin{restatable}{claim}{GVcode}
%\label{clm:GV}
%There exists binary code $\cC$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\absv{\cC} > 2^{\frac{\ab}{8}}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{\ab}{8}$,
%\item $\forall c \in \cC, \absv{i:c(i)=1}=\frac{\ab}{2}$.
%\end{enumerate}
%\end{restatable}
%\amargin{We repeat the statement above as well ... I would rather we reduce the number of repeats.}
%WLOG assume $\alpha < 1/24$. Given $c \in \cC$, consider the following distribution  $\p_c$ in $\Delta_\ab$
%\[
%\p_c (i)  = \left\{
%\begin{array}{rcl}
%\frac{1+24\dist}{\ab} ,       &      & \text{when ~ }c(i)=1,\\
%\frac{1-24\dist}{\ab},       &      & \text{when ~ }c(i)=0.
%\end{array} \right.
%\]
%\begin{restatable}{claim}{GVcode}
%\label{clm:GV}
%There exists binary code $\cC$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\absv{\cC} > 2^{\frac{\ab}{8}}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{\ab}{8}$,
%\item $\forall c \in \cC, \absv{i:c(i)=1}=\frac{\ab}{2}$.
%\end{enumerate}
%\end{restatable}
{Suppose $\alpha < 1/48$. Applying Lemma~\ref{lem:GV} with $l={\ab}/{2}$, there exists a constant weight binary code $\cC$ of weight $k/2$, and minimum distance $k/8$, and $|\cC|>2^{7k/128}$. For each codeword $c\in\cC$, a distribution $\p_c$ over $[k]$ is defined as follows:
\[
\p_c (i)  = \left\{
\begin{array}{rcl}
\frac{1+24\dist}{\ab} ,       &      & \text{if ~ }c_i=1,\\
\frac{1-24\dist}{\ab},       &      & \text{if ~ }c_i=0.
\end{array} \right.
\]}

{We choose $\cV = \{ \p_c : c \in \cC \}$ to apply Corollary~\ref{coro:fano}. By the minimum distance property, any two distributions in $\cV$ have a total variation distance of at least $24\alpha/k\cdot k/8=3\alpha$, and at most $24\alpha$. Furthermore, by using $\log (1+x) \le x$, we can bound the KL divergence between distributions by their $\chi^2$ distance, 
\[d_{KL} (\p, \q) \le  \chi^2 (\p,\q)  = \sum_{x=1}^k \frac{\Paren{\p(x) -\q(x)}^2 }{\q(x)} < {10000\alpha^2}.
\]
Setting $\tau=\alpha$, $\gamma=24\alpha$, and $\beta=10000\alpha^2$, and using $\log M > 7\ab/64$ in Corollary~\ref{coro:fano}, we obtain $S(\Delta_{\ab}, d_{TV}, \alpha, \eps)= \Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}.$}
%\amargin{I dont think we can take $\alpha<1/24$, that will break this above, since $q(x)$ can be very close to 0. I have changed it to $\alpha<1/48$. Also, could you check the constant 10000 above.}
\subsubsection{$\ell_2$ distance}
In this section, we derive the sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $\ell_2$ distance, which is stated in Theorem~\ref{thm:pure-l2}.

\medskip

\noindent \textbf{Upper bound:}
We use the same algorithm as in Section~\ref{sec:puredp-tv}. Following the same argument as in Section~\ref{sec:puredp-tv}, the square of expected $\ell_2$ loss of $\hat{p}$ can be upper bounded by
\begin{align}
\Paren{\expectation{\norm{\hat{p}-p}}}^2 &\le \expectation{\norm{h-p}^2} \le \expectation{\norms{p^{\text{erm}}-p}}+\expectation{\norms{h - p^{\text{erm}}}} = O\Paren{\frac1{\ns}+\frac{\ab}{\ns^2\eps^2}}. \nonumber
\end{align}
%And $\expectation{\norm{h-p}} \le \frac1{10}\alpha$ when $n= O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{k}}{\alpha\eps}}$.
Since $\Delta_k$ is convex, we have $\norm{\hat{p}-p} \le\norm{h-p}$. Moreover, the following lemma gives another bound for $\norm{\hat{p}-p}$ (See Corollary 2.3 in~\cite{Bassily18}).
\begin{lemma}
Let $L \subset \RR^d$ be a symmetric convex body of $\ab$ vertices $\{a_j\}_{j=1}^{\ab}$, and let $y \in L$ and $\bar{y} = y+z$ for some $z \in \RR^d$. Let $\hat{y} = \arg \min_{w\in L} \norm{w-\bar{y}}^2$. Then we must have 
$$ \norm{y-\hat{y}}^2 \le 4\max_{j\in[k]} \{ \langle z, a_j \rangle\}. $$
\end{lemma} 

From the lemma, we have $\expectation{\norm{\hat{p}-h}^2}\le 4\cdot \expectation{ \max_{j\in[\ab]} \absv{Z_j}}$, where $\forall j \in [\ab]$, $Z_j \sim \text{Lap}(\frac{2}{\ns\eps})$. Note that $\expectation{ \max \absv{Z_j}} = O\Paren{\frac{\log\ab}{\ns\eps}}$ due to the tail bound of Laplace distribution. We have $\Paren{\expectation{\norm{\hat{p}-p}}}^2 = O\Paren{\frac1{\ns}+ \frac{\log\ab}{\ns\eps}}$. Combined with the previous analysis,  $\Paren{\expectation{\norm{\hat{p}-p}}}^2 = O\Paren{\frac1{\ns}+ \min\Paren{\frac{\ab}{\ns^2\eps^2} ,\frac{\log\ab}{\ns\eps}} }$. Therefore $\expectation{\norm{\hat{p}-p}} \le \frac1{10}\alpha$ when $n= O \Paren{\frac{1}{\alpha^2}+ \min \Paren {\frac{\sqrt{k}}{\alpha\eps}, \frac{\log\ab}{\dist^2\eps} }}$.

\medskip

\noindent \textbf{Lower bound:}
We first consider the case when $\dist < \frac1{\sqrt{\ab}}$, where we can 
derive the lower bound simply by a reduction. By Cauchy-Schwarz 
inequality, for any estimator $\hat{p}$, $ \expectation{\absvn{\hat{p}-p}} 
\le \sqrt{\ab} \cdot \expectation{\norm{\hat{p}-p}}$. Therefore 
$S(\Delta_k,  \ell_2, \alpha, \eps) \ge S(\Delta_k,  d_{TV}, \sqrt{k}\alpha, 
\eps)$, which gives us $S(\Delta_k,  \ell_2, \alpha, \eps)= 
\Omega\Paren{\frac{1}{\dist^2}+\frac{\sqrt{\ab}}{\dist\eps}}$.

Now we consider $\dist \ge \frac1{\sqrt{k}}$. Note that it is enough if we prove the lower bound of $\Omega\Paren{\frac{\log \Paren{\alpha^2\ab}}{\dist^2\eps}}$, since $\Omega\Paren{\frac1{\dist^2}}$ %\zsmargin{How to prove this lower bound for $\dist \ge \frac1{\sqrt{k}}$?} 
is the sample complexity of non-private estimation problem for all range of $\dist$. Similarly, we follow Corollary~\ref{coro:fano}, except that we need to construct a different set of distributions. 
%The following claim can be seen as a corollary of Varshamov-Gilbert's lemma when applied to constant weight binary codes.

%\begin{claim}
%\label{claim:constantGV}
%Given an integer weight $l\le\frac1{50}\ab$, there exists a binary code $\cC$ with code length $\ab$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\forall c \in \cC, \absv{i:c(i)=1}=l$,
%\item $\exists c_1, c_2 > 0 $, $\absv{\cC} > \Paren{  \frac{\ab}{c_1 l}}^{c_2  l}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{l}{4}$,
%\end{enumerate}
%\end{claim}
%
%\begin{proof}
%This proof can be viewed as the standard argument used to prove the Gilbert-Varshamov bound when applied to constant weight codes. The following lemma comes from Theorem 7 in~\cite{GrahamS80},
%\begin{lemma}
%\label{lem:constantGV}
%There exists a binary code $\cC$ with length $\ab$, constant weight $l$ and minimum Hamming weight $2\delta$ ($\min_{i,j \in \cC} \ham{i}{j} $), which satisfies $\absv{\cC} \ge \frac{\binom{\ab}{l}}{\sum_{i=0}^{\delta} \binom{l}{i} \binom{\ab-l}{i}}$.
%\end{lemma}
%
%By applying Lemma~\ref{lem:constantGV}, and replacing $2\delta$ by $\frac{l}{4}$, we have
%\begin{align}
%\absv{\cC} &\ge \frac{\binom{\ab}{l}} {\sum_{j=0}^{l/8} \binom{l}{j} \cdot \binom{\ab-l}{j}}\nonumber  \ge \frac{\binom{\ab}{l}}{\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} \cdot \binom{\ab}{\frac{l}{8}}} \nonumber\\
%  &= \frac1 {\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} } \cdot \prod_{i = 0}^{\frac{7l}{8}- 1} \frac{k - \frac{l}{8}-i}{l - i} 
% \ge 2^{-2l} \cdot \Paren{ \frac{\ab-l}{l}}^{\frac{7l}{8}} \nonumber\\
% &\ge \Paren{  \frac{49}{50} \cdot \frac{\ab}{5l}}^{\frac{7l}{8}}, \nonumber 
%\end{align}
%In the second last inequality, we use $\binom{l}{\frac{l}{8}} \le \binom{l}{\frac{l}{2}} \le 2^l$ and $2^l \ge \frac{l}{8}$ when $l \ge 1$.
%\end{proof}

%\newhzz{
%\begin{claim}
%\label{claim:constantGV}
%Given an integer weight $l\le\frac1{2}\ab$, there exists a binary code $\cC$ with code length $\ab$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\forall c \in \cC, \absv{i:c(i)=1}=l$,
%\item $\exists c_1, c_2, c_3 > 0 $, $\absv{\cC} > c_1\cdot  \Paren{  \frac{\ab}{c_2 l}}^{c_3  l}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{l}{4}$,
%\end{enumerate}
%\end{claim}
%\begin{proof}
%This proof can be viewed as the standard argument used to prove the Gilbert-Varshamov bound when applied to constant weight codes. The following lemma comes from Theorem 7 in~\cite{GrahamS80},
%\begin{lemma}
%\label{lem:constantGV}
%There exists a binary code $\cC$ with length $\ab$, constant weight $l$ and minimum Hamming weight $2\delta$ ($\min_{i,j \in \cC} \ham{i}{j} $), which satisfies $\absv{\cC} \ge \frac{\binom{\ab}{l}}{\sum_{i=0}^{\delta} \binom{l}{i} \binom{\ab-l}{i}}$.
%\end{lemma}
%By applying Lemma~\ref{lem:constantGV}, and replacing $2\delta$ by $\frac{l}{4}$, we have
%\begin{align}
%\absv{\cC} &\ge \frac{\binom{\ab}{l}} {\sum_{j=0}^{l/8} \binom{l}{j} \cdot \binom{\ab-l}{j}}\nonumber  \ge \frac{\binom{\ab}{l}}{\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} \cdot \binom{\ab}{\frac{l}{8}}} \nonumber\\
%  &= \frac1 {\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} } \cdot \prod_{i = 0}^{\frac{7l}{8}- 1} \frac{k - \frac{l}{8}-i}{l - i} 
% \ge \frac{2\sqrt{7} \pi}{e} \cdot (0.59)^{\frac{7l}{8}} \cdot \Paren{ \frac{\ab-\frac{l}{8}}{l}}^{\frac{7l}{8}} \nonumber\\
% &\ge \frac{2\sqrt{7} \pi}{e} \cdot \Paren{  0.55 \cdot \frac{\ab}{l}}^{\frac{7l}{8}}, \nonumber 
%\end{align}
%In the second last inequality, we use the Stirling approximation $\sqrt{2\pi}\cdot l^{l+\frac12} \cdot e^{-l} \le l! \le e \cdot l^{l+\frac12} \cdot e^{-l}$ and $1.1^l \ge \sqrt{l}$ when $l \ge 20$.
%\end{proof}
%}

Without loss of generality, we assume $\dist<0.1$. Now we use the codebook in Lemma~\ref{lem:GV} to construct our distribution set. {We fix weight $l = \lfloor \frac1{50\dist^2} \rfloor$. Note that for any $x>2$, $\lfloor x \rfloor > \frac{x}{2}$. Then we have  $\frac1{100\dist^2} < \lfloor l \rfloor  \le \frac1{50\dist^2} $ since $\frac1{50\dist^2}>2$. Therefore we get a codebook $\cC$ with $|\cC| \ge (k\alpha^2)^{\frac{1}{200 \alpha^2}}$}. Given $c \in \cC$, we construct the following distribution  $\p_c$ in $\Delta_\ab$:
%$$ \p_c (i)  = \left\{
%\begin{array}{cl}
%\frac1{l} ,             & when ~ c(i)=1,\\
%0,             & when ~c(i)=0.
%\end{array} \right. $$
$$ \p_c (i)  = \frac1{l} c_i. $$

We use $\cV_\ab = \{ \p_c : c \in \cC \}$ to denote the set of all these distributions. It is easy to check that $\forall \p \in \cV_\ab$ is a valid distribution. Moreover, for any pair of distributions $\p, \q \in \cV_\ab$, we have $\norm{\p - \q}> \frac1{2\sqrt{l}} = \Omega\Paren{\dist}$.


For any pair $\p,\q \in \cV_k$, $d_{TV} (\p, \q) \le 1$, which is a naive upper bound for $TV$ distance. Finally by setting $\ell$ in Corollary~\ref{coro:fano} to be $\ell_2$ distance, we have $S(\Delta_{\ab}, \ell_2, \alpha, \eps)  =  \Omega \Paren{\frac{\log \absv{\cC} }{\eps}} = \Omega \Paren{\frac{\log ( k\alpha^2)}{\alpha^2\eps}}$.



==> back_up/toolbox copy/related.tex <==
\subsection{Related and prior work}
\label{sec:related}
\subsubsection{Private distribution estimation}
Protecting privacy generally comes at the cost of performance degradation. Previous literature has studied various problems and established utility privacy trade-off bounds, including distribution estimation, hypothesis testing, property estimation, empirical risk minimization, etc~\cite{ChaudhuriMS11, Lei11, BassilyST14, DiakonikolasHS15, CaiDK17, AcharyaSZ18, KamathLSU18, AliakbarpourDR18, AcharyaKSZ18}. 

There has been significant recent interest in differentially private distribution estimation.~\cite{DiakonikolasHS15} gives upper bounds for privately learning $\ab$-ary distributions under total variation distance.~\cite{KamathLSU18, BunKSW2019, KarwaV18} focus on high-dimensional distributions, including product distributions and Gaussian distributions. As discussed in the previous section, our proposed lower bounds improve upon their lower bounds in various settings. \cite{BunNSV15} studies the problem of privately estimating a distribution in Kolmogorov distance, which is weaker than total variation distance. Upper and lower bounds for private estimation of the mean of product distributions in $\ell_\infty$ distance, heavy tailed distributions, and Markov Random fields are studied in~\cite{BlumDMN05, DworkMNS06, SteinkeU17a, BunUV18, KamathSU20, ZhangKKW20}.

Several estimation tasks including distribution estimation and hypothesis testing have also been considered under the distributed notion of local differential privacy, e.g.,~\cite{Warner65, KasiviswanathanLNRS11, ErlingssonPK14, DuchiJW13, KairouzBR16, WangHWNXYLQ16, Sheffet17, YeB18, GaboardiR17, AcharyaSZ18a, AcharyaS19, AcharyaCFT18}.

\subsubsection {Lower bounds in differential privacy}
Several methods have been proposed in the literature to prove lower bounds {under DP constraints}. These include packing argument~\cite{HardtT10,Vadhan17, BeimelKN10}, fingerprinting~\cite{BunNSV15, SteinkeU17a, SteinkeU15, BunSU17, BunUV18, KamathLSU18} and coupling based arguments~\cite{AcharyaSZ18, KarwaV18}. 


\smallskip
\noindent\textit{Binary Testing and Coupling.} Coupling based arguments have been recently used to prove lower bounds for binary hypothesis testing, including the independent works of~\cite{AcharyaSZ18, KarwaV18}.~\cite{AcharyaSZ18} establishes a very similar result to Theorem~\ref{thm:le_cam} and uses it to obtain lower bounds for a composite hypothesis testing problem on discrete distributions.~\cite{KarwaV18} proves a similar result for simple hypothesis testing and uses it to lower bound the sample complexity of estimating the mean of a one-dimensional Gaussian distribution. %In~\cite{KarwaV18}, they construct two different Gaussian distributions with mean $\mu_0$ and $\mu_1$, and point out that the probability of $\mu_1$ in the estimated confidence interval of $\mu_0$ must be connected with $\absv{\mu_0-\mu_1}$ by a coupling argument. 
For both papers, the coupling argument implies that it is hard to 
differentially privately distinguish between two distributions, supposing 
there exists a coupling with small expected Hamming distance. This 
method can be viewed as another form of private Le Cam's method 
(Theorem~\ref{thm:le_cam}) and it can only be applied where binary 
hypothesis testing is involved. \newnewzs{\cite{barber2014privacy} also 
uses a private version of Le 
Cam's method to prove lower bounds for differentially private mean 
estimation. However, instead of the expected Hamming distance between 
any couplings, their method only depends on the TV distance between the 
distributions, which corresponds to the naive independent coupling.}
\newzs{\cite{CanonneKMSU19} uses coupling bounds in~\cite{AcharyaSZ18} to derive instance-optimal bounds for simple binary hypothesis testing under pure DP. They consider a coupling only for symbols whose likelihood ratio between the two hypothesis distributions is large, which results in better bounds for certain instances. The argument only considers pure DP and the case where samples are i.i.d generated while Theorem~\ref{thm:le_cam} and~\cite{AcharyaSZ18} can handle approximate DP and arbitrary distributions (e.g. mixtures of i.i.d distributions considered in this paper) .}
%\snote{Should we state a bit more in detail why it is stronger?}
%\anote{Take a stab at it Ziteng, and I can look again. I think it does not hurt to explain the strength.}
\smallskip

%\newhzn{
%	\smallskip
%	\noindent\textbf{Remark.} Theorem~\ref{thm:dp_fano} can be viewed as a probabilistic version of the classic packing lower bound:
%	
%	\begin{lemma}[Packing lower bound~\cite{Vadhan17}] \label{thm:packing}
%		Let $\cV=\{x_1, x_2,...,x_M\}$ be a set of $M$ datasets over $\cX^n$.  For any pair of datasets $x_i$ and $x_j$, we have $\ham{x_i}{x_j} \le d$. Let $ \{S_{i}\}_{i \in [M]}$ be a collection of disjoint subsets of $\cS$. If there exists an $\eps$-DP algorithm $\cA : \cX^{\ns} \to \cS$ such that for every $i \in [M]$, $\probof{\cA(x_i) \in S_{i}}\ge \frac{9}{10}$, then
%		$$\eps = \Omega \Paren{\frac{\log M}{d}}.$$
%	\end{lemma}
%	
%	Note that $D \le d$ if $d$ is the worst case Hamming distance. This lemma, with its roots in database theory, only considers the worst case Hamming distance between deterministic datasets. However, in the statistical setting, this lemma is too pessimistic. Suppose two data sequences $X$ and $Y$ are generated from two distributions $\p_1$ and $\p_2$, in the worst case, they can be completely different with hamming distance $d$. But if $\p_1$ and $\p_2$ are close in TV distance, their expected hamming distance can be much closer. This lemma fails to take advantage of the fact that the samples are generated from the same distribution to gain a sharper rate.
%}

\noindent\textit{Pure DP Estimation and Packing.} Packing argument~\cite{HardtT10, BeimelKN10, Vadhan17} is a geometric approach to prove lower bounds for estimation under pure DP. We state a form of the packing bound below:
\begin{lemma}[Packing lower bound~\cite{Vadhan17}] \label{thm:packing}
	Let $\cV=\{x_1, x_2,...,x_M\}$ be a set of $M$ datasets over $\cX^n$.  For any pair of datasets $x_i$ and $x_j$, we have $\ham{x_i}{x_j} \le d$. Let $ \{S_{i}\}_{i \in [M]}$ be a collection of disjoint subsets of $\cS$. If there exists an $\eps$-DP algorithm $\cA : \cX^{\ns} \to \cS$ such that for every $i \in [M]$, $\probof{\cA(x_i) \in S_{i}}\ge {9}/{10}$, then
	\[
	\eps = \Omega \Paren{\frac{\log M}{d}}.
	\]
\end{lemma}

Our $\eps$-DP Fano's inequality (Theorem~\ref{thm:dp_fano}) and its corollary for distribution estimation (Corollary~\ref{coro:fano}) can be viewed as a probabilistic packing argument which generalizes Lemma~\ref{thm:packing} to the case where $\cV$ consists of distributions over $\cX^n$ instead of deterministic datasets. The distances between distributions are measured in the minimum expected hamming distance between random datasets generated from a coupling between the distributions. Lemma~\ref{thm:packing} can be obtained from $\eps$-DP Fano's inequality by setting the distributions to be point masses over $\cX^n$. 

Note that $d$ in Lemma~\ref{thm:packing} is an upper bound on the worst-case Hamming distance while $D$ is a bound on the expected Hamming distance and therefore $D \le d$. In statistical applications where $D \ll d$, we can obtain stronger lower bounds by replacing $d$ with $D$. For example, in the $\ab$-ary distribution estimation problem, a naive application of the packing argument can only give a lower bound of $\ns = \Omega\Paren{{\ab \log \Paren{1/\dist}}/{\eps}}$ instead of the optimal $\ns = \Omega\Paren{{\ab}/{\dist \eps}}$ lower bound, where there is an exponential gap in the parameter $1/\dist$.

%This lemma, with its roots in database theory, only considers the worst case Hamming distance between deterministic datasets. However, in the statistical setting, this lemma is too pessimistic. Suppose two data sequences $X$ and $Y$ are generated from two distributions $\p_1$ and $\p_2$, in the worst case, they can be completely different with hamming distance $d$. But if $\p_1$ and $\p_2$ are close in TV distance, their expected hamming distance can be much closer. This lemma fails to take advantage of the fact that the samples are generated from the same distribution to gain a sharper rate.

%Roughly speaking, packing argument tells that if there exists a collection of $M$ datasets such that the Hamming distance between any pair of datasets is at most $d$, any $\eps$-DP algorithm which has disjoint output when the input dataset is different must satisfy $\eps = \Omega\Paren{\frac{\log M}{d}}$.
%{This packing lower} bound~\cite{DworkR14} considers the worst case Hamming distance between deterministic datasets, which in general can be as large as $\ns$. In the statistical settings applying this method directly provides a loose bound. For example, in the $\ab$-ary distribution estimation problem, this method can only give a lower bound of $\ns = \Omega\Paren{\frac{\ab \log \Paren{1/\dist}}{\eps}}$ instead of the optimal $\ns = \Omega\Paren{\frac{\ab}{\dist \eps}}$ lower bound. Theorem~\ref{thm:dp_fano} (DP Fano’s inequality) can be viewed as a packing argument over probabilistic datasets generated by a collection of distributions and with the Hamming distance simply replaced by the expected coupling distance between pairs of distributions in the collection.


\smallskip

\noindent\textit{Approximate DP and Fingerprinting.} Fingerprinting~\cite{SteinkeU15, BunNSV15, DworkSSUV15, SteinkeU17a,  BunSU17, BunUV18, KamathLSU18, CaiWZ19} is a versatile lower bounding method for $(\eps,\delta)$-DP for $\delta=O(1/\ns)$. It has been used to prove lower bounds for several problems, including attribute mean estimation in databases~\cite{SteinkeU17a}, lower bounds on the number of online statistical queries~\cite{BunSU17}, and private selection problem~\cite{SteinkeU17b}.~\cite{KamathLSU18} uses fingerprinting to prove lower bounds on estimating Bernoulli product distributions and Gaussian distributions. We believe fingerprinting and DP Assouad's lemma are both powerful tools for proving lower bounds under approximate DP. In estimating Gaussian distributions, fingerprinting provides strong lower bounds under approximate DP, whereas private Assouad's method gives an additional polynomial blow-up compared to fingerprinting. 
%However, fingerprinting lower bound fails to be applied when the underlying distribution is a $\ab$-ary distribution.
However, for discrete distribution estimation, private Assouad's method provides tight lower bounds, and we do not know how to obtain such bounds from the fingerprinting lemma.

%Furthermore, private Assouad's method is a much more simple and user-friendly method. We consider these two methods as incomparable, and 
%So we think private Assouad's method is a valuable addition to the present toolkit of proving lower bounds under approximate DP, which is notoriously difficult.
%As a side remark, Fingerprinting lower bounds hold for  $(\eps, \delta)$-DP when $\delta=O(1/n)$. This is the interesting case for designing privacy-preserving schemes since otherwise one could blatantly disregard privacy of $\delta\ns$ users, which is a constant. However, our results using private Assouad's method (Theorem~\ref{thm:assouad}) shows that even with large $\delta$ (as large as $\eps$), the same lower bounds hold as with $\delta =O(1/\ns)$ for various statistical estimation tasks. In other words, there is no utility gain by compromising the privacy of a fraction of users, and hence there is no incentive to do it.

%However, this technique has two disadvantages. First, it can only be used under approximate DP when $\delta = O\Paren{\frac1{\ns}}$, whe re $\ns$ is the sample size. Second, this method is defined over the Boolean hypercube, and it remains unclear how to extend this technique to $\ab$-ary alphabets. We note that these two drawbacks can be overcome by private Assouad's method (Theorem~\ref{thm:assouad}).

\cite{DuchiJW13} derives analogues of Le Cam, Assouad, and Fano in the local model of differential privacy, and uses them to establish lower bounds for several problems under local differential privacy.~\cite{AcharyaCT19, acharya2020interactive} proves lower bounds for various testing and estimation problems under local differential privacy using a notion of chi-squared contractions based on Le Cam's method and Fano's inequality. 

%\subsection{Organization of the paper}
%In Section~\ref{sec:prem}, we discuss the definitions and notations. We made a summary of our results in Section~\ref{sec:res}. The proof for Theorem~\ref{thm:coupling} is presented in Section~\ref{sec:private_fano} along with ``private'' Fano's inequality. Section~\ref{sec:pdp_kary} gives upper and lower bounds of $\eps$-DP $\ab$-ary distribution learning. The results under $(\eps,\delta)$-DP are given in Section~\ref{sec:adp_kary}. Finally, we study learning product distributions and Gaussian mixtures under $\eps$-DP in Section~\ref{sec:product} and Section~\ref{sec:gaussian}, respectively.
%1. The Complexity of Differential Privacy: rephrase, only works for data base setting.
%\url{https://privacytools.seas.harvard.edu/files/privacytools/files/complexityprivacy_1.pdf}
%
%2. On the Geometry of Differential Privacy: data base setting, $l_1$ norm dp definition, linear transform
%\url{https://arxiv.org/abs/0907.3754}
%
%3. Raef Bassily DP ERM: mean estimation, still data base setting (no distribution)
%\url{https://arxiv.org/abs/1405.7085}
%
%4. confidence interval: naive coupling, only work in i.i.d. case, doesn't work for mixture, only works for two distributions
%\url{https://arxiv.org/abs/1711.03908}
%
%Finger printing lower bound:
%1. Fingerprinting codes and the price of approximate differential privacy.
%\url{https://arxiv.org/abs/1311.3158}
%
%2. Between pure and approximate differential privacy.
%\url{https://arxiv.org/abs/1501.06095}
%
%3. G's paper
%\url{https://arxiv.org/abs/1805.00216}

==> back_up/toolbox copy/table.tex <==

\begin{table*}[htb]
\centering
      \begin{tabular}{| c | c | c |}
      \hline
      %&\multicolumn{2}{c|} {\bf Sample Complexity Bounds}  \\ \hline
      {\bf Problem} & {\bf Upper Bounds} & {\bf Lower Bounds} \\ \hline
      {\bf $\ab$-ary} & \multicolumn{2}{c|} {\parbox[c][1.2cm]{10cm}{\centering$ \Theta \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha\eps}}$~(\cite{DiakonikolasHS15}, Theorem~\ref{thm:pure-dv})} }\\\hline
 
       {\bf $\ab$-ary, $\ell_2$ distance} &\parbox[c][1.5cm]{5cm}{\centering $O\Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist\eps},\frac{\log\ab}{\dist^2\eps}  } }$ \\\small{(Theorem~\ref{thm:pure-l2}) }}
       & \parbox[c]{5cm}{\centering $\Omega \Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist\eps},\frac{\log (\ab \dist^2)}{\dist^2\eps}  } }$ \\\small{(Theorem~\ref{thm:pure-l2}) } } \\ \hline
       
       {\bf product distribution} & \parbox[c][1.5cm]{5cm}{\centering $O\Paren{\ab\dims \log \Paren{ \frac{\ab\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$ \\\small{\cite{BunKSW2019} }}
       &\parbox[c]{5cm}{\centering $\Omega \Paren{{\ab\dims}\Paren{\frac1{\alpha^2}+\frac1{\alpha \eps}}}$ \\\small{(Theorem~\ref{thm:main_product}) }}\\\hline
       
              {\bf Gaussian mixtures} & \parbox[c][1.5cm]{5cm}{\centering ${O}\Paren{kd\log(\frac{dR}{\alpha})(\frac1{\alpha^2}+ \frac1{\alpha \eps})}$ \\\small{\cite{BunKSW2019} }}
       &\parbox[c]{5cm}{\centering $\Omega \Paren{{\ab\dims}\Paren{\frac1{\alpha^2}+\frac1{\alpha \eps}}}$ \\\small{(Theorem~\ref{thm:main_Gaussian}) }}\\\hline
       
      \end{tabular}
    \caption{\label{tab:pure} Summary of the sample complexity bounds for $\eps$-DP discrete distribution estimation. Unless mentioned, the bounds are all for estimation under total variation distance.}
\end{table*}

%\begin{table}[htbp]
%\centering
%      \begin{tabular}{| c | c |}
%      \hline
%      {\bf Problem} & {\bf Sample Complexity Bounds}    \\ \hline
%      
%      {\bf $\ab$-ary , $d_{TV}$ distance} & {\bf Non-private algorithms:  $\Theta \Paren{\frac{\ab}{\alpha^2}}$ } \\
%      &{\bf $(\eps,\delta)$-DP algorithms:} \\
%      &$\Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha(\eps+\delta)}}\le S(\Delta_k, d_{TV}, \alpha, \eps, \delta) \le O \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}$~[Theorem~\ref{thm:ApproximateDiscreteTotalVariation}] \\\hline
%        {\bf $\ab$-ary, $\ell_2$ distance} & {\bf Non-private algorithms:  $\Theta \Paren{\frac{1}{\alpha^2}}$ } \\
%       &{\bf $(\eps,\delta)$-DP algorithms:} \\
%              & \multicolumn{1}{|l|}{{\bf IF} $\dist \le \ab^{-\frac1{2}}$,}   \\  
%             & $ \Omega \Paren {\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha (\eps+\delta)}} \le S(\Delta_k, \ell_2, \alpha, \eps, \delta) \le O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha\eps}}$ \\ 
%                    & \multicolumn{1}{|l|}{{\bf ELSE}} \\
%       & $\Omega\Paren{\frac{1}{\dist^2}+\frac{1}{\dist^2(\eps+\delta)}}\le  S(\Delta_k, \ell_2, \alpha, \eps, \delta) \le O\Paren{\frac{1}{\dist^2}+\frac{\log\ab}{\dist^2\eps}}$~[Theorem~\ref{thm:ApproximateDiscreteL2}]\\ \hline
%      \end{tabular}
%    \caption{\label{table2} \newhz{Summary of the sample complexity bounds for $(\eps,\delta)$-DP discrete distribution learning.}}
%\end{table}

\begin{table*}[htb]
\centering
      \begin{tabular}{| c | c | c |}
      \hline
      %&\multicolumn{2}{c|} {\bf Sample Complexity Bounds}  \\ \hline
      {\bf Problem} & {\bf Upper Bounds} & {\bf Lower Bounds} \\ \hline
      {\bf $\ab$-ary} &  \parbox[c][1.5cm]{5cm}{\centering $O\Paren{\frac{\ab}{\dist^2}+\frac{\ab} {\dist\eps}}$ \\\small{(\cite{DiakonikolasHS15}, Theorem~\ref{thm:ApproximateDiscreteTotalVariation})} }
       &\parbox[c]{5cm}{\centering $\Omega \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha (\eps+\delta)}}$ \\\small{(Theorem~\ref{thm:ApproximateDiscreteTotalVariation})} }\\\hline
 
       {\bf $\ab$-ary, $\ell_2$ distance} &\parbox[c][1.5cm]{5cm}{\centering 
       $O 
       \Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist\eps},\frac{\log\ab}{\dist^2\eps}
         } }$ \\\small{(Theorem~\ref{thm:ApproximateDiscreteL2}) }}
       & \parbox[c]{5cm}{\centering $\Omega \Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist(\eps+\delta)},\frac{1}{\dist^2(\eps+\delta)}  } }$ \\\small{(Theorem~\ref{thm:ApproximateDiscreteL2}) } } \\ \hline
       
              {\makecell { \bf product distribution \\ ($k = 2$)}} & \parbox[c][1.5cm]{5cm}{\centering $O\Paren{\dims \log \Paren{ \frac{\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$ \\\small{\cite{KamathLSU18, BunKSW2019}}}
       &\parbox[c]{5cm}{\centering $\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha (\eps + \delta)}}$ \\\small{(Theorem~\ref{thm:ApproximateProductTotalVariation},~\cite{KamathLSU18}) }}\\ \hline
      \end{tabular}
    \caption{\label{tab:approx} Summary of the sample complexity bounds for $(\eps,\delta)$-DP discrete distribution estimation. Unless mentioned, the bounds are all for estimation under total variation distance.}
\end{table*}
%
%\begin{table}[t]
%\center
%\begin{tabular}{c c c c c}
%&& Deterministic  & Sample & Stochastic  \\
%&& First-Order Oracle & Complexity & First-Order Oracle \\\hline
%\parbox[t]{1cm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{$\norm{x_0-x^*}\leq R$}}}}
%& \small{Upper:}
%& \parbox[t]{4cm}{\centering $\tilde{O}\prn*{\sqrt{\frac{HR}{\epsilon}}}$\\\small{\cite{nesterov2012make}}}
%& \parbox[t]{3cm}{\centering $O\prn*{\frac{\sigma^2}{\epsilon^2}\log^{3}\parens{\frac{HR}{\epsilon}}}$\\\small{(\pref{cor:sample-complexity-bounded})}}
%& \parbox[t]{3cm}{\centering $\tilde{O}\prn*{\sqrt{\frac{HR}{\epsilon}} + \frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{cor:sgd3-bounded-domain})}}
%\rule[-20pt]{0pt}{37pt}\\ ~\\
%& \small{Lower:}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\sqrt{\frac{HR}{\epsilon}}}$\\\small{\cite{carmon2017lower2}}}
%& \parbox[t]{3cm}{\centering $\Omega\prn*{\frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{thm:statistical-lower-bound})}}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\sqrt{\frac{HR}{\epsilon}} + \frac{\sigma^2}{\epsilon^2}\log\parens{\frac{HR}{\epsilon}}}$\\\small{(\pref{thm:first-order-lower-bound})}}
%\rule[-24pt]{0pt}{28pt}\\ \hline
%\parbox[t]{1cm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\parbox[t]{2.345cm}{\centering \scriptsize{$F(x_0)-F(x^*)\leq \Delta$}}}}}
%& \small{Upper:}
%& \parbox[t]{4cm}{\centering $\tilde{O}\prn*{\frac{\sqrt{H\Delta}}{\epsilon}}$\\\small{\cite{carmon2017lower2}}}
%& \parbox[t]{3cm}{\centering $O\prn*{\frac{\sigma^2}{\epsilon^2}\log^{3}\parens{\frac{H\Delta}{\epsilon^2}}}$\\\small{(\pref{cor:sample-complexity-bounded})}}
%& \parbox[t]{3cm}{\centering $\tilde{O}\prn*{\frac{\sqrt{H\Delta}}{\epsilon} + \frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{cor:sgd3-bounded-domain})}}
%\rule[-24pt]{0pt}{41pt}\\~\\
%& \small{Lower:}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\frac{\sqrt{H\Delta}}{\epsilon}}$\\\small{\cite{carmon2017lower2}}}
%& \parbox[t]{3cm}{\centering $\Omega\prn*{\frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{thm:statistical-lower-bound})}}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\frac{\sqrt{H\Delta}}{\epsilon} + \frac{\sigma^2}{\epsilon^2}\log\parens{\frac{H\Delta}{\epsilon^2}}}$\\\small{(\pref{thm:first-order-lower-bound})}}
%\rule[-24pt]{0pt}{26pt}\\\hline
%\end{tabular}
%\caption{Upper and lower bounds on the complexity of finding $x$
%  such that $\norm{\nabla F(x)}\leq\epsilon$ for convex problems with
%  $H$-Lipschitz gradients, where $\sigma^2$ is a bound on the variance
%  of gradient estimates.}
%  \label{tab:results}
%\end{table}


==> back_up/toolbox copy/uniformity-lower_new.tex <==
\subsection{Sample Complexity Lower bounds for Uniformity Testing}\label{sec:lower-identity}

The first term is the lower bound without privacy constraints, proved in~\cite{Paninski08}. In this section, we prove the terms associated with privacy. 

The simplest argument is for $\ns \ge \frac{\ab}{\alpha^2}$, which hopefully will give the readers a sense of how coupling argument works. We consider the case of binary uniformity testing where the goal is to test whether the bias of a coin is $1/2$ or $\alpha$-far from $1/2$. This is a special case of uniformity testing for distributions over $[\ab]$ (when $\ab-2$ symbols have probability zero). This is strictly harder than the problem of distinguishing between $\Bern{1/2}$ and $\Bern{1/2+\alpha}$. The coupling given in Example~\ref{exm:coin} has expected hamming distance of $\alpha \ns$. Hence combing with Theorem~\ref{thm:le_cam}, by letting the RHS no larger than $\frac13$, we get a lower bound of $ \ns = \Omega\Paren{\min\Paren{\frac1{\dist\eps}, \frac1{\dist\delta} }} = \Omega({\frac{1}{\dist (\eps+\delta)}})$.

We now consider the cases $\ns \le \ab$ and $\ab< \ns \le \frac{\ab}{\alpha^2}$.

%The final term is a lower bound for testing identity to $\Bern{0.5}$, which is easier than uniformity testing by Theorem~\ref{thm:unif-identity}. 

To this end, we invoke our private LeCam's method, and design a hypothesis testing problem that will imply a lower bound on uniformity testing. The testing problem will be to distinguish between the following two cases. 

{\bf Case 1:} We are given $\ns$ independent samples from the uniform distribution $\unifab$.

{\bf Case 2:} Generate a distribution $\p$ with $\dtv{\p}{\unifab}\ge\dist$ according to some prior over all such distributions. We are then given $\ns$ independent samples from this distribution $\p$. 

From Theorem~\ref{thm:le_cam}, any lower bound for distinguishing between these two cases is a lower bound on uniformity testing problem. 

We now describe the prior construction for {\bf Case 2}, which is the same as considered by~\cite{Paninski08} for lower bounds on identity testing without privacy considerations. For each $\textbf{z} \in\{\pm1\}^{\ab/2}$, define a distribution $\p_{\textbf{z}}$ over $[\ab]$ such that 
\begin{align}
\p_{\textbf{z}}(2i-1) = \frac{1+\textbf{z}_i\cdot 2\dist}{\ab}, \text{ and } \p_{\textbf{z}}(2i) = \frac{1-\textbf{z}_i\cdot 2\dist}{\ab}.\nonumber
\end{align}
Then for any $\textbf{z}$, $\dtv{P_{\textbf{z}}}{\unifab}= \alpha$. For {\bf Case 2}, choose  $\p$ uniformly from these $2^{\ab/2}$ distributions. Let $Q_2$ denote the distribution on $[\ab]^\ns$ by this process. In other words, $Q_2$ is a mixture of product distributions over $[\ab]$. 

In {\bf Case 1}, let $Q_1$ be the distribution of $\ns$ $i.i.d.$ samples from $\unifab$. 

To obtain a sample complexity lower bound for distinguishing the two cases, we will design a coupling between $Q_1$, and $Q_2$, and bound its expected Hamming distance. While it can be shown that the Hamming distance of the coupling between the uniform distribution with any \emph{one} of the $2^{\ab/2}$ distributions grows as $\alpha\ns$, it can be significantly smaller, when we consider the mixtures. In particular, the following lemma shows that there exist couplings with bounded Hamming distance. 

\begin{lemma}\label{lem:coupling-hamming}
	There is a coupling between $\Xon$ generated by $Q_1$, and $\Yon$ by $Q_2$ such that 
\begin{center}
   $\expectation{\ham{\Xon}{\Yon}} \le C \cdot \dist^2 \min \{ \frac{\ns^2}{\ab}, \frac{\ns^{3/2}}{{\ab}^{1/2}} \}$.
%    \begin{cases}
%                                   8\frac{\ns^2\dist^2}{\ab}, & \text{when $m \le k$} \\
%                                    C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}}, & \text{when $k< m \le \frac{k}{\alpha^2}$}.
%    \end{cases}
\end{center}
\end{lemma}
We refer the proof of the lemma to~\cite{AcharyaSZ18}. Now applying Theorem~\ref{thm:le_cam}, we get the bound in Theorem~\ref{thm:main-identity}.
%\begin{enumerate}
%	\item \newhz{For $m \le k$, $8\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/2}}{\alpha \eps^{1/2}}}$.}
%	\item \newhz{For $k< m \le \frac{k}{\alpha^2}$, $C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}} = \Omega \Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/3}}{\alpha^{4/3}\eps^{2/3}}}$.}
%\end{enumerate}

%\begin{lemma}
%There is a coupling between $\Xon$  generated by $Q_2$, and $\Yon$ by $Q_1$ such that for 
%\[
%\expectation{\ham{\Xon}{\Yon}} \le
%\begin{cases}
%O\Paren{\dist^2\cdot\frac{\ns^2}{\ab}} & \ns\le \ab,\\
%O\Paren{\dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}}& k\le \ns\le \ab/\alpha^2,\\
%%O\Paren{\alpha\ns}&  \ab/\alpha^2\le\ns.
%\end{cases}
%\]
%\label{lem:coupling-uniform}
%\end{lemma}

%We can rewrite this result as
%\begin{align}
%\expectation{\ham{\Xon}{\Yon}} \le
%O\Paren{\min\left\{\dist^2\cdot\frac{\ns^2}{\ab}, \dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}, \alpha\ns\right\}}\label{eq:coup-ub}
%\end{align}
%	For the proof of this lemma, we can refer to lemma
%
%
%
%Using lemma~\ref{lem:coupling-uniform}, we can apply the coupling lower bound to prove the lower bound. 
%\begin{theorem}
%\[
%\Sitd\ge \Omega\Paren{\max\left\{\frac{\ab^{1/2}}{\alpha(\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3}(\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.
%\]
%\end{theorem}


%This is proved in the following lemma. 


%The construction of $Q_2$, and the proof of Lemma~\ref{lem:coup_unif} is slightly technical and is given in Section~\ref{app:lb-unif}.
%Assuming this lemma, by Theorem~\ref{thm:coupling}, we need $\expectation{\ham{\Xon}{\Yon}}=\Omega\Paren{\frac1{\eps+\delta}}$ to distinguish between $Q_1$, and $Q_2$. For this to hold, we need $\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps+\delta}}$, which gives us 
%$\ns\ge \Omega\Paren{\frac{\sqrt \ab}{\dist\sqrt{\eps+\delta}}}$.




==> back_up/toolbox copy/uniformity.tex <==
\section{$(\eps,\delta)$-DP uniformity testing}
\label{sec:identity}

\newhzn{
In this section, we give a proof sketch of sample complexity lower bound of uniformity testing. The full detail can be referred to~\cite{AcharyaSZ18}. The main result is the following. }

\begin{theorem}
\label{thm:main-identity}
The sample complexity of $(\eps,\delta)$-DP identity testing is
$$\Sutd = \Theta\Paren{\frac{k^{1/2}}{\dist^2}+\max\left\{\frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.$$
%
%Or we can write it according to the parameter range,
%\[
%    \Sit =
%    \begin{cases}
%                                   \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}}, & \text{when $k = \Omega \Paren{\frac1{\alpha^4}}$ and $k = \Omega \Paren{\frac1{\alpha^2 (\eps+\delta)}}$,} \\
%              		  \Theta\Paren{\frac{\sqrt k}{\alpha^2} +\frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}}, & \text{when $k = \Omega \Paren{\frac{\alpha}{(\eps+\delta)}}$ and $k = O \Paren{\frac1{\alpha^4}+\frac1{\alpha^2 (\eps+\delta)} }$,}\\
%              		               \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac1{\alpha (\eps+\delta)}}, & \text{when  $k = O \Paren{\frac{\alpha}{(\eps+\delta)}}$.}\\ 
%    \end{cases}
%\]
\end{theorem}
We note that the lower bound is tight up to constant factors in all parameters. 

%In~\cite{AcharyaSZ18}, they show a reduction from identity to uniformity testing under differential privacy and design algorithms which achieve the matching upper bounds.
% 
%In this work, we focus on the lower bounds for identity testing. Since uniformity testing is a special case of identity testing, any lower bound for uniformity will port over to identity, and we give such bounds in Section~\ref{sec:lower-identity}.







==> commondefs <==
#
# Rules and definitions for building various things, especially 
# TeX documents.
# -- Andrew Myers
# Last updated April 2007
#

MAKEDIR = .
INCLDIR = .
TEXDIR = .

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux *.dvi *.log *.stamp *.i *.bbl *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS=$(TEXINPUTS) latex
PDFLATEX = TEXINPUTS=$(TEXINPUTS) pdflatex


==> commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	rm -f temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

.tex.pdf:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then \
	   echo makeindex $*.idx; \
	   makeindex $*.idx; \
	else \
	   echo touch $@; \
	   touch $@; \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo bibtex $*; sh -c "bibtex $(BIBOPTS) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules


==> cu_thesis-2.9/README <==
cornell-thesis 2.9
------------------

This package provides a "style file" for producing Ph.D. dissertations
at Cornell University using the new version of LaTeX, LaTeX 2e
which is now the only officially supported one. (If you haven't
upgraded to it yet, this file won't be of much use to you. Consider
upgrading.)

The distribution contains two source files:
cornell.dtx -- self-documenting LaTeX source code for the style file.
cornell.ins -- installation "script" for the docstrip package.

To install, you need to say "latex cornell.ins", then move the resulting
cornell.cls file somewhere where latex will find it.

Detailed (albeit still incomplete in places) documentation can be be
found in the file "cornell.pdf". This documentation can also be generated
by saying "pdflatex cornell.dtx" twice (or use latex if you want a .dvi file).

There is also a sample thesis document that you can use as a template
for writing your thesis, in "sampleThesis.tex". You can build this by
running "latex sampleThesis" and "bibtex sampleThesis" until things
converge (usually this takes three runs of "latex").

If you don't like typing "latex" so much, and you have "make" available,
you can type "make" to build the document class file and the sample
thesis document. You may also want to use the supplied Makefile as a starting
point for building your own thesis.

Comments from Sergio:

    This style file does not have official status: I just happen to have
    typeset my thesis with the new LateX 2e, using this style file, and the
    thesis secretary seemed fairly pleased with the result. I am making it
    available in the hope that the horror stories about people's encounters
    with the thesis secretary may become a thing of the past... but remember:
    requirements do change, and this style file doesn't remove the need for you
    to heed TeX's warning messages about overfull boxes and pages.

    An older style file for LaTeX 2.09 is still available in various places on
    campus. I used it as a starting point, but added a few enhancements of my
    own.

    I have no plans to maintain this thing. Users are on their own.  But at
    least I tried to document it as fully as time allowed me.

Change Log

v1.0d Converted ## to # as per changes in June 1995 LaTeX release.
v1.1  Changed openbib conditionals to a single command as per changes
           in December 1995 LaTeX release.
v1.2  Moved headers for opening pages to top of page.
v2.0  Chapter headers now consistent throughout.
      Fixed margins.
v2.1  Bug fix for titles containing \\
v2.5  Addition of halfcornellheadings and smallerheadings options
v2.6  Addition of draft, semifinal and final options
v2.7  Corrected interline spacing to really be double spacing
      (i.e, 24pt for 12pt text).  Changed ``cornell'' pagestyle to
      center page numbers at the bottom of the page.
v2.8  When using pdflatex, page size is set to 8.5x11 automatically.
      Copyright and dedication now center properly on page without special hacks.
      \ifpdf macro added to detect use of pdflatex
      A sample thesis document is included in the package.
      A sample Makefile is included in the package (use is optional).
v2.9  Made "cornellheadings" the default, as the thesis guidelines now
      require them for appendices. Also fixed line spacing and margins
      on the title page. Changed sample document to palatino, since
      Times 12 is not approved.


==> cu_thesis-2.9/commondefs <==
#
# Rules and definitions for building various things, especially 
# TeX documents.
# -- Andrew Myers
# Last updated April 2007
#

MAKEDIR = .
INCLDIR = .
TEXDIR = .

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux *.dvi *.log *.stamp *.i *.bbl *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS=$(TEXINPUTS) latex
PDFLATEX = TEXINPUTS=$(TEXINPUTS) pdflatex


==> cu_thesis-2.9/commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	rm -f temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

.tex.pdf:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then \
	   echo makeindex $*.idx; \
	   makeindex $*.idx; \
	else \
	   echo touch $@; \
	   touch $@; \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo bibtex $*; sh -c "bibtex $(BIBOPTS) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules


==> distribution_estimation/abstract.tex <==
Le Cam's method, Fano's inequality, and Assouad's lemma are three widely used techniques to prove lower bounds for statistical estimation tasks. We propose their analogues under central differential privacy. Our results are simple, easy to apply and we use them to establish sample complexity bounds in several estimation tasks. 

\noindent{We establish the optimal sample complexity of discrete distribution estimation under total variation distance and $\ell_2$ distance. We also provide lower bounds for several other distribution classes, including product distributions and Gaussian mixtures that are tight up to logarithmic factors. The technical component of our paper relates coupling between distributions to the sample complexity of estimation under differential privacy. 
}
%\anote{Perhaps add more in terms of upper bounds and some applications in the abstract?}
%Learning distributions from samples is a fundamental statistical learning task. When the samples are collected from users, how to protect each user's privacy has garnered wide interest in the recent years. We study the problem of learning $\ab$-ary discrete distributions under differential privacy. We show that the sample complexity of learning a distribution up to TV distance $\alpha$ ($\ell_2$ distance $\beta$) under $\eps$ pure differential privacy is $\Theta(\frac{k}{\alpha^2} + \frac{k}{\alpha \eps})$ ($\tilde{\Theta}(\frac{1}{\beta^2} + \frac{\min \{\sqrt{k}, 1/\beta\}}{\beta\eps})$ ). %\todo{HZ: this is incorrect, even if we change max to min. We do not have tight bounds in l2 distance.}
%The upper bound is obtained by adding Laplace noise to the empirical estimator. For the lower bound part, we extend the classical Fano's inequality to the case with differential privacy constraint, which can be of independent interest. The technique also gives tight lower bounds for learning product distributions and Gaussian mixtures.

==> distribution_estimation/glodef.tex <==
% Theorem-like environments

\usepackage{lmodern}
%\usepackage{xspace}
\usepackage[protrusion=true,expansion=true]{microtype}
%\usepackage{fullpage}
\usepackage{amsfonts, pbox}

% Colors (with names)

% Colors (with names)
%\usepackage[usenames,dvipsnames,table,xcdraw]{xcolor}


%\usepackage[usenames,dvipsnames,table]{xcolor}
%\usepackage[colorlinks,citecolor=blue, bookmarks=true]{hyperref}

% Required for the table of results
\usepackage{multirow}
\usepackage{dsfont} %\indic
%\usepackage{fullpage}

\newcommand{\insertref}[1]{\todo[color=green!40]{#1}}
\newcommand{\explainindetail}[1]{\todo[color=red!30]{#1}}
\newcommand{\inlinetodo}[1]{\todo[color=blue!25,inline]{#1}}

% Algorithm environment
%\usepackage{algorithmicx,algpseudocode,  algorithm}
\providecommand\algorithmname{Algorithm}
\providecommand*{\factautorefname}{Fact}

% compact lists, and handy shortcuts for items
\usepackage[shortlabels]{enumitem}
\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
\setenumerate{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}


\makeatletter
\@ifundefined{theorem}{% Theorems (each with its own style)
  \theoremstyle{plain}
  \newtheorem{theorem}{Theorem}
  \newtheorem{corollary}[theorem]{Corollary}
  %\newtheorem{corollary}{Corollary}
  \newtheorem{lemma}[theorem]{Lemma}
  \newtheorem{claim}[theorem]{Claim}
  \newtheorem{fact}{Fact}
  \newtheorem*{unnumberedfact}{Fact}
   \theoremstyle{definition}
  \newtheorem{definition}[theorem]{Definition}
  \theoremstyle{remark}
  \newtheorem{remark}{Remark}
  \newtheorem{question}{Question}
  \newtheorem*{notation}{Notation}
  \newtheorem{example}{Example}
  \newtheorem{observation}{Observation}
}{}
\makeatother
\newenvironment{proofof}[1]{\noindent{\bf Proof of {#1}:~~}}{\(\qed\)}

% Begin / End Theorems

\def \bthm#1{\begin{#1}\upshape\quad}
\def \ethm#1{\rqed\end{#1}}
\def \ethmp#1{\end{#1}}     % No box, when ends in displayed equation

\def \bClaim     {\bthm{Claim}}
\def \eClaim     {\ethm{Claim}}
\def \eClaimp    {\ethmp{Claim}}
\def \bConjecture {\bthm{Conjecture}}
\def \eConjecture {\ethm{Conjecture}}
\def \eConjecturep{\ethmp{Conjecture}}
\def \bCorollary {\bthm{Corollary}}
\def \eCorollary {\ethm{Corollary}}
\def \eCorollaryp{\ethmp{Corollary}}
\def \bCounter   {\bthm{CounterExample*}}
\def \eCounter   {\ethm{CounterExample*}}
\def \eCounterp  {\ethmp{CounterExample}}
\def \bDefinition{\bthm{Definition}}
\def \eDefinition{\ethm{Definition}}
\def \eDefinitionp{\ethmp{Definition}}
\def \bExample   {\bthm{Example}}
\def \eExample   {\ethm{Example}}
\def \eExamplep  {\ethmp{Example}}
\def \bExercise  {\bthm{Exercise}}
\def \eExercise  {\ethm{Exercise}}
\def \eExercisep {\ethmp{Exercise}}
\def \bIntuition {\bthm{Intuition}}
\def \eIntuition {\ethmp{Intuition}}
\def \bJoke      {\bthm{Joke}}
\def \eJoke      {\ethm{Joke}}
\def \bLemma     {\bthm{Lemma}}
\def \eLemma     {\ethm{Lemma}}
\def \eLemmap    {\ethmp{Lemma}}
\def \bOpen      {\bthm{Open problem}}
\def \eOpen      {\ethm{Open problem}}
\def \eOpenp     {\ethmp{Open problem}}
\def \bProperty  {\bthm{Property}}
\def \eProperty  {\ethm{Property}}
\def \ePropertyp {\ethmp{Property}}
\def \bQuestion  {\bthm{Question}}
\def \eQuestion  {\ethm{Question}}
%\def \bRemark    {\bthm{Remark}}
%\def \eRemark    {\ethm{Remark}}
\def \bResult    {\bthm{Result}}
\def \eResult    {\ethm{Result}}
\def \bTheorem   {\bthm{Theorem}}
\def \eTheorem   {\ethm{Theorem}}
\def \eTheoremp  {\ethmp{Theorem}}

% Environments

\newenvironment{Problem}{\textbf{Problem}\\ \begin{enumerate}}{\end{enumerate}}
\newenvironment{Problems}{\textbf{Problems}\\ \begin{enumerate}}{\end{enumerate}}

%\newenvironment{Problems}{\begin{trivlist}\item[]{\textbf{Problems}}{\end{trivlist}}}

% Headers

\def \skpbld#1{\par\noindent\textbf{#1}\quad}
\def \skpblds#1{\skpbld{#1}\par\noindent}

\def \Answer   {\skpbld{Answer}}
\def \Answers  {\skpblds{Answers}}
\def \Basis    {\skpbld{Basis}}
\def \Check    {\skpbld{Check}}
%\def \Example  {\skpbld{Example}}
\def \Examples {\skpbld{Examples}}
\def \Intuition{\skpbld{Intuition}}
\def \Method   {\skpbld{Method}}
\def \Methods  {\skpblds{Methods}}
\def \Outline  {\skpbld{Outline}}
\def \Proof    {\skpbld{Proof}}
\def \Proofs   {\skpblds{Proofs}}
%\def \Problem  {\skpbld{Problem}}
%\def \Problems {\skpblds{Problems}}
\def \Proline  {\skpbld{Proof Outline}}
%\def \Remark   {\skpbld{Remark}}
\def \Remarks  {\skpblds{Remarks}}
\def \Solution {\skpbld{Solution}}
\def \Solutions{\skpblds{Solutions}}
\def \Verify   {\skpbld{Verify}}
\def \Step     {\skpbld{Step}}

% Ignores

\newcommand{\ignore}[1]{}

% Problems & solutions

\newcommand{\problem}[1]{#1}
\newcommand{\solution}[1]{{\\ \bf Solution}\quad #1}
%\newcommand{\solution}[1]{\mbox{}\\ \medskip\noindent{\bf Solution\medskip}#1}
%\newcommand{\solution}[1]{}

\newcommand{\source}[1]{(Taken from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\modifiedfrom}[1]{(Modified from~\cite{#1})}
%\newcommand{\modifiedfrom}[1]{}

\newcommand{\takenfrom}[1]{(Taken from~\cite{#1})}
%\newcommand{\takenfrom}[1]{}

\newcommand{\reportedby}[1]{Reported by #1.}
%\newcommand{\reportedby}[1]{}

\newcommand{\hint}[1]{Hint: #1}
%\newcommand{\hint}[1]{}

\newcommand{\joke}[1]{\footnote{#1}}
\newcommand{\trivia}[1]{\footnote{#1}}

% Equation formatting

\newcommand{\spreqn}[1]{{\qquad\text{#1}\qquad}}

% Blackboard fonts
\newcommand{\II}{\mathbb{I}} % Added by Theertha on April 16th 2013.
\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}

% probability
\newcommand{\expectation}[1]{\EE\left[#1\right]}
\newcommand{\variance}[1]{Var\left(#1\right)}

% Number sets

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\positives}{\PP}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}

\newcommand{\realsge}{{\reals_{\ge}}}
\newcommand{\realsp}{\reals^+}
\newcommand{\integersp}{\integers^+}
\newcommand{\integerss}[1]{\integers_{\ge{#1}}}

% boldface

\def \ba     {{\bf a}}
\def \bx     {{\bf x}}
\def \by     {{\bf y}}

\def \bA     {{\bf A}}
\def \bB     {{\bf B}}
\def \bC     {{\bf C}}
\def \bD     {{\bf D}}
\def \bF     {{\bf F}}
\def \bG     {{\bf G}}
\def \bL     {{\bf L}}
\def \bQ     {{\bf Q}}
\def \bR     {{\bf R}}
\def \bS     {{\bf S}}
\def \bT     {{\bf T}}
\def \bX     {{\bf X}}
\def \bY     {{\bf Y}}
\def \bZ     {{\bf Z}}

% caligraphics

\def \cA     {{\cal A}}
\def \cB     {{\cal B}}
\def \cC     {{\cal C}}
\def \cD     {{\cal D}}
\def \cE     {{\cal E}}
\def \cF     {{\cal F}}
\def \cG     {{\cal G}}
\def \cH     {{\cal H}}
\def \cI     {{\cal I}}
\def \cK     {{\cal K}}
\def \cL     {{\cal L}}
\def \cM     {{\cal M}}
\def \cN     {{\cal N}}
\def \cO     {{\cal O}}
\def \cP     {{\cal P}}
\def \cQ     {{\cal Q}}
\def \cR     {{\cal R}}
\def \cS     {{\cal S}}
\def \cT     {{\cal T}}
\def \cU     {{\cal U}}
\def \cV     {{\cal V}}
\def \cW     {{\cal W}}
\def \cX     {{\cal X}}
\def \cY     {{\cal Y}}
\def \cZ     {{\cal Z}}

% vectors

\def \vct#1{{\overline{#1}}}

\def \vcta  {{\vct a}}
\def \vctb  {{\vct b}}
\def \vctq  {{\vct q}}
\def \vcts  {{\vct s}}
\def \vctu  {{\vct u}}
\def \vctv  {{\vct v}}
\def \vctx  {{\vct x}}
\def \vcty  {{\vct y}}
\def \vctz  {{\vct z}}
\def \vctp  {{\vct p}}

\def \vctV  {{\vct V}}
\def \vctX  {{\vct X}}
\def \vctY  {{\vct Y}}
\def \vctZ  {{\vct Z}}

\def \vctbeta  {{\vct\beta}}

% Random variables

\newcommand{\rnd}[1]{{\boldsymbol #1}}

\newcommand{\rndd}{{\rnd d}}
\newcommand{\rndl}{{\rnd l}}
\newcommand{\rndp}{{\rnd p}}
\newcommand{\rnds}{{\rnd s}}
\newcommand{\rndx}{{\rnd x}}
\newcommand{\rndy}{{\rnd y}}
\newcommand{\rndz}{{\rnd z}}

%\newcommand{\poi}{{\rm poi}}
\newcommand{\Var}{{\rm Var}}

% following should not exist (indicate random sets)

\newcommand{\rndR}{{\rnd R}}
\newcommand{\rndT}{{\rnd T}}

% arrow vectors

\newcommand{\rvc}{{\overrightarrow c}}

% Abbreviations - \xspace puts space iff there is space after command

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish
%\newcommand{\iid}{\textit{i.i.d.}\xspace} 
\newcommand{\iid}{\textit{i.i.d.}} % Edit by Theertha, \xspace not compiling

\newcommand{\etc}{etc.\@\xspace}

% Colors

%\definecolor{light}{gray}{.75}


% marginal notes

\newcommand{\mrgs}[2]{\# #1 \#{\marginpar{#2}}}

\newcommand{\mrgcgd}[1]{\mrgs{#1}{CHANGED}}
\newcommand{\mrgchk}[1]{\mrgs{#1}{CHECK}}
\newcommand{\mrgfix}[1]{\mrgs{#1}{FIX}}
\newcommand{\mrgnew}[1]{\mrgs{#1}{NEW}}

% qed's --  Also consider \qedhere

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}

\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \ok    {1\upto k}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \set#1#2{{\sets{{#1}\upto{#2}}}}

\def \setpmo   {\sets{\pm 1}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \setok    {\{\ok\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \inseg#1{{[#1]}} % use \intsgm instead
\newcommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations


%\DeclareMathOperator*{\union}{\cup}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Union}{\bigcup}  %Commented by Theertha on April 15

\newcommand{\unionl}{\union\limits}
\newcommand{\Unionl}{\Union\limits}
 
%\DeclareMathOperator*{\inter}{\cap}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Inter}{\bigcap}   %Commented by Theertha on April 15

\newcommand{\interl}{\inter\limits}
\newcommand{\Interl}{\Inter\limits}

% Floors, Ceilings, Absolute value

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}
\def \absvlu#1{{|#1|}}
\def \Absvlu#1{{\left|{#1}\right|}}
\newcommand{\absv}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|_2}
% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}
\def \Brace#1{\left\{#1\right\}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory

\newcommand{\base}[2]{{[#1]_{#2}}}

% equalities

\newcommand{\ed}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{{:=}}

\newcommand{\cnvprb}{\stackrel{\mathrm{p}}{\to}}
\newcommand{\cnvdst}{\stackrel{\mathrm{d}}{\to}}
\newcommand{\cnvas}{\stackrel{\mathrm{a.s.}}{\to}}

\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

\newcommand{\al}[1]{\stackrel{\mathit{{#1}}}{<}}
\newcommand{\ag}[1]{\stackrel{\mathit{{#1}}}{>}}
\newcommand{\ale}[1]{\stackrel{\mathit{{#1}}}{\le}}
\newcommand{\age}[1]{\stackrel{\mathit{{#1}}}{\ge}}
\newcommand{\aeq}[1]{\stackrel{\mathit{{#1}}}{=}}

%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

\newcommand{\re}{\sim}
\newcommand{\rle}{\stackrel<\sim} % roughly (asymptotically taken) <=
%\newcommand{\rl}{\stackrel<\sim}
\newcommand{\rge}{\stackrel>\sim}
%\newcommand{\rg}{\stackrel>\sim}

\newcommand{\ere}{\approx} % exponentially roughly equal
\newcommand{\erle}{\stackrel<\approx}
%\newcommand{\erl}{\stackrel<\approx}
\newcommand{\erge}{\stackrel>\approx}
%\newcommand{\erg}{\stackrel>\approx}

% Relations

\newcommand{\independent}{\perp\!\!\!\perp}

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% probability

\newcommand{\pr}{{p}} % phase out in favor of \prb
\newcommand{\prb}{{p}} 

\newcommand{\prbs}[1]{{\prb^{(#1)}}}

\newcommand{\Prb}{\text{Pr}}
%\newcommand{\Pr}{{\text{Pr}}} % phase out in favor of \Prb
\newcommand{\Prn}{\text{Pr}}  % phase out in favor of \Prb

\newcommand{\Prs}[1]{\Pr\Paren{#1}} % phase out in favor of \Prbs
\newcommand{\Prbs}[1]{{\Prb^{(#1)}}} % Check if used - phase out
\newcommand{\probof}[1]{\Pr\Paren{#1}}

% notation

\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\newcommand{\flnpwr}[2]{{#1^{\underline{#2}}}} % Falling power

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\pfx}{{\prec}}
\newcommand{\pfxeq}{{\preceq}}

\newcommand{\sfx}{{\succ}}
\newcommand{\sfxeq}{{\succeq}}

% for old documents

\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{				% grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}


\newcommand{\Sparen}[1]{\left[#1\right]}
\newcommand{\Order}{O}
\newcommand{\order}{o}


\newtheorem{prop2}[theorem]{Proposition}
\newtheorem{lem2}[theorem]{Lemma}
\newtheorem{coro2}[theorem]{Corollary}







==> distribution_estimation/intro2.tex <==
\section{Introduction}
{
Statistical estimation tasks are often characterized by the optimal trade-off between the sample size and estimation error. There are two steps in establishing tight sample complexity bounds: An information theoretic lower bound on sample complexity and an algorithmic upper bound that achieves it.}
%Statistical estimation tasks are often characterized by their rates or sample complexity which characterizes the optimal trade-off between the sample size and error in estimation. There are two parts to establishing sample complexity bounds: An information theoretic lower bound on sample complexity, and an algorithmic upper bound that achieves it.
Several works %\amargin{Get bunch of references from YU, BIN?}
have developed general tools to obtain the lower bounds (e.g.,~\cite{LeCam73, Assouad83, IbragimovK13, BickelR88, devroye1987course, verdu1994generalizing, CoverT06, ScarlettC19}, and references therein), {and three prominent techniques are Le Cam's method, Fano's inequality, and Assouad's lemma.} An exposition of {these three methods and their connections} is presented in~\cite{Yu97}\footnote{The title of~\cite{Yu97}, ``Assouad, Fano, and Le Cam'' is the inspiration for our title.}. 

%\noindent\textbf{Setting.} Let $\cP$ be a family of distributions over $\cX^\ns$, and let $\ell:\cP\times\cP\to\RR_{\ge0}$ be a distance measure between distributions in $\cP$. Here $\ns$ denotes the number of samples, and $\cX$ is the underlying domain of the individual samples.

In several estimation tasks, individual samples have sensitive information that must be protected. 
%has gathered much attention when the samples are collected from different users with the concern of each user's privacy.  %The data samples used in several applications can contain sensitive information about individuals who contribute to the samples. 
This is particularly of concern in applications such as healthcare, finance, geo-location, etc. Privacy-preserving computation has been studied in various fields including database, cryptography, statistics and machine learning~\cite{Warner65, Dalenius77, DinurN03, WassermanZ10, DuchiJW13, ChaudhuriMS11}. Differential privacy (DP)~\cite{DworkMNS06}, which allows statistical inference while preserving the privacy of the individual samples, has become one of the most {popular notions of privacy}~\cite{DworkMNS06, WassermanZ10, DworkRV10, BlumLR13, McSherryT07, DworkR14, KairouzOV17}. Differential privacy has been adopted by the US Census Bureau for the 2020 census and several large technology companies, including Google, Apple, and Microsoft~\cite{ErlingssonPK14, AppleDP17, DingKY17}.

\medskip
\noindent\textit{Differential privacy}~\cite{DworkMNS06}. {Let $\cX$ denote an underlying data domain of individual data samples} and {$\cX^\ns$ be the set of all possible length-$n$ sequences over $\cX$}. For $x, y\in \cX^\ns$, $\ham{x}{y}$ is their Hamming distance, the number of coordinates they differ at. A (randomized) estimator $\hat\theta:\cX^\ns\to\Theta$ is \emph{$(\eps,\delta)$-differentially private} (denoted {as} $(\eps,\delta)$-DP) if for any $S \subseteq \Theta$, and all $x, y\in\cX^\ns$ with $\ham{x}{y}\le 1$, the following holds:
	\begin{align}
		\probof{\hat\theta(x)\in S}\le e^{\eps} \cdot \probof{\hat\theta(y)\in S}+\delta.\label{eqn:dp-definition}
	\end{align}

The case $\delta=0$ is \emph{pure differential privacy} and is denoted by $\eps$-DP. We consider problems of parameter estimation and {goodness-of-fit (hypothesis testing)} under differential privacy constraints.
\medskip

\noindent\textbf{Setting.} Let $\cP$ be \emph{{any}} collection of distributions over $\cX^\ns$, {where $\ns$ denotes the number of samples.}\footnote{In the general setting, we are not assuming i.i.d. distribution over $\cX^\ns$, although we will specialize to this case later.} {Let $\theta:\cP\to\Theta$ be a parameter of the distribution that we want to estimate}. {Let $\ell:\Theta\times\Theta\to\RR_+$ be a pseudo-metric which is the loss function for estimating $\theta$. We now describe the minimax framework of parameter estimation, and hypothesis testing.}
%Let $\ell:\Theta\times\Theta\to\RR_+$ be a loss function (distance) between parameters.

\medskip

\noindent\textit{Parameter estimation.} The risk of an estimator $\hat{\theta}:\cX^\ns\to\Theta$ under loss $\ell$ is $\max_{\p \in \cP} \EE_{X \sim \p}\left[\ell(\hat \theta (X),\theta(p))\right]$, {the worst case expected loss of $\hat\theta$ over $\cP$. Note that $X\in\cX^\ns$, since $\p$ is a distribution over $\cX^\ns$. The minimax risk of estimation under $\ell$ for the class $\cP$ is}
\begin{align*}
R(\cP, \ell) := \min_{\hat \theta}\ \max_{\p \in \cP}\ \EE_{X \sim \p}\left[\ell(\hat \theta (X),\theta(p))\right].
\end{align*}
{The minimax risk under differentially private protocols is given by restricting $\hat\theta$ to be differentially private. For $(\eps, \delta)$-DP, we study the following minimax risk:} 
\begin{align}
R(\cP, \ell, \eps, \delta) := \min_{\hat \theta \text{ is }(\eps,\delta)\text{-DP}}\ \max_{\p \in \cP}\ \EE_{X \sim \p}\left[\ell(\hat \theta (X),\theta(p))\right].\label{eqn:minmax-risk}
\end{align}
For $\delta=0$, the above minimax risk under $\eps$-DP is denoted as $R(\cP, \ell, \eps)$. 

\medskip

\noindent\textit{Hypothesis testing.} Hypothesis testing can be cast in the framework of parameter estimation as follows. {Let $\cP_1\subset \cP$, and $\cP_2\subset \cP$ be two disjoint subsets of distributions denoting the two hypothesis classes. Let $\Theta=\{1,2\}$, such that for $\p\in\cP_i$, let $\theta(p)=i$. For a test $\hat\theta:\cX^n\to \{1,2\}$, and $\ell(\theta, \theta')=\II\{\theta\ne\theta'\}=|\theta-\theta'|$,} {the error probability is the worst case risk under this loss function:}
\begin{align}
P_e(\hat\theta, \cP_1, \cP_2):= \max_i \max_{\p\in \cP_i}\probofsub{ 
\newnewzs{X\sim \p}}{\hat\theta(X)\ne i } = \max_i \max_{\p\in 
\cP_i}\EE_{X\sim \p} 
\left[{|\hat\theta(X)-\theta(p)}|\right].\label{eqn:error-prob}
\end{align}


%\noindent\textit{Hypothesis testing.} Hypothesis testing can be cast in the framework of parameter estimation as follows. \newa{Let $\cP_1\subset \cP$, and $\cP_2\subset \cP$ be two disjoint subsets of distributions denoting the two hypothesis classes. Let $\Theta=\{1,2\}$, such that for $\p\in\cP_i$, let $\theta(p)=i$. For a test $\hat\theta:\cX^n\to \{1,2\}$, and $\ell(\theta, \theta')=\II\{\theta\ne\theta'\}=|\theta-\theta'|$. The error probability is the minimax risk under this loss function:}
%\begin{align}
%P_e(\hat\theta, \cP_1, \cP_2):= \max_i \max_{\p\in \cP_i}\probof{\hat\theta(X)\ne i \mid X\sim \p} = \max_i \max_{\p\in \cP_i}\EE_{X\sim \p} \left[{|\hat\theta(X)-\theta(p)}|\right].\label{eqn:error-prob}
%\end{align}



%\vspace{-20pt}

\smallskip
\noindent\textbf{Organization.} The remainder of the paper is organized as follows. In Section~\ref{sec:dp-lecam},~\ref{sec:dp-fano}, and~\ref{sec:dp-assouad} we state the privatized versions of Le Cam, Fano, and Assouad's method respectively. In Section~\ref{sec:applications} we discuss the applications of these results to several estimation tasks. In Section~\ref{sec:related} we discuss some related and prior work. In Section~\ref{sec:pdp_estimation} and~\ref{sec:adp_applications} we prove the bounds for distribution estimation under pure DP and approximate DP respectively. In Section~\ref{sec:proofs}, we prove the main theorems stated in Section~\ref{sec:results}.  
 
\section{Results}
\label{sec:results}
Le Cam's method is used to establish lower bounds for hypothesis testing and functional estimation. Fano's inequality, and Assouad's lemma prove {lower bounds} for multiple hypothesis testing problems and can be applied to parameter estimation tasks such as estimating distributions. We \newhzn{develop} extensions of these results with differential privacy. 


\medskip

{
\noindent\textit{An observation.} 
A \emph{coupling} between distributions $\p_1$ and $\p_2$ over 
$\cX^\ns$ is a joint distribution $(X,Y)$ over $\cX^\ns \times\cX^\ns$ 
whose marginals satisfy $X \sim \p_1$ and $Y \sim 
\p_2$\footnote{\newnewzs{We use the term coupling to refer to both the random 
variable $(X,Y)$ and the joint distribution.}}. 
%For simplicity, we treat coupling as a randomized function $f: \cX^\ns\to\cX^\ns$ such that if $X\sim\p$, then $Y=f(X)\sim\q$. Note that $X$, and $Y$ are not necessarily independent. 
Our lower bounds are based on the following observation. If there is a coupling $(X,Y)$ between distributions $\p_1$ and $\p_2$ over $\cX^\ns$ with $\expectation{\ham{X}{Y}}=D$, then a draw from $\p_1$ can be converted to a draw from $\p_2$ by changing $D$ coordinates in expectation. 
%We then apply~\eqref{eqn:dp-definition} for any DP algorithm that distinguishes $p_1$ and $p_2$ about $D$ times.}
\newzs{By the group property of differential privacy, roughly speaking, for 
any $(\eps,\delta)$-DP estimator $\hat{\theta}$, it must satisfy $$\forall 
S\subseteq \Theta, \probofsub{ 
		\newnewzs{X\sim \p}}{\hat\theta(X) \in S} \le e^{D\eps}\cdot 
		\probofsub{ 
		\newnewzs{X\sim \q}}{\hat\theta(Y) \in S}+ \delta D e^{\eps(D-1)}.$$
	Hence, if there exists an algorithm that distinguishes between $\p_1$ and $\p_2$ reliably, $D$ must be large ($\Omega\Paren{1/\eps+\delta}$).}


\subsection{DP Le Cam's method}
\label{sec:dp-lecam}
\newhz{
Le Cam's method (Lemma 1 of~\cite{Yu97}) is widely used to prove lower bounds for composite hypothesis testings such as uniformity testing~\cite{Paninski08}, density estimation~\cite{Yu97, ray2016cam}, and estimating functionals of distributions~\cite{JiaoVHW15, WuY16, polyanskiy2019dualizing}.}
%\amargin{Find more applications ... check this paper to add ... Dualizing le cam by Yihong wu and yury}  

%We use the expected Hamming distance between couplings of distributions in the two classes to obtain the following extension of Le Cam's method with $(\eps, \delta)$-DP. \anew{Coupling based lower bounds for DP appeared independently in~\cite{AcharyaSZ18, KarwaV18}.~\cite{KarwaV18} established their results for simple hypothesis testing where $\p_1$ and $\p_2$ below are i.i.d. distributions. The result below is similar to the result in~\cite{AcharyaSZ18} which was stated for arbitrary distributions over $\cX^\ns$ and used to establish sample complexity lower bounds for composite hypothesis testing problems.} For the hypothesis testing problem described above, let $\text{co}(\cP_i)$ be the convex hull of distributions in $\cP_i$, which are also families of distributions over $\cX^\ns$.

We use the expected Hamming distance between couplings of distributions in the two classes to obtain the following extension of Le Cam's method with $(\eps, \delta)$-DP, which is an adaptation of a similar result in~\cite{AcharyaSZ18}. For the hypothesis testing problem described above, let $\text{co}(\cP_i)$ be the convex hull of distributions in $\cP_i$, which are also families of distributions over $\cX^\ns$.

\begin{restatable}[$(\eps, \delta)$-DP Le Cam's method]{theorem}{dplecam}
	\label{thm:le_cam}
	Let $\p_1\in\text{co}(\cP_1)$ and $\p_2\in\text{co}(\cP_2)$. Let $(X,Y)$ be a coupling between $\p_1$ and $\p_2$ with $D=\expectation{\ham{X}{Y}}$. Then for $\eps\ge0, \delta\ge0$, any $(\eps,\delta)$-differentially private  hypothesis testing algorithm $\hat{\theta}$ must satisfy 
	\begin{align}
	P_e(\hat{\theta}, \cP_1, \cP_2)  \ge  \frac12 \max \left\{  1-\dtv{p_1}{p_2}, 0.9 e^{-10 \eps D} - 10 D \delta\right\},\label{eqn:le-cam}
	\end{align}
	{where $\dtv{p_1}{p_2} := \sup_{A \subseteq \cX^\ns} 
	\Paren{p_1(A)-p_2(A)}=\frac12\|\p_1 -  \p_2\|_1$ is the total 
	variation (TV) distance of $p_1$ and $p_2$.}
\end{restatable}
%\begin{theorem}[$(\eps, \delta)$-DP Le Cam's method]
%\label{thm:le_cam}
%Let $\p_1\in\text{co}(\cP_1)$ and $\p_2\in\text{co}(\cP_2)$. Let $(X,Y)$ be a coupling between $\p_1$ and $\p_2$ with $D=\expectation{\ham{X}{Y})}$. Then for $\eps\ge0, \delta\ge0$, any $(\eps,\delta)$-differentially private binary hypothesis testing algorithm $\cA$ must satisfy 
%\begin{align*}
%	P_e(\cA, \cP_1, \cP_2)  \ge  \frac12 \max \big\{  1-\dtv{p_1}{p_2}, \left(0.9 e^{-10 \eps D} - 10 D \delta\right) \big\}.
%\end{align*}
%\end{theorem}
The first term here is the original Le Cam's result~\cite{LeCam73, LeCam86, Yu97, Canonne15} and the second term is a lower bound on the additional error due to privacy. \newzs{Note that the second term increases when $D$ decreases. Choosing $\p_1, \p_2$ with small $D$ makes the RHS of~\eqref{eqn:le-cam} large, hence giving better testing lower bounds.} {A similar result (Theorem 1 in~\cite{AcharyaSZ18})}, along with a suitable coupling was used in~\cite{AcharyaSZ18} to obtain the optimal sample {complexity of testing discrete distributions}. We defer the proof of this theorem to Section~\ref{sec:le}.
%{~\cite{AcharyaSZ18} used their result with a suitable coupling to obtain the optimal sample complexity of the composite hypothesis testing problem of testing discrete distributions (see Section~\ref{??}). \anew{An independent result of~\cite{KarwaV18} obtained a similar result for testing simple hypotheses, where $\p_1$ and $\p_2$ are both i.i.d. distributions over $\cX^\ns$, and $D$ is }
%\medskip

%\noindent\textbf{Applications.} The \newhz{private} Le Cam's method has found usage in several applications. Theorem~\ref{thm:le_cam} can be used to establish optimal sample complexity for testing uniformity of discrete distributions~\cite{AcharyaSZ18, AliakbarpourDR18}, and for establishing lower bounds of differentially private entropy and support size estimation~\cite{AcharyaKSZ18}. The key component to use this result is to design couplings with small \newhz{expected} Hamming distance. 

\subsection{DP Fano's inequality}
\label{sec:dp-fano}
\newzs{Theorem~\ref{thm:le_cam} (DP Le Cam's method) characterizes lower bounds for binary hypothesis testing. In estimation problems with multiple parameters, it is common to reduce the problem to a multi-way hypothesis testing problem. The following theorem, proved in Section~\ref{sec:fano_pro}, provides a lower bound on the risk of multi-way hypothesis testing under $\eps$-DP.}
%\amargin{I am adding definition of KL, not sure if we ever did.}
Let 
\[
D_{KL}\Paren{\p_i,\p_j}:=\sum_{x\in\cX^\ns}p_i(x)\log \frac{p_i(x)}{p_j(x)}
\]
 be the $KL$ divergence between (discrete) distributions $\p_i$ and $\p_j$. \footnote{\newzs{For continuous distributions, the summation is replaced with an integral and the probability mass functions are replaced with densities. We focus on discrete distributions in the proof while the results hold for continuous distributions as well.}}
%\begin{theorem} [$\eps$-DP Fano's inequality] \label{thm:dp_fano}
%	Let $\p_1, \p_2,...,\p_M\in\cP$ such that 
%	\begin{enumerate}[label=(\alph*)]
%		\item $\forall i \neq j \in [M]$, $\ell \Paren{\theta(\p_i),\theta(\p_j)} \ge \alpha$,
%		\item $\forall i,j \in [M]$, $D_{KL} \Paren{\p_i,\p_j} \le \beta$,
%		\item \label{item:dham} $\forall i,j \in [M]$, there exists a coupling $(X, Y)$ between $\p_i$ and $\p_j$ such that
%		\[
%		\expectation{\ham{X}{Y}} \le D, 
%		\]
%	\end{enumerate}
%	then
%	\begin{align} \label{eqn:fano_result}
%	R(\cP, \ell, \eps) \ge \max \Bigg\{ & \frac{\alpha}{2} \left(1 - \frac{\beta + \log 2}{\log M}\right), 0.4\alpha \min\left\{1, \frac{M}{e^{10\eps D}}\right\} \Bigg\}. \nonumber 
%	\end{align}
%\end{theorem}
%\amargin{remember to define coupling.}
\begin{restatable} [$\eps$-DP Fano's inequality] {theorem}{dpfano}
	\label{thm:dp_fano}
	Let $\cV=\{\p_1, \p_2,...,\p_M\}\subseteq \cP$ such that {for all $i\ne j$,} 
	\begin{enumerate}[label=(\alph*)]
		\item  $\ell \Paren{\theta(\p_i),\theta(\p_j)} \ge \alpha$,
		\item $D_{KL} \Paren{\p_i,\p_j} \le \beta$,
		\item \label{item:dham} there exists a coupling $(X, Y)$ between $\p_i$ and $\p_j$ such that $\expectation{\ham{X}{Y}} \le D$, then
	\end{enumerate}
	\begin{align} \label{eqn:fano_result}
		R(\cP, \ell, \eps) \ge \max \Bigg\{ & \frac{\alpha}{2} \left(1 - \frac{\beta + \log 2}{\log M}\right), 0.4\alpha \min\left\{1, \frac{M}{e^{10\eps D}}\right\} \Bigg\}. 
	\end{align}
\end{restatable}

\newzs{Under pure DP constraints, Theorem~\ref{thm:dp_fano} extends Theorem~\ref{thm:le_cam} to the multiple hypothesis case.} Non-private Fano's inequality (e.g., Lemma 3 of~\cite{Yu97}) requires only conditions $(a)$ and $(b)$ and provides the first term of the risk bound above. {Now, if we consider the second term, which is the additional cost due to privacy, we would require $\exp(10\eps D)\ge M$, \ie $D \ge {\log M}/{(10\eps)}$ to achieve a risk less than $0.4\alpha$.} Therefore, for reliable estimation, the expected Hamming distance between any pair of distributions cannot be too small. In Corollary~\ref{coro:fano}, we provide a corollary of this result to establish sample complexity lower bounds for several distribution estimation tasks.

	Theorem~\ref{thm:dp_fano} ($\eps$-DP Fano's inequality) can also be seen as a probabilistic generalization of the classic packing lower bound~\cite{Vadhan17}. The packing argument, with its roots in database theory, considers inputs to be deterministic datasets whose pairwise Hamming distances are bounded with probability one, while Theorem~\ref{thm:dp_fano} considers randomly generated datasets whose Hamming distances are bounded in expectation. This difference makes Theorem~\ref{thm:dp_fano} better suited for proving lower bounds for statistical estimation problems. We discuss this difference in details in Section~\ref{sec:related}.

\smallskip
\noindent\textbf{Remark.} {Theorem~\ref{thm:dp_fano} is a bound on the risk for pure differential privacy ($\delta=0$). Our proof extends to $(\eps,\delta)$-DP for \newhz{$\delta = O \Paren{\frac1M}$},  which is not sufficient to establish meaningful bounds since in most problems $M$ will be chosen to be exponential in the problem parameters. To circumvent this difficulty, in the next section we provide a private analogue of Assouad's method, which also works for $(\eps,\delta)$-DP.} 


%\noindent\textbf{Remark.} In Corollary~\ref{coro:fano} we present a corollary of this theorem that is easily applicable to establish sample complexity lower bounds for distribution estimation problems under $\eps$-DP.

%\medskip

%\noindent\textbf{Applications.} We use this theorem to establish the optimal sample complexity of estimating $k$-ary discrete distributions under total variation distance (Theorem~\ref{thm:pure-dv}), $k$-ary discrete distributions under $\ell_2$ distance (Theorem~\ref{thm:pure-l2}), and improved \newhz{sample complexity} lower bounds for product distributions (Theorem~\ref{thm:main_product}) and Gaussian mixtures (Theorem~\ref{thm:main_Gaussian}). 

\subsection{DP Assouad's method}
\label{sec:dp-assouad}
{Our next result is a private version of Assouad's lemma (Lemma 2 of~\cite{Yu97}, and~\cite{Assouad83}). Recall that $\cP$ is a set of distributions over $\cX^\ns$. Let $\cV\subseteq\cP$ be} a set of distributions indexed by the hypercube $ \cE_{\ab} := \{\pm 1\}^{\ab}$, and the loss  $\ell$ is such that
\begin{align}
\forall u,v \in \cE_{\ab}, \ell(\theta(\p_u), \theta(\p_v)) \ge 2\tau \cdot \sum_{i=1}^{\ab} \mathbb{I}\Paren{u_i\neq v_i}.
\label{eqn:assouad-loss}
\end{align}

{Assouad's method provides a lower bound on the estimation risk for distributions in $\cV$, which is a lower bound for $\cP$. For each coordinate $i\in[k]$, consider the following mixture distributions obtained by averaging over all distributions with a fixed value at the $i$th coordinate,}
\[
	\p_{+i}  =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e_i= + 1}\p_e, ~~~ \p_{-i}  =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e_i= -1}\p_e.
\]
Assouad's lemma provides a lower bound on the risk by using~\eqref{eqn:assouad-loss} and considering the problem of distinguishing $\p_{+i}$ and $\p_{-i}$. 
{Analogously, we prove the following privatized version of Assouad's lemma by considering the minimax risk of a private hypothesis testing $\phi:\cX^\ns\to\{-1,+1\}$ between $\p_{+i}$ and $\p_{-i}$. The detailed proof is in Section~\ref{sec:private_assouad}.
}
%In particular, we consider the minimax risk of a hypothesis test $\phi:\cX^\ns\to\{-1,+1\}$ between $\p_{+i}$ and $\p_{-i}$ to prove the following privatized version of Assouad's lemma, and prove it in Section~\ref{sec:private_assouad}. 
\begin{restatable} [DP Assouad's method] {theorem} {dpassouad}
	\label{thm:assouad} 
{$\forall i \in [k]$, let $\phi_i:\cX^\ns\to\{-1,+1\}$ be a binary classifier.%\amargin{I dont understand how we can have $\phi$ inside the summation below, and define one $\phi$ above.
	\begin{align*}
	R(\cP, \ell, \eps, \delta) \ge \frac{\tau}{2} \cdot \sum_{i=1}^{\ab} \min_{\phi_i \text{ is $(\eps, \delta)$-DP}}   ( \probofsub{ X\sim \p_{+i} }{ \phi_i(X) \neq 1 } 
	+ \probofsub{X\sim \p_{-i} }{\phi_i(X) \neq -1 } ). \nonumber
	\end{align*}
	Moreover, if $\forall i\in [\ab]$, there exists a coupling $(X,Y)$ between $\p_{+i}$ and $\p_{-i}$ with $\expectation{\ham {X} {Y}} \le D$,
	\begin{equation} \label{eqn:assouad}
	R(\cP, \ell, \eps, \delta) \ge \frac{\ab \tau}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}. 
	\end{equation} }
%	\begin{align*}
%	R(\cP, \ell, \eps, \delta) \ge R_1:= \frac{\tau}{2} \cdot \sum_{i=1}^{\ab} \min_{\phi_i \text{ is $(\eps, \delta)$-DP}}   ( \probofsub{ X\sim \p_{+i} }{ \phi_i(X) \neq 1 } 
%	+ \probofsub{X\sim \p_{-i} }{\phi_i(X) \neq -1 } ). \nonumber
%	\end{align*}
%Moreover, if $\forall i\in [\ab]$, there exists a coupling $(X,Y)$ between $\p_{+i}$ and $\p_{-i}$ with $\expectation{\ham {X} {Y}} \le D$,
%	\begin{equation} \label{eqn:assouad}
%	R(\cP, \ell, \eps, \delta) \ge \max\left\{R_1, \frac{\ab \tau}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}\right\}.
%	\end{equation}
\end{restatable}

%\begin{theorem}
%\label{thm:assouad}
%Let $\cE_{\ab}$, \newhz{ $\cV_k \subseteq \cP$} be as previously defined, and $\phi: X \rightarrow \{\pm1\}$ be a binary classifier.
%\begin{align*}
%	R(\cP, \ell, \eps, \delta) \ge \frac{\tau}{2} \cdot \sum_{i=1}^{\ab} \min_{ \phi: \phi \text{ is DP}}   ( \probofsub{ X\sim \p_{+i} }{ \phi(X) \neq 1 } 
%	+ \probofsub{X\sim \p_{-i} }{\phi(X) \neq -1 } ). \nonumber
%\end{align*}
%
%%\begin{equation}
%%\sup_{\p \in \cV_{\ab} } \EE_{X \sim \p} \left[ \ell(\p_{\he}, \p )\right] \ge \tau \cdot \sum_{i=1}^{\ab} \inf_{ \phi: \phi \text{ is DP}}  \Paren{ \probofsub{ X\sim \p_{+i} }{ \phi(X) \neq 1 } + \probofsub{X\sim \p_{-i} }{\phi(X) \neq -1 }}. \nonumber
%%\end{equation}
%Moreover, if $\forall i\in [\ab]$, there exists a coupling $(X,Y)$ between $\p_{+i}$ and $\p_{-i}$ with $\expectation{\ham {X} {Y}} \le D$,
%\begin{equation} \label{eqn:assouad}
%	R(\cP, \ell, \eps, \delta) \ge \frac{\ab \tau}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}. \nonumber
%\end{equation}
%\end{theorem}
\noindent The first bound is the classic Assouad's Lemma and~\eqref{eqn:assouad} is the loss due to privacy constraints. Once again note that~\eqref{eqn:assouad} grows with decreasing $D$. \newzs{Compared to Theorem~\ref{thm:dp_fano} (DP Fano's inequality), Theorem~\ref{thm:assouad} works under $(\eps, \delta)$-DP, which is a less stringent privacy notion.}
%\medskip
%\noindent\textbf{Applications.} We use Theorem~\ref{thm:assouad} to establish optimal sample complexity for $k$-ary discrete distributions under total variation distance (Theorem~\ref{thm:ApproximateDiscreteTotalVariation}), and $\ell_2$ distance (Theorem~\ref{thm:ApproximateDiscreteL2}). \newhz{say something about product}



 

==> distribution_estimation/locdef.tex <==
 \newcommand{\anew}[1]{{\color{black}#1}}
 \newcommand{\newzs}[1]{{\color{black}#1}}
  \newcommand{\newnewzs}[1]{{\color{black}#1}}
  
 \newcommand{\newhz}[1]{{\color{black}#1}}
 \newcommand{\newhzz}[1]{{\color{black}#1}}
 \newcommand{\newzz}[1]{{\color{black}#1}}
 
  \newcommand{\newhzn}[1]{{\color{black}#1}}

\newcommand{\Dk}{\Delta_k}
\newcommand{\D}{\Delta}
\newcommand{\Du}{\Delta_u}

\newcommand{\absz}{k}
\newcommand{\ab}{k}
\newcommand{\dims}{d}
\newcommand{\ns}{n}
\newcommand{\ber}{\cB}
\newcommand{\dP}{p}
\newcommand{\dQ}{q}
\newcommand{\mP}{p}
\newcommand{\mQ}{q}


\newcommand{\verify}[1]{\textcolor{black}{#1}}


\newcommand{\p}{p}
\newcommand{\q}{q}
\newcommand{\pn}[1]{\p^{#1}}
\newcommand{\qn}[1]{\q^{#1}}


\newcommand{\expectationsub}[2]{\EE_{#1}\left[#2\right]}
\newcommand{\probofsub}[2]{\Pr\nolimits_{#1}\Paren{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Sitnp}{S({\tt IT}, \ab, \dist)}

\newcommand{\Sit}{S({\tt IT}, \ab, \dist,\eps)}
\newcommand{\Sitd}{S({\tt IT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sut}[2]{S({\tt UT}, #1, #2,\eps)}
\newcommand{\Sutd}{S({\tt UT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sutnp}[2]{S({\tt UT}, #1, #2)}
\newcommand{\Sittwo}{S({\tt IT}, \ab, \dist,\eps)}
\newcommand{\Sct}{S({\tt CT}, \ab, \dist,\eps)}
\newcommand{\Sctd}{S({\tt CT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sctnp}{S({\tt CT}, \ab, \dist)}

\newcommand{\Smc}[1]{S({\tt MC},#1)}
\newcommand{\Sdl}[1]{S({\tt DL},\Delta_{\ab}, \alpha,\eps, #1)}
\newcommand{\Sdla}[1]{S({\tt DL},\Delta_{\ab}, \alpha,\eps,\delta, #1)}
\newcommand{\Sdlat}[2]{S({\tt DL},#1, \alpha,\eps,\delta, #2)}

\newcommand{\Pds}{C_{\ab, \dims}}
\newcommand{\Spl}{S({\tt PL},\Pds, \alpha,\eps, d_{TV})}
\newcommand{\Spla}{S({\tt PL},\Pds, \alpha,\eps, \delta, d_{TV})}

\newcommand{\absvn}[1]{\left\|#1\right\|_1}



\newcommand{\unif}{u}
\newcommand{\unifab}{\unif[{\ab}]}
\newcommand{\unifabs}[1]{\unif[{#1}]}


\newcommand{\smb}{x}
\newcommand{\psmb}{\p_\smb}
\newcommand{\ps}[1]{\p_{#1}}
\newcommand{\Xon}{X^\ns}
\newcommand{\Yon}{Y^\ns}
\newcommand{\Zon}{Z^\ns}
\newcommand{\xon}{x^\ns}
\newcommand{\yon}{y^\ns}
\newcommand{\Xot}{X_1^t}
\newcommand{\Yot}{Y_1^t}
\newcommand{\Xos}{X_1^s}
\newcommand{\Xosp}{X_1^{'s}}
\newcommand{\Yos}{Y_1^s}
\newcommand{\Yosp}{Y_1^{'s}}
\newcommand{\Xosmo}{X_1^{s-1}}
\newcommand{\Yosmo}{Y_1^{s-1}}




\newcommand{\Mestxon}{\Mest\Paren{\Xon}}
\newcommand{\Mest}{{M}}
\newcommand{\Mestgtxon}{\Mest^{\texttt{GT}}\Paren{\Xon}}


\newcommand{\Moxon}{M_0(\Xon)}

\newcommand{\prf}[2]{\Phi_{#1}(#2)}
\newcommand{\prfi}[1]{\Phi_{#1}}

\newcommand{\kp}{k^{'}}

\newcommand{\eps}{\varepsilon}
\newcommand{\he}{\hat{E}}

\newcommand{\mltx}[1]{\mu_{#1}}
\newcommand{\mlty}[1]{\nu_{#1}}

\newcommand{\bias}{b}
\newcommand{\Bern}[1]{B(#1)}

\newcommand{\ham}[2]{d_{\text{Ham}}(#1,#2)}
\newcommand{\alg}{\hat \theta}


\newcommand{\Mltsmb}[2]{M_{#1}(#2)}
\newcommand{\prfsmb}[2]{\Phi_{#1}(#2)}


\newcommand{\dist}{\alpha}

\newcommand{\dtv}[2]{d_{TV}(#1, #2)}
\newcommand{\dkl}[2]{d_{KL}(#1, #2)}


%\ifnum\withcolors=1
%  \newcommand{\new}[1]{{\color{red} {#1}}} % new
%  \newcommand{\newer}[1]{{\color{blue} {#1}}} % even newer
%  \newcommand{\newest}[1]{{\color{orange} {#1}}} % even even newer
%  \newcommand{\newerest}[1]{{\color{blue!10!black!40!green} {#1}}} % you get the idea.
%  \newcommand{\acolor}[1]{{\color{ForestGreen}#1}} % Jayadev
%  \newcommand{\scolor}[1]{{\color{RubineRed}#1}} % Clement
%  \newcommand{\zcolor}[1]{{\color{Orange}#1}} % Himanshu
%  \newcommand{\zscolor}[1]{{\color{Purple}#1}} % Himanshu
%\else
%  \newcommand{\new}[1]{{{#1}}}
%  \newcommand{\newer}[1]{{{#1}}}
%  \newcommand{\newest}[1]{{{#1}}}
%  \newcommand{\newerest}[1]{{{#1}}}
%  \newcommand{\acolor}[1]{{#1}}
%  \newcommand{\scolor}[1]{{#1}}
%  \newcommand{\zcolor}[1]{{#1}}
%\fi
%
%\ifnum\withnotes=1
%  \newcommand{\anote}[1]{\par\acolor{\textbf{J: }\sf #1}} % Jayadev
%  \newcommand{\snote}[1]{\par\scolor{\textbf{ZS: }\sf #1}} % Clement
%  \newcommand{\znote}[1]{\par\zcolor{\textbf{H: }\sf #1}} % Himanshu
%  \newcommand{\afootnote}[1]{\footnote{{\bf \acolor{Jayadev}}: {#1}}}
%  \newcommand{\sfootnote}[1]{\footnote{{\bf \scolor{Cl\'ement}}: {#1}}}
%  \newcommand{\zfootnote}[1]{\footnote{{\bf \zcolor{Himanshu}}: {#1}}}
%
%
%  \newcommand{\todonote}[2][]{\todo[size=\scriptsize,color=red!40,#1]{#2}}  
%	\newcommand{\questionnote}[2][]{\todo[size=\tiny,color=blue!30]{#2}}
%	\newcommand{\todonotedone}[2][]{\todo[size=\scriptsize,color=green!40]{$\checkmark$ #2}}
%	\newcommand{\todonoteinline}[2][]{\todo[inline,size=\scriptsize,color=orange!40,#1]{#2}}  
%  \newcommand{\marginnote}[1]{\todo[color=white,linecolor=black]{{#1}}}
%\else
%  \newcommand{\anote}[1]{}
%  \newcommand{\snote}[1]{}
%  \newcommand{\znote}[1]{}
%  \newcommand{\todonote}[2][]{\ignore{#2}}
%	\newcommand{\questionnote}[2][]{\ignore{#2}}
%	\newcommand{\todonotedone}[2][]{\ignore{#2}}
%	\newcommand{\todonoteinline}[2][]{\ignore{#2}}
%  \newcommand{\marginnote}[1]{\ignore{#1}}
%\fi
%
%\newcommand{\amargin}[1]{\questionnote{\acolor{#1}}} % Jayadev
%\newcommand{\smargin}[1]{\questionnote{\ccolor{#1}}} % Clement
%\newcommand{\zmargin}[1]{\questionnote{\hcolor{#1}}} % Himanshu
%\newcommand{\zsmargin}[1]{\questionnote{\zscolor{#1}}} %Ziteng
%
%\ifnum\withnotes=1
%  \usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}
%\fi



%%%%%%%%%%%%%%%%%%%%%%

==> distribution_estimation/proof_of_theorem.tex <==
\section{Proof of Theorems}
\label{sec:proofs}

\subsection{Proof of Corollary~\ref{coro:fano}} \label{sec:coro_fano_proof}
%{We restate the corollary before proving it.} 
%
\distest*
%\amargin{Dont know how to make the number to Corollary 4.}
\begin{proof}
Recall that $\cQ^{\ns} := \{ \q^\ns | \q \in \cQ \}$ is the set of induced distributions over $\cX^\ns$ and $\q^\ns \in \cQ^\ns, \theta(\q^\ns) = \q$. Then,
	$\forall i \neq j \in [M]$,
$\ell \Paren{\theta(\q_i^n),\theta(\q_j^n)} \ge 3 \tau$, and $D_{KL} \Paren{\q_i^n,\q_j^n} = n D_{KL} \Paren{\q_i,\q_j}  \le n \beta.$

{The following lemma is a corollary of maximal coupling~\cite{Hollander12}, which states that for two distributions there is a coupling of their $n$ fold product distributions with an expected Hamming distance $n$ times their total variation distance.}
	\begin{lemma}
		\label{lem:couplingdistance}
		Given distributions $\q_1,\q_2$ over $\cX$, there exists a coupling $(X,Y)$ between $\q_1^n$ and $\q_2^n$ such that  
		\[\expectation{\ham{X}{Y}} = \ns \cdot d_{TV} \Paren{\q_1,\q_2},
		\]
		where $X \sim \q_1^n$ and $Y \sim \q_2^n.$
	\end{lemma}
\noindent By Lemma~\ref{lem:couplingdistance}, $\forall i,j \in [M]$, there exists a coupling $(X, Y)$ between $\q_i^n$ and $\q_j^n$ such that $\expectation{\ham{X}{Y}} \le n\gamma. $
	Now by Theorem~\ref{thm:dp_fano},
	\begin{align}
	R(\cQ^*, \ell, \eps) \ge \max \Bigg\{\frac{3\tau}{2} \left(1 - \frac{n \beta + \log 2}{\log M}\right), 1.2\tau \min\left\{1, \frac{M}{e^{10\eps n \gamma}}\right\} \Bigg\}.
	\end{align}
Therefore, for $R(\cQ^\ns, \ell, \eps) \le \tau$, 
	\[
	S(\cQ, \ell, \tau, \eps) = \Omega\Paren{\frac{\log M}{\beta}+ \frac{\log M}{\gamma \eps}}.
	\]
\end{proof}

==> distribution_estimation/table.tex <==

\begin{table*}[htb]
\centering
      \begin{tabular}{| c | c | c |}
      \hline
      %&\multicolumn{2}{c|} {\bf Sample Complexity Bounds}  \\ \hline
      {\bf Problem} & {\bf Upper Bounds} & {\bf Lower Bounds} \\ \hline
      {\bf $\ab$-ary} & \multicolumn{2}{c|} {\parbox[c][1.2cm]{10cm}{\centering$ \Theta \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha\eps}}$~(\cite{DiakonikolasHS15}, Theorem~\ref{thm:pure-dv})} }\\\hline
 
       {\bf $\ab$-ary, $\ell_2$ distance} &\parbox[c][1.5cm]{5cm}{\centering $O\Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist\eps},\frac{\log\ab}{\dist^2\eps}  } }$ \\\small{(Theorem~\ref{thm:pure-l2}) }}
       & \parbox[c]{5cm}{\centering $\Omega \Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist\eps},\frac{\log (\ab \dist^2)}{\dist^2\eps}  } }$ \\\small{(Theorem~\ref{thm:pure-l2}) } } \\ \hline
       
       {\bf product distribution} & \parbox[c][1.5cm]{5cm}{\centering $O\Paren{\ab\dims \log \Paren{ \frac{\ab\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$ \\\small{\cite{BunKSW2019} }}
       &\parbox[c]{5cm}{\centering $\Omega \Paren{{\ab\dims}\Paren{\frac1{\alpha^2}+\frac1{\alpha \eps}}}$ \\\small{(Theorem~\ref{thm:main_product}) }}\\\hline
       
              {\bf Gaussian mixtures} & \parbox[c][1.5cm]{5cm}{\centering ${O}\Paren{kd\log(\frac{dR}{\alpha})(\frac1{\alpha^2}+ \frac1{\alpha \eps})}$ \\\small{\cite{BunKSW2019} }}
       &\parbox[c]{5cm}{\centering $\Omega \Paren{{\ab\dims}\Paren{\frac1{\alpha^2}+\frac1{\alpha \eps}}}$ \\\small{(Theorem~\ref{thm:main_Gaussian}) }}\\\hline
       
      \end{tabular}
    \caption{\label{tab:pure} Summary of the sample complexity bounds for $\eps$-DP discrete distribution estimation. Unless mentioned, the bounds are all for estimation under total variation distance.}
\end{table*}

%\begin{table}[htbp]
%\centering
%      \begin{tabular}{| c | c |}
%      \hline
%      {\bf Problem} & {\bf Sample Complexity Bounds}    \\ \hline
%      
%      {\bf $\ab$-ary , $d_{TV}$ distance} & {\bf Non-private algorithms:  $\Theta \Paren{\frac{\ab}{\alpha^2}}$ } \\
%      &{\bf $(\eps,\delta)$-DP algorithms:} \\
%      &$\Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha(\eps+\delta)}}\le S(\Delta_k, d_{TV}, \alpha, \eps, \delta) \le O \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}$~[Theorem~\ref{thm:ApproximateDiscreteTotalVariation}] \\\hline
%        {\bf $\ab$-ary, $\ell_2$ distance} & {\bf Non-private algorithms:  $\Theta \Paren{\frac{1}{\alpha^2}}$ } \\
%       &{\bf $(\eps,\delta)$-DP algorithms:} \\
%              & \multicolumn{1}{|l|}{{\bf IF} $\dist \le \ab^{-\frac1{2}}$,}   \\  
%             & $ \Omega \Paren {\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha (\eps+\delta)}} \le S(\Delta_k, \ell_2, \alpha, \eps, \delta) \le O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha\eps}}$ \\ 
%                    & \multicolumn{1}{|l|}{{\bf ELSE}} \\
%       & $\Omega\Paren{\frac{1}{\dist^2}+\frac{1}{\dist^2(\eps+\delta)}}\le  S(\Delta_k, \ell_2, \alpha, \eps, \delta) \le O\Paren{\frac{1}{\dist^2}+\frac{\log\ab}{\dist^2\eps}}$~[Theorem~\ref{thm:ApproximateDiscreteL2}]\\ \hline
%      \end{tabular}
%    \caption{\label{table2} \newhz{Summary of the sample complexity bounds for $(\eps,\delta)$-DP discrete distribution learning.}}
%\end{table}

\begin{table*}[htb]
\centering
      \begin{tabular}{| c | c | c |}
      \hline
      %&\multicolumn{2}{c|} {\bf Sample Complexity Bounds}  \\ \hline
      {\bf Problem} & {\bf Upper Bounds} & {\bf Lower Bounds} \\ \hline
      {\bf $\ab$-ary} &  \parbox[c][1.5cm]{5cm}{\centering $O\Paren{\frac{\ab}{\dist^2}+\frac{\ab} {\dist\eps}}$ \\\small{(\cite{DiakonikolasHS15}, Theorem~\ref{thm:ApproximateDiscreteTotalVariation})} }
       &\parbox[c]{5cm}{\centering $\Omega \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha (\eps+\delta)}}$ \\\small{(Theorem~\ref{thm:ApproximateDiscreteTotalVariation})} }\\\hline
 
       {\bf $\ab$-ary, $\ell_2$ distance} &\parbox[c][1.5cm]{5cm}{\centering 
       $O 
       \Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist\eps},\frac{\log\ab}{\dist^2\eps}
         } }$ \\\small{(Theorem~\ref{thm:ApproximateDiscreteL2}) }}
       & \parbox[c]{5cm}{\centering $\Omega \Paren{\frac{1}{\dist^2}+\min\Paren{\frac{\sqrt{\ab}}{\dist(\eps+\delta)},\frac{1}{\dist^2(\eps+\delta)}  } }$ \\\small{(Theorem~\ref{thm:ApproximateDiscreteL2}) } } \\ \hline
       
              {\makecell { \bf product distribution \\ ($k = 2$)}} & \parbox[c][1.5cm]{5cm}{\centering $O\Paren{\dims \log \Paren{ \frac{\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$ \\\small{\cite{KamathLSU18, BunKSW2019}}}
       &\parbox[c]{5cm}{\centering $\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha (\eps + \delta)}}$ \\\small{(Theorem~\ref{thm:ApproximateProductTotalVariation},~\cite{KamathLSU18}) }}\\ \hline
      \end{tabular}
    \caption{\label{tab:approx} Summary of the sample complexity bounds for $(\eps,\delta)$-DP discrete distribution estimation. Unless mentioned, the bounds are all for estimation under total variation distance.}
\end{table*}
%
%\begin{table}[t]
%\center
%\begin{tabular}{c c c c c}
%&& Deterministic  & Sample & Stochastic  \\
%&& First-Order Oracle & Complexity & First-Order Oracle \\\hline
%\parbox[t]{1cm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\small{$\norm{x_0-x^*}\leq R$}}}}
%& \small{Upper:}
%& \parbox[t]{4cm}{\centering $\tilde{O}\prn*{\sqrt{\frac{HR}{\epsilon}}}$\\\small{\cite{nesterov2012make}}}
%& \parbox[t]{3cm}{\centering $O\prn*{\frac{\sigma^2}{\epsilon^2}\log^{3}\parens{\frac{HR}{\epsilon}}}$\\\small{(\pref{cor:sample-complexity-bounded})}}
%& \parbox[t]{3cm}{\centering $\tilde{O}\prn*{\sqrt{\frac{HR}{\epsilon}} + \frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{cor:sgd3-bounded-domain})}}
%\rule[-20pt]{0pt}{37pt}\\ ~\\
%& \small{Lower:}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\sqrt{\frac{HR}{\epsilon}}}$\\\small{\cite{carmon2017lower2}}}
%& \parbox[t]{3cm}{\centering $\Omega\prn*{\frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{thm:statistical-lower-bound})}}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\sqrt{\frac{HR}{\epsilon}} + \frac{\sigma^2}{\epsilon^2}\log\parens{\frac{HR}{\epsilon}}}$\\\small{(\pref{thm:first-order-lower-bound})}}
%\rule[-24pt]{0pt}{28pt}\\ \hline
%\parbox[t]{1cm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\parbox[t]{2.345cm}{\centering \scriptsize{$F(x_0)-F(x^*)\leq \Delta$}}}}}
%& \small{Upper:}
%& \parbox[t]{4cm}{\centering $\tilde{O}\prn*{\frac{\sqrt{H\Delta}}{\epsilon}}$\\\small{\cite{carmon2017lower2}}}
%& \parbox[t]{3cm}{\centering $O\prn*{\frac{\sigma^2}{\epsilon^2}\log^{3}\parens{\frac{H\Delta}{\epsilon^2}}}$\\\small{(\pref{cor:sample-complexity-bounded})}}
%& \parbox[t]{3cm}{\centering $\tilde{O}\prn*{\frac{\sqrt{H\Delta}}{\epsilon} + \frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{cor:sgd3-bounded-domain})}}
%\rule[-24pt]{0pt}{41pt}\\~\\
%& \small{Lower:}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\frac{\sqrt{H\Delta}}{\epsilon}}$\\\small{\cite{carmon2017lower2}}}
%& \parbox[t]{3cm}{\centering $\Omega\prn*{\frac{\sigma^2}{\epsilon^2}}$\\\small{(\pref{thm:statistical-lower-bound})}}
%& \parbox[t]{4cm}{\centering $\Omega\prn*{\frac{\sqrt{H\Delta}}{\epsilon} + \frac{\sigma^2}{\epsilon^2}\log\parens{\frac{H\Delta}{\epsilon^2}}}$\\\small{(\pref{thm:first-order-lower-bound})}}
%\rule[-24pt]{0pt}{26pt}\\\hline
%\end{tabular}
%\caption{Upper and lower bounds on the complexity of finding $x$
%  such that $\norm{\nabla F(x)}\leq\epsilon$ for convex problems with
%  $H$-Lipschitz gradients, where $\sigma^2$ is a bound on the variance
%  of gradient estimates.}
%  \label{tab:results}
%\end{table}


==> distribution_estimation/uniformity-lower_new.tex <==
\subsection{Sample Complexity Lower bounds for Uniformity Testing}\label{sec:lower-identity}

The first term is the lower bound without privacy constraints, proved in~\cite{Paninski08}. In this section, we prove the terms associated with privacy. 

The simplest argument is for $\ns \ge \frac{\ab}{\alpha^2}$, which hopefully will give the readers a sense of how coupling argument works. We consider the case of binary uniformity testing where the goal is to test whether the bias of a coin is $1/2$ or $\alpha$-far from $1/2$. This is a special case of uniformity testing for distributions over $[\ab]$ (when $\ab-2$ symbols have probability zero). This is strictly harder than the problem of distinguishing between $\Bern{1/2}$ and $\Bern{1/2+\alpha}$. The coupling given in Example~\ref{exm:coin} has expected hamming distance of $\alpha \ns$. Hence combing with Theorem~\ref{thm:le_cam}, by letting the RHS no larger than $\frac13$, we get a lower bound of $ \ns = \Omega\Paren{\min\Paren{\frac1{\dist\eps}, \frac1{\dist\delta} }} = \Omega({\frac{1}{\dist (\eps+\delta)}})$.

We now consider the cases $\ns \le \ab$ and $\ab< \ns \le \frac{\ab}{\alpha^2}$.

%The final term is a lower bound for testing identity to $\Bern{0.5}$, which is easier than uniformity testing by Theorem~\ref{thm:unif-identity}. 

To this end, we invoke our private LeCam's method, and design a hypothesis testing problem that will imply a lower bound on uniformity testing. The testing problem will be to distinguish between the following two cases. 

{\bf Case 1:} We are given $\ns$ independent samples from the uniform distribution $\unifab$.

{\bf Case 2:} Generate a distribution $\p$ with $\dtv{\p}{\unifab}\ge\dist$ according to some prior over all such distributions. We are then given $\ns$ independent samples from this distribution $\p$. 

From Theorem~\ref{thm:le_cam}, any lower bound for distinguishing between these two cases is a lower bound on uniformity testing problem. 

We now describe the prior construction for {\bf Case 2}, which is the same as considered by~\cite{Paninski08} for lower bounds on identity testing without privacy considerations. For each $\textbf{z} \in\{\pm1\}^{\ab/2}$, define a distribution $\p_{\textbf{z}}$ over $[\ab]$ such that 
\begin{align}
\p_{\textbf{z}}(2i-1) = \frac{1+\textbf{z}_i\cdot 2\dist}{\ab}, \text{ and } \p_{\textbf{z}}(2i) = \frac{1-\textbf{z}_i\cdot 2\dist}{\ab}.\nonumber
\end{align}
Then for any $\textbf{z}$, $\dtv{P_{\textbf{z}}}{\unifab}= \alpha$. For {\bf Case 2}, choose  $\p$ uniformly from these $2^{\ab/2}$ distributions. Let $Q_2$ denote the distribution on $[\ab]^\ns$ by this process. In other words, $Q_2$ is a mixture of product distributions over $[\ab]$. 

In {\bf Case 1}, let $Q_1$ be the distribution of $\ns$ $i.i.d.$ samples from $\unifab$. 

To obtain a sample complexity lower bound for distinguishing the two cases, we will design a coupling between $Q_1$, and $Q_2$, and bound its expected Hamming distance. While it can be shown that the Hamming distance of the coupling between the uniform distribution with any \emph{one} of the $2^{\ab/2}$ distributions grows as $\alpha\ns$, it can be significantly smaller, when we consider the mixtures. In particular, the following lemma shows that there exist couplings with bounded Hamming distance. 

\begin{lemma}\label{lem:coupling-hamming}
	There is a coupling between $\Xon$ generated by $Q_1$, and $\Yon$ by $Q_2$ such that 
\begin{center}
   $\expectation{\ham{\Xon}{\Yon}} \le C \cdot \dist^2 \min \{ \frac{\ns^2}{\ab}, \frac{\ns^{3/2}}{{\ab}^{1/2}} \}$.
%    \begin{cases}
%                                   8\frac{\ns^2\dist^2}{\ab}, & \text{when $m \le k$} \\
%                                    C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}}, & \text{when $k< m \le \frac{k}{\alpha^2}$}.
%    \end{cases}
\end{center}
\end{lemma}
We refer the proof of the lemma to~\cite{AcharyaSZ18}. Now applying Theorem~\ref{thm:le_cam}, we get the bound in Theorem~\ref{thm:main-identity}.
%\begin{enumerate}
%	\item \newhz{For $m \le k$, $8\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/2}}{\alpha \eps^{1/2}}}$.}
%	\item \newhz{For $k< m \le \frac{k}{\alpha^2}$, $C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}} = \Omega \Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/3}}{\alpha^{4/3}\eps^{2/3}}}$.}
%\end{enumerate}

%\begin{lemma}
%There is a coupling between $\Xon$  generated by $Q_2$, and $\Yon$ by $Q_1$ such that for 
%\[
%\expectation{\ham{\Xon}{\Yon}} \le
%\begin{cases}
%O\Paren{\dist^2\cdot\frac{\ns^2}{\ab}} & \ns\le \ab,\\
%O\Paren{\dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}}& k\le \ns\le \ab/\alpha^2,\\
%%O\Paren{\alpha\ns}&  \ab/\alpha^2\le\ns.
%\end{cases}
%\]
%\label{lem:coupling-uniform}
%\end{lemma}

%We can rewrite this result as
%\begin{align}
%\expectation{\ham{\Xon}{\Yon}} \le
%O\Paren{\min\left\{\dist^2\cdot\frac{\ns^2}{\ab}, \dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}, \alpha\ns\right\}}\label{eq:coup-ub}
%\end{align}
%	For the proof of this lemma, we can refer to lemma
%
%
%
%Using lemma~\ref{lem:coupling-uniform}, we can apply the coupling lower bound to prove the lower bound. 
%\begin{theorem}
%\[
%\Sitd\ge \Omega\Paren{\max\left\{\frac{\ab^{1/2}}{\alpha(\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3}(\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.
%\]
%\end{theorem}


%This is proved in the following lemma. 


%The construction of $Q_2$, and the proof of Lemma~\ref{lem:coup_unif} is slightly technical and is given in Section~\ref{app:lb-unif}.
%Assuming this lemma, by Theorem~\ref{thm:coupling}, we need $\expectation{\ham{\Xon}{\Yon}}=\Omega\Paren{\frac1{\eps+\delta}}$ to distinguish between $Q_1$, and $Q_2$. For this to hold, we need $\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps+\delta}}$, which gives us 
%$\ns\ge \Omega\Paren{\frac{\sqrt \ab}{\dist\sqrt{\eps+\delta}}}$.




==> distribution_estimation/uniformity.tex <==
\section{$(\eps,\delta)$-DP uniformity testing}
\label{sec:identity}

\newhzn{
In this section, we give a proof sketch of sample complexity lower bound of uniformity testing. The full detail can be referred to~\cite{AcharyaSZ18}. The main result is the following. }

\begin{theorem}
\label{thm:main-identity}
The sample complexity of $(\eps,\delta)$-DP identity testing is
$$\Sutd = \Theta\Paren{\frac{k^{1/2}}{\dist^2}+\max\left\{\frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.$$
%
%Or we can write it according to the parameter range,
%\[
%    \Sit =
%    \begin{cases}
%                                   \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}}, & \text{when $k = \Omega \Paren{\frac1{\alpha^4}}$ and $k = \Omega \Paren{\frac1{\alpha^2 (\eps+\delta)}}$,} \\
%              		  \Theta\Paren{\frac{\sqrt k}{\alpha^2} +\frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}}, & \text{when $k = \Omega \Paren{\frac{\alpha}{(\eps+\delta)}}$ and $k = O \Paren{\frac1{\alpha^4}+\frac1{\alpha^2 (\eps+\delta)} }$,}\\
%              		               \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac1{\alpha (\eps+\delta)}}, & \text{when  $k = O \Paren{\frac{\alpha}{(\eps+\delta)}}$.}\\ 
%    \end{cases}
%\]
\end{theorem}
We note that the lower bound is tight up to constant factors in all parameters. 

%In~\cite{AcharyaSZ18}, they show a reduction from identity to uniformity testing under differential privacy and design algorithms which achieve the matching upper bounds.
% 
%In this work, we focus on the lower bounds for identity testing. Since uniformity testing is a special case of identity testing, any lower bound for uniformity will port over to identity, and we give such bounds in Section~\ref{sec:lower-identity}.







==> inspec/abs.tex <==
We develop differentially private methods for estimating various distributional properties.
Given a sample from a discrete distribution $p$, some functional $f$, and accuracy and privacy parameters $\dist$ and $\eps$, the goal is to estimate $f(p)$ up to accuracy $\dist$, while maintaining $\eps$-differential privacy of the sample.
We prove almost-tight bounds on the sample size required for this problem for several functionals of interest, including support size, support coverage, and entropy.
We show that the cost of privacy is negligible in a variety of settings, both theoretically and experimentally.
Our methods are based on a sensitivity analysis of several state-of-the-art methods for estimating these properties with sublinear sample complexities.


==> inspec/empirical.tex <==
\subsubsection{Upper Bound for Entropy Estimation: The Empirical Estimator}
\label{sec:entropy-ub-empirical}


Let $\emp$ be the empirical distribution, and let $\entemp$ be the entropy of the empirical distribution.

\begin{theorem}\label{thm:empirical}
\[
C(H, \dist, \eps) = O\Paren{\frac{\ab}{\dist}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}+\frac{1}{\dist\eps}\log\Paren{\frac1{\dist\eps}}}.
\]
\end{theorem}

\begin{proof}
We present the entire argument for completeness. We will show that the theorem is implied by the following three results. 
\begin{align}
&\absv{\entp{\p}-\expectation{\entemp}} =O\Paren{\frac{\ab}{\ns}},\label{eq:bias-emp}\\
&\variance{\entemp} =O\Paren{\frac{\log^2(\min\{\ab,\ns\})}{\ns}},\label{eq:variance-emp}\\
&\Delta(\entemp) = O\Paren{\frac{\log\ns}{\ns}}.\label{eqn:sensitivity-emp}
\end{align}
Using these three equations, we are done.
\end{proof}

\paragraph{Proof of~\eqref{eq:bias-emp}.} By the concavity of entropy function, we know that 
\[
\expectation{\entp{\emp}} \le \entp{\p}.
\]
Therefore, 
\begin{align}
\expectation{\absv{\entp{\p}-\entp{\emp}}} &=  \entp{\p}-\expectation{{\entp{\emp}}}\nonumber\\
&=  \expectation{\sum_{\smb}\Paren{\pemps\log \pemps-\ps\log\ps}} \nonumber\\
&=  \expectation{\sum_{\smb}\pemps\log \frac{\pemps}{\ps}}+\expectation{\sum_{\smb}(\pemps-\ps)\log\ps}\nonumber\\
&=  \expectation{\kldist{\emp}{\p}}\label{eqn:kl-exp}\\
&\leq \expectation{\chisquare{\emp}{\p}}\label{eqn:kl-chisq}\\
&=  \expectation{\sum_{\smb}\frac{(\pemps-\ps)^2}{\ps}}\nonumber\\
&\le  {\sum_{\smb}\frac{(\ps/\ns)}{\ps}}\label{eqn:var-bin}\\
&= \frac\ab\ns.
\end{align}

\paragraph{Proof of~\eqref{eqn:sensitivity-emp}.}
The largest change in any $\nsmb$ when we change one symbol is one. Moreover, at most two $\nsmb$ changes. Therefore, 
\begin{align}
\Delta(\entemp) &\leq  2\cdot \max_{j=1\ldots \ns-1} \absv{ \frac{j+1}{n}\log\frac{n}{j+1}-\frac{j}{n}\log\frac{n}{j}}\nonumber\\
&=  2\cdot \max_{j=1\ldots \ns-1}\absv{\frac{j}{\ns}\log \frac{j}{j+1}+\frac1{\ns}\log \frac{\ns}{j+1}}\label{eqn:sum-one}\\
&\leq  2 \cdot \max_{j=1\ldots \ns-1}\max\left\{\absv{\frac{j}{\ns}\log \frac{j}{j+1}}, \absv{ \frac1{\ns}\log \frac{\ns}{j+1}}\right\}\label{eqn:sum-two}\\
&\leq  2\cdot \max\left\{\frac 1\ns, \frac{\log \ns}{\ns}\right\},\nonumber\\
& = 2\cdot \frac{\log \ns}{\ns}.
\end{align}

\paragraph{Proof of~\eqref{eq:variance-emp}.}The variance bound of $\frac{\log k}{n}$ is given precisely in~\cite[Lemma 15]{JiaoVHW17}.
To obtain the other half of the bound of, we apply the bounded differences inequality.

\begin{lemma}[BLM-Cor 3.2]
	\label{lem:bdd-diff-var}
	Let $f:\Omega^{\ns}\to\RR$ be a function. Suppose further that 
	\[
	\max_{z_1,\ldots, z_n, z_{i}^{'}} \absv{f(z_1,\ldots,z_n) - f(z_1,\ldots, z_{i-1}, z_i^{'},\ldots,z_n)}\le c_i.
	\]
	Then for independent variables $Z_1,\ldots,Z_{\ns}$, 
	\[
	\Var\Paren{f(Z_1,\ldots,Z_{\ns})} \le \frac14\sum_{i=1}^{\ns} c_i^2.
	\]
\end{lemma}

Therefore, using Lemma~\ref{lem:bdd-diff-var} and Equation~\eqref{eqn:sensitivity-emp}
\[
\variance{\entemp}\le \ns\cdot\Paren{\frac{4\log^2\ns}{\ns^2}} = \frac{4\log^2\ns}{\ns}.
\]

%\begin{theorem}\label{lb:all}
%Any entropy estimator must take 
%\[
%\Omega\Paren{\frac{\ab}{\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}+\frac{\log\ab}{\dist\eps}}
%\]
%samples to estimate $\entp{\p}$ up to $\pm\eps$. Therefore, 
%\[
%\variance{\entemp}\le \ns\cdot\Paren{\frac{4\log^2\ns}{\ns^2}} = \frac{4\log^2\ns}{\ns}.
%\]
%\end{theorem}
%
%As a corollary, note that when $\eps$, and $\dist$ are at most inverse polynomial in $\ab$, then the dependence of the sample complexity is optimal in terms of the privacy parameter. 


==> inspec/lb.tex <==
\subsubsection{Lower Bound for Entropy Estimation}

\begin{theorem}\label{lb:all}
\[
C(H, \dist, \eps) =\Omega\Paren{\frac{\ab}{\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}+\frac{\log\ab}{\dist\eps}}.
\]
\end{theorem}
\begin{proof}
The first two terms in the lower bound follows from the entropy estimation lower bounds, even without privacy requirements. For the final term, we will invoke the lower bound arguments from~\cite{AcharyaSZ18}.\todo{Do we need to state the lemma here?} Consider the two distributions below (which are also used in~\cite{WuY16}). The first distribution assigns probability $2/3$ to the first element, and is uniform over the remaining $\ab-1$ elements, and the second distribution assigns probability $(2-\eta)/3$ to the first element, and is uniform over the rest. Then, the entropy of the two distributions differ by $\Theta(\eta\log\ab)$. Therefore, when $\eta = \dist/\log\ab$, the entropy of the two distributions differ by $\Theta(\dist)$. There is a coupling between the two distributions with expected Hamming distance $\expectation{D} = {\eta\ns}/3$. Therefore, 
\[
\eta\ns\ge\frac1\eps \Rightarrow \ns\ge\frac1{\eta\eps}.
\]
Substituting, $\eta = \dist/\log\ab$, gives
\[
\ns\ge \frac{\log\ab}{\dist\eps}.
\]
\end{proof}




==> inspec/polynomial.tex <==
\subsubsection{Upper Bound for Entropy Estimation: Best-Polynomial Approximation}
The upper bound should be straightforward from the sensitivity bound in Lemma 2 of~\cite{AcharyaDOS17}.


The optimal sample complexity of estimating $\entp{\p}$ to $\pm \dist$ is~\cite{WuY16}
\[
O\Paren{\frac{\ab}{\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2}}.
\]
However, \todo{which two papers?}both these papers propose estimators that can have a high sensitivity.~\cite{AcharyaDOS17} propose technical modifications to these approaches to obtain an estimator that has the following properties. We denote their estimator with $H^\beta$, where $\beta>0$ is a fixed constant (say 0.01 or something).  Then the estimator satisfies the followings:
\begin{itemize}
\item
The sample complexity of the estimator is at most a factor $1/\beta^2$ of the optimal, which is sample order-optimal for any constant $\beta$. 
\item
The sensitivity of $H^{\beta}$ is at most $O(\ns^{\beta}/\ns)$. 
\end{itemize}

This shows the following bound on the sample complexity of estimating $\entp{\p}$ under $\eps$-differential privacy. 
\begin{theorem}
Let $\beta>0$ be a small fixed constant. Then,  
\[
C(H, \dist, \eps) = O\Paren{\frac{\ab}{\beta^2\dist\log\ab}+\frac{\log^2(\min\{\ab,\ns\})}{\dist^2} + \Paren{\frac1{\dist\eps}}^{1+\beta}}.
\]
which can estimate $\entp{\p}$ up to $\pm \dist$ with success probability of 2/3.
\end{theorem}





==> inspec/preamble.tex <==


%%% USED FOR COMMENTS

\def\a{\alpha}
\def\b{\beta}
%\def\c{\chi}
\def\d{\delta}
\def\D{\Delta}
%\def\e{\epsilon}
\def\e{\eta}
\def\eps{\varepsilon}
\renewcommand{\epsilon}{\ve}
\def\ve{\varepsilon}
\def\f{\phi}
\def\F{\Phi}
\def\g{\gamma}
\def\G{\Gamma}
\def\k{\kappa}
\def\K{\Kappa}
\def\z{\zeta}
\def\th{\theta}
\def\Th{\Theta}
\def\l{\lambda}
\def\la{\lambda}
%\def\L{\Lambda}
\def\m{\mu}
\def\n{\nu}
%\def\p{\pi}
\def\P{\Pi}
\def\r{\rho}
\def\R{\Rho}
\def\s{\sigma}
\def\S{\Sigma}
\def\t{\tau}
\def\om{\omega}
\def\Om{\Omega}
\def\smallo{{\rm o}}
\def\bigo{{\rm O}}
\def\to{\rightarrow}
\def\ex{{\bf Exp}}
\def\cd{{\cal D}}
\def\rme{{\rm e}}
\def\hf{{1\over2}}
\def\R{{\bf  R}} 
\def\cala{{\cal A}}
\def\calt{{\cal T}}
\def\cale{{\cal E}}
\def\Fscr{{\cal F}}
\def\cc{{\cal C}}
\def\calc{{\cal C}}
\def\call{{\cal L}}
\def\calm{{\cal M}}
\def\calh{{\cal H}}
\def\cali{{\cal I}}
\def\bk{\backslash}


\newcommand{\Exp}{\mbox{\bf Exp}}
\newcommand{\E}{\mbox{\bf E}}
%\newcommand{\Var}{\mbox{\bf Var}}
\newcommand{\sign}{\mbox{\bf sign}}

\newcommand{\erf}{\mbox{\text erf}}
\newcommand{\erfc}{\mbox{\text erfc}}

%\newcommand{\pr}[2][]{\mbox{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[#2\right]}
\newcommand{\given}{\ \mid\ }
%\newcommand{\reals}{\mathbb{R}}

\newcommand{\U}{\mathcal{U}_n}


\newcommand{\limninf}{\lim_{n \rightarrow \infty}}
\newcommand{\proofstart}{{\bf Proof\hspace{2em}}}
\newcommand{\tset}{\mbox{$\cal T$}}
\newcommand{\proofend}{\hspace*{\fill}\mbox{$\Box$}}
\newcommand{\bfm}[1]{\mbox{\boldmath $#1$}}
%\newcommand{\reals}{\mbox{\bfm{R}}}
%\newcommand{\expect}{\mbox{\bf Exp}}
\newcommand{\he}{\hat{\e}}
\newcommand{\card}[1]{\mbox{$|#1|$}}
\newcommand{\rup}[1]{\mbox{$\lceil{ #1}\rceil$}}
\newcommand{\rdn}[1]{\mbox{$\lfloor{ #1}\rfloor$}}
\newcommand{\ov}[1]{\mbox{$\overline{ #1}$}}
\newcommand{\inv}[1]{$\frac{1}{ #1}$}
\newcommand{\dtv}{d_{\mathrm {TV}}}
\newcommand{\dk}{d_{\mathrm K}}
\newcommand{\dkl}{d_{\mathrm {KL}}}
\newcommand{\dskl}{d_{\mathrm {SKL}}}
\newcommand{\Tr}{{\mathrm {Tr}}}

\newtheorem{theorem}{Theorem}
\newtheorem{nontheorem}{Non Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{observation}{Observation}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}
\newtheorem{case}{Case}
\newtheorem{dfn}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{question}{Question}
\newtheorem{openquestion}{Open Question}
\newtheorem{res}{Result}
%\newcommand{\ignore}[1]{}
\providecommand{\poly}{\operatorname*{poly}}

\newenvironment{proofsketch}{\noindent {\em {Proof (sketch):}}}{$\blacksquare$\vskip \belowdisplayskip}
\newenvironment{prevproof}[2]{\noindent {\em {Proof of {#1}~\ref{#2}:}}}{$\hfill\qed$\vskip \belowdisplayskip}

%\newenvironment{prevproof}[2]{\noindent {\em {Proof of
%{#1}~\ref{#2}:}}}{$\blacksquare$\vskip \belowdisplayskip}

% Allow argmax operation
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\img}{img}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\avg}{avg}

%\def\qedsymbol{\blksquare}
\newcommand{\bg}[1]{\medskip\noindent{\bf #1}}
%\newcommand{\ed}{{\hfill\qedsymbol}\medskip}
%\newenvironment{proofof}[1]{\bg{Proof of #1 : }}{\qed}



%%%
%%% Packed enumerate / itemize
%%%

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\definecolor{Red}{rgb}{1,0,0}
\def\red{\color{Red}}
\newcommand{\costasnote}[1]{{\red #1}}
\newcommand{\oldbound}[1]{{}}


\newcommand{\sparse}{\mathrm{sparse}}
\newcommand{\lrg}{\mathrm{large}}

\newcommand{\goodgamma}{\chi_{\tau_1, \tau_2}}


==> phs/preamble.tex <==
\def\eps{\ve}
\renewcommand{\epsilon}{\ve}
\def\ve{\varepsilon}

\newcommand{\Exp}{\mbox{\bf Exp}}
\newcommand{\E}{\mbox{\bf E}}
\newcommand{\Var}{\mbox{\bf Var}}
\newcommand{\sign}{\mbox{\bf sign}}
\newcommand{\erf}{\mbox{\text erf}}
\newcommand{\erfc}{\mbox{\text erfc}}
\newcommand{\pr}[2][]{\mathrm{Pr}\ifthenelse{\not\equal{}{#1}}{_{#1}}{}\!\left[#2\right]}
\newcommand{\R}{\mathbb{R}}
\newcommand{\U}{\mathcal{U}_n}
\newcommand{\dtv}{d_{\mathrm {TV}}}
\newcommand{\dk}{d_{\mathrm K}}
\newcommand{\dkl}{d_{\mathrm {KL}}}
\newcommand{\dskl}{d_{\mathrm {SKL}}}
\newcommand{\tr}{{\mathrm {tr}}}
\DeclareMathOperator{\argmax}{argmax}
\providecommand{\poly}{\operatorname*{poly}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\id}{\mathbb{I}}

\def \Paren#1{{\left({#1}\right)}}


\newtheorem{theorem}{Theorem}
\newtheorem{nontheorem}[theorem]{Non Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{case}[theorem]{Case}
\newtheorem{dfn}[theorem]{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{res}[theorem]{Result}
\numberwithin{theorem}{section} 
\numberwithin{nontheorem}{section} 
\numberwithin{proposition}{section} 
\numberwithin{observation}{section} 
\numberwithin{remark}{section} 
\numberwithin{fact}{section} 
\numberwithin{lemma}{section} 
\numberwithin{claim}{section} 
\numberwithin{corollary}{section} 
\numberwithin{case}{section} 
\numberwithin{dfn}{section} 
\numberwithin{definition}{section} 
\numberwithin{question}{section} 
\numberwithin{openquestion}{section} 
\numberwithin{res}{section} 


\newenvironment{proofsketch}{\noindent {\em {Proof (sketch):}}}{$\blacksquare$\vskip \belowdisplayskip}
\newenvironment{prevproof}[2]{\noindent {\em {Proof of {#1}~\ref{#2}:}}}{$\hfill\qed$\vskip \belowdisplayskip}

\ifnum\withcolors=1
  \newcommand{\new}[1]{{\color{red} {#1}}} % new
  \newcommand{\newer}[1]{{\color{blue} {#1}}} % even newer
  \newcommand{\newest}[1]{{\color{orange} {#1}}} % even even newer
  \newcommand{\newerest}[1]{{\color{blue!10!black!40!green} {#1}}} % you get the idea.
  \newcommand{\gcolor}[1]{{\color{red}#1}} 
  
  \newcommand{\hcolor}[1]{{\color{blue}#1}} %Huanyu
\else
  \newcommand{\new}[1]{{{#1}}}
  \newcommand{\newer}[1]{{{#1}}}
  \newcommand{\newest}[1]{{{#1}}}
  \newcommand{\newerest}[1]{{{#1}}}
  \newcommand{\gcolor}[1]{{#1}}
  
  \newcommand{\hcolor}[1]{{#1}} %Huanyu
\fi

\ifnum\withnotes=1
  \newcommand{\gnote}[1]{\par\gcolor{\textbf{G: }\sf #1}} % Gautam
  \newcommand{\gfootnote}[1]{\footnote{{\bf \gcolor{Gautam}}: {#1}}}
  
  \newcommand{\hnote}[1]{ \hcolor{\textbf{H: }\sf #1}} %Huanyu
  \newcommand{\snote}[1]{ \hcolor{\textbf{SW: }\sf #1}} %Huanyu
  \newcommand{\todonote}[2][]{\todo[size=\scriptsize,color=red!40,#1]{#2}}  
	\newcommand{\questionnote}[2][]{\todo[size=\tiny,color=blue!30]{#2}}
	\newcommand{\todonotedone}[2][]{\todo[size=\scriptsize,color=green!40]{$\checkmark$ #2}}
	\newcommand{\todonoteinline}[2][]{\todo[inline,size=\scriptsize,color=orange!40,#1]{#2}}  
  \newcommand{\marginnote}[1]{\todo[color=white,linecolor=black]{{#1}}}
\else
  \newcommand{\gnote}[1]{}
  \newcommand{\hnote}[1]{}
    \newcommand{\snote}[1]{}

  \newcommand{\gfootnote}[1]{}
  \newcommand{\todonote}[2][]{\ignore{#2}}
	\newcommand{\questionnote}[2][]{\ignore{#2}}
	\newcommand{\todonotedone}[2][]{\ignore{#2}}
	\newcommand{\todonoteinline}[2][]{\ignore{#2}}
  \newcommand{\marginnote}[1]{\ignore{#1}}
\fi
\newcommand{\ignore}[1]{\leavevmode\unskip} % eat unnecessary spaces before
\newcommand{\gmargin}[1]{\questionnote{\gcolor{#1}}} 

\newcommand{\ellone}[1]{||#1||_{\ell_1}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\Dinfty}{D_\infty}
\newcommand{\Lap}{\mathrm{Lap}}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\DKL}{D_{\mathrm{KL}}}


==> testing/Identity_Sample_Complexity.tex <==
\section{Sample Complexity Bound of Algorithm~\ref{algorithm_uniformity}} \label{sec:sample_complexity_unifrom}
In this section, we prove the sample complexity bound of Algorithm~\ref{algorithm_uniformity} where we privatize the statistic proposed in~\cite{diakonikolas2017sample} to achieve the sample complexity in Theorem~\ref{thm:main-identity} for all parameter ranges.

Because of the normalization in Equation~\ref{eqn:statistic} and lemma~\ref{lem:diako}, for $\Xon$ drawn from $\unifab$
\begin{equation}\label{eqn:statistic-expectation-uniform}
\expectation{Z (\Xon)} \le
\begin{cases}
- \frac1{2} c \alpha^2 \cdot  \frac{m^2}{k}, & \text{when $m \le k$,} \\
- \frac1{2} c \alpha^2 \cdot  { \frac{m^{3/2}}{k^{1/2}} }, & \text{when $k< m \le \frac{k}{\alpha^2}$,} \\
-\frac1{2} cm \alpha, & \text{when  $m \ge \frac{k}{\alpha^2}$ . } 
\end{cases}
\end{equation}

For $\Xon$ drawn from $\p$ with $\dtv{\p}{\unifab}\ge\alpha$, 
\begin{equation}\label{eqn:statistic-expectation-far}
\expectation{Z (\Xon)} \ge
\begin{cases}
\frac1{2} c \alpha^2 \cdot  \frac{m^2}{k}, & \text{when $m \le k$,} \\
\frac1{2} c \alpha^2 \cdot  { \frac{m^{3/2}}{k^{1/2}} }, & \text{when $k< m \le \frac{k}{\alpha^2}$,} \\
\frac1{2} c m\alpha, & \text{when  $m \ge \frac{k}{\alpha^2}$ . } 
\end{cases}
\end{equation}

In order to prove the utility bounds, we also need the following (weak) version of the result of~\cite{diakonikolas2017sample}, which is sufficient to prove the sample complexity bound for constant error probability.
\begin{lemma}
	\label{lem:identityerror}
	There is a constant $C>0$, such that when $\ns>C\sqrt{\ab}/\dist^2$, then for $\Xon\sim \p$, where either $\p=\unifab$, or $\dtv{\p}{\unifab}\ge\alpha$, 
	\[
	\probof{\absv{{Z(\Xon)-\expectation{Z(\Xon)}}}> \frac{2\expectation{Z(\Xon)}}{3} }<0.01.
	\]
\end{lemma}
\noindent The proof of this result is in Appendix~\ref{app:iden-lemma}.

We now proceed to prove the sample complexity bounds. Assume that $\ns>C\sqrt{\ab}/\alpha^2$, so Lemma~\ref{lem:identityerror} holds. Suppose $\eps$ be any real number such that $\eps|\expectation{Z(\Xon)}|>3\log {100}$. Let $\cA(\Xon)$ be the output of Algorithm~\ref{algorithm_uniformity}. Denote the output by 1 when $\cA(\Xon)$ is ``$\p\ne\unifab$'', and 0 otherwise. Consider the case when $\Xon\sim \p$, and $\dtv{\p}{\unifab}\ge\alpha$. Then, 
\begin{align*}
\probof{\cA(\Xon) = 1} &\ge  \probof{\cA(\Xon) = 1 \text{ and } Z(\Xon)>\frac{\expectation{Z(\Xon)}}3}\\
& =\probof{Z(\Xon)>\frac{\expectation{Z(\Xon)}}3}\cdot \probof{\cA(\Xon) = 1|Z(\Xon)>\frac{\expectation{Z(\Xon)}}3}\\
& \ge 0.99\cdot \probof{B\Paren{\sigma(\eps\cdot \frac{\expectation{Z(\Xon)}}3)}=1}\\
&\ge 0.99 \cdot 0.99 \ge 0.9,
\end{align*}
where the last step uses that $\eps \expectation{Z(\Xon)}/3>\log {100}$, along with Lemma~\ref{lem:sig-cont}. The case of $\p=\unifab$ follows from the same argument. 

Therefore, the algorithm is correct with probability at least $0.9$, whenever, $\ns>C\sqrt{\ab}/\dist^2$, and $\eps|\expectation{Z(\Xon)}|>3\log {100}$. By ~\eqref{eqn:statistic-expectation-far}, note that $\eps|\expectation{Z(\Xon)}|>3\log {100}$ is satisfied when, 
\begin{align*}
c \alpha^2 \cdot  {m^2}/{k}\ge&(6\log {100})/\eps ,\ \text{ for $m \le k$}, &\\
c \alpha^2 \cdot  { {m^{3/2}}/{k^{1/2}} }\ge&(6\log {100})/\eps,  \ \text{ for $k< m \le {k}/{\alpha^2}$}, &\\
c \alpha\cdot \ns\ge& (6\log {100})/\eps,\ \text{ for  $m \ge {k}/{\alpha^2}$}.&
\end{align*}
This gives the upper bounds for all the three regimes of $\ns$. 


%We first consider the case when $k< m \le \frac{k}{\alpha^2}$. When $p=\unifab$, we get $\expectation{Z(\Xon)} = - \frac1{2} c m \alpha^2 \cdot \sqrt { \frac{m}{k} }$, then according to Lemma~\ref{lem:identityerror}, when $\ns>C\sqrt{\ab}/\dist^2$,
% \begin{align}
%\probof{Z(\Xon)> -   \frac1{6} c m \dist^2 \cdot \sqrt{\frac{m}{k}}}  = 
% \probof{Z(\Xon) > \frac1{3} \expectation{Z(\Xon) }} \le 0.01
%\end{align}
%
%Furthermore, if $\eps c \cdot m \dist^2 \cdot \sqrt{\frac{m}{k}}>6\log(25)$, then for all $\Xon$ with $Z(\Xon)<-   \frac1{6} c m \dist^2 \cdot \sqrt{\frac{m}{k}} $, with probability at least 0.95, the algorithm outputs the uniform distribution. Combining the conditions, we obtain that there is a constant $C_1$ such that for $\ns = C_1\Paren{\frac{\sqrt{\absz}}{\alpha^2}+ \frac{ k^{ 1/3 } } { \alpha^{4/3}  \eps^{ 2/3 } }}$, with probability at least $0.95\times 0.99 > 0.9$, the algorithm outputs uniform distribution when the input distribution is indeed uniform.  The case of non-uniform distribution is similar because Lemma~\ref{lem:identityerror} holds for both the cases, and is omitted.
%
%Then we consider the case when $\frac{k}{\alpha^2} < m$. When $p=\unifab$, we get $\expectation{Z(\Xon)} = - \frac1{2} c m \alpha$, then using totally the same argument we get 
%\begin{align}
%\probof{Z(\Xon)> -   \frac1{6} c m \dist}   =
%\probof{Z(\Xon) > \frac1{3} \expectation{Z(\Xon) }} \le & 0.01
%\end{align}
%
%If $\eps c \cdot m  \dist>6\log(25)$, then for all $\Xon$ with $Z(\Xon)<-   \frac1{6} c m \dist $, with probability at least 0.95, the algorithm outputs the uniform distribution. 
%Therefore, there exists a constant $C_2$ such that for $\ns = C_2\Paren{\frac{\sqrt{\absz}}{\alpha^2}+ \frac1{\alpha \eps}}$, with probability at least 0.9, the algorithm outputs uniform distribution when the input distribution is indeed uniform. The case of non-uniform distribution is omitted for the same reason.

%%%%%%%%
\iffalse
Therefore, there is a $C_1$ such that if $\ns\ge C_1/\alpha^2$, then under the uniform distribution $\probof{Z(\Xon)>-\frac{c \ns \dist}{6}}$ is at most 1/100. Now furthermore, if $\eps \cdot c m \dist>\log(25)$, then for all $\Xon$ with $Z(\Xon)<-\frac{c\ns\dist}{6}$, with probability at least 0.95, the algorithm outputs the uniform distribution. Combining the conditions, we obtain that there is a constant $C_2$ such that for $\ns = C_2\Paren{\frac{\sqrt{\absz}}{\alpha^2}+ \frac1{\alpha \eps}}$, with probability at least 0.9, the algorithm outputs uniform distribution when the input distribution is indeed uniform.The case of non-uniform distribution is similar since the variance bounds hold for both the cases, and is omitted.
\fi
%%%%%%%%

%At last we consider the case when $m \le k$. When $p=\unifab$, we get $\expectation{Z(\Xon)} = - \frac1{2} c \alpha^2 \cdot \frac{m^2}{k}$, then by Lemma~\ref{lem:identityerror},

==> testing/abstract.tex <==
We study the fundamental problems of identity testing (goodness of fit), and closeness testing (two sample test) of distributions over $k$ elements, under differential privacy. While the problems have a long history in statistics,  finite sample bounds for these problems have only been established recently. 

In this work, we derive upper and lower bounds on the sample complexity of both the problems under $(\varepsilon, \delta)$-differential privacy. We provide sample optimal algorithms for identity testing problem for all parameter ranges, and  the first results for closeness testing. Our closeness testing bounds are optimal in the sparse regime where the number of samples is at most $k$. 

Our upper bounds are obtained by privatizing non-private estimators for these problems. The non-private estimators are chosen to have small sensitivity. We propose a general framework to establish lower bounds on the sample complexity of statistical tasks under differential privacy. We show a bound on differentially private algorithms in terms of a coupling between the two hypothesis classes we aim to test. By carefully constructing chosen priors over the hypothesis classes, and using Le Cam's two point theorem we provide a general mechanism for proving lower bounds.  We believe that the framework can be used to obtain strong lower bounds for other statistical tasks under privacy.

==> testing/app-closeness-testing.tex <==
\section{Proof of Theorem~\ref{thm:close-main} } \label{app:close:}

\subsection{Closeness Testing -- Upper Bounds} \label{sec:close-upper}

%In this section, we only consider the case when $\delta = 0$, which would suffice by lemma~\ref{lm:epsdelta}.
%
%To prove the upper bounds, we privatize the closeness testing algorithm of~\cite{chan2014optimal}. To reduce the strain on the readers, we drop the sequence notations explicitly and let
%\[
%\mltx i \ed \Mltsmb{i}{\Xon}, \text{ and } \mlty i\ed \Mltsmb{i}{\Yon}. 
%\]
%
%Variants of the chi-squared test have been used to test closeness of distributions in the recent years~\cite{AcharyaDJOPS12, chan2014optimal}. In particular,  the statistic used by~\cite{chan2014optimal} is
%\[
% Z(\Xon,\Yon) \ed \sum_{i\in[\ab]} \frac{(\mltx i-\mlty i)^2-\mltx i-\mlty i}{\mltx i+\mlty i},
%\]
%where we assume that $((\mltx i-\mlty i)^2-\mltx i-\mlty i)/({\mltx i+\mlty i})=0$, when $\mltx i +\mlty i = 0$.

%The results in~\cite{chan2014optimal} were proved under Poisson sampling, and we also use Poisson sampling, with only a constant factor effect on the number of samples for the same error probability. They showed the following bounds:
%\begin{align}
%\expectation{ Z(\Xon,\Yon) } &= 0 \text{ when } \p=\q,\label{eqn:expectation-equal}\\
%\Var\Paren{Z(\Xon,\Yon)} &\le 2\min\{\ab, \ns\} \text{ when } \p=\q,\label{eqn:variance-equal}\\
%\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns ^2\alpha^2}{4\ab+2\ns}  \text{ when } \dtv{\p}{\q}\ge\dist,\label{eqn:expectation-unequal}\\
%\Var\Paren{Z(\Xon,\Yon)} &\le \frac1{1000}\expectation{Z(\Xon,\Yon)}^2 \text{ when } \p\ne\q, \text{ and } \ns=\Omega\Paren{\frac1{\alpha^2}}. \label{eqn:variance-equal}
%\end{align}

% We use the same approach with the test statistic as with binary testing and uniformity testing to obtain a differentially private closeness testing method, described in Algorithm~\ref{algorithm_closeness}.
%  \begin{algorithm}
%  	\caption{}
%  	\label{algorithm_closeness}
%  	\hspace*{\algorithmicindent} \textbf{Input:}
%  	$\eps$, $\alpha$, sample access to distribution $p$ and $q$
%  	\begin{algorithmic}[1] 
%  		\State $Z' \gets Z(\Xon,\Yon) - \frac12\frac{\ns^2 \alpha^2}{4\ab+2\ns}$
%  		\State Generate $Y\sim\Bern{\sigma\Paren{\exp(\eps\cdot Z'}}$
%    \State{ {\bf if} $Y=0$, {\bf return} $\p=\q$}
%    \State{ {\bf else}, {\bf return} $\p\ne\q$}
%  	\end{algorithmic}
%  \end{algorithm}

In this section, we will show that Algorithm~\ref{algorithm_closeness} satisfies sample complexity upper bounds described in Theorem~\ref{thm:close-main}.

The results in~\cite{chan2014optimal} were proved under Poisson sampling, and we also use Poisson sampling, with only a constant factor effect on the number of samples for the same error probability. They showed the following bounds:
\begin{align}
\expectation{ Z(\Xon,\Yon) } &= 0 \text{ when } \p=\q,\label{eqn:expectation-equal}\\
\Var\Paren{Z(\Xon,\Yon)} &\le 2\min\{\ab, \ns\} \text{ when } \p=\q,\label{eqn:variance-equal}\\
\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns ^2\alpha^2}{4\ab+2\ns}  \text{ when } \dtv{\p}{\q}\ge\dist,\label{eqn:expectation-unequal}\\
\Var\Paren{Z(\Xon,\Yon)} &\le \frac1{1000}\expectation{Z(\Xon,\Yon)}^2 \text{ when } \p\ne\q, \text{ and } \ns=\Omega\Paren{\frac1{\alpha^2}}. \label{eqn:variance-equal}
\end{align}

%\noindent We first bound the sensitivity (Definition~\ref{def:sensitivity}) of the test statistic to prove privacy bounds. 
%\begin{lemma} \label{sens_close}
%$\Delta(Z(\Xon, \Yon))\le14$. 
%\end{lemma}
%\begin{proof}
%Since $Z(\Xon, \Yon)$ is symmetric, without loss of generality assume that one of the symbols is changed in $\Yon$. This would cause at most two of the $\mlty i$'s to change. Suppose $\mlty i\ge1$, and it changed to $\mlty i-1$. Suppose, $\mltx i+\mlty i > 1$, the absolute change in the $i$th term of the statistic is
%\begin{align}
%\absv{\frac{(\mltx i-\mlty i)^2}{\mltx i+\mlty i}  - \frac{(\mltx i-\mlty i+1)^2}{\mltx i+\mlty i-1} }
%=&    \absv{\frac{(\mltx i+\mlty i) (2\mltx i-2\mlty i+1) +(\mltx i-\mlty i)^2} {(\mltx i+\mlty i) (\mltx i+\mlty i-1)  } } \nonumber \\
%\leq&  \absv{\frac{2\mltx i-2\mlty i+1}{\mltx i+\mlty i-1} }+ \absv {\frac{\mltx i-\mlty i}{\mltx i+\mlty i-1} }\nonumber \\
%\leq&   \frac{3\absv{\mltx i-\mlty i} +1}{\mltx i+\mlty i-1} \nonumber \\
%\leq&    3+ \frac{4}{\mltx i+\mlty i-1}\leq  7.\nonumber
%\end{align}
%When $\mltx i+\mlty i = 1$, the change can again be bounded by 7.  Since at most two of the $\nu_i$'s change, we obtain the desired bound.
%\end{proof}
%
%\noindent Since the sensitivity of the statistic is at most 14, the input to the sigmoid changes by at most $14\eps$ when any input sample is changed.  Invoking Lemma~\ref{lem:sig-cont}, the probability of any output changes by a multiplicative $\exp(14\eps)$, and the algorithm is $14\eps$-differentially private. 
%
%We now prove the correctness of the algorithm:

\textbf{Case 1: $\dist^2>\frac1{\sqrt \ab}$, and $\dist^2\eps>\frac1{\ab}$.} 
In this case, we will show that $\Sct  = O \Paren{ \frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}}$. In this case, $\frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}  \le 2\ab$.

 We consider the case when $\p = \q$, then $\Var\Paren{Z(\Xon,\Yon)} \le 2\min\{\ab, \ns\}$. Let $\Var\Paren{Z(\Xon,\Yon)} \le c \ns$ for some constant $c$. By the Chebyshev's inequality,

\begin{align}
\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}} \le& 
\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns^2 \alpha^2}{8\ab}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} >  \Paren{c\ns}^{1/2} \cdot \frac{\ns^{3/2} \alpha^2}{24c^{1/2} \ab}}  \nonumber\\
\le & 576c\cdot \frac{\ab^2}{\ns^3 \dist^4},\nonumber
\end{align}
where we used that $4k+2m\le 8\ab$. 

Therefore, there is a $C_1$ such that if $\ns \ge C_1 \ab^{2/3} / \alpha^{4/3}$, 
then under $\p=\q$, $\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}$ is at most 1/100. Now furthermore, if $\eps\cdot\ns^2\dist^2 / (672\ab)>\log(20)$, then for all $Z' <  -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}$, with probability at least 0.95, the algorithm outputs the $\p=\q$. Combining the conditions, we obtain that there is a constant $C_2$ such that for $\ns = C_2 \Paren{ \frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}} $, with probability at least 0.9, the algorithm outputs the correct answer when the input distributions satisfy $\p=\q$. The case of  $\dtv{\p}{\q} > \dist$ distribution is similar and is omitted. 


\textbf{Case 2: $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$.} In this case, we will prove a bound of $O \Paren{ \frac{\sqrt\ab}{\alpha^{2}} + \frac{1}{\alpha^2\eps}}$ on the sample complexity. We still consider the case when $\p = \q$. We first note that when $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$, then either $\frac{\sqrt\ab}{\alpha^{2}}+\frac{1}{\alpha^2\eps}>\ab$.  Hence we can assume that the sample complexity bound we aim for is at least $\Omega(\ab)$. So $\Var\Paren{Z(\Xon,\Yon)} \le c \ab$ for constant $c$. By the Chebyshev's inequality,

\begin{align}
\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}} \le& 
\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns \alpha^2}{6}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} >  \Paren{c \ab}^{1/2} \cdot \frac{\ns \alpha^2}{18c^{1/2} \ab^{1/2} }}  \nonumber\\
\le & 144\cdot c\cdot \frac{\ab}{\ns^2 \dist^4}.\nonumber
\end{align}

Therefore, there is a $C_1$ such that if $\ns \ge C_1 \ab^{1/2} / \alpha^{2}$, 
then under $\p=\q$, $\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}$ is at most 1/100. In this situation, if $\eps\cdot\ns \dist^2 / 504>\log(20)$, then for all $Z' <  -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}$, with probability at least 0.95, the algorithm outputs the $\p=\q$. Combining with the previous conditions, we obtain that there also exists a constant $C_2$ such that for $\ns = C_2 \Paren{ \frac{\sqrt\ab}{\alpha^{2}} + \frac{1}{\alpha^2\eps}}$, with probability at least 0.9, the algorithm outputs the correct answer when the input distribution is $\p=\q$. The case of  $\dtv{\p}{\q} > \dist$ distribution is similar and is omitted. 




\subsection{Closeness Testing -- Lower Bounds}  \label{sec:close:lower}

To show the lower bound part of Theorem~\ref{thm:close-main}, we need the following simple result.

\begin{lemma}  \label{lem:close-to-ident}
	%Closeness testing is at least as hard as identity testing.
	 $\Sit \leq \Sct$. 
\end{lemma}

\begin{proof}
Suppose we want to test identity with respect to $\q$. Given $\Xon$ from $\p$, generate $\Yon$ independent samples from $\q$. If $\p=\q$, then the two samples are generated by the same distribution, and otherwise they are generated by distributions that are at least $\eps$ far in total variation. Therefore, we can simply return the output of an \newhz{$(\ab,\dist,\eps)$}-closeness testing algorithm on $\Xon$, and $\Yon$. 
\end{proof}

By Lemma~\ref{lem:close-to-ident} we know that a lower bound for identity testing is also a lower bound on closeness testing.

We first consider the sparse case, when $\dist^2>\frac1{\sqrt \ab}$, and \newhz{$\dist^2 \eps>\frac1{\ab}$}. In this case, we show that 
\newhz{
\[
\Sct= \Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha\sqrt{\eps}}}.
\]
}
When $\alpha>\frac1{k^{1/4}}$, $\frac{\ab^{2/3}}{\alpha^{4/3}}$ is the dominating term in the sample complexity $\Sctnp = \Theta\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^{2}}}$, giving us the first term. By Lemma~\ref{lem:close-to-ident} we know that a lower bound for identity testing is also a lower bound on closeness testing giving the second term, and the lower bound of Theorem~\ref{thm:main-identity} contains the second term as a summand.

In the dense case, when $\dist^2<\frac1{\sqrt \ab}$, or \newhz{$\dist^2 \eps<\frac1{\ab}$}, we show that 
\newhz{
\[
\Sctd = \Omega\Paren{\frac{\sqrt \ab}{\alpha^{2}}+\frac{\sqrt\ab}{\alpha\sqrt{\eps}}+\frac1{\dist \eps}}.
\]
}
In the dense case, using the non-private lower bounds of $\Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^{2}}}$ along with the identity testing bound of sample complexity lower bounds of note that $\frac{\sqrt\ab}{\alpha\sqrt{\eps}}+\frac1{\dist \eps}$ gives a lower bound of $\Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^{2}}+\frac{\sqrt\ab}{\alpha\sqrt{\eps}}+\frac1{\dist \eps} }$. However, in the dense case, it is easy to see that $\frac{\ab^{2/3}}{\alpha^{4/3}}=O\Paren{\frac{\sqrt \ab}{\alpha^{2}}+\frac{\sqrt\ab}{\alpha\sqrt{\eps}}}$ giving us the bound. 




%The first two terms are from the sample complexity bounds for 
%Using this lemma, we get that any lower bound for identity testing will also be a lower bound for closeness testing. Combining with the fact that $\Sct \geq \Sctnp$, we get lower bounds for $\eps$-differentially private closeness testing.
%
%When $\dist^2>\frac1{\sqrt \ab}$, and $\dist^2\eps>\frac1{\ab}$,
%\begin{equation}
%	m = \max\{\Omega\Paren{\frac{\ab^{2/3}}{ \alpha^{4/3}} }, \Omega\Paren{\frac{\sqrt{k}}{\alpha \sqrt{\eps}}}\} = \Omega\Paren{\frac{\ab^{2/3}}{ \alpha^{4/3}} + \frac{\sqrt{k}}{\alpha \sqrt{\eps}} }
%\end{equation}
%
%	which matches the upper bound for closeness testing, hence we get optimal sample complexity in this regime.
%	
%	Otherwise, we have:
%	
%\begin{equation}
%m = \max\{\Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^2}}, \Omega\Paren{\frac{\sqrt \ab}{\alpha\sqrt\eps}+\frac{1}{\alpha \eps} }\} =\Omega\Paren{\frac{\sqrt \ab}{\alpha^2}+\frac{\sqrt \ab}{\alpha\sqrt\eps}+\frac{1}{\alpha \eps}}
%\end{equation}
%












  
  \iffalse
  Similar to uniformity, and binary testing, to get privacy guarantee, it would suffice if the difference in the expectations of the test statistic in two cases is at most $O(\frac{1}{\eps})$.
  \fi


\iffalse
%%begin{comment}
\textbf{Case 1: $\dist^2>\frac1{\sqrt \ab}$, and $\dist^2\eps>\frac1{\ab}$.} 
In this case, we will prove a bound of $O \Paren{ \frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}}$ on the sample complexity. The first term is sufficient for a non-private algorithm in this case. We now show that the second term gives the privacy guarantee. As in lemma~\ref{sens_close}, we will show that $Z(\Xon, \Yon)$ has a sensitivity of at most 7. Using this, it would be enough if the difference in expectations of the statistic is at most $O(1/\eps)$. Assuming $\ns <\ab$, note that
\begin{align}
	\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns ^2\alpha^2}{4\ab},  
\end{align}
which would be at elast $\Omega(1/\eps)$, for $\ns = O\Paren{\frac{\sqrt{\ab}}{\dist\sqrt\eps}}$.

\textbf{Case 2: $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$.} In this case, we will prove a bound of $O \Paren{ \frac{\sqrt\ab}{\alpha^{2}} + \frac{1}{\alpha^2\eps}}$ on the sample complexity. The first term is sufficient for a non-private algorithm in this case. The second term ensures that the privacy conditions are preserved. We first note that when $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$, then either $\frac{\sqrt\ab}{\alpha^{2}}+\frac{1}{\alpha^2\eps}>\ab$.  Hence we can assume that the sample complexity bound we aim for is at least $\Omega(\ab)$. Therefore, in this case, 
\begin{align}
	\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns\alpha^2}{4},  
\end{align}
which would be at least $\Omega(1/\eps)$, for $\ns = O\Paren{\frac1{\dist^2\eps}}$.
\fi
%%end{comment}









%\begin{theorem}
%Algorithm~\ref{algorithm_closeness} is an $\eps$-differentially private algorithm for testing if $\p = \q$ or $ \dtv{\p}{\q}\ge\alpha$ for the closeness testing problem. Moreover, it has error probability at most $1/3$, with sample complexity $O \Paren{ \ab^{2/3} / \alpha^{4/3} + \ab^{1/2}/ \alpha^{2} + \ab^{1/2}/  (\alpha \eps^{1/2}) + 1/ (\alpha^2 \eps)}$.
%\end{theorem}
%
%We proceed to prove the two aspects of the algorithm, correctness and privacy.
%
%First we consider the correctness. We use the following two properties of the statistics, which rely on the condition that $O \Paren{ \ab^{2/3} / \alpha^{4/3}+ \ab^{1/2}/ \alpha^{2}}$. The proof for the two claims can be found in ~\cite{chan2014optimal}.
%
%\begin{claim}
%	Given $\p=\q$, $\expectation{Z} = 0$. Given $ \dtv{\p}{\q}\ge\alpha$, $\expectation{Z}\ge 1$.
%\end{claim}
%
%\begin{claim}
%	Given $\p=\q$, $\variance{Z} \le \frac1{1000}$. Given $ \dtv{\p}{\q}\ge\alpha$, $\variance{Z} \le \frac1{1000} \expectation{E}^2(Z)$.
%\end{claim}
%
%
%We consider the case $\p=\q$. According to Chebyshev's inequality, we get that $Z \le 1/10$ with probability at least $9/10$, and we output  $\p = \q$ with probability $1/10+4/5*(9/10)^2 \ge 2/3$ . Similarly, when $ \dtv{\p}{\q}\ge\alpha$, $E(Z) \ge 1$, $Z \ge 9/10$ with probability at least $9/10$, and we get the right answer with probability greater than $2/3$. 
%
%Then we consider the privacy. We will prove the algorithm is $(0,\frac1{10} \eps)$ differentially private. Because each output for the algorithm is at least $1/10$, so the $(0,\frac1{10} \eps)$ differential privacy will imply $(\eps,0)$ differential privacy.
%
%Now we consider the value of $Z$ for two neighbouring datasets $D$ and $D ^ \prime$, where  $D ^ \prime$ has one fewer occurrence of sample. Without loss of generality, we assume $D^\prime$ has one fewer occurrence of symbol $i$ from distribution $q$.  When $\mltx i+\mlty i > 1$, we have
%\begin{align}
%&\absv{Z(D) - Z(D^\prime)} \\
%= &  \frac{4\ab+2\ns}{\ns^2 \alpha^2} \absv{\frac{(\mltx i-\mlty i)^2}{\mltx i+\mlty i}  - \frac{(\mltx i-\mlty i+1)^2}{\mltx i+\mlty i-1} }\\
%=&   \frac{4\ab+2\ns}{\ns^2 \alpha^2} \cdot \frac{(\mltx i+\mlty i) (2\mltx i-2\mlty i+1) +(\mltx i-\mlty i)^2} {(\mltx i+\mlty i) (\mltx i+\mlty i-1)  }   \\
%\leq&   \frac{4\ab+2\ns}{\ns^2 \alpha^2}  \cdot  \Brack{\frac{2\mltx i-2\mlty i+1}{\mltx i+\mlty i-1}+ \frac{\mltx i-\mlty i}{\mltx i+\mlty i-1} }\\
%\leq&  \frac{4\ab+2\ns}{\ns^2 \alpha^2} \cdot  \Brack{ \frac{3\absv{\mltx i-\mlty i} +1}{\mltx i+\mlty i-1} }\\
%\leq&    \frac{4\ab+2\ns}{\ns^2 \alpha^2} \cdot  \Brack{3+ \frac{4}{\mltx i+\mlty i-1}}\\
%\leq&  \frac{4\ab+2\ns}{\ns^2 \alpha^2} \cdot 7
%\end{align}
%When $\mltx i+\mlty i = 1$, it is easy to get $Z(D)- Z(D^\prime) = 0$.
%
%Then we prove under our constraint, $\absv{Z(D) - Z(D^\prime)} \le \frac1{8} \eps$. When $\ns < \ab$, $\absv{Z(D) - Z(D^\prime)} \le \ab/ (\ns^2 \alpha^2)$. Under the constraint of $m = \Omega \Paren {\ab^{1/2}/  (\alpha \eps^{1/2}) }$. We get $\absv{Z(D) - Z(D^\prime)} \le \frac1{8} \eps $. Else when $\ns > \ab$, $\absv{Z(D) - Z(D^\prime)} \le 6 / (\ns \alpha^2)$. Using the constraint of $\ns = \Omega \Paren {1/ (\alpha^2 \eps)}$, we get the same result.
%
%Now suppose the algorithm outputs $\p=\q$, the difference of the output probability for $D$ and $D^\prime$ is at most $4/5 * \absv{T(D)- T(D^\prime)} \le \frac1{10} \eps$. And things are similar if we output $ \dtv{\p}{\q}\ge\alpha$. So we have proved our algorithm is $(0,\frac1{10} \eps)$. Combining with the previous argument, the algorithm is also $(\eps,0)$ differentially private.
%


==> testing/app-group-property.tex <==
\subsection{Proof of Lemmas}

\subsubsection{Proof of Lemma~\ref{lem:group}}
\label{app:group}
%
%\begin{lemma}
%	Let $\alg$ be a $(\eps,\delta)$-DP algorithm, then for sequences $\xon$, and $\yon$ with $\ham{\xon}{\yon} \le t$, and $\forall S$, 
%$		\probof{\cA(\xon)\in S}\le e^{t\eps}\cdot\probof{\cA(\yon)\in S}+ \delta t e^{\eps (t-1)}$. 
%\end{lemma}

\begin{proof}
Let $\ham{\xon}{\yon}= \hat D$. When $\hat D = 0$ or $1$, the lemma is trivially true.  Then, suppose $\hat D \ge 2$ we can find $\hat D-1$ sequences  $z^m_1, \ldots, z^m_{\hat D-1}$ over $\cX^\ns$ with $\ham{\xon}{z^m_1} =1, \ham{z^m_{\hat D - 1} }{\yon} = 1$ and $\ham{z^m_i}{z^m_{i+1}} = 1$ for $i \in \{1,2,...,\hat D - 2\}$. 
Hence, by the condition of $(\eps,\delta)$ - differential privacy,
\begin{align}
	\probof{\alg\Paren{\xon}=\q} & \leq  e^{\eps} \probof{\alg\Paren{z^m_{1}}=\q} + \delta 
	\leq e^{\eps} (e^{\eps} \probof{\alg\Paren{z^m_{2}}=\q} + \delta) + \delta \le \ldots \nonumber\\
	&\leq  e^{\hat D\eps} \probof{\alg\Paren{\yon}=\q}+ \delta\cdot\sum_{i = 0}^{\hat D - 1} e^{i\eps} 
	\leq  e^{\hat D\eps} \probof{\alg\Paren{\yon}=\q}  + \delta \hat D e^{(\hat D-1) \eps } \nonumber \\ 
	%\frac{e^{\eps \hat D} - 1}{e^{\eps} - 1} \nonumber \\
	&\leq  e^{t\eps} \probof{\alg\Paren{\yon}=\q}  + \delta t e^{\eps(t-1)}. \nonumber
%	\leq  e^{t\eps} \probof{\alg\Paren{\xon}=\q}  + \delta t e^{\eps t} \nonumber
\end{align}
\end{proof}

\subsubsection{Proof of Lemma~\ref{lm:epsdelta}} \label{app:epsdelta}
\begin{proof}
	Suppose $\cA$ is a $(\eps+\delta)$-differentially private algorithm. Then for any $\Xon$ and $\Yon$ with $\ham{\Xon}{\Yon}\le 1$ and any $S\subset \text{range}(\cA)$, we have
	\begin{align*}
		% \probof{\cA(\Xon)\in S} \le e^{\eps+\delta}\cdot\probof{\cA(\Yon)\in S} 
		% 									 = e^{\eps}\cdot\probof{\cA(\Yon)\in S} + (e^{\delta} - 1)\cdot e^{\eps}\probof{\cA(\Yon)\in S}. 
		\probof{\cA(\Xon)\in S} \le e^{\eps}\cdot\probof{\cA(\Yon)\in S} + (e^{\delta} - 1)\cdot e^{\eps}\probof{\cA(\Yon)\in S}. 
	\end{align*}
	If $e^{\eps}\cdot\probof{\cA(\Yon)\in S} > 1-\delta$, then $\probof{\cA(\Xon)\in S}\le1< e^{\eps}\cdot\probof{\cA(\Yon)\in S}+\delta$.
	Otherwise, $e^{\eps}\cdot\probof{\cA(\Yon)\in S} \leq 1 - \delta$. To prove $(e^{\delta}-1)\cdot e^{\eps}\cdot\probof{\cA(\Yon)\in S}<\delta$, it suffices to show $(e^{\delta} - 1)(1 - \delta) \le \delta$, which is equivalent to $e^{-\delta} \ge 1 - \delta$, completing the proof.
\end{proof}

==> testing/app-uniformity-to-identity.tex <==
\section{Proof of Theorem~\ref{thm:unif-identity}}
\label{app:iden-unif}

\begin{proof} We first briefly describe the essential components of the construction of~\cite{goldreich2016uniform}. Given an explicit distribution $\q$ over $[\ab]$, there exists a randomized function $F_{\q}:[\ab]\to[6\ab]$  such that if $X\sim\q$, then $F_{\q}(X)\sim \unifabs{6\ab}$, and if $X\sim\p$ for a distribution with $\dtv{\p}{\q}\ge\dist$, then the distribution of $F_{\q}(X)$ has a total variation distance of at least $\dist/3$ from $\unifabs{6\ab}$. 
Given $s$ samples $X_1^s$ from a distribution $\p$ over $[\ab]$. Apply $F_\q$ independently to each of the $X_i$ to obtain a new sequence $Y_1^s = F_\q(X_1^s)\ed F_q(X_1)\ldots F_{\q}(X_s)$. Let $\cA$ be an algorithm that distinguishes $\unifabs{6\ab}$ from all distributions with total variation distance at least $\dist/3$ from it. Then consider the algorithm $\cA^{'}$ that outputs $\p=\q$ if $\cA$ outputs ``$\p = \unifabs{6k}$'', and outputs $\p\ne \q$ otherwise. This shows that without privacy constraints, $\Sitnp \le \Sutnp{6\ab}{\dist/3}$ (See~\cite{goldreich2016uniform} for details). 

We now prove that if further $\cA$ was an $\eps$-DP algorithm, then $\cA^{'}$ is also an $\eps$-DP algorithm. Suppose $X_1^s$, and $X_1^{'s}$ be two sequences in $[\ab]^s$ that could differ only on the last coordinate, namely $\Xos = \Xosmo X_s$, and $\Xosp = \Xosmo X_s^{'}$. 

Consider two sequences $\Yos= \Yosmo Y_s$, and $\Yosp= \Yosmo Y_s^{'}$ in $[6\ab]^s$ that could differ on only the last coordinate. Since $\cA$ is $\eps$-DP, 
\begin{align}
\cA(\Yos=\unifabs{6\ab}) \le \cA(\Yosp=\unifabs{6\ab})\cdot e^{\eps}.\label{eqn:dp-unif}
\end{align}
Moreover, since $F_{\q}$ is applied independently to each coordinate, 
\[
\probof{F_{\q}(\Xos) = \Yos} = \probof{F_{\q}(\Xosmo) = \Yosmo}\probof{F_{\q}(X_s) = Y_s}.
\]
Then, 
\begin{align}
&\ \ \ \ \probof{\cA^{'}(\Xos) = \q} \nonumber\\
& = \probof{\cA(F_{\q}(X_1^s)) = \unifabs{6\ab}}\nonumber\\
& = \sum_{\Yos}\ \probof{\mathcal{A}(Y^s_1) = \unifabs{6\ab}}\probof{F_{\q}(\Xos) = \Yos)}\nonumber\\
& = \sum_{\Yosmo} \sum_{Y_s\in[6\ab]}\ \probof{\mathcal{A}(Y^s_1) = \unifabs{6\ab}} \probof{F_{\q}(\Xosmo) = \Yosmo}\probof{F_{\q}(X_s) = Y_s}\nonumber\\
& = \sum_{\Yosmo}\probof{F_{\q}(\Xosmo) = \Yosmo}\Brack{ \sum_{Y_s\in[6\ab]}\ \probof{\mathcal{A}(Y^s_1) = \unifabs{6\ab}} \probof{F_{\q}(X_s) = Y_s}}.\label{eqn:first-term-prob}
\end{align}
Similarly, 
\begin{align}
\probof{\cA^{'}(\Xosp) = \q}
 \!\!=\!\! \sum_{\Yosmo}\probof{F_{\q}(\Xosmo)\!\! = \!\!\Yosmo}\Brack{ \sum_{Y_s^{'}\in[6\ab]} \probof{\mathcal{A}(\Yosp) = \unifabs{6\ab}} \probof{F_{\q}(X_s^{'}) = Y_s^{'}}}.\label{eqn:second-term-prob}
\end{align}
For a fixed $\Yosmo$, the term within the bracket in~\eqref{eqn:first-term-prob}, and~\eqref{eqn:second-term-prob} are both expectations over the final coordinate. However, by~\eqref{eqn:dp-unif} these expectations differ at most by a multiplicative $e^{\eps}$ factor. This implies that
\begin{align}
	\probof{\cA'(\Xos) = \q}\le \probof{\cA'(\Xosp) = \q}e^{\eps}.\nonumber
\end{align}
The argument is similar for the case when the testing output is \textbf{not $\unifabs{6\ab}$}, and is omitted here. We only considered sequences that differ on the last coordinate, and the proof remains the same when any of the coordinates is changed. This proves the privacy guarantees of the algorithm.
\end{proof}


==> testing/closeness-testing.tex <==
\section{Closeness Testing} \label{sec:close:}

Recall the closeness testing problem from Section~\ref{sec:testing_preliminaries}, and the tight non-private bounds from Table~\ref{fig:badass:table}. Our main result in this section is the following theorem characterizing the sample complexity of differentially private algorithms for closeness testing. 
\newhz{
\begin{theorem}
	\label{thm:close-main}
		If $\alpha>1/\ab^{1/4}$, and $\eps\dist^2>1/\ab$,
		\[
		\Sct= \Theta \Paren{ \frac{\ab^{2/3}} {\alpha^{4/3}} + \frac{\ab^{1/2}}{  \alpha \sqrt{\eps} }},
		\]
		otherwise, 
		\[
	\Omega \Paren{ \frac{\ab^{1/2}}{ \alpha^{2}} + \frac{\ab^{1/2} }{ \alpha\sqrt{\eps}}+ \frac{1}{ \alpha \eps}}\le	\Sct\le O \Paren{ \frac{\ab^{1/2}}{ \alpha^{2}} + \frac{1}{ \alpha^2 \eps}}.
		\]
\end{theorem}
}
{
This theorem shows that in the sparse regime, when $\ns=O(\ab)$, our bounds are tight up to constant factors in all parameters. 

\subsection{Closeness Testing -- Upper Bounds} \label{sec:close-upper}

To prove the upper bounds, we only consider the case when $\delta = 0$, which would suffice by lemma~\ref{lm:epsdelta}. We privatize the closeness testing algorithm of~\cite{ChanDVV14}. To reduce the strain on the readers, we drop the sequence notations explicitly and let
\[
\mltx i \ed \Mltsmb{i}{\Xon}, \text{ and } \mlty i\ed \Mltsmb{i}{\Yon}. 
\]
The statistic used by~\cite{ChanDVV14} is
\[
Z(\Xon,\Yon) \ed \sum_{i\in[\ab]} \frac{(\mltx i-\mlty i)^2-\mltx i-\mlty i}{\mltx i+\mlty i},
\]
where we assume that $((\mltx i-\mlty i)^2-\mltx i-\mlty i)/({\mltx i+\mlty i})=0$, when $\mltx i +\mlty i = 0$. It turns out that this statistic has a constant sensitivity, as shown in Lemma~\ref{sens_close}.
%\noindent We first bound the sensitivity (Definition~\ref{def:sensitivity}) of the test statistic to prove privacy bounds. 
\begin{lemma} \label{sens_close}
	$\Delta(Z(\Xon, \Yon))\le14$. 
\end{lemma}
\begin{proof}
	Since $Z(\Xon, \Yon)$ is symmetric, without loss of generality assume that one of the symbols is changed in $\Yon$. This would cause at most two of the $\mlty i$'s to change. Suppose $\mlty i\ge1$, and it changed to $\mlty i-1$. Suppose, $\mltx i+\mlty i > 1$, the absolute change in the $i$th term of the statistic is
	\begin{align}
	\absv{\frac{(\mltx i-\mlty i)^2}{\mltx i+\mlty i}  - \frac{(\mltx i-\mlty i+1)^2}{\mltx i+\mlty i-1} }
	=&    \absv{\frac{(\mltx i+\mlty i) (2\mltx i-2\mlty i+1) +(\mltx i-\mlty i)^2} {(\mltx i+\mlty i) (\mltx i+\mlty i-1)  } } \nonumber \\
	\leq&  \absv{\frac{2\mltx i-2\mlty i+1}{\mltx i+\mlty i-1} }+ \absv {\frac{\mltx i-\mlty i}{\mltx i+\mlty i-1} }\nonumber \\
	\leq&   \frac{3\absv{\mltx i-\mlty i} +1}{\mltx i+\mlty i-1} \leq    3+ \frac{4}{\mltx i+\mlty i-1}\leq  7.\nonumber
	\end{align}
	When $\mltx i+\mlty i = 1$, the change can again be bounded by 7.  Since at most two of the $\nu_i$'s change, we obtain the desired bound.
\end{proof}
We use the same approach with the test statistic as with uniformity testing to obtain a differentially private closeness testing method, described in Algorithm~\ref{algorithm_closeness}. Since the sensitivity of the statistic is at most 14, the input to the sigmoid changes by at most $\eps$ when any input sample is changed.  Invoking Lemma~\ref{lem:sig-cont}, the probability of any output changes by a multiplicative $\exp(\eps)$, and the algorithm is $\eps$-differentially private. 
\begin{algorithm}
	\caption{}
	\label{algorithm_closeness}
	\hspace*{\algorithmicindent} \textbf{Input:}
	$\eps$, $\alpha$, sample access to distribution $p$ and $q$
	\begin{algorithmic}[1] 
		\State $Z' \gets (Z(\Xon,\Yon) - \frac12\frac{\ns^2 \alpha^2}{4\ab+2\ns})/14$
		\State Generate $Y\sim\Bern{\sigma\Paren{\exp(\eps\cdot Z'}}$
		\State{ {\bf if} $Y=0$, {\bf return} $\p=\q$}
		\State{ {\bf else}, {\bf return} $\p\ne\q$}
	\end{algorithmic}
\end{algorithm}
}

%The remaining part is to show that Algorithm~\ref{algorithm_closeness} satisfies sample complexity upper bounds described in theorem~\ref{thm:close-main}. We will give the details in Appendix~\ref{app:close:}, where the analysis of the lower bound is also given.


%In this section, we only consider the case when $\delta = 0$, which would suffice by lemma~\ref{lm:epsdelta}.
%
%To prove the upper bounds, we privatize the closeness testing algorithm of~\cite{chan2014optimal}. To reduce the strain on the readers, we drop the sequence notations explicitly and let
%\[
%\mltx i \ed \Mltsmb{i}{\Xon}, \text{ and } \mlty i\ed \Mltsmb{i}{\Yon}. 
%\]
%
%Variants of the chi-squared test have been used to test closeness of distributions in the recent years~\cite{AcharyaDJOPS12, chan2014optimal}. In particular,  the statistic used by~\cite{chan2014optimal} is
%\[
% Z(\Xon,\Yon) \ed \sum_{i\in[\ab]} \frac{(\mltx i-\mlty i)^2-\mltx i-\mlty i}{\mltx i+\mlty i},
%\]
%where we assume that $((\mltx i-\mlty i)^2-\mltx i-\mlty i)/({\mltx i+\mlty i})=0$, when $\mltx i +\mlty i = 0$.

%The results in~\cite{chan2014optimal} were proved under Poisson sampling, and we also use Poisson sampling, with only a constant factor effect on the number of samples for the same error probability. They showed the following bounds:
%\begin{align}
%\expectation{ Z(\Xon,\Yon) } &= 0 \text{ when } \p=\q,\label{eqn:expectation-equal}\\
%\Var\Paren{Z(\Xon,\Yon)} &\le 2\min\{\ab, \ns\} \text{ when } \p=\q,\label{eqn:variance-equal}\\
%\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns ^2\alpha^2}{4\ab+2\ns}  \text{ when } \dtv{\p}{\q}\ge\dist,\label{eqn:expectation-unequal}\\
%\Var\Paren{Z(\Xon,\Yon)} &\le \frac1{1000}\expectation{Z(\Xon,\Yon)}^2 \text{ when } \p\ne\q, \text{ and } \ns=\Omega\Paren{\frac1{\alpha^2}}. \label{eqn:variance-equal}
%\end{align}

% We use the same approach with the test statistic as with binary testing and uniformity testing to obtain a differentially private closeness testing method, described in Algorithm~\ref{algorithm_closeness}.
%  \begin{algorithm}
%  	\caption{}
%  	\label{algorithm_closeness}
%  	\hspace*{\algorithmicindent} \textbf{Input:}
%  	$\eps$, $\alpha$, sample access to distribution $p$ and $q$
%  	\begin{algorithmic}[1] 
%  		\State $Z' \gets Z(\Xon,\Yon) - \frac12\frac{\ns^2 \alpha^2}{4\ab+2\ns}$
%  		\State Generate $Y\sim\Bern{\sigma\Paren{\exp(\eps\cdot Z'}}$
%    \State{ {\bf if} $Y=0$, {\bf return} $\p=\q$}
%    \State{ {\bf else}, {\bf return} $\p\ne\q$}
%  	\end{algorithmic}
%  \end{algorithm}

In this section, we will show that Algorithm~\ref{algorithm_closeness} satisfies sample complexity upper bounds described in Theorem~\ref{thm:close-main}.

The results in~\cite{ChanDVV14} were proved under Poisson sampling, and we also use Poisson sampling, with only a constant factor effect on the number of samples for the same error probability. They showed the following bounds:
\begin{align}
\expectation{ Z(\Xon,\Yon) } &= 0 \text{ when } \p=\q,\label{eqn:expectation-equal}\\
\Var\Paren{Z(\Xon,\Yon)} &\le 2\min\{\ab, \ns\} \text{ when } \p=\q,\label{eqn:variance-equal}\\
\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns ^2\alpha^2}{4\ab+2\ns}  \text{ when } \dtv{\p}{\q}\ge\dist,\label{eqn:expectation-unequal}\\
\Var\Paren{Z(\Xon,\Yon)} &\le \frac1{1000}\expectation{Z(\Xon,\Yon)}^2 \text{ when } \p\ne\q, \text{ and } \ns=\Omega\Paren{\frac1{\alpha^2}}. \label{eqn:variance-equal}
\end{align}

%\noindent We first bound the sensitivity (Definition~\ref{def:sensitivity}) of the test statistic to prove privacy bounds. 
%\begin{lemma} \label{sens_close}
%$\Delta(Z(\Xon, \Yon))\le14$. 
%\end{lemma}
%\begin{proof}
%Since $Z(\Xon, \Yon)$ is symmetric, without loss of generality assume that one of the symbols is changed in $\Yon$. This would cause at most two of the $\mlty i$'s to change. Suppose $\mlty i\ge1$, and it changed to $\mlty i-1$. Suppose, $\mltx i+\mlty i > 1$, the absolute change in the $i$th term of the statistic is
%\begin{align}
%\absv{\frac{(\mltx i-\mlty i)^2}{\mltx i+\mlty i}  - \frac{(\mltx i-\mlty i+1)^2}{\mltx i+\mlty i-1} }
%=&    \absv{\frac{(\mltx i+\mlty i) (2\mltx i-2\mlty i+1) +(\mltx i-\mlty i)^2} {(\mltx i+\mlty i) (\mltx i+\mlty i-1)  } } \nonumber \\
%\leq&  \absv{\frac{2\mltx i-2\mlty i+1}{\mltx i+\mlty i-1} }+ \absv {\frac{\mltx i-\mlty i}{\mltx i+\mlty i-1} }\nonumber \\
%\leq&   \frac{3\absv{\mltx i-\mlty i} +1}{\mltx i+\mlty i-1} \nonumber \\
%\leq&    3+ \frac{4}{\mltx i+\mlty i-1}\leq  7.\nonumber
%\end{align}
%When $\mltx i+\mlty i = 1$, the change can again be bounded by 7.  Since at most two of the $\nu_i$'s change, we obtain the desired bound.
%\end{proof}
%
%\noindent Since the sensitivity of the statistic is at most 14, the input to the sigmoid changes by at most $14\eps$ when any input sample is changed.  Invoking Lemma~\ref{lem:sig-cont}, the probability of any output changes by a multiplicative $\exp(14\eps)$, and the algorithm is $14\eps$-differentially private. 
%
%We now prove the correctness of the algorithm:

\textbf{Case 1: $\dist^2>\frac1{\sqrt \ab}$, and $\dist^2\eps>\frac1{\ab}$.} 
In this case, we will show that $\Sct  = O \Paren{ \frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}}$. In this case, $\frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}  \le 2\ab$.

 We consider the case when $\p = \q$, then $\Var\Paren{Z(\Xon,\Yon)} \le 2\min\{\ab, \ns\}$. Let $\Var\Paren{Z(\Xon,\Yon)} \le c \ns$ for some constant $c$. By the Chebyshev's inequality,

\begin{align}
\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}} \le& 
\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns^2 \alpha^2}{8\ab}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} >  \Paren{c\ns}^{1/2} \cdot \frac{\ns^{3/2} \alpha^2}{24c^{1/2} \ab}}  \nonumber\\
\le & 576c\cdot \frac{\ab^2}{\ns^3 \dist^4},\nonumber
\end{align}
where we used that $4k+2\ns\le 8\ab$. 

Therefore, there is a $C_1$ such that if $\ns \ge C_1 \ab^{2/3} / \alpha^{4/3}$, 
then under $\p=\q$, $\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}$ is at most 1/100. Now furthermore, if $\eps\cdot\ns^2\dist^2 / (672\ab)>\log(20)$, then for all $Z' <  -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}$, with probability at least 0.95, the algorithm outputs the $\p=\q$. Combining the conditions, we obtain that there is a constant $C_2$ such that for $\ns = C_2 \Paren{ \frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}} $, with probability at least 0.9, the algorithm outputs the correct answer when the input distributions satisfy $\p=\q$. The case of  $\dtv{\p}{\q} > \dist$ distribution is similar and is omitted. 


\textbf{Case 2: $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$.} In this case, we will prove a bound of $O \Paren{ \frac{\sqrt\ab}{\alpha^{2}} + \frac{1}{\alpha^2\eps}}$ on the sample complexity. We still consider the case when $\p = \q$. We first note that when $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$, then either $\frac{\sqrt\ab}{\alpha^{2}}+\frac{1}{\alpha^2\eps}>\ab$.  Hence we can assume that the sample complexity bound we aim for is at least $\Omega(\ab)$. So $\Var\Paren{Z(\Xon,\Yon)} \le c \ab$ for constant $c$. By the Chebyshev's inequality,

\begin{align}
\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}} \le& 
\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} > \frac13 \cdot \frac{\ns \alpha^2}{6}}  \nonumber\\
\le&\probof{Z(\Xon, \Yon)  -\expectation{Z (\Xon, \Yon)} >  \Paren{c \ab}^{1/2} \cdot \frac{\ns \alpha^2}{18c^{1/2} \ab^{1/2} }}  \nonumber\\
\le & 144\cdot c\cdot \frac{\ab}{\ns^2 \dist^4}.\nonumber
\end{align}

Therefore, there is a $C_1$ such that if $\ns \ge C_1 \ab^{1/2} / \alpha^{2}$, 
then under $\p=\q$, $\probof{Z' > -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}}$ is at most 1/100. In this situation, if $\eps\cdot\ns \dist^2 / 504>\log(20)$, then for all $Z' <  -\frac1{84} \cdot \frac{\ns^2 \alpha^2}{4\ab+2\ns}$, with probability at least 0.95, the algorithm outputs the $\p=\q$. Combining with the previous conditions, we obtain that there also exists a constant $C_2$ such that for $\ns = C_2 \Paren{ \frac{\sqrt\ab}{\alpha^{2}} + \frac{1}{\alpha^2\eps}}$, with probability at least 0.9, the algorithm outputs the correct answer when the input distribution is $\p=\q$. The case of  $\dtv{\p}{\q} > \dist$ distribution is similar and is omitted. 




\subsection{Closeness Testing -- Lower Bounds}  \label{sec:close:lower}

To show the lower bound part of Theorem~\ref{thm:close-main}, we need the following simple result.

\begin{lemma}  \label{lem:close-to-ident}
	%Closeness testing is at least as hard as identity testing.
	 $\Sit \leq \Sct$. 
\end{lemma}

\begin{proof}
Suppose we want to test identity with respect to $\q$. Given $\Xon$ from $\p$, generate $\Yon$ independent samples from $\q$. If $\p=\q$, then the two samples are generated by the same distribution, and otherwise they are generated by distributions that are at least $\eps$ far in total variation. Therefore, we can simply return the output of an \newhz{$(\ab,\dist,\eps)$}-closeness testing algorithm on $\Xon$, and $\Yon$. 
\end{proof}

By Lemma~\ref{lem:close-to-ident} we know that a lower bound for identity testing is also a lower bound on closeness testing.

We first consider the sparse case, when $\dist^2>\frac1{\sqrt \ab}$, and \newhz{$\dist^2 \eps>\frac1{\ab}$}. In this case, we show that 
\newhz{
\[
\Sct= \Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha\sqrt{\eps}}}.
\]
}
When $\alpha>\frac1{k^{1/4}}$, $\frac{\ab^{2/3}}{\alpha^{4/3}}$ is the dominating term in the sample complexity $\Sctnp = \Theta\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^{2}}}$, giving us the first term. By Lemma~\ref{lem:close-to-ident} we know that a lower bound for identity testing is also a lower bound on closeness testing giving the second term, and the lower bound of Theorem~\ref{thm:main-identity} contains the second term as a summand.

In the dense case, when $\dist^2<\frac1{\sqrt \ab}$, or \newhz{$\dist^2 \eps<\frac1{\ab}$}, we show that 
\newhz{
\[
\Sctd = \Omega\Paren{\frac{\sqrt \ab}{\alpha^{2}}+\frac{\sqrt\ab}{\alpha\sqrt{\eps}}+\frac1{\dist \eps}}.
\]
}
In the dense case, using the non-private lower bounds of $\Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^{2}}}$ along with the identity testing bound of sample complexity lower bounds of note that $\frac{\sqrt\ab}{\alpha\sqrt{\eps}}+\frac1{\dist \eps}$ gives a lower bound of $\Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^{2}}+\frac{\sqrt\ab}{\alpha\sqrt{\eps}}+\frac1{\dist \eps} }$. However, in the dense case, it is easy to see that $\frac{\ab^{2/3}}{\alpha^{4/3}}=O\Paren{\frac{\sqrt \ab}{\alpha^{2}}+\frac{\sqrt\ab}{\alpha\sqrt{\eps}}}$ giving us the bound. 




%The first two terms are from the sample complexity bounds for 
%Using this lemma, we get that any lower bound for identity testing will also be a lower bound for closeness testing. Combining with the fact that $\Sct \geq \Sctnp$, we get lower bounds for $\eps$-differentially private closeness testing.
%
%When $\dist^2>\frac1{\sqrt \ab}$, and $\dist^2\eps>\frac1{\ab}$,
%\begin{equation}
%	m = \max\{\Omega\Paren{\frac{\ab^{2/3}}{ \alpha^{4/3}} }, \Omega\Paren{\frac{\sqrt{k}}{\alpha \sqrt{\eps}}}\} = \Omega\Paren{\frac{\ab^{2/3}}{ \alpha^{4/3}} + \frac{\sqrt{k}}{\alpha \sqrt{\eps}} }
%\end{equation}
%
%	which matches the upper bound for closeness testing, hence we get optimal sample complexity in this regime.
%	
%	Otherwise, we have:
%	
%\begin{equation}
%m = \max\{\Omega\Paren{\frac{\ab^{2/3}}{\alpha^{4/3}}+\frac{\sqrt \ab}{\alpha^2}}, \Omega\Paren{\frac{\sqrt \ab}{\alpha\sqrt\eps}+\frac{1}{\alpha \eps} }\} =\Omega\Paren{\frac{\sqrt \ab}{\alpha^2}+\frac{\sqrt \ab}{\alpha\sqrt\eps}+\frac{1}{\alpha \eps}}
%\end{equation}
%












  
  \iffalse
  Similar to uniformity, and binary testing, to get privacy guarantee, it would suffice if the difference in the expectations of the test statistic in two cases is at most $O(\frac{1}{\eps})$.
  \fi


\iffalse
%%begin{comment}
\textbf{Case 1: $\dist^2>\frac1{\sqrt \ab}$, and $\dist^2\eps>\frac1{\ab}$.} 
In this case, we will prove a bound of $O \Paren{ \frac{\ab^{2/3}}{\alpha^{4/3}} + \frac{\ab^{1/2}}{\alpha\sqrt\eps}}$ on the sample complexity. The first term is sufficient for a non-private algorithm in this case. We now show that the second term gives the privacy guarantee. As in lemma~\ref{sens_close}, we will show that $Z(\Xon, \Yon)$ has a sensitivity of at most 7. Using this, it would be enough if the difference in expectations of the statistic is at most $O(1/\eps)$. Assuming $\ns <\ab$, note that
\begin{align}
	\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns ^2\alpha^2}{4\ab},  
\end{align}
which would be at elast $\Omega(1/\eps)$, for $\ns = O\Paren{\frac{\sqrt{\ab}}{\dist\sqrt\eps}}$.

\textbf{Case 2: $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$.} In this case, we will prove a bound of $O \Paren{ \frac{\sqrt\ab}{\alpha^{2}} + \frac{1}{\alpha^2\eps}}$ on the sample complexity. The first term is sufficient for a non-private algorithm in this case. The second term ensures that the privacy conditions are preserved. We first note that when $\dist^2<\frac1{\sqrt \ab}$, or $\dist^2\eps<\frac1{\ab}$, then either $\frac{\sqrt\ab}{\alpha^{2}}+\frac{1}{\alpha^2\eps}>\ab$.  Hence we can assume that the sample complexity bound we aim for is at least $\Omega(\ab)$. Therefore, in this case, 
\begin{align}
	\expectation{ Z(\Xon,\Yon) } &\ge \frac{ \ns\alpha^2}{4},  
\end{align}
which would be at least $\Omega(1/\eps)$, for $\ns = O\Paren{\frac1{\dist^2\eps}}$.
\fi






==> testing/coupling.tex <==
\section{Privacy Bounds via Coupling} 
\label{sec:coupling}

Recall that \emph{coupling} between distributions $\p$ and $\q$  over $\cX$, and $\cY$, is a distribution over $\cX\times\cY$ whose marginal distributions are $\p$ and $\q$ (Definition~\ref{def:coupling}). For simplicity, we treat coupling as a randomized function $f: \cX\to\cY$ such that if $X\sim\p$, then $Y=f(X)\sim\q$. Note that $X$, and $Y$ are not necessarily independent. 

\begin{example}
\label{exm:coin}
Let $\Bern{b_1}$, and $\Bern{b_2}$ be Bernoulli distributions with bias $b_1$, and $b_2$ such that $b_1<b_2$. Let $\p$, and $\q$ be distributions over $\{0,1\}^\ns$ obtained by $\ns$ \emph{i.i.d.} samples from $\Bern{b_1}$, and $\Bern{b_2}$ respectively. Let $\Xon$ be distributed according to $\p$. Generate a sequence $\Yon$ as follows: If $X_i=1$, then $Y_i=1$. If $X_i=0$, we flip another coin with bias $(b_2-b_1)/(1-b_1)$, and let $Y_i$ be the output of this coin. Repeat the process independently for each $i$, such that the $Y_i$'s are all independent of each other. Then $\probof{Y_i=1} = b_1 +(1-b_1) (b_2-b_1)/(1-b_1) = b_2$, and $\Yon$ is distributed according to $\q$.
\end{example}

We would like to use coupling to prove lower bounds on differentially private algorithms for testing problems. Let $\p$ and $\q$ be distributions over $\cX^\ns$. If there is a coupling between $\p$ and $\q$ with a small \emph{expected} Hamming distance, we might expect that the algorithm cannot have strong privacy guarantees. The following theorem formalizes this intuition:

Our lower bound is based on the following theorem, 

\begin{theorem}
\label{thm:coupling}
Suppose there is a coupling between $\p$ and $\q$ over $\cX^\ns$, such that $\expectation{\ham{\Xon}{\Yon}} \le D$ where $\Xon \sim p, \Yon \sim q$. Then, any $(\eps,\delta)$-differentially private \newhz{hypothesis testing} algorithm $\cA:\cX^\ns\to\{\p,\q\}$ on $\p$ and $\q$
%with $\probof{\alg\Paren{\Xon}=\q}<0.1$ and $\probof{\alg\Paren{\Yon}=\p}<0.1$
must satisfy $\eps+\delta = \Omega\Paren{\frac1{D}}$ .%.\todo{J: The statement is correct, but is it too DENSE?}
\end{theorem}
\begin{proof}
%\vspace{-5pt}
%Let $\cA:\cX^\ns\to\{\p,\q\}$ be an $(\eps,\delta)$-DP algorithm with error probability at most 0.1. 
Let $(\Xon, \Yon)$ be distributed according to a coupling of $\p$, and $\q$ with $\expectation{\ham{\Xon}{\Yon}} \le D$. 
By Markov's inequality, 
$\probof{\ham{\Xon}{\Yon}>10D}<\probof{\ham{\Xon}{\Yon}>10\cdot\expectation{\ham{\Xon}{\Yon}}}<0.1$.
Let $\xon$ and $\yon$ be the realization of $\Xon$ and $\Yon$. 
% We use $W$ to denote the set where the hamming distance between $\xon$ and $\yon$ is less than $10D$. 
\newhz{Let $W = \{ (\xon,\yon) | \ham{\xon}{\yon} \le 10D \}$. }Then we have 
\begin{center}
	 $0.1 \ge\probof{\alg\Paren{\Xon}=\q} \ge  \sum_{(\xon,\yon)\in W} \probof{\Xon = \xon, \Yon = \yon} \cdot \probof{\alg\Paren{\xon}=\q}$.
	 %= & \sum_{\xon,\yon} \probof{\Xon = \xon, \Yon = \yon} \cdot \probof{\alg\Paren{\xon}=\q} \nonumber\\
\end{center}

% \newhz{Next, we need the group property of $(\eps,\delta)$-differentially privacy. We give a proof of the following lemma in Appendix~\ref{app:group}.}
% \begin{lemma} \label{lem:group}
% 	Let $\alg$ be a $(\eps,\delta)$-DP algorithm, then for sequences $\xon$, and $\yon$ with $\ham{\xon}{\yon} \le t$, and $\forall S$, 
% $		\probof{\cA(\xon)\in S}\le e^{t\eps}\cdot\probof{\cA(\yon)\in S}+ \delta t e^{\eps (t-1)}$. 
% \end{lemma}
\noindent By Lemma~\ref{lem:group}, and $\probof{\ham{\Xon}{\Yon}>10D}<0.1$, and $\probof{\alg\Paren{\yon}=\q}\le 1$,

\begin{align}
	\probof{\alg\Paren{\Yon}=\q} & \leq  
	\sum_{(\xon,\yon)\in W} \probof{\xon,\yon}  \cdot \probof{\alg\Paren{\yon}=\q}+ 
	 %\sum_{(\xon,\yon)\notin W} \probof{\xon,\yon} \cdot \probof{\alg\Paren{\yon}=\q} \nonumber \\
	 \sum_{(\xon,\yon)\notin W} \probof{\xon,\yon} \cdot 1 \nonumber \\
	 & \leq  \sum_{(\xon,\yon)\in W} \probof{\xon,\yon}  \cdot ( e^{\eps \cdot 10D} \probof{\alg\Paren{\xon}=\q} + 10 D\delta \cdot e^{\eps \cdot 10(D-1)}) +0.1	 \nonumber \\
	 & \leq  0.1 e^{\eps\cdot 10 D} +  10 D\delta \cdot e^{\eps \cdot 10D} + 0.1. \nonumber
\end{align}
Since we know $\probof{\alg\Paren{\Yon}=\q} > 0.9$, then
$0.9 < \probof{\alg\Paren{\Yon}=\q} < 0.1 e^{\eps\cdot 10 D} +  10 D\delta \cdot e^{\eps \cdot 10D} +0.1 \nonumber$.
Hence, either $e^{\eps\cdot 10 D} = \Omega(1)$ or $10 D \delta = \Omega(1)$, which implies that 
$D = \Omega\Paren{\min \left\{\frac1\eps, \frac1\delta \right\}} = \Omega\Paren{\frac1{\eps + \delta}},$
proving the theorem.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent Set $\delta=0$, we obtain the bound for pure differential privacy. In the next few sections, we use this theorem to get sample complexity bounds for differentially private testing problems.



==> toolbox/abstract.tex <==
Le Cam's method, Fano's inequality, and Assouad's lemma are three widely used techniques to prove lower bounds for statistical estimation tasks. We propose their analogues under central differential privacy. Our results are simple, easy to apply and we use them to establish sample complexity bounds in several estimation tasks. 

\noindent{We establish the optimal sample complexity of discrete distribution estimation under total variation distance and $\ell_2$ distance. We also provide lower bounds for several other distribution classes, including product distributions and Gaussian mixtures that are tight up to logarithmic factors. The technical component of our paper relates coupling between distributions to the sample complexity of estimation under differential privacy. 
}
%\anote{Perhaps add more in terms of upper bounds and some applications in the abstract?}
%Learning distributions from samples is a fundamental statistical learning task. When the samples are collected from users, how to protect each user's privacy has garnered wide interest in the recent years. We study the problem of learning $\ab$-ary discrete distributions under differential privacy. We show that the sample complexity of learning a distribution up to TV distance $\alpha$ ($\ell_2$ distance $\beta$) under $\eps$ pure differential privacy is $\Theta(\frac{k}{\alpha^2} + \frac{k}{\alpha \eps})$ ($\tilde{\Theta}(\frac{1}{\beta^2} + \frac{\min \{\sqrt{k}, 1/\beta\}}{\beta\eps})$ ). %\todo{HZ: this is incorrect, even if we change max to min. We do not have tight bounds in l2 distance.}
%The upper bound is obtained by adding Laplace noise to the empirical estimator. For the lower bound part, we extend the classical Fano's inequality to the case with differential privacy constraint, which can be of independent interest. The technique also gives tight lower bounds for learning product distributions and Gaussian mixtures.

==> toolbox/applications.tex <==
\subsection{Applications}
\label{sec:applications}
We now describe several applications of the theorems above. 

\medskip
\noindent\textbf{Applications of Theorem~\ref{thm:le_cam}.} 
%A result similar to Theorem 1 was developed by~\cite{AcharyaSZ18} who used it to establish sample complexity of differentially private uniformity testing  of $k$-ary distributions under total variation distance~\cite{AcharyaSZ18, AliakbarpourDR18}. and for differentially private entropy and support size estimation~\cite{AcharyaKSZ18}.  
~\cite{AcharyaSZ18} developed a result similar to Theorem~\ref{thm:le_cam}, which is used to establish sample complexity lower bounds for differentially private uniformity testing under total variation distance~\cite{AcharyaSZ18, AliakbarpourDR18}, and for differentially private entropy and support size estimation~\cite{AcharyaKSZ18}. In this paper, we use Theorem~\ref{thm:le_cam} as a stepping stone to prove private Assouad's method (Theorem~\ref{thm:assouad}). 

\medskip
\noindent\textbf{Distribution Estimation and Applications of Theorem~\ref{thm:dp_fano} and~\ref{thm:assouad}.} {We will apply Theorem~\ref{thm:dp_fano} (private Fano's inequality) and Theorem~\ref{thm:assouad} (private Assouad's lemma) to some classic distribution estimation problems. The results are summarized in Table~\ref{tab:pure} and Table~\ref{tab:approx}. Before presenting the results, we describe the framework of minimax distribution estimation.}

\medskip
\noindent\textit{Distribution estimation framework.} Let $\cQ$ be a collection of distributions over $\cX$, and for this $\cQ$, let $\cP=\cQ^{\ns}:=\{q^\ns:q\in\cQ\}$ be the collection of $n$-fold distributions over $\cX^\ns$ induced by i.i.d. draws from a distribution over $\cQ$. The parameter space is $\Theta=\cQ$, where $\theta(\q^n)=\q$, and $\ell$ is a distance measure between distributions in $\cQ$. 
Let $\alpha>0$ be a fixed parameter. The sample complexity,  $S(\cQ, \ell, \alpha, \eps, \delta)$ is the smallest number of samples $n$ to make $R(\cQ^\ns, \ell, \eps, \delta)\le \alpha$, \ie
\[
S(\cQ, \ell, \alpha, \eps, \delta)= \min \{n: R(\cQ^\ns, \ell, \eps, \delta)\le \alpha\}.
\]
When $\delta = 0$, we denote the sample complexity by $S(\cQ, \ell, \alpha, \eps)$. We will state our results in terms of sample complexity. The following corollary of Theorem~\ref{thm:dp_fano} can be used to prove lower bounds on the sample complexity in this distribution estimation framework.  The detailed proof of the corollary is in Section~\ref{sec:coro_fano_proof}.

\begin{restatable}[$\eps$-DP distribution estimation]{coro2}{distest}
	\label{coro:fano}
	Given $\eps>0$, let $\cV=\{\q_1, \q_2,...,\q_M\} \subseteq \cQ$ be a set distributions over $\cX$ with size $M$, such that for all $i\ne j$, 	\begin{enumerate}[label=(\alph*)]
		\item $\ell \Paren{\q_i, \q_j} \ge 3 \tau$,
		\item $D_{KL} \Paren{\q_i,\q_j} \le \beta$,
		\item $d_{TV} \Paren{\q_i,\q_j} \le \gamma$,
	\end{enumerate}
	then
\[
		S(\cQ, \ell, \tau, \eps) = \Omega\Paren{\frac{\log M}{\beta}+ \frac{\log M}{\gamma \eps}}.
\]
\end{restatable}
\noindent\textbf{Remark.} With only conditions $(a)$ and $(b)$, we obtain 
the first term of the sample complexity lower bound which is the original 
Fano's bound for sample complexity. \newnewzs{By Pinsker's inequality, 
a bound on the KL divergence (Condition $(c)$) would imply a bound on TV 
distance (Condition $(b)$), i.e., $\gamma \le \sqrt{\beta/2}$. Hence 
Conditions $(a)$ and $(b)$ can also imply a lower bound on the sample 
complexity. We include all three conditions here since it is possible that in 
certain applications $\gamma \ll \sqrt{\beta/2}$, and hence a better bound 
can be obtained.}
\input{toolbox/table}
\medskip

\medskip
\noindent We now present examples of distribution classes we consider.

\medskip
\noindent\textit{$k$-ary discrete distribution estimation.} {Suppose $\cX=[k]:=\{1, \ldots, \ab\}$, and $\cQ:=\Delta_k$ is the simplex of $k$-ary distributions over $[k]$.  We consider estimation in both total variation and $\ell_2$ distance.} 

\medskip
\noindent\textit{$(k,d)$-product distributions.} Consider $\cX=[k]^d$, and let $\cQ:=\Delta_k^d$ be the set of product distributions over $[k]^d$, where the marginal distribution on each coordinate is over $[k]$ and independent of the other coordinates. We study estimation under total variation distance. A special case of this is Bernoulli product distributions ($k=2$), where each of the $d$ coordinates is an independent Bernoulli random variable.  

\medskip
\noindent\textit{$d$-dimensional Gaussian mixtures.} Suppose $\cX=\RR^{\dims}$, and $\cG_{\dims} := \{ \cN (\mu, I_d): \norm{\mu}\le R\}$ is the set of all Gaussian distributions in $\RR^d$ with bounded mean and identity covariance matrix. The bounded mean assumption is unavoidable, since by~\cite{BunKSW2019}, it is not possible to learn a single Gaussian distribution under pure DP without this assumption. {We consider 
\[
\cQ = \cG_{\ab, \dims} :=\left\{\sum_{j=1}^{\ab} w_j \p_j: \forall j \in [k], w_j \ge 0, \p_j\in\cG_\dims, w_1+\ldots+w_k =1\right\},
\] the collection of mixtures of $k$ distributions from $\cG_\dims$.} 

\medskip
\noindent\textbf{Applications of Theorem~\ref{thm:dp_fano}.}
We apply Corollary~\ref{coro:fano} and obtain sample complexity lower bounds for the tasks mentioned above under pure  differential privacy.

\medskip
{\noindent\textit{$\ab$-ary distribution estimation.} Without privacy constraints, the sample complexity of $\ab$-ary discrete distributions under total variation, and $\ell_2$ distance is $\Theta(k/\alpha^2)$ and $\Theta(1/\alpha^2)$ respectively, achieved by the empirical estimator. Under $\eps$-DP constraint, an upper bound of $O \Paren{\ab/\alpha^2+\ab/\alpha\eps}$
%$O \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha\eps}}$
samples for total variation distance is known using Laplace 
mechanism~\cite{DworkMNS06} (e.g.~\cite{DiakonikolasHS15}). In 
Theorem~\ref{thm:pure-dv}, we establish the sample complexity of this 
problem by providing a lower bound that matches this upper 
bound. \newnewzs{The bound shows that when $\eps \ll \alpha$, the cost 
due 
to privacy dominates the statistical error and when $\eps \ge \alpha$, the 
privacy cost is almost negligible. The same break point (up to logarithmic 
factors) has also been observed for product distributions and mixtures of 
Gaussian distributions, as listed below.}} 

Under $\ell_2$ distance, in Theorem~\ref{thm:pure-l2} we design estimators and establish their optimality whenever $\dist< \ab^{-1/2}$ or $\dist \ge \ab^{-0.499}$, which contains almost all the parameter range. Note that under $\ell_2$ distance, estimation without privacy has sample complexity independent of $k$, whereas {an unavoidable} logarithmic dependence on $\ab$ is introduced due to privacy requirements. The results are presented in Section~\ref{sec:pdp_kary}. 
 
\medskip
\noindent\textit{$(\ab,\dims)$-product distribution estimation.} For $(\ab,\dims)$-product distribution estimation under $\eps$-DP,~\cite{BunKSW2019} proposed an algorithm that uses
%$O\Paren{\ab\dims \log \Paren{ \frac{\ab\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$ 
$O\Paren{\ab\dims \log \Paren{ \ab\dims/\dist} \Paren{1/\dist^2+1/\dist\eps}}$ samples. 
%For the lower bound, they argue that given the existence of an $\dist$-packing set of size M, there exists a lower bound of $\Omega\Paren{\frac{M}{\eps}}$.\amargin{I dont understand the previous sentence about packing. Could we clarify a bit?} However, no packing set is explicitly constructed in the paper. 
In this paper, we present a lower bound of $\Omega\Paren{{\ab\dims}/{\dist^2}+{\ab\dims}/{\dist\eps}}$, which matches their upper bound up to logarithmic factors. For Bernoulli product distributions, \cite{KamathLSU18} proved a lower bound of $\Omega\Paren{{d}/{\alpha \eps}}$ under $(\eps,{3}/{64\ns})$-DP, which is naturally a lower bound for pure DP. %Their proof is based on fingerprinting lemma~\cite{SteinkeU15}, \newhz{ which is defined for Boolean hypercube. It remains unclear whether the proof can be extended to $k$-ary product distributions.}  
The details are presented in Section~\ref{sec:product}.

\medskip
\noindent\textit{Estimating Gaussian mixtures.}{~\cite{BunKSW2019} provided an upper bound of $\widetilde{O}\Paren{{\ab\dims}/{\dist^2}+{\ab\dims}/{\dist\eps}}$ samples.} Without privacy, a tight bounds of $\Omega({\ab\dims}/{\alpha^2})$ was shown in~\cite{SureshOAJ14, DaskalakisK14, AshtianiBHLMP18}. {In this paper, we prove a lower bound of $\Omega\Paren{{\ab\dims}/{\dist^2}+{\ab\dims}/{\dist\eps}}$, which matches the upper bound up to logarithmic factors.} \newzs{For the special case of estimating a single Gaussian ($k=1$), a lower bound of $\ns = {\Omega}\Paren{{\dims}/{(\alpha\eps\log \dims)}}$ was given in~\cite{KamathLSU18} for $(\eps,{3}/{64\ns})$-DP, which implies a lower bound that is $\log d$ factor weaker than our result under pure DP.}
	%Our lower bound for $k = 1$ improves their result under pure DP.} The details are given in Section~\ref{sec:gaussian}.

%\newhzn{
%\noindent\textbf{Remark.} Using the classic packing lower bound instead of Corollary~\ref{coro:fano} leads to loose lower bounds for these estimation problems. For example, in the $\ab$-ary distribution estimation problem, the packing lemma can only give a lower bound of $\ns = \Omega\Paren{\frac{\ab \log \Paren{1/\dist}}{\eps}}$ instead of the optimal $\ns = \Omega\Paren{\frac{\ab}{\dist \eps}}$ lower bound, where there exists an exponential gap in the parameter $\frac1\dist$. This is non-trivial when $\dist$ is small, e.g., $\dist = \frac1{\ab}$.}

\medskip
\noindent\textbf{Applications of Theorem~\ref{thm:assouad}.} As remarked earlier, Theorem~\ref{thm:dp_fano} only works for pure DP (or approximate DP with very small $\delta$). 
%However, it was easy to use as Corollary~\ref{coro:fano}. 
Assouad's lemma can be used to obtain lower bounds for distribution estimation under $(\eps,\delta)$-DP. For $k$-ary distribution estimation under $TV$ distance, we get a lower bound of $\Omega\Paren{{k}/{\alpha^2} + {k}/{\alpha(\eps + \delta)}}$. This shows that even up to $\delta=O(\eps)$, the sample complexity for $(\eps,\delta)$-DP is the same as that under $\eps$-DP.

\newzs{For Bernoulli ($k = 2$) product distributions, \cite{KamathLSU18} provides an efficient $(\eps, \delta)$-DP algorithm that achieves an upper bound of $O\Paren{\dims \log \Paren{ \dims/\dist} \Paren{1/\dist^2+1/\dist\eps}}$.\footnote{\newzs{The algorithm in~\cite{BunKSW2019} works for $\eps$-DP and general $k$ but it is not computationally efficient.}}} The lower bound $\Omega ({d}/{\alpha^2} + {d}/{\alpha \eps})$ obtained in~\cite{KamathLSU18} by fingerprinting holds for small values of $\delta = O(1/\ns)$. Note by the definition of DP~\eqref{eqn:dp-definition}, if $\delta>1/\ns$, a DP algorithm can blatantly disregard the privacy of $\delta\ns$ users. Therefore in most of the literature, $\delta$ is assumed to be $O(1/\ns)$. We want to make a complimentary remark that we
%\footnote{\newhzn{In fact, their lower bound only holds given the loss is in the form of expectation. When the loss is in the form of high probability, they derive a worse lower bound of $\Omega\Paren{\frac{d}{\dist\eps\log d}}$. However, our lower bound holds for both cases.}} \snote{I think we agreed on not putting this footnote since it is not well justified in the current write up. Am I right?}
% We 
can obtain the same lower bound all the way up to $\delta = O(\eps)$. This shows that there is no gain even if we compromise the privacy of a $\delta$ fraction of users. Therefore, there is no incentive to do it. We describe the details about these applications in Section~\ref{sec:adp_applications}. 
%\newzs{
%Note that $\delta=O(1/n)$ is the interesting case for designing privacy-preserving schemes since otherwise one could blatantly disregard privacy of $\delta\ns$ users, which is a constant. However, our results improves our understanding of the estimation risk by showing that even with large $\delta$ (even as large as $\eps$), the same lower bounds hold as with $\delta =O(1/\ns)$ for various statistical estimation tasks. In other words, there is no utility gain by compromising the privacy of a fraction of users, and hence there is no incentive to do it.
%}
%For the results above, we note that while DP with $\delta>1/n$ is not really a privacy guarantee since the privacy of $\delta\ns$ users can be compromised. 
%\newhzn{
%Someone may argue that DP with $\delta>1/n$ is not really a privacy guarantee since the privacy of $\delta\ns$ users can be compromised.
%However, our results above show that the utility can not be improved even sacrificing the privacy of a constant fraction of the users. In other words there is no motivation for using large $\delta$ as opposed to $\delta=O(1/\ns)$. 
%}

==> toolbox/approx_dp_new2.tex <==
\section{$(\eps,\delta)$-DP distribution estimation} \label{sec:adp_applications}
{In the previous section we used Theorem~\ref{thm:dp_fano} to obtain sample complexity lower bounds for pure differential privacy. We will now use Theorem~\ref{thm:assouad} to prove sample complexity lower bounds under $(\eps, \delta)$-DP.}

\subsection{$\ab$-ary distribution estimation} \label{sec:adp_kary}
%In this section, we consider $\ab$-ary distribution estimation under $(\eps, \delta)$-DP.

%\approxdtv*

\begin{theorem}
\label{thm:ApproximateDiscreteTotalVariation}
The sample complexity of $(\eps, \delta)$-DP $\ab$-ary distribution estimation under total variation distance is 
\[
S(\Delta_k,  d_{TV}, \alpha, \eps, \delta) =\Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha(\eps+\delta)}}.
\]
\end{theorem}
{In practice, $\delta$ is chosen to be $\delta = O\Paren{\frac1\ns}$, and the privacy parameter is chosen as a small constant, $\eps = \Theta(1)$. In particular, when $\delta\le \eps$, the theorem above shows
\[
S(\Delta_k,  d_{TV}, \alpha, \eps, \delta) =\Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}.
\]
Since the sample complexity of $\eps$-DP is at most the sample complexity of $(\eps,\delta)$-DP, this shows that the bound above is tight for {$ \delta\le \eps$}. The lower bound part is proved using Theorem~\ref{thm:assouad} in Section~\ref{sec:approximate-tv}.}

\begin{theorem}
\label{thm:ApproximateDiscreteL2}
The sample complexity of $(\eps, \delta)$-DP discrete distribution estimation under $\ell_2$ distance,
\[
 \Omega \Paren {\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha (\eps+\delta)}} \le S(\Delta_k, \ell_2, \alpha, \eps, \delta) \le O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{\ab}}{\alpha\eps}},\ \ \ \ \text{for $\dist < \frac1{\sqrt{\ab}}$},
\] 
\begin{align}
\Omega\Paren{\frac{1}{\dist^2}+\frac{1}{\dist^2(\eps+\delta)}}\le S(\Delta_k, \ell_2, \alpha, \eps, \delta)  \le O\Paren{\frac{1}{\dist^2}+\frac{\log\ab}{\dist^2\eps}}, \ \ \ \text{for $\dist > \frac1{\sqrt{\ab}}$}. \nonumber
\end{align}
\end{theorem}
%{When $\delta = O(\eps)$, by Theorem~\ref{thm:pure-l2}, the bounds are tight up to logarithmic factor. We prove this result in Section~\ref{sec:approximate-l2}.}
{When $\delta = O(\eps)$, the bounds are tight when $\dist < 1/\sqrt{\ab}$ and differ by a factor of $\log k$ when $\dist \ge 1/\sqrt{\ab}$. We prove this result in Section~\ref{sec:approximate-l2}.}

\subsubsection{Proof of Theorem~\ref{thm:ApproximateDiscreteTotalVariation}.}
\label{sec:approximate-tv}

{The first term $k/\alpha^2$ is the tight sample complexity without privacy. We prove that $S(\Delta_{\ab}, d_{TV}, \alpha, \eps, \delta) = \Omega \Paren{\frac{\ab}{\alpha(\eps+\delta)}}$.} 

{Suppose $k$ is even and $\dist < 1/10$. Let $ \cE_{k/2} =\{-1,+1\}^{k/2}$, for  $e \in \cE_{k/2}$, we define $\p_e\in\Delta_k$ as follows. 
\begin{align}
\text{For $i=1, \ldots, k/2$}~~~~ \p_e(2i-1) = \frac{1+ 10 e_i \cdot \alpha}{\ab},  ~~ \p_e(2i) = \frac{1- 10e_i  \cdot \dist}{\ab}. \label{eqn:constr-approx-k-ary}
\end{align}}
{To apply Theorem~\ref{thm:assouad}, let $\cV_{\ab/2} = \{ \p_e^n, e \in \cE_{\ab/2}\}$. $\p_e^n$ is the distribution of $n$ i.i.d. samples from distribution $\p_e$, and $\theta(\p_e^n) = \p_e$. For $u, v \in \cE_{\ab/2}$,
\[
\ell( \theta(\p_u^n),  \theta(\p_v^n)) = d_{TV} (p_{u},p_{v}) = \frac{20\dist}{\ab} \cdot \sum_{i=1}^{\frac{k}{2}}\mathbb{I}\Paren{u_i \neq v_i}, 
\]
thus obeying~\eqref{eqn:assouad-loss} with $\tau=10\dist/k$.}
%\amargin{is the inequality an equality above? \newhzz{HZ: Yes}}

%First, we prove that
%\[
%	R(n, \Delta_{\ab}, d_{TV}, \eps, \delta) \ge \frac{1}{2}\min_{\he: \he \text{ is  $(\eps, \delta)$-DP}} ~ \max_{ e \in \cE_{\ab/2} } \EE_{\Xon \sim  \p_e^n} \left[ d_{TV}(\p_{\he},\p_e )\right].
%\]
%
%Given $\Xon$ generated from unknown $\p_e^{\ns} \in \cV_{\ab/2}$, for any distribution estimator $\hat p: \Xon \rightarrow \Delta_{\ab}$, we define $\he \in \{\pm1\}^{k/2}$ as follows:
%$$ \he(i)  = \left\{
%\begin{array}{rcl}
%1 ,       &      & when ~ \hat p (2i-1) \ge \hat p (2i),\\
%-1,       &      & when ~ \hat p (2i-1) < \hat p (2i).
%\end{array} \right. $$
%
%% We note that, given $\Xon$ generated from unknown $\p_e \in \cV_{\ab/2}$, it is enough if we can construct an index estimator $\hat e: \Xon \rightarrow  \{\pm1\}^{k/2}$ according to a feasible distribution estimator $\hat p: \Xon \rightarrow \Delta_{\ab}$ and we show that they have ``similar' performance. We define $\hat {e} \in \{\pm1\}^{k/2}$ as follows:
%%$$ \hat {e}(i)  = \left\{
%%\begin{array}{rcl}
%%1 ,       &      & when ~ \hat p (2i-1) \ge \hat p (2i),\\
%%-1,       &      & when ~ \hat p (2i-1) < \hat p (2i).
%%\end{array} \right. $$
%
%Since $\he$ is a post-processing of $\hat{p}$, so it also satisfies $(\eps,\delta)$-DP. Note that for any estimator $\hat {\p}$ and any distribution $\p_e$, if we have $\hat p (2i-1) < \hat p(2i) $ and $e(i)=1$. Then
%\[
%	\frac{1}{2} \Paren{ |\hat{\p}(2i -1) - \p_e(2i-1)| + |\hat{\p}(2i) - \p_e(2i)|} \ge \frac12|\p_e(2i-1) - \p_e(2i)| = \frac{10 \alpha}{k}.
%\]
%
%The same inequality holds if $\hat p (2i-1) \ge \hat p(2i) $ and $e(i)= -1$. For event $S$, let $\probofsub{e}{S}$ denote $\probofsub{\Xon \sim \p_e^{\ns}}{S}$. Hence for any $e \in \{\pm1\}^{k/2}$, we have
%\begin{align}
%          \expectationsub{\p_{e}}{d_{TV}(\hat p, \p_{e})} & = \frac{1}{2}\sum_{i = 1}^{k/2} \expectationsub{\p_{e}}{ |\hat{\p}(2i -1) - \p_e(2i-1)| + |\hat{\p}(2i) - \p_e(2i)|} \nonumber \\
%          %& \ge  \frac{10\alpha}{k} \sum_{i=1}^{k/2} \Big[ \mathbb{I} (e(i)=1) \cdot \probofsub{e}{\hat p (2i-1) < \hat p(2i) } 
%          %+  \mathbb{I} (e(i)  = -1) \cdot \probofsub{e}{\hat p (2i-1) >\hat p(2i) } \Big] \nonumber \\
%          &\ge  \frac{10\alpha}{k} \sum_{i=1}^{k/2} \Big[ \mathbb{I} (e(i)  =1 ) \cdot \probofsub{e}{\he(i)  =-1} 
%           +  \mathbb{I} ({e(i)}  = -1) \cdot \probofsub{e}{ \he_i =+1} \Big] \nonumber\\
%	 &= \frac1{2}\expectationsub{\p_{e}}{d_{TV}(\p_{\he},\p_{e})}.\nonumber
%\end{align}
%
%Hence we have:
%\begin{align}
%	R(n, \Delta_{\ab}, d_{TV}, \eps, \delta) & %= \min_{\hat p: \hat p \text{ is }(\eps,\delta)-DP} \max_{\p \in \cP} \EE_{\Xon \sim \p^n}\left[d_{TV}(\hat p(\Xon),\p)\right] \nonumber \\
%		 \ge  \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}} \max_{e \in \cE_{\ab/2} } \EE_{\Xon \sim \p_e^n} \left[d_{TV}(\hat p,\p_e)\right] \nonumber \\
%		& \ge \frac{1}{2} \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}}\max_{e \in \cE_{\ab/2}} \EE_{\Xon \sim \p^{\ns}_e} \left[d_{TV}(\p_{\he},\p_e)\right] \nonumber \\
%		& = \frac{1}{2} \min_{\he: \he \text{ is $(\eps,\delta)$-DP}} \max_{\p_e^{\ns} \in \cV_{\ab/2} } \EE_{\Xon \sim \p_e^{\ns}} \left[\ell(\p^{\ns}_{\he},\p_e^{\ns})\right]. \nonumber 
%\end{align}
%
%%Since $\sup_{\p_e \in \cV_{\ab} }\mathbb{E}_{\p_e} [d_{TV}(\hat{\p}, \p_e)]<  \sup_{\p \in \Delta_{\ab} }\mathbb{E}_{\p} [d_{TV}(\hat{\p}, \p)] \le \dist$, we have $R(n,  \cV_{\ab/2}, \ell, \eps, \delta) \le 2\dist$. By Theorem~\ref{thm:assouad}, we have
%%$$\sum_{i=1}^{\frac{\ab}{2}} \probofsub{+i }{ \hat {E}(i) \neq 1 } + \probofsub{-i }{\hat {E}(i) \neq -1 } \leq \frac{k}{5},$$
%%where
%%\[
%%\probofsub{+i }{S} = \probof{S | e(i) = +1} =   \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= + 1}\probof{S| E= e},
%%\]
%%\[
%%\probofsub{-i }{ S } =\probof{S | e(i) = -1} =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= - 1}\probof{S | E= e} .
%%\]
{Recall the mixture distributions $\p_{+i}$ and $\p_{-i}$,} 
\[
\dP_{+i}  =  \frac{2}{|\cE_{\ab/2}|} \sum_{e \in \cE_{\ab/2}: e_i= + 1} \p^{\ns}_e, ~~~ \dP_{-i}  =  \frac{2}{|\cE_{\ab/2}|} \sum_{e \in \cE_{\ab/2}: e_i= -1}\p^{\ns}_e.
\]
{To apply Theorem~\ref{thm:assouad}, we prove the following bound on the Hamming distance between a coupling between $\p_{+i}$ and $\p_{-i}$.
\begin{lemma} \label{lem:coupling_distance}
For any $i$, there is a coupling $(X,Y)$ between $\dP_{+i}$ and $\dP_{-i}$, such that
\[
\expectation{\ham{X}{Y}} \le \frac{20\dist \ns}{\ab}.
\]
\end{lemma}}
\begin{proof}
{By the construction in~\eqref{eqn:constr-approx-k-ary}, note that the distributions $\dP_{+i}$ and $\dP_{-i}$ only have a difference in the number of times $2i-1$ and $2i$ appear. To generate $Y\sim \p_{-i}$ from from $X\sim\p_{+i}$, we scan through $X$ and independently change the coordinates that have the symbol $2i-1$ to the symbol $2i$ with probability $\frac{20\alpha}{1+10\alpha}$. The expected Hamming distance is bounded by $\frac{20\alpha}{1+10\alpha} \cdot \frac{1+10\alpha}{\ab} \cdot \ns = \frac{20\alpha \ns}{\ab}$.}
\end{proof}

Note that $\cV\subset\cP := \{\p^n | \p \in \Delta_k \}$. By Theorem~\ref{thm:assouad}, using the bound on $D$ from Lemma~\ref{lem:coupling_distance}, and $\tau=10\dist/k$,
\[
R(\cP, d_{TV}, \eps, \delta) \ge \frac{5\alpha}{\ab} \cdot \ab \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}\ge  {5\alpha} \cdot \Paren{0.9 e^{-200 n\eps\alpha/k} - 200 \frac{n\eps\alpha\delta}k}.
\]
{To achieve $R(\cP, d_{TV}, \eps, \delta) \le \alpha$, either $n\eps\alpha/k=\Omega(1)$ or ${n\eps\alpha\delta}/k=\Omega(1)$, which implies that $n=\Omega( \frac{k}{\alpha(\eps+\delta)})$}.
%\amargin{Please check the constants above.}

\subsubsection{Proof of Theorem~\ref{thm:ApproximateDiscreteL2}} \label{sec:approximate-l2}

We first consider the case where $\dist < \frac1{\sqrt{\ab}}$.  By Cauchy-Schwarz inequality, $S(\Delta_k, \ell_2, \alpha, \eps, \delta) \ge S(\Delta_k,  d_{TV}, \sqrt{k}\alpha, \eps, \delta) $, and therefore $S(\Delta_k, \ell_2, \alpha, \eps, \delta) = \Omega\Paren{\frac{1}{\dist^2}+\frac{\sqrt{\ab}}{\dist (\eps+\delta)}}$ by Theorem~\ref{thm:ApproximateDiscreteTotalVariation}.

For $\alpha \ge \frac{1}{\sqrt{k}}$, we have $l = \lfloor \frac1{16\dist^2}\rfloor \le k$. Therefore, $\Delta_l \subset \Delta_k$ and $\dist < \frac1{\sqrt{l}}$. Hence,
\[
	S(\Delta_k, \ell_2, \alpha, \eps, \delta) \ge S(\Delta_l, \ell_2, \alpha, \eps, \delta) = \Omega\Paren{\frac{1}{\alpha^2} + \frac1{\dist^2(\eps+\delta)}}.
\]


==> toolbox/approx_dp_product.tex <==
\subsection{Binary product distribution estimation} 
\label{sec:adp_product}

{We now consider estimation of Bernoulli product distributions under total variation distance. A Bernoulli product distribution in $d$ dimensions is a distribution over $\{0,1\}^\dims$ parameterized by $\mu\in [0,1]^\dims$, where the $i$th coordinate is distributed $\ber(\mu_i)$, where $\ber(\cdot)$ is a Bernoulli distribution. Let $\Delta_{2,\dims}$ be the class of Bernoulli product distributions in $\dims$ dimensions.} 

\begin{theorem}
\label{thm:ApproximateProductTotalVariation}
The sample complexity of $(\eps, \delta)$-DP  binary product  distribution estimation satisfies 
\[
S(\Delta_{2,\dims}, d_{TV}, \alpha, \eps, \delta)  =\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha(\eps+\delta)}}.
\]
%Further, when $\delta\le\eps$,
%\[
%S(\Delta_{2,\dims}, d_{TV}, \alpha, \eps, \delta)   =\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha\eps}}.
%\]
\end{theorem}

\newzs{Compared to the upper bound of $O\Paren{\dims \log \Paren{\dims/\dist} \Paren{1/\dist^2+1/\dist\eps}}$ in~\cite{BunKSW2019, KamathLSU18}, our bound is tight up to logarithmic factors when $\delta \le \eps$. \cite{KamathLSU18} also presents a lower bound of $\Omega \Paren{\frac{\dims}{\alpha^2}+\frac{\dims}{\alpha(\eps+\delta)}}$ under $(\eps, \delta)$-DP when $\delta = O(1/\ns)$. Although $\delta = O(1/\ns)$ is the more interesting regime in practice, our bound complements the result by stating that the utility will not improve even if $\delta$ can be as large as $\eps$.}
\begin{proof}	
{Since $\Theta(\dims/\eps^2)$ is an established tight bound for non-private estimation, we only prove the second term.}

{We start by constructing a set of Bernoulli product distributions indexed by $\cE_{\dims} = \{ \pm1\}^{\dims}$. For all $e \in \cE_{\dims}$, let $\p_e = \ber(\mu^e_1) \times \ber(\mu^e_2) \times \cdots \times \ber(\mu^e_\dims)$, where 
\[
\mu^e_i = \frac{1+ e_i\cdot 20\dist}{\dims}.
\]}
%\amargin{I am changing the definitions here, since we wrote $e_i$ to be in 0,1 earlier.}
{Let $\cV = \{ \p_e^{\ns}, e \in \cE_{\dims}\}$, the set of distributions of 
$n$ i.i.d samples from $\p_e$, and $\theta\Paren{\p_e^{\ns}} = \p_e$. For 
$u, v\in \cE_{\dims},$, 	$\ell( \theta(\p_u^n),  \theta(\p_v^n)) = d_{TV} 
(p_{u},p_{v})$. We first prove that~\eqref{eqn:assouad-loss} holds under 
total variation distance for an appropriate $\tau$.} 


%By Lemma 6.4 in~\cite{KamathLSU18}, 
%for any pair of distributions $\p_i, \p_j \in \cV_{\dims}$, $C_1 \dist \le \dtv{\p_i}{\p_j} \le C_2\dist$, where $C_1$ and $C_2$ are some constants.

%We need the following lemma.
\begin{lemma}
\label{lem:binaryproducttv}
There exists a constant $C_1 > 5 $ such that $ \forall u, v \in \cE_{\dims}$,
\[ 
d_{TV} (\p_{u},\p_{v}) \ge \frac{C_1 \dist}{\dims}\cdot  \sum_{i=1}^{\dims}\mathbb{I}\Paren{u_i \neq v_i}.
\]
\end{lemma}

\begin{proof}
Let $S = \{i \in [\dims] : u_i \neq v_i\}$, and $S^{\prime} = \{i \in S : u_i = 1\} $. WLOG, let $\absv{S^{\prime}} \ge \frac12 \absv{S}$ (or else we can define $S^{\prime} = \{i \in S : u_i = -1\}$). Given a random sample $Z \in \{ \pm1\}^{\dims}$, we define an event $A = \{\forall i \in S^{\prime}, Z_i=0\}$. Now we consider the difference between the following two probabilities, which is a lower bound of the total variation distance between $\p_u$ and $\p_v$.
\begin{align}
d_{TV} (\p_{u},\p_{v}) &\ge \absv{\probofsub{Z \sim \p_{u}} {A} - \probofsub{Z \sim \p_{v}} {A}} \nonumber\\
&= \Paren{1-\frac{1-20\dist}{\dims}}^{\absv{S^{\prime}}} - \Paren{1-\frac{1+20\dist}{\dims}}^{\absv{S^{\prime}}} \nonumber\\
&\ge \frac{40\dist}{\dims} \cdot  \absv{S^{\prime}} \cdot  \Paren{1-\frac{1+20\dist}{\dims}}^{\absv{S^{\prime}}} \nonumber \\
& \ge \frac{40 \dist}{\dims} \cdot \absv{S'} e^{-(1+20\dist)} \ge \frac{C_1\dist}{\dims} \cdot \ham{u}{v}, \nonumber
\end{align}
where in the last two inequalities, we assume $\dims \ge 1000$ and $\dist<0.01$.
\end{proof} 

%First, we prove that
%\[
%	R(n, \cC_{\dims}, d_{TV}, \eps, \delta) \ge \frac{1}{2}\min_{\he: \he \text{ is  $(\eps, \delta)$-DP}} ~ \max_{ e \in \cE_{\dims} } \EE_{\Xon \sim  \p_e^n} \left[ d_{TV}(\p_{\he},\p_e )\right].
%\]
%
%Given $\Xon$ generated from unknown $\p_e^{\ns} \in \cV_{\dims}$, for any distribution estimator $\hat \p: \Xon \rightarrow \cC_{\dims}$, we define $\he \in \{\pm1\}^{\dims}$ as follows:
%$$ \he(i)  = \left\{
%\begin{array}{rcl}
%1 ,       &      & when ~ \hat \mu (i) \ge \frac1{\dims},\\
%-1,       &      & when ~ \hat \mu (i) < \frac1{\dims}.
%\end{array} \right. $$
%
%% We note that, given $\Xon$ generated from unknown $\p_e \in \cV_{\dims}$, it is enough if we can construct an index estimator $\hat e: \Xon \rightarrow  \{\pm1\}^{\dims}$ according to a feasible distribution estimator $\hat p: \Xon \rightarrow \cC_{\dims}$ and we show that they have ``similar' performance. We define $\hat {e} \in \{\pm1\}^{\dims}$ as follows:
%%$$ \hat {e}(i)  = \left\{
%%\begin{array}{rcl}
%%1 ,       &      & when ~ \hat p (2i-1) \ge \hat p (2i),\\
%%-1,       &      & when ~ \hat p (2i-1) < \hat p (2i).
%%\end{array} \right. $$
%
%Since $\he$ is a post-processing of $\hat{p}$, so it also satisfies $(\eps,\delta)$-DP. 
%%Note that for any estimator $\hat {\mu}$ and any distribution $\p_e$, if we have $\hat p (2i-1) < \hat p(2i) $ and $e(i)=1$. Then
%%\[
%%	\frac{1}{2} \Paren{ |\hat{\p}(2i -1) - \p_e(2i-1)| + |\hat{\p}(2i) - \p_e(2i)|} \ge \frac12|\p_e(2i-1) - \p_e(2i)| = \frac{10 \alpha}{k}.
%%\]
%%
%%The same inequality holds if $\hat p (2i-1) \ge \hat p(2i) $ and $e(i)= -1$.
% For event $S$, let $\probofsub{e}{S}$ denote $\probofsub{\Xon \sim \p_e^{\ns}}{S}$. Hence for any $e \in \{\pm1\}^{\dims}$, we have
%\begin{align}
%          \expectationsub{\p_{e}}{d_{TV}(\hat p, \p_{e})} & \ge C_1 \sum_{i = 1}^{\dims} \expectationsub{\p_{e}}{ |\hat{\mu}(i) - \mu_e(i)|} \nonumber \\
%          %& \ge  \frac{10\alpha}{k} \sum_{i=1}^{\dims} \Big[ \mathbb{I} (e(i)=1) \cdot \probofsub{e}{\hat p (2i-1) < \hat p(2i) } 
%          %+  \mathbb{I} (e(i)  = -1) \cdot \probofsub{e}{\hat p (2i-1) >\hat p(2i) } \Big] \nonumber \\
%          &\ge  \frac{C_1\alpha}{\dims} \sum_{i=1}^{\dims} \Big[ \mathbb{I} (e(i)  =1 ) \cdot \probofsub{e}{\he(i)  =-1} 
%           +  \mathbb{I} ({e(i)}  = -1) \cdot \probofsub{e}{ \he_i =+1} \Big] \nonumber\\
%	 &\ge \frac{C_1}{C_2}\expectationsub{\p_{e}}{d_{TV}(\p_{\he},\p_{e})}.\nonumber
%\end{align}
%
%Hence we have:
%\begin{align}
%	R(n, \cC_{\dims}, d_{TV}, \eps, \delta) & %= \min_{\hat p: \hat p \text{ is }(\eps,\delta)-DP} \max_{\p \in \cP} \EE_{\Xon \sim \p^n}\left[d_{TV}(\hat p(\Xon),\p)\right] \nonumber \\
%		 \ge  \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}} \max_{e \in \cE_{\dims} } \EE_{\Xon \sim \p_e^n} \left[d_{TV}(\hat p,\p_e)\right] \nonumber \\
%		& \ge\frac{C_1}{C_2} \min_{\hat p: \hat p \text{ is $(\eps,\delta)$-DP}}\max_{e \in \cE_{\dims}} \EE_{\Xon \sim \p^{\ns}_e} \left[d_{TV}(\p_{\he},\p_e)\right] \nonumber \\
%		& =\frac{C_1}{C_2} \min_{\he: \he \text{ is $(\eps,\delta)$-DP}} \max_{\p_e^{\ns} \in \cV_{\dims} } \EE_{\Xon \sim \p_e^{\ns}} \left[\ell(\p^{\ns}_{\he},\p_e^{\ns})\right]. \nonumber 
%\end{align}

%Since $\sup_{\p_e \in \cV_{\ab} }\mathbb{E}_{\p_e} [d_{TV}(\hat{\p}, \p_e)]<  \sup_{\p \in \cC_{\dims} }\mathbb{E}_{\p} [d_{TV}(\hat{\p}, \p)] \le \dist$, we have $R(n,  \cV_{\dims}, \ell, \eps, \delta) \le 2\dist$. By Theorem~\ref{thm:assouad}, we have
%$$\sum_{i=1}^{\frac{\ab}{2}} \probofsub{+i }{ \hat {E}(i) \neq 1 } + \probofsub{-i }{\hat {E}(i) \neq -1 } \leq \frac{k}{5},$$
%where
%\[
%\probofsub{+i }{S} = \probof{S | e(i) = +1} =   \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= + 1}\probof{S| E= e},
%\]
%\[
%\probofsub{-i }{ S } =\probof{S | e(i) = -1} =  \frac{2}{|\cE_{k}|} \sum_{e \in \cE_{k}: e(i)= - 1}\probof{S | E= e} .
%\]
%Recall the definition of the two mixtures of distributions: \amargin{We just recalled this two pages ago. How many times should we recall?}
%$$
%\dP_{+i}  =  \frac{2}{|\cE_{\dims}|} \sum_{e \in \cE_{\dims}: e(i)= + 1} \p^{\ns}_e, ~~~ \dP_{-i}  =  \frac{2}{|\cE_{\dims}|} \sum_{e \in \cE_{\dims}: e(i)= -1}\p^{\ns}_e.
%$$
{Let $D$ be an upper bound on the expected Hamming distance for a coupling between $\dP_{+i}$ and $\dP_{-i}$ over all $i$.  Since $\cV_{\dims} \subset \Delta_{2,\dims}$, applying Theorem~\ref{thm:assouad} with Lemma~\ref{lem:binaryproducttv} we have
\[
R(\cP, d_{TV}, \eps, \delta) \ge \frac{C_1\alpha}{2\dims} \cdot \dims \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta} = \frac{C_1\alpha}{2} \cdot \Paren{0.9 e^{-10 \eps D} - 10 D \delta}. 
\]}

{Setting $R(\cP, d_{TV}, \eps, \delta) \le \alpha$, we get $D =\Omega\Paren{\frac1\eps}$ or $D =\Omega\Paren{\frac1\delta}$, or equivalently, $D =\Omega\Paren{\frac1{\eps+\delta}}$. Lemma~\ref{lem:coupling_distance} below shows that we can take $ D =\frac{40\dist\ns}{\dims}$, which proves the result.}
\end{proof}

\begin{lemma} \label{lem:coupling_distance}
There is a coupling between $(X,Y)$ between $\dP_{+i}$ and $\dP_{-i}$, such that
$\expectation{\ham{X}{Y}} \le \frac{40\dist \ns}{\dims}.$
\end{lemma}

\begin{proof}
We generate $Y\sim \dP_{-i}$ from $X\sim\dP_{+i}$ as follows. If the $i$th coordinate of a sample $X$ is $+1$, we independently flip it to $-1$ with probability  $\frac{40\alpha}{1+20\alpha}$ to obtain a sample $Y$. The expected Hamming distance is bounded by $\frac{40\alpha}{1+20\alpha} \cdot \frac{1+20\alpha}{\dims} \cdot \ns = \frac{40\alpha \ns}{\dims}$. 
\end{proof}



==> toolbox/coding-proofs.tex <==
\section{Proofs of existence of codes (Lemma~\ref{lem:GV} and Lemma~\ref{lem:constantGV2})}
\label{sec:codes}
%\amargin{This entire section is new, please read it thoroughly. I have changed the equations in Lemma~\ref{lem:GV}!}

\begin{proof}[Proof of Lemma~\ref{lem:GV}]
{This proof is a standard argument for Gilbert-Varshamov bound applied to constant weight codes. We use the following version (Theorem 7 in~\cite{GrahamS80}).}
\begin{lemma}
\label{lem:constantGV}
{There exists a length-$k$ constant weight binary code $\cC$ with weight $l$ and minimum Hamming distance $2\delta$, with $$\absv{\cC} \ge \frac{\binom{\ab}{l}}{\sum_{i=0}^{\delta} \binom{l}{i} \binom{\ab-l}{i}}.$$}
\end{lemma}
Applying this Lemma with $2\delta=\frac{l}{4}$, we have
\begin{align}
\absv{\cC} &\ge \frac{\binom{\ab}{l}} {\sum_{j=0}^{l/8} \binom{l}{j} \cdot \binom{\ab-l}{j}}\nonumber  \ge \frac{\binom{\ab}{l}}{\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} \cdot \binom{\ab}{\frac{l}{8}}}
  = \frac1 {\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} } \cdot \prod_{i = 0}^{\frac{7l}{8}- 1} \frac{k - \frac{l}{8}-i}{l - i} \\
& \ge \frac{2\sqrt{7} \pi}{e} \cdot (0.59)^{\frac{7l}{8}} \cdot \Paren{ \frac{\ab-\frac{l}{8}}{l}}^{\frac{7l}{8}} \label{eqn:gv-step}\\
 &\ge \Paren{\frac{\ab}{2^{7/8}l}}^{\frac{7l}{8}}, \nonumber 
\end{align}
{In~\eqref{eqn:gv-step}, we note that $\frac{k - \frac{l}{8}-i}{l - i}$ is monotonically increasing as $i$ increases.} And the first part is obtained by the Stirling's approximation $\sqrt{2\pi}\cdot l^{l+\frac12} \cdot e^{-l} \le l! \le e \cdot l^{l+\frac12} \cdot e^{-l}$ and the fact that $1.1^l \ge \sqrt{l}$ when $l \ge 20$. The last inequality comes from $l \le k/2$ and $15/16 \times 0.59 > 1/2^{7/8}$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:constantGV2}]
By the Gilbert-Varshamov bound (Lemma~\ref{lem:constantGV}),
\[
	\absv{\cH} \ge \frac{h^\dims}{\sum_{j=0}^{\frac{d}{2}-1} \binom{\dims}{j}(h-1)^j} \ge \frac{h^\dims}{\frac{\dims}{2} \cdot \binom{\dims}{\frac{\dims}{2}} \cdot h^{\frac{\dims}{2}}} \ge
	\frac{h^{\frac{\dims}{2}}} { \dims \cdot 2^{\dims} }  \ge \left(\frac{h}{16}\right)^{\frac{\dims}{2}}.
\]
\end{proof}

==> toolbox/gaussian.tex <==
\subsection{Gaussian mixtures 	estimation} \label{sec:gaussian}

%In this section, we show that our private Fano's inequality can be applied to derive the sample complexity lower bound of learning mixtures of distributions.   

%\begin{definition}
%	Let $\cG$ be some set of distributions. A $\ab$-mixture of $\cG$ is a distribution with density $\sum_{j=1}^{\ab} w_j \p_j$, where each $\p_j \in \cG$ and $\sum_{j=1}^{\ab} w_j =1$.
%\end{definition}

Recall $\cG_{\dims} = \{ \cN (\mu, I_d): \norm{\mu}\le R\}$ is the set of $\dims$-dimensional spherical Gaussians with unit variance and bounded mean and $\cG_{\ab,\dims} = \{ \p: \p \text{ is a $\ab$-mixture of } \cG_{\dims} \}$ consists of mixtures of $k$ distributions in $\cG_{\dims}$.~\cite{BunKSW2019} proves an upper bound of $\widetilde{O}\Paren{\frac{\ab\dims}{\dist^2}+\frac{\dims}{\dist\eps}}$ for estimating $k$-mixtures of Gaussians. We provide a sample complexity lower bound for estimating mixtures of Gaussians in Theorem~\ref{thm:main_Gaussian}, which matches the upper bound up to logarithmic factors. 

\begin{theorem}
\label{thm:main_Gaussian}
Given $\ab \le \dims$ and $R\ge \sqrt{64\log\Paren{\frac{8\ab}{\dist}}}$, {or $\ab \ge \dims$ and $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$,}
\begin{align}
&S(\cG_{\ab, \dims}, d_{TV}, \alpha, \eps) = \Omega \Paren{\frac{\ab\dims}{\dist^2}+\frac{\ab\dims}{\dist \eps}}. \nonumber
\end{align}
\end{theorem}

\begin{proof}
	
{We first consider the case when $\ab \le \dims$ and $R\ge \sqrt{64\log\Paren{\frac{8\ab}{\dist}}}$.} Let $\cC$ denote the codebook in Lemma~\ref{lem:GV} with weight $l=\frac{\dims}{2}$. Then we have $|\cC| \ge 2^{\frac{7\ab}{128}}$. Given $c_i$ in codebook $\cC$, we construct the following $\dims$-dimensional Gaussian distribution $\p_i$, with identity covariance matrix and mean $\mu_i$ satisfying %\amargin{This looks like the third time ... but this is ok this time I think}
%\[\mu_{i} (j)  = \left\{
%\begin{array}{rcl}
%+ \frac{\dist}{\sqrt{ \dims}} ,       &      & \text{for ~ } c_i (j)=1,\\
%- \frac{\dist}{\sqrt{\dims}},       &      & \text{for ~ } c_i (j)=0.
%\end{array} \right.
%\]

\[\mu_{i,j}  = \frac{\dist}{\sqrt{ \dims}} c_{i,j},\]
{ where   $\mu_{i,j}$ denotes the $j$-th coordinate of $\mu_i$.}

{Let $h = \absv{\cC}$. Similar to the product distribution case, using Lemma~\ref{lem:constantGV2}, we can get an $h$-ary codebook $\cH$ with length $d$ and minimum hamming distance $d/2$. Moreover, $|\cH| \ge (\frac{h}{16})^{\frac{\dims}{2}}$. }


$\forall i \in [h]$ and $j \in k$, define $\p_{i}^{(j)} = \cN(\mu_i + \frac{R}{2}e_j , I_d)$, where $e_j$ is the $j$th standard basis vector. It is easy to verify their means satisfy the norm bound. %By Claim~\ref{claim:constantGV2}, there exists an $h$-ary code $\cH \subset [h]^\ab$ with code length $\ab$ and minimum Hamming distance $\frac{\ab}{2}$, which satisfies $\absv{\cH} \ge (\frac{h}{16})^{\frac{\ab}{2}}$. 
For a codeword $b \in \cH$, let
\[
	\mP_b = \frac1k \Paren{ \p_{b_1}^{(1)} +  \p_{b_2}^{(2)}  +\ldots + \p_{b_k}^{(k)} }.
\]

Let $\cV_{\cG} = \{ \mP_b: b \in \cH\}$ be the set of the distributions defined above. Next we prove that $\forall \mP_b \neq \mP_{b'}\in \cV_{\cG}$, 
\begin{align}
	\dtv{\mP_b}{\mP_{b'}} \ge C \alpha, \label{eqn:dtv_gaussian} \\
	\dkl{\mP_b}{\mP_{b'}} \le 4 \alpha^2.\label{eqn:dkl_gaussian}
\end{align}
where $C$ is a constant. If these two inequalities hold, using~\eqref{eqn:dkl_gaussian}, by Pinsker's Inequality, we get $\dtv{\mP_b}{\mP_{b'}} \le \sqrt{2\dkl{\mP_b}{\mP_{b'}}  } \le 2\sqrt2\alpha$. Using Corollary~\ref{coro:fano}, we get
\[
S(\cG_{\ab, \dims}, d_{TV}, \alpha, \eps) =\Omega \Paren{\frac{\ab\dims}{\alpha^2}+\frac{\ab\dims}{\alpha \eps}}.
\]
It remains to prove~\eqref{eqn:dtv_gaussian} and~\eqref{eqn:dkl_gaussian}.

For~\eqref{eqn:dkl_gaussian}, note that for any distribution pair $\mP_b \neq \mP_{b'} \in \cV_{\cG}$,
\begin{align}
\dkl{\mP_b}{\mP_{b'}} &\le \frac1{k} \sum_{t=1}^{\ab} \dkl{\p^{(t)}_{b_t}}{\p^{(t)}_{b'_{t}}}\le \max_{i,j \in [h]} d_{KL}\Paren{\p_i, \p_j} \le 4\dist^2, \nonumber
\end{align}
{where the first inequality comes from the convexity of $KL$ divergence and the last inequality uses the fact that the KL divergence between two Gaussians with identity covariance is at most the $\ell_2^2$ distance between their means.} 

Next we prove~\eqref{eqn:dtv_gaussian}. Let $B_j = B_{j,1} \times \cdots \times B_{j,\dims}$, where

$$B_{j,i}=
\begin{cases}
[ \frac{R}{4}, \frac{3R}{4}], & \text{when $i=j$,}\\
[ -\frac{R}{4}, \frac{R}{4} ], & \text{when $i \neq j$ and $i \le \ab$,}\\
[-\infty, \infty], & \text{when $\ab<i \le \dims$.}
\end{cases}$$

Then by Gaussian tail bound and union bound, for any $\mP \in \cV_{\cG}$, the mass of the $j$-th Gaussian component outside $B_j$ is at most $2ke^{-\frac12 \cdot \Paren{\frac1{4} R}^2}$. And the mass of other Gaussian components inside $B_j$ is at most $e^{-\frac12 \cdot \Paren{\frac1{4} R}^2}$. Hence we have:
\begin{align}
	\dtv{\mP_b}{\mP_{b'}} &= \frac1{2\ab} \int_{z \in \RR^{\dims}} \absv{ \p_{b_1}^{(1)}(z) +\cdots+ \p_{b_{\ab}}^{(\ab)}(z)  - \p_{b'_{1}}^{(1)}(z)  - \cdots -  \p_{b'_{\ab}}^{(\ab)}(z) }  dz \nonumber\\
	&\ge \frac1{2\ab}  \sum_{j=1}^{\ab} \int_{z \in B_j} \absv{ \p_{b_1}^{(1)}(z) +\cdots+ \p_{b_{\ab}}^{(\ab)}(z)  - \p_{b'_{1}}^{(1)}(z)  - \cdots -  \p_{b'_{\ab}}^{(\ab)}(z) }  dz \nonumber\\
	& \ge \frac1{2\ab} \cdot \sum_{j=1}^{\ab} (\int_{z \in B_j}  \absv{  \p_{b_{j}}^{(j)}(z)  - \p_{b'_{j}}^{(j)}(z) } dz -(\ab - 1) \cdot e^{-\frac12 \cdot \Paren{\frac1{4} R}^2}) \nonumber \\
	& \ge \frac1{2\ab} \cdot \sum_{j=1}^{\ab} (\int_{z \in \RR^{\dims}}  \absv{  \p_{b_{j}}^{(j)}(z)  - \p_{b'_{j}}^{(j)}(z) } dz - 3\ab \cdot e^{-\frac12 \cdot \Paren{\frac1{4} R}^2}) \nonumber \\
	& = \frac1{2\ab} \cdot \sum_{j=1}^{\ab} \dtv{\p_{b_{j}}}{\p_{b'_{j}}} - \frac{3\dist^2}{64k}. \nonumber
\end{align}
By Fact 6.6 in~\cite{KamathLSU18}, there exists a constant $C_1$ such that for any pair $i \neq j \in [h]$, 
$$\dtv{\p_i}{\p_j} \ge C_1\dist.$$
Hence we have
\[
	\frac1{2\ab} \cdot \sum_{j=1}^{\ab} \dtv{\p_{b_{j}}}{\p_{b'_{j}}} \ge \frac{C_1\dist}{2\ab} \ham{b}{b'} \ge \frac{C_1\dist}{4},
\]
where the last inequality comes from the property of the codebook. WLOG, we can assume $
\frac{3\dist}{64k} < C_1/8$. Taking $C = \frac{C_1}{8}$ completes the proof of~\eqref{eqn:dtv_gaussian}.

%\begin{align}
%\dtv{P}{Q} &= \frac1{2\ab} \int_{z \in \RR^{\dims}} \absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%&\ge \frac1{2\ab}  \sum_{j=1}^{\ab} \int_{z \in B_j}\absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%& \ge \frac1{2\ab} \cdot \frac{\ab}{2} (C_1\dist - 2\ab\cdot e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}) \ge \frac14 \Paren{C_1 -\frac{1}{4}}\dist.
%\end{align}
%where in the last inequality, we only look at the balls such that $i_j$ differs from $i^{\prime}_j$, and there exists at least $\frac{\ab}{2}$ such balls by the property of the codebook. Besides, by Gaussian tail bound, for the other component other than $j$, it has at most $e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}$ mass in ball $j$.
%

%Let $h = \absv{\cC}$ denote the size of the codebook. Now we have designed a class of $h > 2^{\frac{\dims}{8}}$ distributions around the origin. Let $\cG = \{ \p_1, \p_2,\cdots, \p_h\}$. We note that by  For a distribution $\p$ over $\reals^{\dims}$ and $v \in \RR^{\dims}$, we define $\p+ v$ to be the distribution $\p$ shifted by $v$. 
%
%Now we are able to design the set of Gaussian mixtures. Each $(i_1, \cdots,i_k) \in [h]^\ab$ corresponds to the mixture of $\ab$ spherical Gaussians, with density
%$$ \frac1k \Paren{ \p_{i_1,1} +  \p_{i_2,2} +\cdots+ \p_{i_k,k}},$$
%where for $i \in [h]$ and $j \in [\ab]$, $\p_{i,j}\coloneqq \p_i + v_j$.
%Then by Claim~\ref{claim:constantGV}, there exists a $h$-ary code $\cH$ with code length $\ab$ and minimum Hamming distance $\frac{\ab}{2}$, which satisfies $\absv{\cH} \ge (\frac{h}{16})^{\frac{\ab}{2}}$. This implies that among the $h^{\ab}$ distributions, there exist a set of $\absv{\cH} \ge (\frac{h}{16})^{\frac{\ab}{2}}$ distributions among which any pair of tuples $(i_1,\cdots,i_k)$ and $(i^{\prime}_1,\cdots,i^{\prime}_k)$ corresponding to two distributions has Hamming distance at least $\frac{\ab}{2}$. We denote this distribution set as 
%$\cV_{\ab, \dims}$.
%
%Now let we set $v_j, j \in [\ab]$ far apart each other, in order to reduce the overlapping between each component of the mixture. To be specific, we set 
%$j \in [\ab], v_j = B \cdot t_j$, where $t_j$ is $j$-th standard basis vector. %We note that for any pair $i,j \in [\ab]$, $\norm{v_i-v_j} = \sqrt{2}B$.
%
%Following the same routine, we want to prove that for any pair $P, Q \in \cV_{\ab,\dims}$, $\dtv{P}{Q} \ge C_2\dist$ for some constant $C_2$. Let $P = \frac1\ab \Paren{ \p_{i_1,1} +  \p_{i_2,2} +\cdots+ \p_{i_\ab,\ab}}$, $Q  = \frac1\ab \Paren{ \p_{i^{\prime}_1,1} +  \p_{i^{\prime}_2,2} +\cdots+ \p_{i^{\prime}_\ab,\ab}}$, and we use $B_j$ to denote the $\dims$-dimensional ball with centre $v_j$ and radius $\frac{R}{2}$,
%\begin{align}
%\dtv{P}{Q} &= \frac1{2\ab} \int_{z \in \RR^{\dims}} \absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%&\ge \frac1{2\ab}  \sum_{j=1}^{\ab} \int_{z \in B_j}\absv{ \p_{i_1,1}(z) +\cdots+ \p_{i_\ab,\ab}(z)  - \p_{i^{\prime}_1,1} (z)  - \cdots - \p_{i^{\prime}_\ab,\ab} (z)}  dz \nonumber\\
%& \ge \frac1{2\ab} \cdot \frac{\ab}{2} (C_1\dist - 2\ab\cdot e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}) \ge \frac14 \Paren{C_1 -\frac{1}{4}}\dist.
%\end{align}
%where in the last inequality, we only look at the balls such that $i_j$ differs from $i^{\prime}_j$, and there exists at least $\frac{\ab}{2}$ such balls by the property of the codebook. Besides, by Gaussian tail bound, for the other component other than $j$, it has at most $e^{-\frac12 \cdot \Paren{\frac1{2} R}^2}$ mass in ball $j$.
%
%
%By similar argument with Lemma~\ref{lem:reduction}, we can show $S(\cG_{\ab, \dims}, d_{TV}, \alpha, \eps)  \ge \Smc{\cV_{\ab, \dims}, \eps}$. Hence it is enough to show  $\Smc{\cV_{\ab, \dims}, \eps}=\Omega \Paren{\frac{\ab\dims}{\alpha^2}+\frac{\ab \dims}{\alpha \eps}}.$ Note that for any distribution pair $P,Q \in \cV_{\ab,\dims}$,
%\begin{align}
%	D_{KL} (P,Q) &\le \frac1{k} \sum_{j=1}^{\ab} D_{KL} (\p_{i_j},\p_{i^{\prime}_j}) \le \max_{i,j \in [h]} d_{KL}\Paren{\p_i, \p_j} \le 4\dist^2, \nonumber
%\end{align}
%where the first equality comes from the convexity of KL divergence. By Pinsker's inequality, $d_{TV}(P, Q) \le \sqrt{2D_{KL} (P,Q) } \le 2\sqrt2\alpha$.  Finally by Theorem~\ref{thm:fano} and the fact that $\exists c_1, c_2>0 , \absv{\cH} > c_1 \cdot 2^{c_2 \cdot \ab \dims}$, we have $\Smc{\cV_{\ab,\dims}, \eps} =\Omega \Paren{\frac{\ab\dims}{\alpha^2}+\frac{\ab\dims}{\alpha \eps}}$.

%\newhzz{Now we move to the case when $\ab \ge \dims$ and $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$. Let $r = \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$, we note that there exists a $r$-packing $S \subset \mathbb{R}^{\dims}$ with $|S| = \ab$ since $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$. Here we consider the same construction of the set of distributions as in the previous case, except that we set the centers of the $\ab$ components to be the points in $S$. Let $B_j$ denote the $\ell_2$ ball centering at the $j$-th point of $S$ with radius $\frac{r}{2}$. We note that by the tail bound of the Chi-squared distribution, the mass of the $j$-th Gaussian component outside $B_j$ is at most $O\Paren{\frac{\dist}{\ab}}$. Meanwhile, the mass of other Gaussian components inside $B_j$ is also at most $O\Paren{\frac{\dist}{\ab}}$. All the other analysis follows from the previous case.}

{Now we considers the case when $\ab \ge \dims$ and $R\ge (\ab)^{\frac1\dims} \cdot \sqrt{64\dims \log\Paren{\frac{8\ab}{\dist}}}$. Let $r = \sqrt{16\dims \log\Paren{\frac{8\ab}{\dist}}}$, we note that there exists a packing set $S = \{v_1, v_2, ..., v_k\} \subset \mathbb{R}^{\dims}$ which satisfies $\forall u, v \in S$,
	\[
		\norm{u - v} > r,~~~~ \norm{u}\le R,~~~~, \norm{v}\le R/3, 
	\]
	and $|S| = \ab$ since $R\ge 2 (\ab)^{\frac1\dims}  r$. Consider the set of mixture distributions as following: 
	For a codeword $b \in \cH$, let
	\[
		\mP'_b = \frac1k \Paren{ \p_{b_1}^{(1)'} +  \p_{b_{2}}^{(2)'}  +\ldots + \p_{b_{\ab}}^{(k)'} },
	\]
	where $\forall i \in [k], \p_{b_j}^{(j)'} = \cN(\mu_{b_j} + v_j, I_d)$.
	Let $B'_j$ denote the $\ell_2$ ball centering at the $v_j$ with radius $\frac{r}{2}$. We note that by similar analysis using the tail bound of the Gaussian distribution, the mass of the $j$-th Gaussian component outside $B_j'$ is at most $\frac{\dist^2}{64\ab^2}$. Meanwhile, the mass of other Gaussian components inside $B_j'$ is also at most $\frac{\dist^2}{64\ab^2}$. Hence the remaining analysis follows from the previous case.}
\end{proof}

==> toolbox/glodef.tex <==
% Theorem-like environments

\usepackage{lmodern}
%\usepackage{xspace}
\usepackage[protrusion=true,expansion=true]{microtype}
%\usepackage{fullpage}
\usepackage{amsfonts, pbox}

% Colors (with names)

% Colors (with names)
%\usepackage[usenames,dvipsnames,table,xcdraw]{xcolor}


%\usepackage[usenames,dvipsnames,table]{xcolor}
%\usepackage[colorlinks,citecolor=blue, bookmarks=true]{hyperref}

% Required for the table of results
\usepackage{multirow}
\usepackage{dsfont} %\indic
%\usepackage{fullpage}

\newcommand{\insertref}[1]{\todo[color=green!40]{#1}}
\newcommand{\explainindetail}[1]{\todo[color=red!30]{#1}}
\newcommand{\inlinetodo}[1]{\todo[color=blue!25,inline]{#1}}

% Algorithm environment
%\usepackage{algorithmicx,algpseudocode,  algorithm}
\providecommand\algorithmname{Algorithm}
\providecommand*{\factautorefname}{Fact}

% compact lists, and handy shortcuts for items
\usepackage[shortlabels]{enumitem}
\setitemize{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
\setenumerate{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}


\makeatletter
\@ifundefined{theorem}{% Theorems (each with its own style)
  \theoremstyle{plain}
  \newtheorem{theorem}{Theorem}
  \newtheorem{corollary}[theorem]{Corollary}
  %\newtheorem{corollary}{Corollary}
  \newtheorem{lemma}[theorem]{Lemma}
  \newtheorem{claim}[theorem]{Claim}
  \newtheorem{fact}{Fact}
  \newtheorem*{unnumberedfact}{Fact}
   \theoremstyle{definition}
  \newtheorem{definition}[theorem]{Definition}
  \theoremstyle{remark}
  \newtheorem{remark}{Remark}
  \newtheorem{question}{Question}
  \newtheorem*{notation}{Notation}
  \newtheorem{example}{Example}
  \newtheorem{observation}{Observation}
}{}
\makeatother
\newenvironment{proofof}[1]{\noindent{\bf Proof of {#1}:~~}}{\(\qed\)}

% Begin / End Theorems

\def \bthm#1{\begin{#1}\upshape\quad}
\def \ethm#1{\rqed\end{#1}}
\def \ethmp#1{\end{#1}}     % No box, when ends in displayed equation

\def \bClaim     {\bthm{Claim}}
\def \eClaim     {\ethm{Claim}}
\def \eClaimp    {\ethmp{Claim}}
\def \bConjecture {\bthm{Conjecture}}
\def \eConjecture {\ethm{Conjecture}}
\def \eConjecturep{\ethmp{Conjecture}}
\def \bCorollary {\bthm{Corollary}}
\def \eCorollary {\ethm{Corollary}}
\def \eCorollaryp{\ethmp{Corollary}}
\def \bCounter   {\bthm{CounterExample*}}
\def \eCounter   {\ethm{CounterExample*}}
\def \eCounterp  {\ethmp{CounterExample}}
\def \bDefinition{\bthm{Definition}}
\def \eDefinition{\ethm{Definition}}
\def \eDefinitionp{\ethmp{Definition}}
\def \bExample   {\bthm{Example}}
\def \eExample   {\ethm{Example}}
\def \eExamplep  {\ethmp{Example}}
\def \bExercise  {\bthm{Exercise}}
\def \eExercise  {\ethm{Exercise}}
\def \eExercisep {\ethmp{Exercise}}
\def \bIntuition {\bthm{Intuition}}
\def \eIntuition {\ethmp{Intuition}}
\def \bJoke      {\bthm{Joke}}
\def \eJoke      {\ethm{Joke}}
\def \bLemma     {\bthm{Lemma}}
\def \eLemma     {\ethm{Lemma}}
\def \eLemmap    {\ethmp{Lemma}}
\def \bOpen      {\bthm{Open problem}}
\def \eOpen      {\ethm{Open problem}}
\def \eOpenp     {\ethmp{Open problem}}
\def \bProperty  {\bthm{Property}}
\def \eProperty  {\ethm{Property}}
\def \ePropertyp {\ethmp{Property}}
\def \bQuestion  {\bthm{Question}}
\def \eQuestion  {\ethm{Question}}
%\def \bRemark    {\bthm{Remark}}
%\def \eRemark    {\ethm{Remark}}
\def \bResult    {\bthm{Result}}
\def \eResult    {\ethm{Result}}
\def \bTheorem   {\bthm{Theorem}}
\def \eTheorem   {\ethm{Theorem}}
\def \eTheoremp  {\ethmp{Theorem}}

% Environments

\newenvironment{Problem}{\textbf{Problem}\\ \begin{enumerate}}{\end{enumerate}}
\newenvironment{Problems}{\textbf{Problems}\\ \begin{enumerate}}{\end{enumerate}}

%\newenvironment{Problems}{\begin{trivlist}\item[]{\textbf{Problems}}{\end{trivlist}}}

% Headers

\def \skpbld#1{\par\noindent\textbf{#1}\quad}
\def \skpblds#1{\skpbld{#1}\par\noindent}

\def \Answer   {\skpbld{Answer}}
\def \Answers  {\skpblds{Answers}}
\def \Basis    {\skpbld{Basis}}
\def \Check    {\skpbld{Check}}
%\def \Example  {\skpbld{Example}}
\def \Examples {\skpbld{Examples}}
\def \Intuition{\skpbld{Intuition}}
\def \Method   {\skpbld{Method}}
\def \Methods  {\skpblds{Methods}}
\def \Outline  {\skpbld{Outline}}
\def \Proof    {\skpbld{Proof}}
\def \Proofs   {\skpblds{Proofs}}
%\def \Problem  {\skpbld{Problem}}
%\def \Problems {\skpblds{Problems}}
\def \Proline  {\skpbld{Proof Outline}}
%\def \Remark   {\skpbld{Remark}}
\def \Remarks  {\skpblds{Remarks}}
\def \Solution {\skpbld{Solution}}
\def \Solutions{\skpblds{Solutions}}
\def \Verify   {\skpbld{Verify}}
\def \Step     {\skpbld{Step}}

% Ignores

\newcommand{\ignore}[1]{}

% Problems & solutions

\newcommand{\problem}[1]{#1}
\newcommand{\solution}[1]{{\\ \bf Solution}\quad #1}
%\newcommand{\solution}[1]{\mbox{}\\ \medskip\noindent{\bf Solution\medskip}#1}
%\newcommand{\solution}[1]{}

\newcommand{\source}[1]{(Taken from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\modifiedfrom}[1]{(Modified from~\cite{#1})}
%\newcommand{\modifiedfrom}[1]{}

\newcommand{\takenfrom}[1]{(Taken from~\cite{#1})}
%\newcommand{\takenfrom}[1]{}

\newcommand{\reportedby}[1]{Reported by #1.}
%\newcommand{\reportedby}[1]{}

\newcommand{\hint}[1]{Hint: #1}
%\newcommand{\hint}[1]{}

\newcommand{\joke}[1]{\footnote{#1}}
\newcommand{\trivia}[1]{\footnote{#1}}

% Equation formatting

\newcommand{\spreqn}[1]{{\qquad\text{#1}\qquad}}

% Blackboard fonts
\newcommand{\II}{\mathbb{I}} % Added by Theertha on April 16th 2013.
\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}

% probability
\newcommand{\expectation}[1]{\EE\left[#1\right]}
\newcommand{\variance}[1]{Var\left(#1\right)}

% Number sets

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\positives}{\PP}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}

\newcommand{\realsge}{{\reals_{\ge}}}
\newcommand{\realsp}{\reals^+}
\newcommand{\integersp}{\integers^+}
\newcommand{\integerss}[1]{\integers_{\ge{#1}}}

% boldface

\def \ba     {{\bf a}}
\def \bx     {{\bf x}}
\def \by     {{\bf y}}

\def \bA     {{\bf A}}
\def \bB     {{\bf B}}
\def \bC     {{\bf C}}
\def \bD     {{\bf D}}
\def \bF     {{\bf F}}
\def \bG     {{\bf G}}
\def \bL     {{\bf L}}
\def \bQ     {{\bf Q}}
\def \bR     {{\bf R}}
\def \bS     {{\bf S}}
\def \bT     {{\bf T}}
\def \bX     {{\bf X}}
\def \bY     {{\bf Y}}
\def \bZ     {{\bf Z}}

% caligraphics

\def \cA     {{\cal A}}
\def \cB     {{\cal B}}
\def \cC     {{\cal C}}
\def \cD     {{\cal D}}
\def \cE     {{\cal E}}
\def \cF     {{\cal F}}
\def \cG     {{\cal G}}
\def \cH     {{\cal H}}
\def \cI     {{\cal I}}
\def \cK     {{\cal K}}
\def \cL     {{\cal L}}
\def \cM     {{\cal M}}
\def \cN     {{\cal N}}
\def \cO     {{\cal O}}
\def \cP     {{\cal P}}
\def \cQ     {{\cal Q}}
\def \cR     {{\cal R}}
\def \cS     {{\cal S}}
\def \cT     {{\cal T}}
\def \cU     {{\cal U}}
\def \cV     {{\cal V}}
\def \cW     {{\cal W}}
\def \cX     {{\cal X}}
\def \cY     {{\cal Y}}
\def \cZ     {{\cal Z}}

% vectors

\def \vct#1{{\overline{#1}}}

\def \vcta  {{\vct a}}
\def \vctb  {{\vct b}}
\def \vctq  {{\vct q}}
\def \vcts  {{\vct s}}
\def \vctu  {{\vct u}}
\def \vctv  {{\vct v}}
\def \vctx  {{\vct x}}
\def \vcty  {{\vct y}}
\def \vctz  {{\vct z}}
\def \vctp  {{\vct p}}

\def \vctV  {{\vct V}}
\def \vctX  {{\vct X}}
\def \vctY  {{\vct Y}}
\def \vctZ  {{\vct Z}}

\def \vctbeta  {{\vct\beta}}

% Random variables

\newcommand{\rnd}[1]{{\boldsymbol #1}}

\newcommand{\rndd}{{\rnd d}}
\newcommand{\rndl}{{\rnd l}}
\newcommand{\rndp}{{\rnd p}}
\newcommand{\rnds}{{\rnd s}}
\newcommand{\rndx}{{\rnd x}}
\newcommand{\rndy}{{\rnd y}}
\newcommand{\rndz}{{\rnd z}}

%\newcommand{\poi}{{\rm poi}}
\newcommand{\Var}{{\rm Var}}

% following should not exist (indicate random sets)

\newcommand{\rndR}{{\rnd R}}
\newcommand{\rndT}{{\rnd T}}

% arrow vectors

\newcommand{\rvc}{{\overrightarrow c}}

% Abbreviations - \xspace puts space iff there is space after command

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish
%\newcommand{\iid}{\textit{i.i.d.}\xspace} 
\newcommand{\iid}{\textit{i.i.d.}} % Edit by Theertha, \xspace not compiling

\newcommand{\etc}{etc.\@\xspace}

% Colors

%\definecolor{light}{gray}{.75}


% marginal notes

\newcommand{\mrgs}[2]{\# #1 \#{\marginpar{#2}}}

\newcommand{\mrgcgd}[1]{\mrgs{#1}{CHANGED}}
\newcommand{\mrgchk}[1]{\mrgs{#1}{CHECK}}
\newcommand{\mrgfix}[1]{\mrgs{#1}{FIX}}
\newcommand{\mrgnew}[1]{\mrgs{#1}{NEW}}

% qed's --  Also consider \qedhere

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}

\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \ok    {1\upto k}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \set#1#2{{\sets{{#1}\upto{#2}}}}

\def \setpmo   {\sets{\pm 1}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \setok    {\{\ok\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \inseg#1{{[#1]}} % use \intsgm instead
\newcommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations


%\DeclareMathOperator*{\union}{\cup}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Union}{\bigcup}  %Commented by Theertha on April 15

\newcommand{\unionl}{\union\limits}
\newcommand{\Unionl}{\Union\limits}
 
%\DeclareMathOperator*{\inter}{\cap}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Inter}{\bigcap}   %Commented by Theertha on April 15

\newcommand{\interl}{\inter\limits}
\newcommand{\Interl}{\Inter\limits}

% Floors, Ceilings, Absolute value

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}
\def \absvlu#1{{|#1|}}
\def \Absvlu#1{{\left|{#1}\right|}}
\newcommand{\absv}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|_2}
% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}
\def \Brace#1{\left\{#1\right\}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory

\newcommand{\base}[2]{{[#1]_{#2}}}

% equalities

\newcommand{\ed}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{{:=}}

\newcommand{\cnvprb}{\stackrel{\mathrm{p}}{\to}}
\newcommand{\cnvdst}{\stackrel{\mathrm{d}}{\to}}
\newcommand{\cnvas}{\stackrel{\mathrm{a.s.}}{\to}}

\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

\newcommand{\al}[1]{\stackrel{\mathit{{#1}}}{<}}
\newcommand{\ag}[1]{\stackrel{\mathit{{#1}}}{>}}
\newcommand{\ale}[1]{\stackrel{\mathit{{#1}}}{\le}}
\newcommand{\age}[1]{\stackrel{\mathit{{#1}}}{\ge}}
\newcommand{\aeq}[1]{\stackrel{\mathit{{#1}}}{=}}

%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

\newcommand{\re}{\sim}
\newcommand{\rle}{\stackrel<\sim} % roughly (asymptotically taken) <=
%\newcommand{\rl}{\stackrel<\sim}
\newcommand{\rge}{\stackrel>\sim}
%\newcommand{\rg}{\stackrel>\sim}

\newcommand{\ere}{\approx} % exponentially roughly equal
\newcommand{\erle}{\stackrel<\approx}
%\newcommand{\erl}{\stackrel<\approx}
\newcommand{\erge}{\stackrel>\approx}
%\newcommand{\erg}{\stackrel>\approx}

% Relations

\newcommand{\independent}{\perp\!\!\!\perp}

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% probability

\newcommand{\pr}{{p}} % phase out in favor of \prb
\newcommand{\prb}{{p}} 

\newcommand{\prbs}[1]{{\prb^{(#1)}}}

\newcommand{\Prb}{\text{Pr}}
%\newcommand{\Pr}{{\text{Pr}}} % phase out in favor of \Prb
\newcommand{\Prn}{\text{Pr}}  % phase out in favor of \Prb

\newcommand{\Prs}[1]{\Pr\Paren{#1}} % phase out in favor of \Prbs
\newcommand{\Prbs}[1]{{\Prb^{(#1)}}} % Check if used - phase out
\newcommand{\probof}[1]{\Pr\Paren{#1}}

% notation

\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\newcommand{\flnpwr}[2]{{#1^{\underline{#2}}}} % Falling power

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\pfx}{{\prec}}
\newcommand{\pfxeq}{{\preceq}}

\newcommand{\sfx}{{\succ}}
\newcommand{\sfxeq}{{\succeq}}

% for old documents

\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{				% grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}


\newcommand{\Sparen}[1]{\left[#1\right]}
\newcommand{\Order}{O}
\newcommand{\order}{o}


\newtheorem{prop2}[theorem]{Proposition}
\newtheorem{lem2}[theorem]{Lemma}
\newtheorem{coro2}[theorem]{Corollary}







==> toolbox/locdef.tex <==
 \newcommand{\anew}[1]{{\color{black}#1}}
 \newcommand{\newzs}[1]{{\color{black}#1}}
  \newcommand{\newnewzs}[1]{{\color{black}#1}}
  
 \newcommand{\newhz}[1]{{\color{black}#1}}
 \newcommand{\newhzz}[1]{{\color{black}#1}}
 \newcommand{\newzz}[1]{{\color{black}#1}}
 
  \newcommand{\newhzn}[1]{{\color{black}#1}}

\newcommand{\Dk}{\Delta_k}
\newcommand{\D}{\Delta}
\newcommand{\Du}{\Delta_u}

\newcommand{\absz}{k}
\newcommand{\ab}{k}
\newcommand{\dims}{d}
\newcommand{\ns}{n}
\newcommand{\ber}{\cB}
\newcommand{\dP}{p}
\newcommand{\dQ}{q}
\newcommand{\mP}{p}
\newcommand{\mQ}{q}


\newcommand{\verify}[1]{\textcolor{black}{#1}}


\newcommand{\p}{p}
\newcommand{\q}{q}
\newcommand{\pn}[1]{\p^{#1}}
\newcommand{\qn}[1]{\q^{#1}}


\newcommand{\expectationsub}[2]{\EE_{#1}\left[#2\right]}
\newcommand{\probofsub}[2]{\Pr\nolimits_{#1}\Paren{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Sitnp}{S({\tt IT}, \ab, \dist)}

\newcommand{\Sit}{S({\tt IT}, \ab, \dist,\eps)}
\newcommand{\Sitd}{S({\tt IT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sut}[2]{S({\tt UT}, #1, #2,\eps)}
\newcommand{\Sutd}{S({\tt UT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sutnp}[2]{S({\tt UT}, #1, #2)}
\newcommand{\Sittwo}{S({\tt IT}, \ab, \dist,\eps)}
\newcommand{\Sct}{S({\tt CT}, \ab, \dist,\eps)}
\newcommand{\Sctd}{S({\tt CT}, \ab, \dist,\eps,\delta)}
\newcommand{\Sctnp}{S({\tt CT}, \ab, \dist)}

\newcommand{\Smc}[1]{S({\tt MC},#1)}
\newcommand{\Sdl}[1]{S({\tt DL},\Delta_{\ab}, \alpha,\eps, #1)}
\newcommand{\Sdla}[1]{S({\tt DL},\Delta_{\ab}, \alpha,\eps,\delta, #1)}
\newcommand{\Sdlat}[2]{S({\tt DL},#1, \alpha,\eps,\delta, #2)}

\newcommand{\Pds}{C_{\ab, \dims}}
\newcommand{\Spl}{S({\tt PL},\Pds, \alpha,\eps, d_{TV})}
\newcommand{\Spla}{S({\tt PL},\Pds, \alpha,\eps, \delta, d_{TV})}

\newcommand{\absvn}[1]{\left\|#1\right\|_1}



\newcommand{\unif}{u}
\newcommand{\unifab}{\unif[{\ab}]}
\newcommand{\unifabs}[1]{\unif[{#1}]}


\newcommand{\smb}{x}
\newcommand{\psmb}{\p_\smb}
\newcommand{\ps}[1]{\p_{#1}}
\newcommand{\Xon}{X^\ns}
\newcommand{\Yon}{Y^\ns}
\newcommand{\Zon}{Z^\ns}
\newcommand{\xon}{x^\ns}
\newcommand{\yon}{y^\ns}
\newcommand{\Xot}{X_1^t}
\newcommand{\Yot}{Y_1^t}
\newcommand{\Xos}{X_1^s}
\newcommand{\Xosp}{X_1^{'s}}
\newcommand{\Yos}{Y_1^s}
\newcommand{\Yosp}{Y_1^{'s}}
\newcommand{\Xosmo}{X_1^{s-1}}
\newcommand{\Yosmo}{Y_1^{s-1}}




\newcommand{\Mestxon}{\Mest\Paren{\Xon}}
\newcommand{\Mest}{{M}}
\newcommand{\Mestgtxon}{\Mest^{\texttt{GT}}\Paren{\Xon}}


\newcommand{\Moxon}{M_0(\Xon)}

\newcommand{\prf}[2]{\Phi_{#1}(#2)}
\newcommand{\prfi}[1]{\Phi_{#1}}

\newcommand{\kp}{k^{'}}

\newcommand{\eps}{\varepsilon}
\newcommand{\he}{\hat{E}}

\newcommand{\mltx}[1]{\mu_{#1}}
\newcommand{\mlty}[1]{\nu_{#1}}

\newcommand{\bias}{b}
\newcommand{\Bern}[1]{B(#1)}

\newcommand{\ham}[2]{d_{\text{Ham}}(#1,#2)}
\newcommand{\alg}{\hat \theta}


\newcommand{\Mltsmb}[2]{M_{#1}(#2)}
\newcommand{\prfsmb}[2]{\Phi_{#1}(#2)}


\newcommand{\dist}{\alpha}

\newcommand{\dtv}[2]{d_{TV}(#1, #2)}
\newcommand{\dkl}[2]{d_{KL}(#1, #2)}


%\ifnum\withcolors=1
%  \newcommand{\new}[1]{{\color{red} {#1}}} % new
%  \newcommand{\newer}[1]{{\color{blue} {#1}}} % even newer
%  \newcommand{\newest}[1]{{\color{orange} {#1}}} % even even newer
%  \newcommand{\newerest}[1]{{\color{blue!10!black!40!green} {#1}}} % you get the idea.
%  \newcommand{\acolor}[1]{{\color{ForestGreen}#1}} % Jayadev
%  \newcommand{\scolor}[1]{{\color{RubineRed}#1}} % Clement
%  \newcommand{\zcolor}[1]{{\color{Orange}#1}} % Himanshu
%  \newcommand{\zscolor}[1]{{\color{Purple}#1}} % Himanshu
%\else
%  \newcommand{\new}[1]{{{#1}}}
%  \newcommand{\newer}[1]{{{#1}}}
%  \newcommand{\newest}[1]{{{#1}}}
%  \newcommand{\newerest}[1]{{{#1}}}
%  \newcommand{\acolor}[1]{{#1}}
%  \newcommand{\scolor}[1]{{#1}}
%  \newcommand{\zcolor}[1]{{#1}}
%\fi
%
%\ifnum\withnotes=1
%  \newcommand{\anote}[1]{\par\acolor{\textbf{J: }\sf #1}} % Jayadev
%  \newcommand{\snote}[1]{\par\scolor{\textbf{ZS: }\sf #1}} % Clement
%  \newcommand{\znote}[1]{\par\zcolor{\textbf{H: }\sf #1}} % Himanshu
%  \newcommand{\afootnote}[1]{\footnote{{\bf \acolor{Jayadev}}: {#1}}}
%  \newcommand{\sfootnote}[1]{\footnote{{\bf \scolor{Cl\'ement}}: {#1}}}
%  \newcommand{\zfootnote}[1]{\footnote{{\bf \zcolor{Himanshu}}: {#1}}}
%
%
%  \newcommand{\todonote}[2][]{\todo[size=\scriptsize,color=red!40,#1]{#2}}  
%	\newcommand{\questionnote}[2][]{\todo[size=\tiny,color=blue!30]{#2}}
%	\newcommand{\todonotedone}[2][]{\todo[size=\scriptsize,color=green!40]{$\checkmark$ #2}}
%	\newcommand{\todonoteinline}[2][]{\todo[inline,size=\scriptsize,color=orange!40,#1]{#2}}  
%  \newcommand{\marginnote}[1]{\todo[color=white,linecolor=black]{{#1}}}
%\else
%  \newcommand{\anote}[1]{}
%  \newcommand{\snote}[1]{}
%  \newcommand{\znote}[1]{}
%  \newcommand{\todonote}[2][]{\ignore{#2}}
%	\newcommand{\questionnote}[2][]{\ignore{#2}}
%	\newcommand{\todonotedone}[2][]{\ignore{#2}}
%	\newcommand{\todonoteinline}[2][]{\ignore{#2}}
%  \newcommand{\marginnote}[1]{\ignore{#1}}
%\fi
%
%\newcommand{\amargin}[1]{\questionnote{\acolor{#1}}} % Jayadev
%\newcommand{\smargin}[1]{\questionnote{\ccolor{#1}}} % Clement
%\newcommand{\zmargin}[1]{\questionnote{\hcolor{#1}}} % Himanshu
%\newcommand{\zsmargin}[1]{\questionnote{\zscolor{#1}}} %Ziteng
%
%\ifnum\withnotes=1
%  \usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}
%\fi



%%%%%%%%%%%%%%%%%%%%%%

==> toolbox/product_new.tex <==
\subsection{Product distribution estimation} \label{sec:product}

%\begin{definition}
%A $(\ab,\dims)$-product distribution is a distribution over $[\ab]^{\dims}$, such that its marginal distribution on each dimension is independent.
%\end{definition}

Recall that $\Delta_{\ab, \dims}$ is the set of all $(\ab,\dims)$-product distributions.~\cite{BunKSW2019} proves an upper bound of $O\Paren{\ab\dims \log \Paren{ \frac{\ab\dims}{\dist}} \Paren{\frac1{\dist^2}+\frac1{\dist\eps}}}$. We prove a sample complexity lower bound for $\eps$-DP $(\ab,\dims)$-product distribution estimation in Theorem~\ref{thm:main_product}, which is optimal up to logarithmic factors.

%\product*
\begin{theorem}
\label{thm:main_product}
The sample complexity of $\eps$-DP $(\ab,\dims)$-product distribution estimation satisfies
\begin{align}
&S(\Delta_{\ab, \dims}, d_{TV}, \alpha, \eps) = \Omega \Paren{\frac{\ab\dims}{\dist^2}+\frac{\ab\dims}{\dist \eps}}. \nonumber
\end{align}
\end{theorem}

\begin{proof}
%We start with the construction of the distribution set. First we utilize the same binary code as in Claim~\ref{clm:GV}, restated below:
%\amargin{A total repeat again ...!}
%\GVcode*
{
We start with the construction of the distribution set. First we use the same binary code as in Lemma~\ref{lem:GV} with weight $l = \frac{\ab}{2}$.
Let $h := \absv{\cC}$ denote the size of the codebook. Given $j \in [h]$, we construct the following $\ab$-ary distribution $\p_j$ based on $c_j \in \cC$:}

{$$ \p_{j} (i)  = \frac{1}{\ab} +\frac{\dist}{\ab\sqrt{\dims}} \cdot \mathbb{I}\Paren{ c_{j,i}=1},$$}
{ where $ c_{j,i}$ denotes the $i$-th coordinate of $c_j$.}
%
%$$ \p_{j} (i)  = \left\{
%\begin{array}{rcl}
%\frac{1}{\ab} + \frac{\dist}{\ab \sqrt{ \dims}} ,       &      & when ~ c_j (i)=1,\\
%\frac{1}{\ab} - \frac{\dist}{\ab\sqrt{\dims}},       &      & when ~c_j (i)=0.
%\end{array} \right. $$


Now we have designed a set of $\ab$-ary distributions of size $h = \Omega \Paren{2^{\frac{7\ab}{128}}}$. To construct a set of product distributions, {we use the codebook construction in Lemma~\ref{lem:constantGV2} to get an $h$-ary codebook $\cH$ with length $d$ and minimum hamming distance $d/2$. Moreover, $|\cH| \ge (\frac{h}{16})^{\frac{\dims}{2}}$. }

Now we can construct the distribution set of $(\ab,\dims)$-product distributions.
Given $b \in \cH$, define
$$\dP_b = \p_{b_1} \times  \p_{b_2}\times \cdots \times \p_{b_d}.$$

Let $\cV_{\ab,\dims}$ denote the set of distributions induced by $\cH$. We want to prove that $\forall \dP \neq \dQ \in \cV_{\ab,\dims},$
\begin{align}
	\dtv{\dP}{\dQ} \ge C\dist, \label{eqn:dtv_prod}\\
	D_{KL} (\dP,\dQ)  \le 4\dist^2, \label{eqn:dkl_prod}
\end{align}
for some constant $C$. Suppose these two inequalities hold, using~\eqref{eqn:dkl_prod}, by Pinsker's Inequality, we get $d_{TV}(\dP, \dQ) \le \sqrt{2D_{KL} (\dP, \dQ) } \le 2\sqrt2\alpha$. Then using Corollary~\ref{coro:fano}, we can get
\begin{align}
&S(\Delta_{\ab, \dims}, d_{TV}, \alpha, \eps) = \Omega \Paren{\frac{\ab\dims}{\dist^2}+\frac{\ab\dims}{\dist \eps}}. \nonumber
\end{align}
Now it remains to prove~\eqref{eqn:dtv_prod} and~\eqref{eqn:dkl_prod}. For~\eqref{eqn:dkl_prod}, note that for any distribution pair $\dP,\dQ \in \cV_{\ab,\dims}$,
\begin{align}
	D_{KL} (\dP,\dQ) \le \dims \cdot \max_{i, j \in [h]} d_{KL}\Paren{\p_i, \p_j} \le 4\dist^2, \nonumber
\end{align}
\newzs{
where the first inequality comes from the additivity of $KL$ divergence for independent distributions and $\forall i, j \in [h]$, 
\[
	d_{KL}\Paren{\p_i, \p_j} = \sum_{x \in [k]} \p_i(x) \log \frac{\p_i(x)}{\p_j(x)} \le \sum_{x \in [\dims]} \frac{(\p_i(x) - \p_j(x))^2}{\p_j(x)} \le \ab \Paren{\frac{\dist}{\ab\sqrt{\dims}}}^2/ \frac{1}{\ab} = \frac{\alpha^2}{d}.
\]
}
Next we prove~\eqref{eqn:dtv_prod}. For any $b \in \cH$ and $\forall i \in[k]$, define set
\[
	S_i  = \{j \in [\ab] : c_{ b_{i},j} = 1\},
\]
which contains the locations of $+1$'s in the code at the $i$th coordinate of $b$. Based on this, we define a product distribution
\[
	\dP'_{b} = \prod_{i = 1}^{d} \cB(\mu_{i} ),
\]
where $\mu_{i} = \sum_{j \in S_i} \p_{b_{i}} (j)$ and $\cB(t)$ is a Bernoulli distribution with mean $t$. For any $b' \neq b \in \cH$, we define
\[
	\dP'_{b'} = \prod_{i = 1}^{d} \cB(\mu'_{i} ),
\]
 where $\mu'_{i} = \sum_{j \in S_i} \p_{b'_{i}}(j)$. Then we have:
 \[
 	\dtv{\dP'_{b}}{\dP'_{b'}} \le \dtv{\dP_{b}}{\dP_{b'}},
 \]
since $\dP'_{b}$ and $\dP'_{b'}$ can be viewed as a post processing of $\dP_{b}$ and $\dP_{b'}$ by mapping elements in $S_i$ to 1 and others to 0 at the $i$-th coordinate. Moreover, we have $\ham{b}{b'} \ge \frac{d}{2}$, and $\forall i$, if $b_{i} \neq b'_{i}$, we have $d_{H}(c_{b_{i}}, c_{b'_{i}}) > \frac{k}{8}$. By the definition of $\p_i$'s, we have
\[
	\| \mu_1 - \mu_2 \|_2^2 \ge \frac{d}{2} \times \left( \frac{\ab}{8} \times \frac{\dist}{\ab \sqrt{d}} \right)^2 = \frac{\dist^2}{128}.
\] 
By Lemma 6.4 in~\cite{KamathLSU18}, there exists a constant $C$ such that $\dtv{\dP'_{b}}{\dP'_{b'}} \ge C\dist$, proving~\eqref{eqn:dtv_prod}.

%start by looking at the marginal distribution of $\dP$ and $\dQ$ on the first coordinate, which we denote as $\p$ and $\q$.  Let $S(\p) = \{j \in [\ab] : \p(j) = \frac{1}{\ab} + \frac{\dist}{\ab \sqrt{ \dims}} \}$, and we design the following mapping $f: \Delta_{\ab} \to \Delta_2$ such that given distribution $\p^{\prime}$, $f (\p^{\prime}) = \cB(\mu_{\p^{\prime}})$, with $\mu_{\p^{\prime}} = \sum_{j \in S(\p)} \p^{\prime}(j)$. By the properties of the code $\cC$, we note that $\mu_{\p} = \frac12+ \frac{\dist}{\sqrt{\dims}}$ and $\mu_p - \mu_q \ge \frac{\dist}{8\sqrt{\dims}}$. Now we apply similar mapping on all the dimensions and after the mapping, we get two $(2,\dims)$-product distributions $\dP^{\prime}$ and $\dQ^{\prime}$, such that $\norm{\mu(\dP^{\prime}) - \mu(\dQ^{\prime})} \ge \frac{\dist}{8}$, where $\mu(\dP^{\prime})$ is the bias vector of the $(2,\dims)$-product distribution $\dP^{\prime}$. By Lemma 6.4 in~\cite{KamathLSU18}, there exists some constant $C$ such that $\dtv{\dP^{\prime}}{\dQ^{\prime}}  \ge C\dist$.  Besides, by the definition of TV distance, we have $\dtv{\dP}{\dQ} \ge \dtv{\dP^{\prime}}{\dQ^{\prime}}\ge C\dist$. 


\end{proof}

==> toolbox/pure_dp.tex <==
\section{$\eps$-DP distribution estimation} \label{sec:pdp_estimation}
In this section, we use Corollary~\ref{coro:fano} to prove sample complexity lower bounds for various $\eps$-DP distribution estimation problems. The general idea is to construct a subset of distributions in $\cQ$ such that they are close in both $TV$ distance and $KL$ divergence while being separated {in the loss function $\ell$}. The larger the subsets we construct, {the better} the lower bounds we can get. In Section~\ref{sec:pdp_kary}, we {derive} sample complexity lower bounds for $k$-ary distribution estimation under both \emph{TV} and $\ell_2$ distance that are tight up to constant factors. Tight sample complexity lower bounds up to logarithmic factors for $(k,d)$-product distributions and $d$-dimensional Gaussian mixtures are derived in Section~\ref{sec:product} and~\ref{sec:gaussian} respectively. 

{Corollary~\ref{coro:fano} requires a \emph{packing} of distributions with pairwise distance at least $3\tau$ apart in $\ell$. A standard method to construct such distributions is using results from coding theory.}

\newzs{We start with some definitions. An $h$-ary code of length $k$ is a set $\cC\subseteq \{0,1, \ldots, h-1\}^k$, and each $c\in\cC$ is a \emph{codeword}. The \emph{minimum distance} of a code $\cC$ is the smallest Hamming distance between two codewords in $\cC$. The code is called binary when $h = 2$. The weight of a binary codeword $c\in\cC$ is $wt(c)= |\{i:c_i=1\}|$, the number of 1's in $c$. A binary code $\cC$ is a \emph{constant weight code} if each $c\in\cC$ has the same weight.  We now present some useful variants of the classic Giblert Varshamov bounds on the existence of codes with certain properties. We prove these in Section~\ref{sec:codes}.
}
{
\begin{lemma}
\label{lem:GV}
Let $l$ be an integer at most $k/2$ and at least $20$. There exists a constant weight binary code $\cC$ which has code length $k$, weight $l$, minimum distance $l/4$ with $|\cC|\ge \Paren{\frac{k}{2^{7/8}l}}^{7l/8}$.
\end{lemma}} 

%\noindent{An $h$-ary code of length-$k$ is a subset of $\{0,1,\ldots, h-1\}^k$. 
\begin{lemma}
\label{lem:constantGV2}
There exists an $h$-ary code $\cH$ with code length $\dims$ and minimum Hamming distance $\frac{\dims}{2}$, which satisfies that $\absv{\cH} \ge (\frac{h}{16})^{\frac{\dims}{2}}$.
\end{lemma}}


%We start with some definitions. A binary code of length $k$ is a set $\cC\subseteq \{0,1\}^k$, and each $c\in\cC$ is a \emph{codeword}. The weight of a binary codeword $c\in\cC$ is $wt(c)= |\{i:c_i=1\}|$, the number of 1's in $c$. $\cC$ is a \emph{constant weight code} if each $c\in\cC$ has the same weight. The \emph{minimum distance} of a code $\cC$ is the smallest Hamming distance between two codewords in $\cC$. We now present some useful variants of the classic Giblert Varshamov bounds on the existence of codes with certain properties. We prove these in Section~\ref{sec:codes}.
%
%{
%	\begin{lemma}
%		\label{lem:GV}
%		Let $l$ be an integer at most $k/2$ and at least $20$. There exists a constant weight binary code $\cC$ which has code length $k$, weight $l$, minimum distance $l/4$ with $|\cC|\ge \Paren{\frac{k}{2^{7/8}l}}^{7l/8}$.
%\end{lemma}} 
%
%\noindent{An $h$-ary code of length-$k$ is a subset of $\{0,1,\ldots, h-1\}^k$. 
%	\begin{lemma}
%		\label{lem:constantGV2}
%		There exists an $h$-ary code $\cH$ with code length $\dims$ and minimum Hamming distance $\frac{\dims}{2}$, which satisfies that $\absv{\cH} \ge (\frac{h}{16})^{\frac{\dims}{2}}$.
%\end{lemma}}

\input{toolbox/pure_dp_kary}

\input{toolbox/product_new}

\input{toolbox/gaussian}

==> toolbox/pure_dp_kary.tex <==
\subsection{$\ab$-ary distribution estimation} \label{sec:pdp_kary}
We establish the sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $TV$ and $\ell_2$ distance. 
%\puredtv*
\begin{theorem}
\label{thm:pure-dv}
The sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $TV$ distance  is
\begin{align}
S(\Delta_{\ab}, d_{TV}, \alpha, \eps)=\Theta \Paren{\frac{\ab}{\alpha^2}+\frac{\ab}{\alpha\eps}}.
\end{align}
\end{theorem}

\begin{theorem}
\label{thm:pure-l2}
The sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $\ell_2$ distance is
\begin{align}
S(\Delta_{\ab}, \ell_2, \alpha, \eps) =\Theta \Paren{\frac{1}{\dist^2}+\frac{\sqrt{\ab}}{\dist\eps}},\ \ \ \text{for $\dist < \frac1{\sqrt{\ab}}$, and}
\end{align}
\begin{align}
\Omega\Paren{\frac{1}{\dist^2}+\frac{\log(\ab\dist^2)}{\dist^2\eps}}\le S(\Delta_{\ab}, \ell_2, \alpha, \eps) \le O\Paren{\frac{1}{\dist^2}+\frac{\log\ab}{\dist^2\eps}} \ \ \ \text{for $\dist > \frac1{\sqrt{\ab}}$.} 
\end{align}
\end{theorem}
 

For $\ell_2$ loss, our bounds are tight within constant factors when $\dist < \frac1{\sqrt{\ab}}$ or $\dist > \ab^{-(\frac12- 0.001)}$.
%With regarding to approximate DP, we have matching upper and lower bounds when $\eps \ge O(\delta)$, which is a weak condition (practically people $\eps = O(1)$ and $\delta = O\Paren{\frac1{\ns}}$). 

\subsubsection {Total variation distance}
\label{sec:puredp-tv}

In this section, we derive the sample complexity of $\eps$-DP $k$-ary distribution estimation under $TV$ distance, which is stated in Theorem~\ref{thm:pure-dv}.

\medskip

\noindent \textbf{Upper bound:}
\cite{DiakonikolasHS15} provides an upper bound based on Laplace mechanism~\cite{DworkMNS06}. {We state the algorithm and a proof for completeness and we will use it for estimation under $\ell_2$ distance.}

Given a $\Xon$ from an unknown distribution $\p$ over $[\ab]$. Let $M_x(\Xon)$ be the number of appearances of $x$ in $\Xon$. {Let $p^{\text{erm}}$ be the empirical estimator where $ p^{\text{erm}}(x) :=\frac{M_x(\Xon)}{\ns}$. We note that changing one $X_i$ in $X^n$ can change at most two coordinates of $p^{\text{erm}}$, each by at most $\frac1n$, and thus changing one $X_i$ changes the $p^{\text{erm}}$ by at most $2/n$ in $\ell_1$ distance. Therefore, by~\cite{DworkMNS06}, adding a Laplace noise of parameter $2/\ns\eps$ to each coordinate of $p^{\text{erm}}$ makes it $\eps$-DP. For $x\in[k]$, let
\[ 
h(x) = p^{\text{erm}}(x)+\text{Lap}\Paren{\frac{2}{n \eps}}, \]
where $Lap(\beta)$ is a Laplace random variable with parameter $\beta$.}
The final output $\hat{p}$ is the projection of $h$ on the simplex $\Delta_k$ {in $\ell_2$ distance}.
%We first give the proof of the sample complexity under $\ell_2$ loss. Then we can attain the result with respect to  total variation distance by Cauchy-Schwartz Inequality.
The expected $\ell_2$ loss between $h$ and $p$ can be upper bounded by
\begin{align}
\Paren{\expectation{\norm{h-p}}}^2 &\le \expectation{\norms{h-p}} \le \expectation{\norms{p^{\text{erm}}-p}}+\expectation{\norms{h - p^{\text{erm}}}}, \nonumber
\end{align}
where the first inequality comes from the Jensen's inequality and the second inequality comes from the triangle inequality.


The first term $\expectation{\norms{p^{\text{erm}} -p}}$ is upper bounded by $\frac{1}{n}$ by an elementary analysis of the empirical estimator. For the second term, note that $\expectation{\norms{h - p^{\text{erm}}}} = \sum_{i=1}^\ab \expectation{Z_i^2}$, where $\forall i, Z_i \sim \text{Lap}\Paren{\frac{2}{\ns\eps}}$. %\amargin{Which property of Laplace distribution?} 
{By the variance of Laplace distribution}, we have $\expectation{\norms{p^{\text{erm}} -h}} = O\Paren{\frac{k}{n^2 \eps^2}}$.  Therefore $\expectation{\norm{h-p}}\le O\Paren{\frac1{\sqrt{\ns}}+\frac{\sqrt{k}}{\ns\eps}}$.
%Therefore $\expectation{\norm{\hat{p}-p}} \le \frac1{10}\alpha$ when $n= O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{k}}{\alpha\eps}}$.
%By simply applying Markov inequality, we have $\norm{h-\p} \le \alpha$ with probability higher than $\frac{9}{10}$.

Note that since $\Delta_k$ is convex, $\norm{\hat{p}-p} \le\norm{h-p}$. Finally, by Cauchy-Schwarz Inequality, $\expectation{\absvn{\hat{p}- p}} \le \sqrt{\ab}\cdot \expectation{\norm{\hat{p}-\p}}  \le \sqrt{\ab}\cdot\expectation{\norm{h-\p}} = O\Paren{\sqrt{\frac{k}{n}}+ {\frac{k}{n \eps}}} $. Therefore $\expectation{\absvn{\hat{p}- p}} \le \alpha$ when $n= O \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}$.

%As to the lower bounds, we first give a proof under total variation distance by a standard packing argument. Then we extend it to $\ell_2$ distance by using Cauchy–Schwarz inequality. We begin by constructing packing set.
\medskip

\noindent \textbf{Lower bound.}
{We will construct a large set of distributions such that the conditions of Corollary~\ref{coro:fano} hold.} 
\ignore{Our lower bound is through the following two steps. The first step is to construct a set of distributions $\cV_\ab \subset \Delta_k$, such that each pair of distributions in $\cV_\ab$ is $\Omega(\dist)$-separated in total variation distance and with $|\cV_\ab|$ as large as possible. 
In the second step, we bound the $KL$ divergence and $TV$ distance between each pair of distributions, and apply Corollary~\ref{coro:fano} to get the sample complexity lower bound.}
%The following claim is a corollary of Varshamov-Gilbert's lemma (Lemma 4.7 in~\cite{Massart07}). First we need the following binary code to construct packing set.
%\begin{restatable}{claim}{GVcode}
%\label{clm:GV}
%There exists binary code $\cC$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\absv{\cC} > 2^{\frac{\ab}{8}}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{\ab}{8}$,
%\item $\forall c \in \cC, \absv{i:c(i)=1}=\frac{\ab}{2}$.
%\end{enumerate}
%\end{restatable}
%\amargin{We repeat the statement above as well ... I would rather we reduce the number of repeats.}
%WLOG assume $\alpha < 1/24$. Given $c \in \cC$, consider the following distribution  $\p_c$ in $\Delta_\ab$
%\[
%\p_c (i)  = \left\{
%\begin{array}{rcl}
%\frac{1+24\dist}{\ab} ,       &      & \text{when ~ }c(i)=1,\\
%\frac{1-24\dist}{\ab},       &      & \text{when ~ }c(i)=0.
%\end{array} \right.
%\]
%\begin{restatable}{claim}{GVcode}
%\label{clm:GV}
%There exists binary code $\cC$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\absv{\cC} > 2^{\frac{\ab}{8}}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{\ab}{8}$,
%\item $\forall c \in \cC, \absv{i:c(i)=1}=\frac{\ab}{2}$.
%\end{enumerate}
%\end{restatable}
{Suppose $\alpha < 1/48$. Applying Lemma~\ref{lem:GV} with $l={\ab}/{2}$, there exists a constant weight binary code $\cC$ of weight $k/2$, and minimum distance $k/8$, and $|\cC|>2^{7k/128}$. For each codeword $c\in\cC$, a distribution $\p_c$ over $[k]$ is defined as follows:
\[
\p_c (i)  = \left\{
\begin{array}{rcl}
\frac{1+24\dist}{\ab} ,       &      & \text{if ~ }c_i=1,\\
\frac{1-24\dist}{\ab},       &      & \text{if ~ }c_i=0.
\end{array} \right.
\]}

{We choose $\cV = \{ \p_c : c \in \cC \}$ to apply Corollary~\ref{coro:fano}. By the minimum distance property, any two distributions in $\cV$ have a total variation distance of at least $24\alpha/k\cdot k/8=3\alpha$, and at most $24\alpha$. Furthermore, by using $\log (1+x) \le x$, we can bound the KL divergence between distributions by their $\chi^2$ distance, 
\[d_{KL} (\p, \q) \le  \chi^2 (\p,\q)  = \sum_{x=1}^k \frac{\Paren{\p(x) -\q(x)}^2 }{\q(x)} < {10000\alpha^2}.
\]
Setting $\tau=\alpha$, $\gamma=24\alpha$, and $\beta=10000\alpha^2$, and using $\log M > 7\ab/64$ in Corollary~\ref{coro:fano}, we obtain $S(\Delta_{\ab}, d_{TV}, \alpha, \eps)= \Omega \Paren{\frac{k}{\alpha^2}+\frac{k}{\alpha\eps}}.$}
%\amargin{I dont think we can take $\alpha<1/24$, that will break this above, since $q(x)$ can be very close to 0. I have changed it to $\alpha<1/48$. Also, could you check the constant 10000 above.}
\subsubsection{$\ell_2$ distance}
In this section, we derive the sample complexity of $\eps$-DP $\ab$-ary distribution estimation under $\ell_2$ distance, which is stated in Theorem~\ref{thm:pure-l2}.

\medskip

\noindent \textbf{Upper bound:}
We use the same algorithm as in Section~\ref{sec:puredp-tv}. Following the same argument as in Section~\ref{sec:puredp-tv}, the square of expected $\ell_2$ loss of $\hat{p}$ can be upper bounded by
\begin{align}
\Paren{\expectation{\norm{\hat{p}-p}}}^2 &\le \expectation{\norm{h-p}^2} \le \expectation{\norms{p^{\text{erm}}-p}}+\expectation{\norms{h - p^{\text{erm}}}} = O\Paren{\frac1{\ns}+\frac{\ab}{\ns^2\eps^2}}. \nonumber
\end{align}
%And $\expectation{\norm{h-p}} \le \frac1{10}\alpha$ when $n= O \Paren{\frac{1}{\alpha^2}+\frac{\sqrt{k}}{\alpha\eps}}$.
Since $\Delta_k$ is convex, we have $\norm{\hat{p}-p} \le\norm{h-p}$. Moreover, the following lemma gives another bound for $\norm{\hat{p}-p}$ (See Corollary 2.3 in~\cite{Bassily18}).
\begin{lemma}
Let $L \subset \RR^d$ be a symmetric convex body of $\ab$ vertices $\{a_j\}_{j=1}^{\ab}$, and let $y \in L$ and $\bar{y} = y+z$ for some $z \in \RR^d$. Let $\hat{y} = \arg \min_{w\in L} \norm{w-\bar{y}}^2$. Then we must have 
$$ \norm{y-\hat{y}}^2 \le 4\max_{j\in[k]} \{ \langle z, a_j \rangle\}. $$
\end{lemma} 

From the lemma, we have $\expectation{\norm{\hat{p}-h}^2}\le 4\cdot \expectation{ \max_{j\in[\ab]} \absv{Z_j}}$, where $\forall j \in [\ab]$, $Z_j \sim \text{Lap}(\frac{2}{\ns\eps})$. Note that $\expectation{ \max \absv{Z_j}} = O\Paren{\frac{\log\ab}{\ns\eps}}$ due to the tail bound of Laplace distribution. We have $\Paren{\expectation{\norm{\hat{p}-p}}}^2 = O\Paren{\frac1{\ns}+ \frac{\log\ab}{\ns\eps}}$. Combined with the previous analysis,  $\Paren{\expectation{\norm{\hat{p}-p}}}^2 = O\Paren{\frac1{\ns}+ \min\Paren{\frac{\ab}{\ns^2\eps^2} ,\frac{\log\ab}{\ns\eps}} }$. Therefore $\expectation{\norm{\hat{p}-p}} \le \frac1{10}\alpha$ when $n= O \Paren{\frac{1}{\alpha^2}+ \min \Paren {\frac{\sqrt{k}}{\alpha\eps}, \frac{\log\ab}{\dist^2\eps} }}$.

\medskip

\noindent \textbf{Lower bound:}
We first consider the case when $\dist < \frac1{\sqrt{\ab}}$, where we can 
derive the lower bound simply by a reduction. By Cauchy-Schwarz 
inequality, for any estimator $\hat{p}$, $ \expectation{\absvn{\hat{p}-p}} 
\le \sqrt{\ab} \cdot \expectation{\norm{\hat{p}-p}}$. Therefore 
$S(\Delta_k,  \ell_2, \alpha, \eps) \ge S(\Delta_k,  d_{TV}, \sqrt{k}\alpha, 
\eps)$, which gives us $S(\Delta_k,  \ell_2, \alpha, \eps)= 
\Omega\Paren{\frac{1}{\dist^2}+\frac{\sqrt{\ab}}{\dist\eps}}$.

Now we consider $\dist \ge \frac1{\sqrt{k}}$. Note that it is enough if we prove the lower bound of $\Omega\Paren{\frac{\log \Paren{\alpha^2\ab}}{\dist^2\eps}}$, since $\Omega\Paren{\frac1{\dist^2}}$ %\zsmargin{How to prove this lower bound for $\dist \ge \frac1{\sqrt{k}}$?} 
is the sample complexity of non-private estimation problem for all range of $\dist$. Similarly, we follow Corollary~\ref{coro:fano}, except that we need to construct a different set of distributions. 
%The following claim can be seen as a corollary of Varshamov-Gilbert's lemma when applied to constant weight binary codes.

%\begin{claim}
%\label{claim:constantGV}
%Given an integer weight $l\le\frac1{50}\ab$, there exists a binary code $\cC$ with code length $\ab$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\forall c \in \cC, \absv{i:c(i)=1}=l$,
%\item $\exists c_1, c_2 > 0 $, $\absv{\cC} > \Paren{  \frac{\ab}{c_1 l}}^{c_2  l}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{l}{4}$,
%\end{enumerate}
%\end{claim}
%
%\begin{proof}
%This proof can be viewed as the standard argument used to prove the Gilbert-Varshamov bound when applied to constant weight codes. The following lemma comes from Theorem 7 in~\cite{GrahamS80},
%\begin{lemma}
%\label{lem:constantGV}
%There exists a binary code $\cC$ with length $\ab$, constant weight $l$ and minimum Hamming weight $2\delta$ ($\min_{i,j \in \cC} \ham{i}{j} $), which satisfies $\absv{\cC} \ge \frac{\binom{\ab}{l}}{\sum_{i=0}^{\delta} \binom{l}{i} \binom{\ab-l}{i}}$.
%\end{lemma}
%
%By applying Lemma~\ref{lem:constantGV}, and replacing $2\delta$ by $\frac{l}{4}$, we have
%\begin{align}
%\absv{\cC} &\ge \frac{\binom{\ab}{l}} {\sum_{j=0}^{l/8} \binom{l}{j} \cdot \binom{\ab-l}{j}}\nonumber  \ge \frac{\binom{\ab}{l}}{\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} \cdot \binom{\ab}{\frac{l}{8}}} \nonumber\\
%  &= \frac1 {\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} } \cdot \prod_{i = 0}^{\frac{7l}{8}- 1} \frac{k - \frac{l}{8}-i}{l - i} 
% \ge 2^{-2l} \cdot \Paren{ \frac{\ab-l}{l}}^{\frac{7l}{8}} \nonumber\\
% &\ge \Paren{  \frac{49}{50} \cdot \frac{\ab}{5l}}^{\frac{7l}{8}}, \nonumber 
%\end{align}
%In the second last inequality, we use $\binom{l}{\frac{l}{8}} \le \binom{l}{\frac{l}{2}} \le 2^l$ and $2^l \ge \frac{l}{8}$ when $l \ge 1$.
%\end{proof}

%\newhzz{
%\begin{claim}
%\label{claim:constantGV}
%Given an integer weight $l\le\frac1{2}\ab$, there exists a binary code $\cC$ with code length $\ab$ which satisfies the following conditions:
%\begin{enumerate}[label=(\alph*)]
%\item $\forall c \in \cC, \absv{i:c(i)=1}=l$,
%\item $\exists c_1, c_2, c_3 > 0 $, $\absv{\cC} > c_1\cdot  \Paren{  \frac{\ab}{c_2 l}}^{c_3  l}$,
%\item $\min_{a,b \in \cC} \ham{a}{b}>\frac{l}{4}$,
%\end{enumerate}
%\end{claim}
%\begin{proof}
%This proof can be viewed as the standard argument used to prove the Gilbert-Varshamov bound when applied to constant weight codes. The following lemma comes from Theorem 7 in~\cite{GrahamS80},
%\begin{lemma}
%\label{lem:constantGV}
%There exists a binary code $\cC$ with length $\ab$, constant weight $l$ and minimum Hamming weight $2\delta$ ($\min_{i,j \in \cC} \ham{i}{j} $), which satisfies $\absv{\cC} \ge \frac{\binom{\ab}{l}}{\sum_{i=0}^{\delta} \binom{l}{i} \binom{\ab-l}{i}}$.
%\end{lemma}
%By applying Lemma~\ref{lem:constantGV}, and replacing $2\delta$ by $\frac{l}{4}$, we have
%\begin{align}
%\absv{\cC} &\ge \frac{\binom{\ab}{l}} {\sum_{j=0}^{l/8} \binom{l}{j} \cdot \binom{\ab-l}{j}}\nonumber  \ge \frac{\binom{\ab}{l}}{\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} \cdot \binom{\ab}{\frac{l}{8}}} \nonumber\\
%  &= \frac1 {\frac{l}{8} \cdot \binom{l}{\frac{l}{8}} } \cdot \prod_{i = 0}^{\frac{7l}{8}- 1} \frac{k - \frac{l}{8}-i}{l - i} 
% \ge \frac{2\sqrt{7} \pi}{e} \cdot (0.59)^{\frac{7l}{8}} \cdot \Paren{ \frac{\ab-\frac{l}{8}}{l}}^{\frac{7l}{8}} \nonumber\\
% &\ge \frac{2\sqrt{7} \pi}{e} \cdot \Paren{  0.55 \cdot \frac{\ab}{l}}^{\frac{7l}{8}}, \nonumber 
%\end{align}
%In the second last inequality, we use the Stirling approximation $\sqrt{2\pi}\cdot l^{l+\frac12} \cdot e^{-l} \le l! \le e \cdot l^{l+\frac12} \cdot e^{-l}$ and $1.1^l \ge \sqrt{l}$ when $l \ge 20$.
%\end{proof}
%}

Without loss of generality, we assume $\dist<0.1$. Now we use the codebook in Lemma~\ref{lem:GV} to construct our distribution set. {We fix weight $l = \lfloor \frac1{50\dist^2} \rfloor$. Note that for any $x>2$, $\lfloor x \rfloor > \frac{x}{2}$. Then we have  $\frac1{100\dist^2} < \lfloor l \rfloor  \le \frac1{50\dist^2} $ since $\frac1{50\dist^2}>2$. Therefore we get a codebook $\cC$ with $|\cC| \ge (k\alpha^2)^{\frac{1}{200 \alpha^2}}$}. Given $c \in \cC$, we construct the following distribution  $\p_c$ in $\Delta_\ab$:
%$$ \p_c (i)  = \left\{
%\begin{array}{cl}
%\frac1{l} ,             & when ~ c(i)=1,\\
%0,             & when ~c(i)=0.
%\end{array} \right. $$
$$ \p_c (i)  = \frac1{l} c_i. $$

We use $\cV_\ab = \{ \p_c : c \in \cC \}$ to denote the set of all these distributions. It is easy to check that $\forall \p \in \cV_\ab$ is a valid distribution. Moreover, for any pair of distributions $\p, \q \in \cV_\ab$, we have $\norm{\p - \q}> \frac1{2\sqrt{l}} = \Omega\Paren{\dist}$.


For any pair $\p,\q \in \cV_k$, $d_{TV} (\p, \q) \le 1$, which is a naive upper bound for $TV$ distance. Finally by setting $\ell$ in Corollary~\ref{coro:fano} to be $\ell_2$ distance, we have $S(\Delta_{\ab}, \ell_2, \alpha, \eps)  =  \Omega \Paren{\frac{\log \absv{\cC} }{\eps}} = \Omega \Paren{\frac{\log ( k\alpha^2)}{\alpha^2\eps}}$.



==> toolbox/uniformity-lower_new.tex <==
\subsection{Sample Complexity Lower bounds for Uniformity Testing}\label{sec:lower-identity}

The first term is the lower bound without privacy constraints, proved in~\cite{Paninski08}. In this section, we prove the terms associated with privacy. 

The simplest argument is for $\ns \ge \frac{\ab}{\alpha^2}$, which hopefully will give the readers a sense of how coupling argument works. We consider the case of binary uniformity testing where the goal is to test whether the bias of a coin is $1/2$ or $\alpha$-far from $1/2$. This is a special case of uniformity testing for distributions over $[\ab]$ (when $\ab-2$ symbols have probability zero). This is strictly harder than the problem of distinguishing between $\Bern{1/2}$ and $\Bern{1/2+\alpha}$. The coupling given in Example~\ref{exm:coin} has expected hamming distance of $\alpha \ns$. Hence combing with Theorem~\ref{thm:le_cam}, by letting the RHS no larger than $\frac13$, we get a lower bound of $ \ns = \Omega\Paren{\min\Paren{\frac1{\dist\eps}, \frac1{\dist\delta} }} = \Omega({\frac{1}{\dist (\eps+\delta)}})$.

We now consider the cases $\ns \le \ab$ and $\ab< \ns \le \frac{\ab}{\alpha^2}$.

%The final term is a lower bound for testing identity to $\Bern{0.5}$, which is easier than uniformity testing by Theorem~\ref{thm:unif-identity}. 

To this end, we invoke our private LeCam's method, and design a hypothesis testing problem that will imply a lower bound on uniformity testing. The testing problem will be to distinguish between the following two cases. 

{\bf Case 1:} We are given $\ns$ independent samples from the uniform distribution $\unifab$.

{\bf Case 2:} Generate a distribution $\p$ with $\dtv{\p}{\unifab}\ge\dist$ according to some prior over all such distributions. We are then given $\ns$ independent samples from this distribution $\p$. 

From Theorem~\ref{thm:le_cam}, any lower bound for distinguishing between these two cases is a lower bound on uniformity testing problem. 

We now describe the prior construction for {\bf Case 2}, which is the same as considered by~\cite{Paninski08} for lower bounds on identity testing without privacy considerations. For each $\textbf{z} \in\{\pm1\}^{\ab/2}$, define a distribution $\p_{\textbf{z}}$ over $[\ab]$ such that 
\begin{align}
\p_{\textbf{z}}(2i-1) = \frac{1+\textbf{z}_i\cdot 2\dist}{\ab}, \text{ and } \p_{\textbf{z}}(2i) = \frac{1-\textbf{z}_i\cdot 2\dist}{\ab}.\nonumber
\end{align}
Then for any $\textbf{z}$, $\dtv{P_{\textbf{z}}}{\unifab}= \alpha$. For {\bf Case 2}, choose  $\p$ uniformly from these $2^{\ab/2}$ distributions. Let $Q_2$ denote the distribution on $[\ab]^\ns$ by this process. In other words, $Q_2$ is a mixture of product distributions over $[\ab]$. 

In {\bf Case 1}, let $Q_1$ be the distribution of $\ns$ $i.i.d.$ samples from $\unifab$. 

To obtain a sample complexity lower bound for distinguishing the two cases, we will design a coupling between $Q_1$, and $Q_2$, and bound its expected Hamming distance. While it can be shown that the Hamming distance of the coupling between the uniform distribution with any \emph{one} of the $2^{\ab/2}$ distributions grows as $\alpha\ns$, it can be significantly smaller, when we consider the mixtures. In particular, the following lemma shows that there exist couplings with bounded Hamming distance. 

\begin{lemma}\label{lem:coupling-hamming}
	There is a coupling between $\Xon$ generated by $Q_1$, and $\Yon$ by $Q_2$ such that 
\begin{center}
   $\expectation{\ham{\Xon}{\Yon}} \le C \cdot \dist^2 \min \{ \frac{\ns^2}{\ab}, \frac{\ns^{3/2}}{{\ab}^{1/2}} \}$.
%    \begin{cases}
%                                   8\frac{\ns^2\dist^2}{\ab}, & \text{when $m \le k$} \\
%                                    C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}}, & \text{when $k< m \le \frac{k}{\alpha^2}$}.
%    \end{cases}
\end{center}
\end{lemma}
We refer the proof of the lemma to~\cite{AcharyaSZ18}. Now applying Theorem~\ref{thm:le_cam}, we get the bound in Theorem~\ref{thm:main-identity}.
%\begin{enumerate}
%	\item \newhz{For $m \le k$, $8\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/2}}{\alpha \eps^{1/2}}}$.}
%	\item \newhz{For $k< m \le \frac{k}{\alpha^2}$, $C\cdot \dist^2\frac{\ns^{3/2}}{{\ab}^{1/2}} = \Omega \Paren{\frac1{\eps}}$, implying $m = \Omega \Paren{\frac{\ab^{1/3}}{\alpha^{4/3}\eps^{2/3}}}$.}
%\end{enumerate}

%\begin{lemma}
%There is a coupling between $\Xon$  generated by $Q_2$, and $\Yon$ by $Q_1$ such that for 
%\[
%\expectation{\ham{\Xon}{\Yon}} \le
%\begin{cases}
%O\Paren{\dist^2\cdot\frac{\ns^2}{\ab}} & \ns\le \ab,\\
%O\Paren{\dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}}& k\le \ns\le \ab/\alpha^2,\\
%%O\Paren{\alpha\ns}&  \ab/\alpha^2\le\ns.
%\end{cases}
%\]
%\label{lem:coupling-uniform}
%\end{lemma}

%We can rewrite this result as
%\begin{align}
%\expectation{\ham{\Xon}{\Yon}} \le
%O\Paren{\min\left\{\dist^2\cdot\frac{\ns^2}{\ab}, \dist^2\cdot\frac{\ns^{3/2}}{\ab^{1/2}}, \alpha\ns\right\}}\label{eq:coup-ub}
%\end{align}
%	For the proof of this lemma, we can refer to lemma
%
%
%
%Using lemma~\ref{lem:coupling-uniform}, we can apply the coupling lower bound to prove the lower bound. 
%\begin{theorem}
%\[
%\Sitd\ge \Omega\Paren{\max\left\{\frac{\ab^{1/2}}{\alpha(\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3}(\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.
%\]
%\end{theorem}


%This is proved in the following lemma. 


%The construction of $Q_2$, and the proof of Lemma~\ref{lem:coup_unif} is slightly technical and is given in Section~\ref{app:lb-unif}.
%Assuming this lemma, by Theorem~\ref{thm:coupling}, we need $\expectation{\ham{\Xon}{\Yon}}=\Omega\Paren{\frac1{\eps+\delta}}$ to distinguish between $Q_1$, and $Q_2$. For this to hold, we need $\frac{\ns^2\dist^2}{\ab} = \Omega\Paren{\frac1{\eps+\delta}}$, which gives us 
%$\ns\ge \Omega\Paren{\frac{\sqrt \ab}{\dist\sqrt{\eps+\delta}}}$.




==> toolbox/uniformity.tex <==
\section{$(\eps,\delta)$-DP uniformity testing}
\label{sec:identity}

\newhzn{
In this section, we give a proof sketch of sample complexity lower bound of uniformity testing. The full detail can be referred to~\cite{AcharyaSZ18}. The main result is the following. }

\begin{theorem}
\label{thm:main-identity}
The sample complexity of $(\eps,\delta)$-DP identity testing is
$$\Sutd = \Theta\Paren{\frac{k^{1/2}}{\dist^2}+\max\left\{\frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.$$
%
%Or we can write it according to the parameter range,
%\[
%    \Sit =
%    \begin{cases}
%                                   \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac{\ab^{1/2}}{\alpha (\eps+\delta)^{1/2}}}, & \text{when $k = \Omega \Paren{\frac1{\alpha^4}}$ and $k = \Omega \Paren{\frac1{\alpha^2 (\eps+\delta)}}$,} \\
%              		  \Theta\Paren{\frac{\sqrt k}{\alpha^2} +\frac{\ab^{1/3}}{\alpha^{4/3} (\eps+\delta)^{2/3}}}, & \text{when $k = \Omega \Paren{\frac{\alpha}{(\eps+\delta)}}$ and $k = O \Paren{\frac1{\alpha^4}+\frac1{\alpha^2 (\eps+\delta)} }$,}\\
%              		               \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac1{\alpha (\eps+\delta)}}, & \text{when  $k = O \Paren{\frac{\alpha}{(\eps+\delta)}}$.}\\ 
%    \end{cases}
%\]
\end{theorem}
We note that the lower bound is tight up to constant factors in all parameters. 

%In~\cite{AcharyaSZ18}, they show a reduction from identity to uniformity testing under differential privacy and design algorithms which achieve the matching upper bounds.
% 
%In this work, we focus on the lower bounds for identity testing. Since uniformity testing is a special case of identity testing, any lower bound for uniformity will port over to identity, and we give such bounds in Section~\ref{sec:lower-identity}.






